Coherence of Type Class Resolution

Elaboration-based type class resolution, as found in languages like Haskell, Mercury and PureScript, is generally nondeterministic: there can be multiple ways to satisfy a wanted constraint in terms of global instances and locally given constraints. Coherence is the key property that keeps this sane; it guarantees that, despite the nondeterminism, programs still behave predictably. Even though elaboration-based resolution is generally assumed coherent, as far as we know, there is no formal proof of this property in the presence of sources of nondeterminism, like superclasses and flexible contexts. This paper provides a formal proof to remedy the situation. The proof is non-trivial because the semantics elaborates resolution into a target language where different elaborations can be distinguished by contexts that do not have a source language counterpart. Inspired by the notion of full abstraction, we present a two-step strategy that first elaborates nondeterministically into an intermediate language that preserves contextual equivalence, and then deterministically elaborates from there into the target language. We use an approach based on logical relations to establish contextual equivalence and thus coherence for the first step of elaboration, while the second step's determinism straightforwardly preserves this coherence property.

==> Makefile <==
OTT_LOC    = ../ott

SOURCE_OTT = $(OTT_LOC)/*.ott

OTT_OPTS  = -tex_show_meta false
OTT_FILES  = $(OTT_LOC)/common.ott $(OTT_LOC)/target.ott $(OTT_LOC)/intermed.ott $(OTT_LOC)/source.ott

MAIN = paper

RULESFILE = ott-rules.tex

SECTIONS_LOC = ./sections
APPENDIX_SECTIONS_LOC = ../doc/sections
FIGURES_LOC = ./figures
EXAMPLES_LOC = ./examples

AUTOGEN = $(SECTIONS_LOC)/source.mng \
$(SECTIONS_LOC)/coherence.mng \
$(SECTIONS_LOC)/coherence2.mng \
$(SECTIONS_LOC)/inter.mng \
$(SECTIONS_LOC)/target.mng \
$(FIGURES_LOC)/source_syntax.mng \
$(FIGURES_LOC)/source_typing.mng \
$(FIGURES_LOC)/source_typing_extra.mng \
$(FIGURES_LOC)/source_typing_extra2.mng \
$(FIGURES_LOC)/source_inst_typing.mng \
$(FIGURES_LOC)/sourceM_typing.mng \
$(FIGURES_LOC)/inter_syntax.mng \
$(FIGURES_LOC)/inter_typing.mng \
$(FIGURES_LOC)/inter_typing_dict.mng \
$(FIGURES_LOC)/inter_eval.mng \
$(FIGURES_LOC)/inter_envwf.mng \
$(FIGURES_LOC)/source_resolution.mng \
$(FIGURES_LOC)/sourceM_resolution.mng \
$(FIGURES_LOC)/target_syntax.mng \
$(FIGURES_LOC)/target_Q.mng \
$(EXAMPLES_LOC)/sielab_example2_env.mng \
$(EXAMPLES_LOC)/itelab_exp1.mng \
$(APPENDIX_SECTIONS_LOC)/typesystem.mng \
$(APPENDIX_SECTIONS_LOC)/logical.mng \
$(APPENDIX_SECTIONS_LOC)/lemmas.mng \
$(APPENDIX_SECTIONS_LOC)/target.mng

WARN_MSG = "%%% !!! WARNING: AUTO GENERATED. DO NOT MODIFY !!! %%%\n"

all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).mng $(wildcard sections/*.tex) macros.tex $(AUTOGEN) $(MAIN).bib figures/*
	@latexmk -pdf $(MAIN).mng
 
$(RULESFILE): $(OTT_FILES)
	ott -tex_wrap false $(OTT_OPTS) -o $@ $^
	@perl -pi -e 'print $(WARN_MSG) if $$. == 1' $@
	@if grep '<<no parses (' $@ >/dev/null 2>&1 && \
		[ -z "$(DONTSTOP)" ]; then \
			echo; \
			echo "***** OTT PARSE ERROR(S) *****"; \
			grep -n '<<no parses (' $@; \
			$(RM) $@; \
			exit 1; \
	fi >&2

%.mng: %.tex $(RULESFILE)
	ott -tex_wrap false $(OTT_OPTS) -tex_filter $*.tex $*.mng $(OTT_FILES)
	@perl -pi -e 'print $(WARN_MSG) if $$. == 1' $@
	@if grep '<<no parses (' $@ >/dev/null 2>&1 && \
		[ -z "$(DONTSTOP)" ]; then \
			echo; \
			echo "***** OTT PARSE ERROR(S) *****"; \
			grep -n '<<no parses (' $@; \
			$(RM) $@; \
			exit 1; \
	fi >&2

export TEXINPUTS := .:./Styles//:${TEXINPUTS}
export BSTINPUTS := .:./Styles//:${BSTINPUTS}
export SHELL := /bin/bash

all: $(MAIN).pdf

clean:
	@latexmk -c
	@rm -Rf $(MAIN).pdf auto/ *.dvi *.aux *.log *.bbl *.blg *.toc *.out *.fls *.haux *.fdb_latexmk paper.lof paper.lot *~

distclean: clean
	$(RM) paper.pdf
	$(RM) *-eps-converted-to.pdf



==> doc/ott-rules.tex <==
%%% !!! WARNING: AUTO GENERATED. DO NOT MODIFY !!! %%%
% generated by Ott 0.28 from: ../ott/common.ott ../ott/target.ott ../ott/intermed.ott ../ott/source.ott
\newcommand{\ottdrule}[4][]{{\displaystyle\frac{\begin{array}{l}#2\end{array}}{#3}\quad\ottdrulename{#4}}}
\newcommand{\ottusedrule}[1]{\[#1\]}
\newcommand{\ottpremise}[1]{ #1 \\}
\newenvironment{ottdefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]}{}
\newenvironment{ottfundefnblock}[3][]{ \framebox{\mbox{#2}} \quad #3 \\[0pt]\begin{displaymath}\begin{array}{l}}{\end{array}\end{displaymath}}
\newcommand{\ottfunclause}[2]{ #1 \equiv #2 \\}
\newcommand{\ottnt}[1]{\mathit{#1}}
\newcommand{\ottmv}[1]{\mathit{#1}}
\newcommand{\ottkw}[1]{\mathbf{#1}}
\newcommand{\ottsym}[1]{#1}
\newcommand{\ottcom}[1]{\text{#1}}
\newcommand{\ottdrulename}[1]{\textsc{#1}}
\newcommand{\ottcomplu}[5]{\overline{#1}^{\,#2\in #3 #4 #5}}
\newcommand{\ottcompu}[3]{\overline{#1}^{\,#2<#3}}
\newcommand{\ottcomp}[2]{\overline{#1}^{\,#2}}
\newcommand{\ottgrammartabular}[1]{\begin{supertabular}{llcllllll}#1\end{supertabular}}
\newcommand{\ottmetavartabular}[1]{\begin{supertabular}{ll}#1\end{supertabular}}
\newcommand{\ottrulehead}[3]{$#1$ & & $#2$ & & & \multicolumn{2}{l}{#3}}
\newcommand{\ottprodline}[6]{& & $#1$ & $#2$ & $#3 #4$ & $#5$ & $#6$}
\newcommand{\ottfirstprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottlongprodline}[2]{& & $#1$ & \multicolumn{4}{l}{$#2$}}
\newcommand{\ottfirstlongprodline}[2]{\ottlongprodline{#1}{#2}}
\newcommand{\ottbindspecprodline}[6]{\ottprodline{#1}{#2}{#3}{#4}{#5}{#6}}
\newcommand{\ottprodnewline}{\\}
\newcommand{\ottinterrule}{\\[5.0mm]}
\newcommand{\ottafterlastrule}{\\}
\newcommand{\ottmetavars}{
\ottmetavartabular{
 $ \ottmv{stypvar} ,\, {\source a } ,\, {\source b } $ &  \\
 $ \ottmv{itypvar} ,\, {\intermed a } ,\, {\intermed b } $ &  \\
 $ \ottmv{sexpvar} ,\, {\source x} ,\, {\source y} $ &  \\
 $ \ottmv{iexpvar} ,\, {\intermed x} ,\, {\intermed y} ,\, {\intermed {\mathit {refl} } } ,\, {\intermed {main} } ,\, {\intermed {test} } $ &  \\
 $ \ottmv{smethodvar} ,\, {\source m} ,\, {\source {base} } ,\, {\source {sub} } ,\, {\source {(==)} } $ &  \\
 $ \ottmv{imethodvar} ,\, {\intermed m} ,\, {\intermed {base} } ,\, {\intermed {sub} } ,\, {\intermed {(==)} } $ &  \\
 $ \ottmv{sclassvar} ,\, {\source {\mathit{TC} } } ,\, {\source {Base} } ,\, {\source {Sub} } ,\, {\source {Eq} } $ &  \\
 $ \ottmv{iclassvar} ,\, {\intermed {\mathit{TC} } } ,\, {\intermed {Base} } ,\, {\intermed {Sub} } ,\, {\intermed {Eq} } $ &  \\
 $ \ottmv{sdictvar} ,\, {\source \delta } $ &  \\
 $ \ottmv{idictvar} ,\, {\intermed \delta } $ &  \\
 $ \ottmv{sdictcon} ,\, {\source D } $ &  \\
 $ \ottmv{idictcon} ,\, {\intermed D } $ &  \\
 $ \ottmv{index} ,\, \ottmv{i} ,\, \ottmv{j} ,\, \ottmv{k} ,\, \ottmv{h} ,\, \ottmv{n} ,\, \ottmv{m} ,\, \ottmv{p} ,\, \ottmv{q} ,\, \ottmv{s} $ & \ottcom{indices} \\
 $ \ottmv{nonuse} ,\, { \intermed { \mathit{ r } } } $ &  \\
 $ \ottmv{ttypvar} ,\, {\target a } ,\, {\target b } $ &  \\
 $ \ottmv{texpvar} ,\, {\target x} ,\, {\target y} ,\, {\target \delta } ,\, {\target {\mathit {refl} } } ,\, {\target {main} } ,\, {\target {test} } $ &  \\
 $ \ottmv{tlabel} ,\, {\target m} ,\, {\target {base} } ,\, {\target {sub} } ,\, {\target {(==)} } $ &  \\
}}

\newcommand{\ottstypvarlist}{
\ottrulehead{\ottnt{stypvarlist}  ,\ {\overline {\source a} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source a} }  \ottsym{,}  {\source a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source a} }  \ottsym{,}  {\source b }}{}{}{}{}}

\newcommand{\ottstypvarblist}{
\ottrulehead{\ottnt{stypvarblist}  ,\ {\overline {\source b} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source b} }  \ottsym{,}  {\source b }}{}{}{}{}}

\newcommand{\ottitypvarlist}{
\ottrulehead{\ottnt{itypvarlist}  ,\ {\overline {\intermed a} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\intermed a} }  \ottsym{,}  {\intermed a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed a }  \ottsym{,}  {\overline {\intermed a} }}{}{}{}{}}

\newcommand{\ottitypvarblist}{
\ottrulehead{\ottnt{itypvarblist}  ,\ {\overline {\intermed b} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\intermed b} }  \ottsym{,}  {\intermed b }}{}{}{}{}}

\newcommand{\ottsdvarlist}{
\ottrulehead{\ottnt{sdvarlist}  ,\ {\overline {\source \delta} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source \delta} }  \ottsym{,}  {\source \delta }}{}{}{}{}}

\newcommand{\ottidvarlist}{
\ottrulehead{\ottnt{idvarlist}  ,\ {\overline {\intermed \delta} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\intermed \delta} }  \ottsym{,}  {\intermed \delta }}{}{}{}{}}

\newcommand{\ottsdictconlist}{
\ottrulehead{\ottnt{sdictconlist}  ,\ {\overline {\source D} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source D} }  \ottsym{,}  {\source D }}{}{}{}{}}

\newcommand{\ottidictconlist}{
\ottrulehead{\ottnt{idictconlist}  ,\ {\overline {\intermed D} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\intermed D} }  \ottsym{,}  {\intermed D }}{}{}{}{}}

\newcommand{\ottttypvarlist}{
\ottrulehead{\ottnt{ttypvarlist}  ,\ {\overline {\target a} }  ,\ {\overline {\target b} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\target a} }  \ottsym{,}  {\target a }}{}{}{}{}}

\newcommand{\ottttmvarlist}{
\ottrulehead{\ottnt{ttmvarlist}  ,\ {\overline {\target \delta} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottkw{txl} \, \ottsym{,}  {\target x}}{}{}{}{}}

\newcommand{\ottttype}{
\ottrulehead{\ottnt{ttype}  ,\ {\target \sigma }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\target {Bool} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{ \target {Int} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{,}  {\target \sigma }_{{\mathrm{2}}}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\target a }  \ottsym{.}  {\target \sigma }}{}{\textsf{bind}\; {\target a }\; \textsf{in}\; {\target \sigma }}{}{}\ottprodnewline
\ottprodline{|}{{\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\target \sigma} }  \rightarrow  {\target \sigma }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  {\target m}  \ottsym{:}  {\target \sigma }  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{} \, \ottcomplu{{\target m}_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}}{{\mathrm{1}}}{..}{\ottmv{n}} \, \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\target \sigma }'  /  {\target a }  ]  {\target \sigma }}{}{}{}{}}

\newcommand{\ottttypelist}{
\ottrulehead{\ottnt{ttypelist}  ,\ {\overline {\target \sigma} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\target \sigma} }  \ottsym{,}  {\target \sigma }}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\target \sigma }'  /  {\target a }  ]  {\overline {\target \sigma} }}{}{}{}{}}

\newcommand{\otttterm}{
\ottrulehead{\ottnt{tterm}  ,\ {\target e }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\target {True} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{\target {False} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target e }}{}{\textsf{bind}\; {\target x}\; \textsf{in}\; {\target e }}{}{}\ottprodnewline
\ottprodline{|}{\lambda  \ottsym{(}  {\target x}_{{\mathrm{1}}}  \ottsym{,}  {\target x}_{{\mathrm{2}}}  \ottsym{)}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target e }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda \, \ottcomp{{\target x}_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  {\target e }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target e }_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\target a }  \ottsym{.}  {\target e }}{}{\textsf{bind}\; {\target a }\; \textsf{in}\; {\target e }}{}{}\ottprodnewline
\ottprodline{|}{{\target e } \, {\target \sigma }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{}  {\target m}  \ottsym{=}  {\target e }  \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{} \, \ottcomplu{{\target m}_{\ottmv{i}}  \ottsym{=}  {\target e }_{\ottmv{i}}}{\ottmv{i}}{{\mathrm{1}}}{..}{\ottmv{n}} \, \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target e }  \ottsym{.}  {\target m}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{=}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}}{}{\textsf{bind}\; {\target x}\; \textsf{in}\; {\target e }_{{\mathrm{2}}}}{}{}\ottprodnewline
\ottprodline{|}{{\target e } \, {\overline {\target \sigma} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target e } \, {\overline {\target e} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\target M }  [  {\target e }  ] }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\target {primEqInt} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\target {(\&\&)} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottsym{5}  \ottsym{,}  \ottsym{42}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottttermlist}{
\ottrulehead{\ottnt{ttermlist}  ,\ {\overline {\target e} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{tel,}  {\target e }}{}{}{}{}}

\newcommand{\otttctx}{
\ottrulehead{\ottnt{tctx}  ,\ {\target \Gamma }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\target {\bullet}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target \Gamma }  \ottsym{,}  {\target a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target \Gamma }  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }}{}{}{}{}}

\newcommand{\otttvalue}{
\ottrulehead{\ottnt{tvalue}  ,\ {\target v}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\target {True} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{\target {False} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target e }}{}{\textsf{bind}\; {\target x}\; \textsf{in}\; {\target e }}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\target a }  \ottsym{.}  {\target e }}{}{\textsf{bind}\; {\target a }\; \textsf{in}\; {\target e }}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{} \, \ottcomplu{{\target m}_{\ottmv{i}}  \ottsym{=}  {\target e }_{\ottmv{i}}}{\ottmv{i}}{{\mathrm{1}}}{..}{\ottmv{n}} \, \ottsym{\}}}{}{}{}{}}

\newcommand{\otttectx}{
\ottrulehead{\ottnt{tectx}  ,\ {\target M }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{[} \, \bullet \, \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{[} \, \target {\bullet} \, \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target M }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda \, \ottcomp{{\target x}_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  {\target M }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target e } \, {\target M }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target M } \, {\target e }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\target a }  \ottsym{.}  {\target M }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\overline {\target a} }  \ottsym{.}  {\target M }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target M } \, {\target \sigma }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{\{} \, \ottcomplu{{\target m}_{\ottmv{i}}  \ottsym{=}  {\target M }_{\ottmv{i}}}{\ottmv{i}}{{\mathrm{1}}}{..}{\ottmv{n}} \, \ottsym{\}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\target M }  \ottsym{.}  {\target m}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{=}  {\target M } \, \textbf{\target {in} } \, {\target e }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{=}  {\target e } \, \textbf{\target {in} } \, {\target M }}{}{}{}{}}

\newcommand{\otticlassconstraint}{
\ottrulehead{\ottnt{iclassconstraint}  ,\ {\intermed Q}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\intermed {\mathit{TC} } } \, {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  \overline {\intermed \sigma}  /  {\overline {\intermed a} }  ]  {\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  \overline {\intermed \sigma}  /  {\overline {\intermed b} }  ]  {\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed R }  \ottsym{(}  {\intermed Q}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { R^{SN} } }  \ottsym{(}  {\intermed Q}  \ottsym{)}}{}{}{}{}}

\newcommand{\otticlassconstraintlist}{
\ottrulehead{\ottnt{iclassconstraintlist}  ,\ {\overline {\intermed Q} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\overline {\intermed Q} }  \Rightarrow  {\intermed Q} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed Q}  \Rightarrow  {\overline {\intermed Q} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  {\overline {\intermed Q} }}{}{}{}{}}

\newcommand{\ottipoly}{
\ottrulehead{\ottnt{ipoly}  ,\ {\intermed \sigma}  ,\ {\intermed \tau}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\intermed {Bool} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{ \intermed {Int} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed b }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed Q}  \Rightarrow  {\intermed \sigma} }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\overline {\intermed Q} }  \Rightarrow  {\intermed \sigma} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}}{}{\textsf{bind}\; {\intermed a }\; \textsf{in}\; {\intermed \sigma}}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\intermed a} }  \ottsym{.}  {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\intermed b} }  \ottsym{.}  {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed \sigma}'}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  \overline {\intermed \sigma}  /  {\overline {\intermed a} }  ]  {\intermed \sigma}'}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed \sigma}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed R }  \ottsym{(}  {\intermed \sigma}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { R^{SN} } }  \ottsym{(}  {\intermed \sigma}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed \sigma}_{{\mathrm{1}}}  \ottsym{,}  {\intermed \sigma}_{{\mathrm{2}}}  \ottsym{)}}{}{}{}{}}

\newcommand{\otticonstraint}{
\ottrulehead{\ottnt{iconstraint}  ,\ {\intermed C}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\intermed a }  \ottsym{.}  {\intermed C}}{}{\textsf{bind}\; {\intermed a }\; \textsf{in}\; {\intermed C}}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\intermed a} }  \ottsym{.}  {\intermed C}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\intermed b} }  \ottsym{.}  {\intermed C}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\intermed a }  \ottsym{.}  {\overline {\intermed Q} }  \Rightarrow  {\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\intermed a} }  \ottsym{.}  {\overline {\intermed Q} }  \Rightarrow  {\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\intermed b} }  \ottsym{.}  {\overline {\intermed Q} }  \Rightarrow  {\intermed Q}}{}{}{}{}}

\newcommand{\ottipolylist}{
\ottrulehead{\ottnt{ipolylist}  ,\ \overline {\intermed \sigma}  ,\ \overline {\intermed \tau}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{\overline {\intermed \sigma}  \ottsym{,}  {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \sigma}  \ottsym{,}  \overline {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed R }  \ottsym{(}  \overline {\intermed \sigma}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  \overline {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { R^{SN} } }  \ottsym{(}  \overline {\intermed \sigma}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \overline {\intermed \sigma}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottidict}{
\ottrulehead{\ottnt{idict}  ,\ {\intermed d}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\intermed \delta }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed D } \, \overline {\intermed \sigma} \, {\overline {\intermed d} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma }  ( {\intermed \phi }  ( {\intermed R }  ( {\intermed d} ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed { \gamma^{SN} } }  ( {\intermed { \phi^{SN} } }  ( {\intermed { R^{SN} } }  ( {\intermed d} ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed d}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \gamma }  \ottsym{(}  {\intermed d}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { \gamma^{SN} } }  \ottsym{(}  {\intermed d}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { R^{SN} } }  \ottsym{(}  {\intermed d}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottidictvalue}{
\ottrulehead{\ottnt{idictvalue}  ,\ {\intermed {dv} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\intermed D } \, \overline {\intermed \sigma} \, {\overline {\intermed { dv } } }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma }  ( {\intermed \phi }  ( {\intermed R }  ( {\intermed d} ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed {dv} }  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \gamma }  \ottsym{(}  {\intermed {dv} }  \ottsym{)}}{}{}{}{}}

\newcommand{\ottidictlist}{
\ottrulehead{\ottnt{idictlist}  ,\ {\overline {\intermed d} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\intermed d} }  \ottsym{,}  {\intermed d}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed d}  \ottsym{,}  {\overline {\intermed d} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma }  ( {\intermed \phi }  ( {\intermed R }  ( {\overline {\intermed d} } ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\overline {\intermed d} }  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed d}  /  {\intermed \delta }  ]  {\overline {\intermed d} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  {\overline {\intermed d} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { \gamma^{SN} } }  \ottsym{(}  {\overline {\intermed d} }  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { R^{SN} } }  \ottsym{(}  {\overline {\intermed d} }  \ottsym{)}}{}{}{}{}}

\newcommand{\ottidictvallist}{
\ottrulehead{\ottnt{idictvallist}  ,\ {\overline {\intermed { dv } } }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\intermed { dv } } }  \ottsym{,}  {\intermed {dv} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed {dv} }  \ottsym{,}  {\overline {\intermed { dv } } }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma }  ( {\intermed \phi }  ( {\intermed R }  ( {\overline {\intermed d} } ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\overline {\intermed { dv } } }  \ottsym{)}}{}{}{}{}}

\newcommand{\ottiexpr}{
\ottrulehead{\ottnt{iexpr}  ,\ {\intermed e}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\intermed {True} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{\intermed {False} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed {\mathit {refl} } }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed {main} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed e}}{}{\textsf{bind}\; {\intermed x}\; \textsf{in}\; {\intermed e}}{}{}\ottprodnewline
\ottprodline{|}{\lambda  \ottsym{(}  {\intermed x}  \ottsym{,}  {\intermed y}  \ottsym{)}  \ottsym{:}  \ottsym{(}  {\intermed a }  \ottsym{,}  {\intermed b }  \ottsym{)}  \ottsym{.}  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed e}_{{\mathrm{1}}} \, {\intermed e}_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\intermed \delta }  \ottsym{:}  {\intermed Q}  \ottsym{.}  {\intermed e}}{}{\textsf{bind}\; {\intermed \delta }\; \textsf{in}\; {\intermed e}}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\overline {\intermed \delta} }  \ottsym{:}  {\overline {\intermed Q} }  \ottsym{.}  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed e} \, {\intermed d}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed e} \, {\overline {\intermed d} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\intermed a }  \ottsym{.}  {\intermed e}}{}{\textsf{bind}\; {\intermed a }\; \textsf{in}\; {\intermed e}}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\overline {\intermed a} }  \ottsym{.}  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\overline {\intermed b} }  \ottsym{.}  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed e} \, {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed e} \, \overline {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed d}  \ottsym{.}  {\intermed m}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed d}  \ottsym{)}  \ottsym{.}  {\intermed m}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{=}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}}{}{\textsf{bind}\; {\intermed x}\; \textsf{in}\; {\intermed e}_{{\mathrm{2}}}}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed M}  [  {\intermed e}  ] }{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed e}'  /  {\intermed x}  ]  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed d}  /  {\intermed \delta }  ]  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\overline {\intermed D} }_{{\mathrm{1}}}  /  {\overline {\intermed D} }_{{\mathrm{2}}}  ]  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed e}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed R }  \ottsym{(}  {\intermed e}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \phi }  \ottsym{(}  {\intermed e}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \gamma }  \ottsym{(}  {\intermed e}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma }  ( {\intermed \phi }  ( {\intermed R }  ( {\intermed e} ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed { \gamma^{SN} } }  ( {\intermed { \phi^{SN} } }  ( {\intermed { R^{SN} } }  ( {\intermed e} ))) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed {primEqInt} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed d}  \ottsym{.}  {\intermed {(==)} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed {(\&\&)} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottsym{5}  \ottsym{,}  \ottsym{42}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottivalue}{
\ottrulehead{\ottnt{ivalue}  ,\ {\intermed v}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\intermed {True} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{\intermed {False} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed e}}{}{\textsf{bind}\; {\intermed x}\; \textsf{in}\; {\intermed e}}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\intermed \delta }  \ottsym{:}  {\intermed Q}  \ottsym{.}  {\intermed e}}{}{\textsf{bind}\; {\intermed \delta }\; \textsf{in}\; {\intermed e}}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\intermed a }  \ottsym{.}  {\intermed e}}{}{\textsf{bind}\; {\intermed a }\; \textsf{in}\; {\intermed e}}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma }  ( {\intermed \phi }  ( {\intermed R }  ( {\intermed e} ))) }{}{}{}{}}

\newcommand{\ottitctx}{
\ottrulehead{\ottnt{itctx}  ,\ {\intermed \Gamma}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,}  {\intermed a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,}  {\overline {\intermed a} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,}  {\overline {\intermed b} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,}  {\intermed \delta }  \ottsym{:}  {\intermed Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,}  {\overline {\intermed \delta} }  \ottsym{:}  {\overline {\intermed Q} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}  \ottsym{,} \, \ottcomp{{\intermed \delta }_{\ottmv{i}}  \ottsym{:}  {\intermed Q}_{\ottmv{i}}}{\ottmv{i}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Gamma}_{{\mathrm{1}}}  \ottsym{,}  {\intermed \Gamma}_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed \Gamma}}{}{}{}{}}

\newcommand{\ottitcctx}{
\ottrulehead{\ottnt{itcctx}  ,\ {\intermed { \Gamma_C } }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { \Gamma_C } }  \ottsym{,}  {\intermed m}  \ottsym{:}  {\intermed {\mathit{TC} } } \, {\intermed a }  \ottsym{:}  {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed { \Gamma_C } }_{{\mathrm{1}}}  \ottsym{,}  {\intermed { \Gamma_C } }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed m}  \ottsym{:}  {\intermed {\mathit{TC} } } \, {\intermed a }  \ottsym{:}  {\intermed \sigma}}{}{}{}{}}

\newcommand{\ottimctx}{
\ottrulehead{\ottnt{imctx}  ,\ {\intermed \Sigma}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Sigma}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  {\intermed C}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed D }  \ottsym{:}  {\intermed C}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed \Sigma}  \ottsym{,}  {\intermed \Sigma}'}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\overline {\intermed D} }_{{\mathrm{1}}}  /  {\overline {\intermed D} }_{{\mathrm{2}}}  ]  {\intermed \Sigma}}{}{}{}{}}

\newcommand{\ottiectx}{
\ottrulehead{\ottnt{iectx}  ,\ {\intermed M}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{[} \, \bullet \, \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\intermed \delta }  \ottsym{:}  {\intermed Q}  \ottsym{.}  {\intermed M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\overline {\intermed \delta} }  \ottsym{:}  {\overline {\intermed Q} }  \ottsym{.}  {\intermed M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed e} \, {\intermed M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed M} \, {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed M} \, {\intermed d}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\intermed a }  \ottsym{.}  {\intermed M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\Lambda  {\overline {\intermed a} }  \ottsym{.}  {\intermed M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed M} \, {\intermed \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{=}  {\intermed M} \, \textbf{\intermed {in} } \, {\intermed e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{=}  {\intermed e} \, \textbf{\intermed {in} } \, {\intermed M}}{}{}{}{}}

\newcommand{\ottR}{
\ottrulehead{{\intermed R }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed R }  ,  {\intermed a }  \mapsto (  {\intermed \sigma} ,  { \intermed { \mathit{ r } } }  ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{{\intermed R }_{{\mathrm{1}}}  \ottsym{,}  {\intermed R }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed R }  \ottsym{)}} {\textsf{S}}{}{}{}}

\newcommand{\ottphi}{
\ottrulehead{{\intermed \phi }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \phi } ,  {\intermed x}  \mapsto ( {\intermed e}_{{\mathrm{1}}} ,  {\intermed e}_{{\mathrm{2}}}  ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \phi } ,  {\intermed x}  \mapsto  {\intermed e} }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed \phi }  \ottsym{)}} {\textsf{S}}{}{}{}}

\newcommand{\ottgamma}{
\ottrulehead{{\intermed \gamma }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma } ,  {\intermed \delta }  \mapsto ( {\intermed {dv} }_{{\mathrm{1}}} ,  {\intermed {dv} }_{{\mathrm{2}}}  ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed \gamma } ,  {\intermed \delta }  \mapsto  {\intermed {dv} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed \gamma }  \ottsym{)}} {\textsf{S}}{}{}{}}

\newcommand{\ottRSN}{
\ottrulehead{{\intermed { R^{SN} } }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed { R^{SN} } }  ,  {\intermed a }  \mapsto (  {\intermed \sigma} ,  { \intermed { \mathit{ r } } }  ) }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\intermed { R^{SN} } }  \ottsym{)}}{}{}{}{}}

\newcommand{\ottphiSN}{
\ottrulehead{{\intermed { \phi^{SN} } }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed { \phi^{SN} } } ,  {\intermed x}  \mapsto  {\intermed e} }{}{}{}{}}

\newcommand{\ottgammaSN}{
\ottrulehead{{\intermed { \gamma^{SN} } }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\intermed { \gamma^{SN} } } ,  {\intermed \delta }  \mapsto  {\intermed d} }{}{}{}{}}

\newcommand{\ottsmono}{
\ottrulehead{\ottnt{smono}  ,\ {\source \tau }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\source {Bool} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{ \source {Int} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\source \tau }_{{\mathrm{1}}}  \ottsym{,}  {\source \tau }_{{\mathrm{2}}}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\source \tau }  /  {\source a }  ]  {\source \tau }'}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\overline {\source \tau} }  /  {\overline {\source a} }  ]  {\source \tau }}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\overline {\source \tau} }  /  {\overline {\source b} }  ]  {\source \tau }}{}{}{}{}}

\newcommand{\ottsmonolist}{
\ottrulehead{\ottnt{smonolist}  ,\ {\overline {\source \tau} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{stl,}  {\source \tau }}{}{}{}{}}

\newcommand{\ottsclassconstraint}{
\ottrulehead{\ottnt{sclassconstraint}  ,\ {\source Q}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\source {\mathit{TC} } } \, {\source \tau }}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\source \tau }  /  {\source a }  ]  {\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\overline {\source \tau} }  /  {\overline {\source a} }  ]  {\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {Base} } \, {\source \tau }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {Sub} } \, {\source \tau }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {Eq} } \, {\source \tau }}{}{}{}{}}

\newcommand{\ottsclassconstraintlist}{
\ottrulehead{\ottnt{sclassconstraintlist}  ,\ {\overline {\source Q} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source Q} }  \ottsym{,}  {\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\overline {\source {\mathit{TC}_i~a } }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source Q} }_{{\mathrm{1}}}  \ottsym{,}  {\overline {\source Q} }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottcomp{{\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }_{\ottmv{i}}}{\ottmv{i}}}{}{}{}{}}

\newcommand{\ottsquan}{
\ottrulehead{\ottnt{squan}  ,\ {\source \rho}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\source \tau }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source Q}  \Rightarrow  {\source \rho}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\overline {\source Q} }  \Rightarrow  {\source \rho}}{}{}{}{}}

\newcommand{\ottspoly}{
\ottrulehead{\ottnt{spoly}  ,\ {\source \sigma}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\source \rho}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\source a }  \ottsym{.}  {\source \sigma}}{}{\textsf{bind}\; {\source a }\; \textsf{in}\; {\source \sigma}}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\source a} }  \ottsym{.}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\source b} }  \ottsym{.}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\source \tau }  /  {\source a }  ]  {\source \sigma}}{}{}{}{}}

\newcommand{\ottsconstraint}{
\ottrulehead{\ottnt{sconstraint}  ,\ {\source C}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\source a }  \ottsym{.}  {\source C}}{}{\textsf{bind}\; {\source a }\; \textsf{in}\; {\source C}}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\source a} }  \ottsym{.}  {\source C}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\source b} }  \ottsym{.}  {\source C}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\source a }  \ottsym{.}  {\overline {\source Q} }  \Rightarrow  {\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\source a} }  \ottsym{.}  {\overline {\source Q} }  \Rightarrow  {\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\forall  {\overline {\source b} }  \ottsym{.}  {\overline {\source Q} }  \Rightarrow  {\source Q}}{}{}{}{}}

\newcommand{\ottsexpr}{
\ottrulehead{\ottnt{sexpr}  ,\ {\source e}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\mathit{\source {True} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{\mathit{\source {False} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source x}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source m}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\source x}  \ottsym{.}  {\source e}}{}{\textsf{bind}\; {\source x}\; \textsf{in}\; {\source e}}{}{}\ottprodnewline
\ottprodline{|}{\lambda  \ottsym{(}  {\source x}_{{\mathrm{1}}}  \ottsym{,}  {\source x}_{{\mathrm{2}}}  \ottsym{)}  \ottsym{.}  {\source e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source e}_{{\mathrm{1}}} \, {\source e}_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\source {let} } \, {\source x}  \ottsym{:}  {\source \sigma}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}}{}{\textsf{bind}\; {\source x}\; \textsf{in}\; {\source e}_{{\mathrm{2}}}}{}{}\ottprodnewline
\ottprodline{|}{{\source e}  ::  {\source \tau }}{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\source M}  [  {\source e}  ] }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\source {primEqInt} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{ {\source {(\&\&)} } }{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  \ottsym{5}  \ottsym{,}  \ottsym{42}  \ottsym{)}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\source e}  \ottsym{)}}{}{}{}{}}

\newcommand{\ottsinst}{
\ottrulehead{{\source {inst} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\textbf{\source {instance} } \, {\overline {\source Q} }  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{=}  {\source e}  \ottsym{\}}}{}{}{}{}}

\newcommand{\ottscls}{
\ottrulehead{{\source {cls} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\textbf{\source {class} } \, {\overline {\source Q} }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{:}  {\source \sigma}  \ottsym{\}}}{}{\textsf{bind}\; {\source a }\; \textsf{in}\; {\source \sigma}}{}{}}

\newcommand{\ottspgm}{
\ottrulehead{{\source {pgm} }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{{\source e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {cls} }  \ottsym{;}  {\source {pgm} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {inst} }  \ottsym{;}  {\source {pgm} }}{}{}{}{}}

\newcommand{\ottstctx}{
\ottrulehead{\ottnt{stctx}  ,\ {\source \Gamma}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}  \ottsym{,}  {\source a }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}  \ottsym{,}  {\overline {\source a} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}  \ottsym{,}  {\overline {\source b} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}  \ottsym{,}  {\source \delta }  \ottsym{:}  {\source Q}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}  \ottsym{,}  {\overline {\source \delta} }  \ottsym{:}  {\overline {\source Q} }}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source \Gamma}_{{\mathrm{1}}}  \ottsym{,}  {\source \Gamma}_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\source \sigma}  /  {\source a }  ]  {\source \Gamma}}{}{}{}{}}

\newcommand{\ottscctx}{
\ottrulehead{\ottnt{scctx}  ,\ {\source { \Gamma_C } }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source { \Gamma_C } }  \ottsym{,}  {\source m}  \ottsym{:}  {\overline {\source Q} }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source m}  \ottsym{:}  {\overline {\source Q} }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source { \Gamma_C } }  \ottsym{,}  {\source { \Gamma_C } }'}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {base} }  \ottsym{:}  {\overline {\source Q} }  \Rightarrow  {\source {Base} } \, {\source a }  \ottsym{:}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {sub} }  \ottsym{:}  {\overline {\source Q} }  \Rightarrow  {\source {Sub} } \, {\source a }  \ottsym{:}  {\source \sigma}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source {(==)} }  \ottsym{:}  {\overline {\source Q} }  \Rightarrow  {\source {Eq} } \, {\source a }  \ottsym{:}  {\source \sigma}}{}{}{}{}}

\newcommand{\ottspgmtheory}{
\ottrulehead{\ottnt{spgmtheory}  ,\ { \source P }}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\bullet}{}{}{}{}\ottprodnewline
\ottprodline{|}{{ \source P }  \ottsym{,}  \ottsym{(}  {\source D }  \ottsym{:}  {\source C}  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  {\source \Gamma}  \ottsym{:}  {\source e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\ottsym{(}  {\source D }  \ottsym{:}  {\source C}  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  {\source \Gamma}  \ottsym{:}  {\source e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{ \source P }_{{\mathrm{1}}}  \ottsym{,}  { \source P }_{{\mathrm{2}}}}{}{}{}{}\ottprodnewline
\ottprodline{|}{[  {\overline {\source D} }_{{\mathrm{1}}}  /  {\overline {\source D} }_{{\mathrm{2}}}  ]  { \source P }}{}{}{}{}}

\newcommand{\ottsectx}{
\ottrulehead{\ottnt{sectx}  ,\ {\source M}}{::=}{}\ottprodnewline
\ottfirstprodline{|}{\ottsym{[} \, \bullet \, \ottsym{]}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\lambda  {\source x}  \ottsym{.}  {\source M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source M} \, {\source e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source e} \, {\source M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\source {let} } \, {\source x}  \ottsym{:}  {\source \sigma}  \ottsym{=}  {\source M} \, \textbf{\source {in} } \, {\source e}}{}{}{}{}\ottprodnewline
\ottprodline{|}{\textbf{\source {let} } \, {\source x}  \ottsym{:}  {\source \sigma}  \ottsym{=}  {\source e} \, \textbf{\source {in} } \, {\source M}}{}{}{}{}\ottprodnewline
\ottprodline{|}{{\source M}  ::  {\source \tau }}{}{}{}{}}

\newcommand{\ottgrammar}{\ottgrammartabular{
\ottstypvarlist\ottinterrule
\ottstypvarblist\ottinterrule
\ottitypvarlist\ottinterrule
\ottitypvarblist\ottinterrule
\ottsdvarlist\ottinterrule
\ottidvarlist\ottinterrule
\ottsdictconlist\ottinterrule
\ottidictconlist\ottinterrule
\ottttypvarlist\ottinterrule
\ottttmvarlist\ottinterrule
\ottttype\ottinterrule
\ottttypelist\ottinterrule
\otttterm\ottinterrule
\ottttermlist\ottinterrule
\otttctx\ottinterrule
\otttvalue\ottinterrule
\otttectx\ottinterrule
\otticlassconstraint\ottinterrule
\otticlassconstraintlist\ottinterrule
\ottipoly\ottinterrule
\otticonstraint\ottinterrule
\ottipolylist\ottinterrule
\ottidict\ottinterrule
\ottidictvalue\ottinterrule
\ottidictlist\ottinterrule
\ottidictvallist\ottinterrule
\ottiexpr\ottinterrule
\ottivalue\ottinterrule
\ottitctx\ottinterrule
\ottitcctx\ottinterrule
\ottimctx\ottinterrule
\ottiectx\ottinterrule
\ottR\ottinterrule
\ottphi\ottinterrule
\ottgamma\ottinterrule
\ottRSN\ottinterrule
\ottphiSN\ottinterrule
\ottgammaSN\ottinterrule
\ottsmono\ottinterrule
\ottsmonolist\ottinterrule
\ottsclassconstraint\ottinterrule
\ottsclassconstraintlist\ottinterrule
\ottsquan\ottinterrule
\ottspoly\ottinterrule
\ottsconstraint\ottinterrule
\ottsexpr\ottinterrule
\ottsinst\ottinterrule
\ottscls\ottinterrule
\ottspgm\ottinterrule
\ottstctx\ottinterrule
\ottscctx\ottinterrule
\ottspgmtheory\ottinterrule
\ottsectx\ottafterlastrule
}}

% defnss
% defns GT_wf
%% defn gt_wf
\newcommand{\ottdruletCxXXEmpty}[1]{\ottdrule[#1]{%
}{
 \vdash_{ctx}  \target {  \target {\bullet}  } }{%
{\ottdrulename{tCx\_Empty}}{}%
}}


\newcommand{\ottdruletCxXXTvar}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \target {  {\target \Gamma }  } }%
\ottpremise{ \target {  {\target a }  }  \notin  \target {  {\target \Gamma }  } }%
}{
 \vdash_{ctx}  \target {  {\target \Gamma }  \ottsym{,}  {\target a }  } }{%
{\ottdrulename{tCx\_Tvar}}{}%
}}


\newcommand{\ottdruletCxXXVar}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \target {  {\target \Gamma }  } }%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }  } }%
\ottpremise{ \target {  {\target x}  }  \notin  \target {  {\target \Gamma }  } }%
}{
 \vdash_{ctx}  \target {  {\target \Gamma }  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }  } }{%
{\ottdrulename{tCx\_Var}}{}%
}}

\newcommand{\ottdefngtXXwf}[1]{\begin{ottdefnblock}[#1]{$ \vdash_{ctx}  \target {  {\target \Gamma }  } $}{}
\ottusedrule{\ottdruletCxXXEmpty{}}
\ottusedrule{\ottdruletCxXXTvar{}}
\ottusedrule{\ottdruletCxXXVar{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsGTXXwf}{
\ottdefngtXXwf{}}

% defns Tty_scope
%% defn tty_sco
\newcommand{\ottdruletTyXXBool}[1]{\ottdrule[#1]{%
}{
 \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  \mathit{\target {Bool} }  } }{%
{\ottdrulename{tTy\_Bool}}{}%
}}


\newcommand{\ottdrulefakeaaaaab}[1]{\ottdrule[#1]{%
}{
 \target {  {\target a }  }  \in  \target {  {\target \Gamma }  } }{%
{\ottdrulename{fakeaaaaab}}{}%
}}


\newcommand{\ottdruletTyXXVar}[1]{\ottdrule[#1]{%
}{
 \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target a }  } }{%
{\ottdrulename{tTy\_Var}}{}%
}}


\newcommand{\ottdruletTyXXAbs}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  \ottsym{,}  {\target a }  }  \vdash_{ty}  \target {  {\target \sigma }  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }  } }{%
{\ottdrulename{tTy\_Abs}}{}%
}}


\newcommand{\ottdruletTyXXArr}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }_{{\mathrm{2}}}  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } }{%
{\ottdrulename{tTy\_Arr}}{}%
}}


\newcommand{\ottdruletTyXXRec}[1]{\ottdrule[#1]{%
\ottpremise{\ottcompu{ \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }_{\ottmv{i}}  } }{\ottmv{i}}{\ottmv{n}}}%
}{
 \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  \ottsym{\{} \, \ottcompu{{\target m}_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}}{\ottmv{n}} \, \ottsym{\}}  } }{%
{\ottdrulename{tTy\_Rec}}{}%
}}

\newcommand{\ottdefnttyXXsco}[1]{\begin{ottdefnblock}[#1]{$ \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }  } $}{}
\ottusedrule{\ottdruletTyXXBool{}}
\ottusedrule{\ottdrulefakeaaaaab{}}
\ottusedrule{\ottdruletTyXXVar{}}
\ottusedrule{\ottdruletTyXXAbs{}}
\ottusedrule{\ottdruletTyXXArr{}}
\ottusedrule{\ottdruletTyXXRec{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsTtyXXscope}{
\ottdefnttyXXsco{}}

% defns Ttm_ty
%% defn ttm_ty
\newcommand{\ottdruletTmXXTrue}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \target {  {\target \Gamma }  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  \mathit{\target {True} }  } : \target {  \mathit{\target {Bool} }  } }{%
{\ottdrulename{tTm\_True}}{}%
}}


\newcommand{\ottdruletTmXXFalse}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \target {  {\target \Gamma }  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  \mathit{\target {False} }  } : \target {  \mathit{\target {Bool} }  } }{%
{\ottdrulename{tTm\_False}}{}%
}}


\newcommand{\ottdruletTmXXVar}[1]{\ottdrule[#1]{%
\ottpremise{ ( \target {  {\target x}  } : \target {  {\target \sigma }  } )  \in  \target {  {\target \Gamma }  } }%
\ottpremise{ \vdash_{ctx}  \target {  {\target \Gamma }  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target x}  } : \target {  {\target \sigma }  } }{%
{\ottdrulename{tTm\_Var}}{}%
}}


\newcommand{\ottdruletTmXXAbs}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  }  \vdash_{tm}  \target {  {\target e }  } : \target {  {\target \sigma }_{{\mathrm{2}}}  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{.}  {\target e }  } : \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } }{%
{\ottdrulename{tTm\_Abs}}{}%
}}


\newcommand{\ottdruletTmXXApp}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{1}}}  } : \target {  {\target \sigma }  \rightarrow  {\target \sigma }'  } }%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{2}}}  } : \target {  {\target \sigma }  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}  } : \target {  {\target \sigma }'  } }{%
{\ottdrulename{tTm\_App}}{}%
}}


\newcommand{\ottdruletTmXXTabs}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  \ottsym{,}  {\target a }  }  \vdash_{tm}  \target {  {\target e }  } : \target {  {\target \sigma }  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  \Lambda  {\target a }  \ottsym{.}  {\target e }  } : \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }  } }{%
{\ottdrulename{tTm\_Tabs}}{}%
}}


\newcommand{\ottdruletTmXXTapp}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }  } : \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }_{{\mathrm{1}}}  } }%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{ty}  \target {  {\target \sigma }_{{\mathrm{2}}}  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e } \, {\target \sigma }  } : \target {  [  {\target \sigma }_{{\mathrm{2}}}  /  {\target a }  ]  {\target \sigma }_{{\mathrm{1}}}  } }{%
{\ottdrulename{tTm\_Tapp}}{}%
}}


\newcommand{\ottdruletTmXXRec}[1]{\ottdrule[#1]{%
\ottpremise{\ottcompu{ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }_{\ottmv{i}}  } : \target {  {\target \sigma }_{\ottmv{i}}  } }{\ottmv{i}}{\ottmv{n}}}%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  \ottsym{\{} \, \ottcompu{{\target m}_{\ottmv{i}}  \ottsym{=}  {\target e }_{\ottmv{i}}}{\ottmv{i}}{\ottmv{n}} \, \ottsym{\}}  } : \target {  \ottsym{\{} \, \ottcompu{{\target m}_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}}{\ottmv{n}} \, \ottsym{\}}  } }{%
{\ottdrulename{tTm\_Rec}}{}%
}}


\newcommand{\ottdruletTmXXProj}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }  } : \target {  \ottsym{\{} \, \ottcompu{{\target m}_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}}{\ottmv{n}} \, \ottsym{\}}  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }  \ottsym{.}  {\target m}_{\ottmv{j}}  } : \target {  {\target \sigma }_{\ottmv{j}}  } }{%
{\ottdrulename{tTm\_Proj}}{}%
}}


\newcommand{\ottdruletTmXXLet}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target \Gamma }  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{2}}}  } : \target {  {\target \sigma }_{{\mathrm{2}}}  } }%
\ottpremise{ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{1}}}  } : \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
}{
 \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } : \target {  {\target \sigma }_{{\mathrm{2}}}  } }{%
{\ottdrulename{tTm\_Let}}{}%
}}

\newcommand{\ottdefnttmXXty}[1]{\begin{ottdefnblock}[#1]{$ \target {  {\target \Gamma }  }  \vdash_{tm}  \target {  {\target e }  } : \target {  {\target \sigma }  } $}{}
\ottusedrule{\ottdruletTmXXTrue{}}
\ottusedrule{\ottdruletTmXXFalse{}}
\ottusedrule{\ottdruletTmXXVar{}}
\ottusedrule{\ottdruletTmXXAbs{}}
\ottusedrule{\ottdruletTmXXApp{}}
\ottusedrule{\ottdruletTmXXTabs{}}
\ottusedrule{\ottdruletTmXXTapp{}}
\ottusedrule{\ottdruletTmXXRec{}}
\ottusedrule{\ottdruletTmXXProj{}}
\ottusedrule{\ottdruletTmXXLet{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsTtmXXty}{
\ottdefnttmXXty{}}

% defns Teval
%% defn t_eval
\newcommand{\ottdruletEvalXXAppAbs}[1]{\ottdrule[#1]{%
}{
 \target {  \ottsym{(}  \lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target e }_{{\mathrm{1}}}  \ottsym{)} \, {\target e }_{{\mathrm{2}}}  }  \longrightarrow  \target {  [  {\target e }_{{\mathrm{1}}}  /  {\target x}  ]  {\target e }_{{\mathrm{2}}}  } }{%
{\ottdrulename{tEval\_AppAbs}}{}%
}}


\newcommand{\ottdruletEvalXXTappTabs}[1]{\ottdrule[#1]{%
}{
 \target {  \ottsym{(}  \Lambda  {\target a }  \ottsym{.}  {\target e }  \ottsym{)} \, {\target \sigma }  }  \longrightarrow  \target {  [  {\target \sigma }  /  {\target a }  ]  {\target e }  } }{%
{\ottdrulename{tEval\_TappTabs}}{}%
}}


\newcommand{\ottdruletEvalXXApp}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target e }_{{\mathrm{1}}}  }  \longrightarrow  \target {  {\target e }'_{{\mathrm{1}}}  } }%
}{
 \target {  {\target e }_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}  }  \longrightarrow  \target {  {\target e }'_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}  } }{%
{\ottdrulename{tEval\_App}}{}%
}}


\newcommand{\ottdruletEvalXXTapp}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target e }_{{\mathrm{1}}}  }  \longrightarrow  \target {  {\target e }'_{{\mathrm{1}}}  } }%
}{
 \target {  {\target e }_{{\mathrm{1}}} \, {\target \sigma }  }  \longrightarrow  \target {  {\target e }'_{{\mathrm{1}}} \, {\target \sigma }  } }{%
{\ottdrulename{tEval\_Tapp}}{}%
}}


\newcommand{\ottdruletEvalXXProj}[1]{\ottdrule[#1]{%
}{
 \target {  \ottsym{\{} \, \ottcomplu{{\target m}_{\ottmv{i}}  \ottsym{=}  {\target e }_{\ottmv{i}}}{\ottmv{i}}{{\mathrm{1}}}{..}{\ottmv{n}} \, \ottsym{\}}  \ottsym{.}  {\target m}_{\ottmv{j}}  }  \longrightarrow  \target {  {\target e }_{\ottmv{j}}  } }{%
{\ottdrulename{tEval\_Proj}}{}%
}}


\newcommand{\ottdruletEvalXXRec}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target e }  }  \longrightarrow  \target {  {\target e }'  } }%
}{
 \target {  {\target e }  \ottsym{.}  {\target m}_{\ottmv{j}}  }  \longrightarrow  \target {  {\target e }'  \ottsym{.}  {\target m}_{\ottmv{j}}  } }{%
{\ottdrulename{tEval\_Rec}}{}%
}}


\newcommand{\ottdruletEvalXXLet}[1]{\ottdrule[#1]{%
}{
 \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{=}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  }  \longrightarrow  \target {  [  {\target e }_{{\mathrm{1}}}  /  {\target x}  ]  {\target e }_{{\mathrm{2}}}  } }{%
{\ottdrulename{tEval\_Let}}{}%
}}

\newcommand{\ottdefntXXeval}[1]{\begin{ottdefnblock}[#1]{$ \target {  {\target e }  }  \longrightarrow  \target {  {\target e }'  } $}{}
\ottusedrule{\ottdruletEvalXXAppAbs{}}
\ottusedrule{\ottdruletEvalXXTappTabs{}}
\ottusedrule{\ottdruletEvalXXApp{}}
\ottusedrule{\ottdruletEvalXXTapp{}}
\ottusedrule{\ottdruletEvalXXProj{}}
\ottusedrule{\ottdruletEvalXXRec{}}
\ottusedrule{\ottdruletEvalXXLet{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsTeval}{
\ottdefntXXeval{}}

% defns GTelab
%% defn gt_eval
\newcommand{\ottdruleCtxXXEmpty}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  }  \rightsquigarrow  \target {  \target {\bullet}  } }{%
{\ottdrulename{Ctx\_Empty}}{}%
}}


\newcommand{\ottdruleCtxXXVar}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}  }  \rightsquigarrow  \target {  {\target \Gamma }  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }  } }{%
{\ottdrulename{Ctx\_Var}}{}%
}}


\newcommand{\ottdruleCtxXXTVar}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed a }  }  \rightsquigarrow  \target {  {\target \Gamma }  \ottsym{,}  {\target a }  } }{%
{\ottdrulename{Ctx\_TVar}}{}%
}}


\newcommand{\ottdruleCtxXXDVar}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed \delta }  \ottsym{:}  {\intermed Q}  }  \rightsquigarrow  \target {  {\target \Gamma }  \ottsym{,}  {\target \delta }  \ottsym{:}  {\target \sigma }  } }{%
{\ottdrulename{Ctx\_DVar}}{}%
}}

\newcommand{\ottdefngtXXeval}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } $}{}
\ottusedrule{\ottdruleCtxXXEmpty{}}
\ottusedrule{\ottdruleCtxXXVar{}}
\ottusedrule{\ottdruleCtxXXTVar{}}
\ottusedrule{\ottdruleCtxXXDVar{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsGTelab}{
\ottdefngtXXeval{}}

% defns Tctx_typing
%% defn tctx_typing
\newcommand{\ottdruletMXXempty}[1]{\ottdrule[#1]{%
}{
 \target {  \ottsym{[} \, \bullet \, \ottsym{]}  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } ) }{%
{\ottdrulename{tM\_empty}}{}%
}}


\newcommand{\ottdruletMXXabs}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } )  \mapsto  ( \target {  {\target \Gamma }'  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{ty}  \target {  {\target \sigma }  } }%
}{
 \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_abs}}{}%
}}


\newcommand{\ottdruletMXXappL}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } ) }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{2}}}  } : \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
}{
 \target {  {\target M } \, {\target e }_{{\mathrm{2}}}  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_appL}}{}%
}}


\newcommand{\ottdruletMXXappR}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } ) }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{1}}}  } : \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } }%
}{
 \target {  {\target e }_{{\mathrm{1}}} \, {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_appR}}{}%
}}


\newcommand{\ottdruletMXXtyAbs}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } )  \mapsto  ( \target {  {\target \Gamma }'  \ottsym{,}  {\target a }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }%
}{
 \target {  \Lambda  {\target a }  \ottsym{.}  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_tyAbs}}{}%
}}


\newcommand{\ottdruletMXXtyApp}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }_{{\mathrm{2}}}  } ) }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{ty}  \target {  {\target \sigma }  } }%
}{
 \target {  {\target M } \, {\target \sigma }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  [  {\target \sigma }  /  {\target a }  ]  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_tyApp}}{}%
}}


\newcommand{\ottdruletMXXletL}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } ) }%
\ottpremise{ \target {  {\target \Gamma }'  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{2}}}  } : \target {  {\target \sigma }_{{\mathrm{2}}}  } }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{ty}  \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
}{
 \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  {\target M } \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_letL}}{}%
}}


\newcommand{\ottdruletMXXletR}[1]{\ottdrule[#1]{%
\ottpremise{ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{tm}  \target {  {\target e }_{{\mathrm{1}}}  } : \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
\ottpremise{ \target {  {\target \Gamma }'  }  \vdash_{ty}  \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
}{
 \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } ) }{%
{\ottdrulename{tM\_letR}}{}%
}}

\newcommand{\ottdefntctxXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \target {  {\target M }  } : ( \target {  {\target \Gamma }  }  \Rightarrow  \target {  {\target \sigma }  } )  \mapsto  ( \target {  {\target \Gamma }'  }  \Rightarrow  \target {  {\target \sigma }'  } ) $}{}
\ottusedrule{\ottdruletMXXempty{}}
\ottusedrule{\ottdruletMXXabs{}}
\ottusedrule{\ottdruletMXXappL{}}
\ottusedrule{\ottdruletMXXappR{}}
\ottusedrule{\ottdruletMXXtyAbs{}}
\ottusedrule{\ottdruletMXXtyApp{}}
\ottusedrule{\ottdruletMXXletL{}}
\ottusedrule{\ottdruletMXXletR{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsTctxXXtyping}{
\ottdefntctxXXtyping{}}

% defns Ity_wf
%% defn iq_wf
\newcommand{\ottdruleiQXXTC}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } = \intermed {  {\intermed { \Gamma_C } }_{{\mathrm{1}}}  }, \intermed {  {\intermed m}  \ottsym{:}  {\intermed {\mathit{TC} } } \, {\intermed a }  \ottsym{:}  {\intermed \sigma}'  }, \intermed {  {\intermed { \Gamma_C } }_{{\mathrm{2}}}  } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }_{{\mathrm{1}}}  } ; \intermed {  \bullet  \ottsym{,}  {\intermed a }  }  \vdash_{ty}  \intermed {  {\intermed \sigma}'  } \itot{ \rightsquigarrow  \target {  {\target \sigma }'  } } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  }\, \itot{ \rightsquigarrow  \target {  [  {\target \sigma }  /  {\target a }  ]  \ottsym{\{}  {\target m}  \ottsym{:}  {\target \sigma }'  \ottsym{\}}  } } }{%
{\ottdrulename{iQ\_TC}}{}%
}}

\newcommand{\ottdefniqXXwf}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } $}{}
\ottusedrule{\ottdruleiQXXTC{}}
\end{ottdefnblock}}

%% defn ic_wf
\newcommand{\ottdruleiCXXabs}[1]{\ottdrule[#1]{%
\ottpremise{\ottcomplu{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\overline {\intermed a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}_{\ottmv{i}}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{i}}  } } }{\ottmv{i}}{{\mathrm{1}}}{..}{\ottmv{n}}}%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\overline {\intermed a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
\ottpremise{ \intermed {  {\overline {\intermed a} }_{\ottmv{j}}  }  \notin  \intermed {  {\intermed \Gamma}  } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {C} }  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed Q}  } }{%
{\ottdrulename{iC\_abs}}{}%
}}

\newcommand{\ottdefnicXXwf}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {C} }  \intermed {  {\intermed C}  } $}{}
\ottusedrule{\ottdruleiCXXabs{}}
\end{ottdefnblock}}

%% defn ity_wf
\newcommand{\ottdruleiTyXXbool}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  \mathit{\intermed {Bool} }  } \itot{ \rightsquigarrow  \target {  \mathit{\target {Bool} }  } } }{%
{\ottdrulename{iTy\_bool}}{}%
}}


\newcommand{\ottdruleiTyXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed a }  }  \in  \intermed {  {\intermed \Gamma}  } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed a }  } \itot{ \rightsquigarrow  \target {  {\target a }  } } }{%
{\ottdrulename{iTy\_var}}{}%
}}


\newcommand{\ottdruleiTyXXarrow}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{iTy\_arrow}}{}%
}}


\newcommand{\ottdruleiTyXXqual}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }'  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {   {\intermed Q}  \Rightarrow  {\intermed \sigma}   } \itot{ \rightsquigarrow  \target {  {\target \sigma }'  \rightarrow  {\target \sigma }  } } }{%
{\ottdrulename{iTy\_qual}}{}%
}}


\newcommand{\ottdruleiTyXXscheme}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed a }  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  \forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }  } } }{%
{\ottdrulename{iTy\_scheme}}{}%
}}

\newcommand{\ottdefnityXXwf}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } $}{}
\ottusedrule{\ottdruleiTyXXbool{}}
\ottusedrule{\ottdruleiTyXXvar{}}
\ottusedrule{\ottdruleiTyXXarrow{}}
\ottusedrule{\ottdruleiTyXXqual{}}
\ottusedrule{\ottdruleiTyXXscheme{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsItyXXwf}{
\ottdefniqXXwf{}\ottdefnicXXwf{}\ottdefnityXXwf{}}

% defns Ictx_wf
%% defn ictx_wf
\newcommand{\ottdruleiCtxXXempty}[1]{\ottdrule[#1]{%
}{
 \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  \bullet  } ; \intermed {  \bullet  } }{%
{\ottdrulename{iCtx\_empty}}{}%
}}


\newcommand{\ottdruleiCtxXXtyEnvTm}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
\ottpremise{ \intermed {  {\intermed x}  }  \notin   \textbf {dom}  ( \intermed {  {\intermed \Gamma}  } ) }%
\ottpremise{ \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}  } }{%
{\ottdrulename{iCtx\_tyEnvTm}}{}%
}}


\newcommand{\ottdruleiCtxXXtyEnvTy}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed a }  }  \notin  \intermed {  {\intermed \Gamma}  } }%
\ottpremise{ \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed a }  } }{%
{\ottdrulename{iCtx\_tyEnvTy}}{}%
}}


\newcommand{\ottdruleiCtxXXtyEnvD}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
\ottpremise{ \intermed {  {\intermed \delta }  }  \notin   \textbf {dom}  ( \intermed {  {\intermed \Gamma}  } ) }%
\ottpremise{ \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed \delta }  \ottsym{:}  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } }{%
{\ottdrulename{iCtx\_tyEnvD}}{}%
}}


\newcommand{\ottdruleiCtxXXclsEnv}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  \ottsym{,}  {\intermed a }  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
\ottpremise{ \intermed {  {\intermed m}  }  \notin   \textbf {dom}  ( \intermed {  {\intermed { \Gamma_C } }  } ) }%
\ottpremise{ \intermed {  {\intermed {\mathit{TC} } } \, {\intermed b }  }  \notin   \textbf {dom}  ( \intermed {  {\intermed { \Gamma_C } }  } ) }%
\ottpremise{ \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  } }%
}{
 \vdash_{ctx}  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  \ottsym{,}  {\intermed m}  \ottsym{:}  {\intermed {\mathit{TC} } } \, {\intermed a }  \ottsym{:}  {\intermed \sigma}  } ; \intermed {  \bullet  } }{%
{\ottdrulename{iCtx\_clsEnv}}{}%
}}


\newcommand{\ottdruleiCtxXXMEnv}[1]{\ottdrule[#1]{%
\ottpremise{ \textbf {unambig}  ( \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } ) }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  }  \vdash_{\mathit {C} }  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } }%
\ottpremise{ ( \intermed {  {\intermed m}  } : \intermed {  {\intermed {\mathit{TC} } } \, {\intermed a }  } : \intermed {  {\intermed \sigma}'  } )  \in  \intermed {  {\intermed { \Gamma_C } }  } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  [  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed \sigma}'   } \itot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \intermed {  {\intermed D }  }  \notin   \textbf {dom}  ( \intermed {  {\intermed \Sigma}  } ) }%
\ottpremise{ ( \intermed {  {\intermed D }'  } : \intermed {  \forall  {\overline {\intermed a} }'_{\ottmv{m}}  \ottsym{.}  {\overline {\intermed Q} }''_{\ottmv{n}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}''  } ) . \intermed {  {\intermed m}'  }  \mapsto  \intermed {  {\intermed e}'  }  \notin  \intermed {  {\intermed \Sigma}  } }%
\ottpremise{ \textbf {where}  \intermed {  [  \overline {\intermed \sigma}_{\ottmv{j}}  /  {\overline {\intermed a} }_{\ottmv{j}}  ]  {\intermed \sigma}  } = \intermed {  [  \overline {\intermed \sigma}'_{\ottmv{m}}  /  {\overline {\intermed a} }'_{\ottmv{m}}  ]  {\intermed \sigma}''  } }%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}  \intermed {  {\intermed \Sigma}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  {\intermed e}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }{%
{\ottdrulename{iCtx\_MEnv}}{}%
}}


\newcommand{\ottdruleiCtxXXMEnvXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ ( \intermed {  {\intermed D }'  } : \intermed {  \forall  {\overline {\intermed a} }'_{\ottmv{m}}  \ottsym{.}  {\overline {\intermed Q} }'_{\ottmv{n}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}'  } ) . \intermed {  {\intermed m}'  }  \mapsto  \intermed {  {\intermed e}'  }  \notin  \intermed {  {\intermed \Sigma}  } }%
\ottpremise{ \textbf {where}  \intermed {  [  \overline {\intermed \sigma}_{\ottmv{j}}  /  {\overline {\intermed a} }_{\ottmv{j}}  ]  {\intermed \sigma}  } = \intermed {  [  \overline {\intermed \sigma}'_{\ottmv{m}}  /  {\overline {\intermed a} }'_{\ottmv{m}}  ]  {\intermed \sigma}'  } }%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
\ottpremise{\ldots}%
}{
 \vdash_{ctx}  \intermed {  {\intermed \Sigma}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  {\intermed e}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }{%
{\ottdrulename{iCtx\_MEnv\_simp}}{}%
}}

\newcommand{\ottdefnictxXXwf}[1]{\begin{ottdefnblock}[#1]{$ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } $}{}
\ottusedrule{\ottdruleiCtxXXempty{}}
\ottusedrule{\ottdruleiCtxXXtyEnvTm{}}
\ottusedrule{\ottdruleiCtxXXtyEnvTy{}}
\ottusedrule{\ottdruleiCtxXXtyEnvD{}}
\ottusedrule{\ottdruleiCtxXXclsEnv{}}
\ottusedrule{\ottdruleiCtxXXMEnv{}}
\ottusedrule{\ottdruleiCtxXXMEnvXXsimp{}}
\end{ottdefnblock}}

%% defn iunambigC
\newcommand{\ottdruleiUnambigXXconstraint}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\overline {\intermed a} }_{\ottmv{j}}  }  \in   \textbf {fv}  ( \intermed {  {\intermed \sigma}  } ) }%
}{
 \textbf {unambig}  ( \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } ) }{%
{\ottdrulename{iUnambig\_constraint}}{}%
}}

\newcommand{\ottdefniunambigC}[1]{\begin{ottdefnblock}[#1]{$ \textbf {unambig}  ( \intermed {  {\intermed C}  } ) $}{}
\ottusedrule{\ottdruleiUnambigXXconstraint{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsIctxXXwf}{
\ottdefnictxXXwf{}\ottdefniunambigC{}}

% defns Itm_ty
%% defn itm_ty
\newcommand{\ottdruleiTmXXtrue}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  \mathit{\intermed {True} }  } : \intermed {  \mathit{\intermed {Bool} }  } \itot{ \rightsquigarrow  \target {  \mathit{\target {True} }  } } }{%
{\ottdrulename{iTm\_true}}{}%
}}


\newcommand{\ottdruleiTmXXfalse}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  \mathit{\intermed {False} }  } : \intermed {  \mathit{\intermed {Bool} }  } \itot{ \rightsquigarrow  \target {  \mathit{\target {False} }  } } }{%
{\ottdrulename{iTm\_false}}{}%
}}


\newcommand{\ottdruleiTmXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ ( \intermed {  {\intermed x}  } : \intermed {  {\intermed \sigma}  } )  \in  \intermed {  {\intermed \Gamma}  } }%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed x}  } : \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target x}  } } }{%
{\ottdrulename{iTm\_var}}{}%
}}


\newcommand{\ottdruleiTmXXlet}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{1}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  \ottsym{=}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{iTm\_let}}{}%
}}


\newcommand{\ottdruleiTmXXmethod}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{d}  \intermed {  {\intermed d}  } : \intermed {  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } \itot{\,  \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ ( \intermed {  {\intermed m}  } : \intermed {  {\intermed {\mathit{TC} } } \, {\intermed a }  } : \intermed {  {\intermed \sigma}'  } )  \in  \intermed {  {\intermed { \Gamma_C } }  } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed d}  \ottsym{.}  {\intermed m}  } : \intermed {  [  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed \sigma}'  } \itot{ \rightsquigarrow  \target {  {\target e }  \ottsym{.}  {\target m}  } } }{%
{\ottdrulename{iTm\_method}}{}%
}}


\newcommand{\ottdruleiTmXXarrI}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  \lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  \ottsym{.}  {\intermed e}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{.}  {\target e }  } } }{%
{\ottdrulename{iTm\_arrI}}{}%
}}


\newcommand{\ottdruleiTmXXarrE}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{1}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{1}}} \, {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{iTm\_arrE}}{}%
}}


\newcommand{\ottdruleiTmXXconstrI}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed \delta }  \ottsym{:}  {\intermed Q}  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  \lambda  {\intermed \delta }  \ottsym{:}  {\intermed Q}  \ottsym{.}  {\intermed e}  } : \intermed {   {\intermed Q}  \Rightarrow  {\intermed \sigma}   } \itot{ \rightsquigarrow  \target {  \lambda  {\target \delta }  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target e }  } } }{%
{\ottdrulename{iTm\_constrI}}{}%
}}


\newcommand{\ottdruleiTmXXconstrE}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {   {\intermed Q}  \Rightarrow  {\intermed \sigma}   } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{d}  \intermed {  {\intermed d}  } : \intermed {  {\intermed Q}  } \itot{\,  \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e} \, {\intermed d}  } : \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{iTm\_constrE}}{}%
}}


\newcommand{\ottdruleiTmXXforallI}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed a }  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target e }  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  \Lambda  {\intermed a }  \ottsym{.}  {\intermed e}  } : \intermed {  \forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  \Lambda  {\target a }  \ottsym{.}  {\target e }  } } }{%
{\ottdrulename{iTm\_forallI}}{}%
}}


\newcommand{\ottdruleiTmXXforallE}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  \forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}'  } \itot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e} \, {\intermed \sigma}  } : \intermed {  [  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed \sigma}'  } \itot{ \rightsquigarrow  \target {  {\target e } \, {\target \sigma }  } } }{%
{\ottdrulename{iTm\_forallE}}{}%
}}

\newcommand{\ottdefnitmXXty}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target e }  } } $}{}
\ottusedrule{\ottdruleiTmXXtrue{}}
\ottusedrule{\ottdruleiTmXXfalse{}}
\ottusedrule{\ottdruleiTmXXvar{}}
\ottusedrule{\ottdruleiTmXXlet{}}
\ottusedrule{\ottdruleiTmXXmethod{}}
\ottusedrule{\ottdruleiTmXXarrI{}}
\ottusedrule{\ottdruleiTmXXarrE{}}
\ottusedrule{\ottdruleiTmXXconstrI{}}
\ottusedrule{\ottdruleiTmXXconstrE{}}
\ottusedrule{\ottdruleiTmXXforallI{}}
\ottusedrule{\ottdruleiTmXXforallE{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsItmXXty}{
\ottdefnitmXXty{}}

% defns D_ty
%% defn d_ty
\newcommand{\ottdruleDXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ ( \intermed {  {\intermed \delta }  } : \intermed {  {\intermed Q}  } )  \in  \intermed {  {\intermed \Gamma}  } }%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{d}  \intermed {  {\intermed \delta }  } : \intermed {  {\intermed Q}  } \itot{\,  \rightsquigarrow  \target {  {\target \delta }  } } }{%
{\ottdrulename{D\_var}}{}%
}}


\newcommand{\ottdruleDXXcon}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  } = \intermed {  {\intermed \Sigma}_{{\mathrm{1}}}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}_{\ottmv{q}}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  \ottsym{.}  {\intermed e}  \ottsym{,}  {\intermed \Sigma}_{{\mathrm{2}}}  } }%
\ottpremise{ \vdash_{ctx}  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
\ottpremise{\ottcomp{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  \ottsym{,}  {\overline {\intermed a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}_{\ottmv{i}}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }'_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{\ottcomp{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{\ottmv{j}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{j}}  } } }{\ottmv{j}}}%
\ottpremise{ \intermed {  {\intermed \Sigma}_{{\mathrm{1}}}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  \ottsym{,}  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  }  \vdash_{tm}  \intermed {  {\intermed e}  } : \intermed {  [  {\intermed \sigma}_{\ottmv{q}}  /  {\intermed a }  ]  {\intermed \sigma}_{\ottmv{m}}  } \itot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{\ottcomp{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{d}  \intermed {  {\intermed d}_{\ottmv{i}}  } : \intermed {  [  \overline {\intermed \sigma}_{\ottmv{j}}  /  {\overline {\intermed a} }_{\ottmv{j}}  ]  {\intermed Q}_{\ottmv{i}}  } \itot{\,  \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
}{
 \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{d}  \intermed {  {\intermed D } \, \overline {\intermed \sigma}_{\ottmv{j}} \, {\overline {\intermed d} }_{\ottmv{i}}  } : \intermed {  {\intermed {\mathit{TC} } } \, [  \overline {\intermed \sigma}_{\ottmv{j}}  /  {\overline {\intermed a} }_{\ottmv{j}}  ]  {\intermed \sigma}_{\ottmv{q}}  } \itot{\,  \rightsquigarrow  \target {  \ottsym{(}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{i}}  \ottsym{:}  {\target \sigma }'_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  \ottsym{\{}  {\target m}  \ottsym{=}  {\target e }  \ottsym{\}}  \ottsym{)} \, {\overline {\target \sigma} }_{\ottmv{j}} \, {\overline {\target e} }_{\ottmv{i}}  } } }{%
{\ottdrulename{D\_con}}{}%
}}

\newcommand{\ottdefndXXty}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \vdash_{d}  \intermed {  {\intermed d}  } : \intermed {  {\intermed Q}  } \itot{\,  \rightsquigarrow  \target {  {\target e }  } } $}{}
\ottusedrule{\ottdruleDXXvar{}}
\ottusedrule{\ottdruleDXXcon{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsDXXty}{
\ottdefndXXty{}}

% defns Ictx_typing
%% defn ictx_typing
\newcommand{\ottdruleiMXXempty}[1]{\ottdrule[#1]{%
}{
 \intermed {  \ottsym{[} \, \bullet \, \ottsym{]}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } ) \itot{ \rightsquigarrow  \target {  \ottsym{[} \, \bullet \, \ottsym{]}  } } }{%
{\ottdrulename{iM\_empty}}{}%
}}


\newcommand{\ottdruleiMXXabs}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  \lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target M }  } } }{%
{\ottdrulename{iM\_abs}}{}%
}}


\newcommand{\ottdruleiMXXappL}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
}{
 \intermed {  {\intermed M} \, {\intermed e}_{{\mathrm{2}}}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M } \, {\target e }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{iM\_appL}}{}%
}}


\newcommand{\ottdruleiMXXappR}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{1}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
}{
 \intermed {  {\intermed e}_{{\mathrm{1}}} \, {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}} \, {\target M }  } } }{%
{\ottdrulename{iM\_appR}}{}%
}}


\newcommand{\ottdruleiMXXdictAbs}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  \ottsym{,}  {\intermed \delta }  \ottsym{:}  {\intermed Q}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{\mathit {Q} }  \intermed {  {\intermed Q}  }\, \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  \lambda  {\intermed \delta }  \ottsym{:}  {\intermed Q}  \ottsym{.}  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {   {\intermed Q}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   } ) \itot{ \rightsquigarrow  \target {  \lambda  {\target \delta }  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target M }  } } }{%
{\ottdrulename{iM\_dictAbs}}{}%
}}


\newcommand{\ottdruleiMXXdictApp}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {   {\intermed Q}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{d}  \intermed {  {\intermed d}  } : \intermed {  {\intermed Q}  } \itot{\,  \rightsquigarrow  \target {  {\target e }  } } }%
}{
 \intermed {  {\intermed M} \, {\intermed d}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M } \, {\target e }  } } }{%
{\ottdrulename{iM\_dictApp}}{}%
}}


\newcommand{\ottdruleiMXXtyAbs}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  \ottsym{,}  {\intermed a }  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
}{
 \intermed {  \Lambda  {\intermed a }  \ottsym{.}  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  \forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  \Lambda  {\target a }  \ottsym{.}  {\target M }  } } }{%
{\ottdrulename{iM\_tyAbs}}{}%
}}


\newcommand{\ottdruleiMXXtyApp}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  \forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{ty}  \intermed {  {\intermed \sigma}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }  } } }%
}{
 \intermed {  {\intermed M} \, {\intermed \sigma}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  [  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M } \, {\target \sigma }  } } }{%
{\ottdrulename{iM\_tyApp}}{}%
}}


\newcommand{\ottdruleiMXXletL}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } } }%
}{
 \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  \ottsym{=}  {\intermed M} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  {\target M } \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{iM\_letL}}{}%
}}


\newcommand{\ottdruleiMXXletR}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } }%
\ottpremise{ \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{tm}  \intermed {  {\intermed e}_{{\mathrm{1}}}  } : \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \vdash_{ty}  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } \itot{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } } }%
}{
 \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}_{{\mathrm{1}}}  \ottsym{=}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } ) \itot{ \rightsquigarrow  \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target M }  } } }{%
{\ottdrulename{iM\_letR}}{}%
}}

\newcommand{\ottdefnictxXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed M}  } : ( \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  }  \Rightarrow  \intermed {  {\intermed \sigma}  } )  \mapsto  ( \intermed {  {\intermed \Sigma}'  } ; \intermed {  {\intermed { \Gamma_C } }'  } ; \intermed {  {\intermed \Gamma}'  }  \Rightarrow  \intermed {  {\intermed \sigma}'  } ) \itot{ \rightsquigarrow  \target {  {\target M }  } } $}{}
\ottusedrule{\ottdruleiMXXempty{}}
\ottusedrule{\ottdruleiMXXabs{}}
\ottusedrule{\ottdruleiMXXappL{}}
\ottusedrule{\ottdruleiMXXappR{}}
\ottusedrule{\ottdruleiMXXdictAbs{}}
\ottusedrule{\ottdruleiMXXdictApp{}}
\ottusedrule{\ottdruleiMXXtyAbs{}}
\ottusedrule{\ottdruleiMXXtyApp{}}
\ottusedrule{\ottdruleiMXXletL{}}
\ottusedrule{\ottdruleiMXXletR{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsIctxXXtyping}{
\ottdefnictxXXtyping{}}

% defns Ievaluate
%% defn i_eval
\newcommand{\ottdruleiEvalXXapp}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e}_{{\mathrm{1}}}  }  \longrightarrow  \intermed {  {\intermed e}'_{{\mathrm{1}}}  } }%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e}_{{\mathrm{1}}} \, {\intermed e}_{{\mathrm{2}}}  }  \longrightarrow  \intermed {  {\intermed e}'_{{\mathrm{1}}} \, {\intermed e}_{{\mathrm{2}}}  } }{%
{\ottdrulename{iEval\_app}}{}%
}}


\newcommand{\ottdruleiEvalXXappAbs}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  \ottsym{(}  \lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed e}_{{\mathrm{1}}}  \ottsym{)} \, {\intermed e}_{{\mathrm{2}}}  }  \longrightarrow  \intermed {  [  {\intermed e}_{{\mathrm{2}}}  /  {\intermed x}  ]  {\intermed e}_{{\mathrm{1}}}  } }{%
{\ottdrulename{iEval\_appAbs}}{}%
}}


\newcommand{\ottdruleiEvalXXtyApp}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e}  }  \longrightarrow  \intermed {  {\intermed e}'  } }%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e} \, {\intermed \sigma}  }  \longrightarrow  \intermed {  {\intermed e}' \, {\intermed \sigma}  } }{%
{\ottdrulename{iEval\_tyApp}}{}%
}}


\newcommand{\ottdruleiEvalXXtyAppAbs}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  \ottsym{(}  \Lambda  {\intermed a }  \ottsym{.}  {\intermed e}  \ottsym{)} \, {\intermed \sigma}  }  \longrightarrow  \intermed {  [  {\intermed \sigma}  /  {\intermed a }  ]  {\intermed e}  } }{%
{\ottdrulename{iEval\_tyAppAbs}}{}%
}}


\newcommand{\ottdruleiEvalXXDApp}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e}  }  \longrightarrow  \intermed {  {\intermed e}'  } }%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e} \, {\intermed d}  }  \longrightarrow  \intermed {  {\intermed e}' \, {\intermed d}  } }{%
{\ottdrulename{iEval\_DApp}}{}%
}}


\newcommand{\ottdruleiEvalXXDAppAbs}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  \ottsym{(}  \lambda  {\intermed \delta }  \ottsym{:}  {\intermed Q}  \ottsym{.}  {\intermed e}  \ottsym{)} \, {\intermed d}  }  \longrightarrow  \intermed {  [  {\intermed d}  /  {\intermed \delta }  ]  {\intermed e}  } }{%
{\ottdrulename{iEval\_DAppAbs}}{}%
}}


\newcommand{\ottdruleiEvalXXmethod}[1]{\ottdrule[#1]{%
\ottpremise{ ( \intermed {  {\intermed D }  } : \intermed {  {\intermed C}  } ) . \intermed {  {\intermed m}  }  \mapsto  \intermed {  {\intermed e}  }  \in  \intermed {  {\intermed \Sigma}  } }%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  \ottsym{(}  {\intermed D } \, \overline {\intermed \sigma} \, {\overline {\intermed d} }  \ottsym{)}  \ottsym{.}  {\intermed m}  }  \longrightarrow  \intermed {  {\intermed e} \, \overline {\intermed \sigma} \, {\overline {\intermed d} }  } }{%
{\ottdrulename{iEval\_method}}{}%
}}


\newcommand{\ottdruleiEvalXXlet}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{=}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  }  \longrightarrow  \intermed {  [  {\intermed e}_{{\mathrm{1}}}  /  {\intermed x}  ]  {\intermed e}_{{\mathrm{2}}}  } }{%
{\ottdrulename{iEval\_let}}{}%
}}

\newcommand{\ottdefniXXeval}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed \Sigma}  }  \vdash  \intermed {  {\intermed e}  }  \longrightarrow  \intermed {  {\intermed e}'  } $}{}
\ottusedrule{\ottdruleiEvalXXapp{}}
\ottusedrule{\ottdruleiEvalXXappAbs{}}
\ottusedrule{\ottdruleiEvalXXtyApp{}}
\ottusedrule{\ottdruleiEvalXXtyAppAbs{}}
\ottusedrule{\ottdruleiEvalXXDApp{}}
\ottusedrule{\ottdruleiEvalXXDAppAbs{}}
\ottusedrule{\ottdruleiEvalXXmethod{}}
\ottusedrule{\ottdruleiEvalXXlet{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsIevaluate}{
\ottdefniXXeval{}}

% defns CtxLog
%% defn ctx_log
\newcommand{\ottdrulectxLogXXempty}[1]{\ottdrule[#1]{%
}{
 \intermed {  {\intermed { \Gamma_C } }  }  \vdash  \intermed {  \bullet  }  \simeq_{log}  \intermed {  \bullet  } }{%
{\ottdrulename{ctxLog\_empty}}{}%
}}


\newcommand{\ottdrulectxLogXXcons}[1]{\ottdrule[#1]{%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  }  \vdash  \intermed {  {\intermed \Sigma}_{{\mathrm{1}}}  }  \simeq_{log}  \intermed {  {\intermed \Sigma}_{{\mathrm{2}}}  } }%
\ottpremise{ \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  }  \vdash  \intermed {  {\intermed \Sigma}_{{\mathrm{1}}}  } : \intermed {  {\intermed e}_{{\mathrm{1}}}  }  \simeq_{log}  \intermed {  {\intermed \Sigma}_{{\mathrm{2}}}  } : \intermed {  {\intermed e}_{{\mathrm{2}}}  } : \intermed {  {\intermed \sigma}'  } }%
}{
 \intermed {  {\intermed { \Gamma_C } }  }  \vdash  \intermed {  {\intermed \Sigma}_{{\mathrm{1}}}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  {\intermed e}_{{\mathrm{1}}}  }  \simeq_{log}  \intermed {  {\intermed \Sigma}_{{\mathrm{2}}}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  {\intermed e}_{{\mathrm{2}}}  } }{%
{\ottdrulename{ctxLog\_cons}}{}%
}}

\newcommand{\ottdefnctxXXlog}[1]{\begin{ottdefnblock}[#1]{$ \intermed {  {\intermed { \Gamma_C } }  }  \vdash  \intermed {  {\intermed \Sigma}_{{\mathrm{1}}}  }  \simeq_{log}  \intermed {  {\intermed \Sigma}_{{\mathrm{2}}}  } $}{}
\ottusedrule{\ottdrulectxLogXXempty{}}
\ottusedrule{\ottdrulectxLogXXcons{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsCtxLog}{
\ottdefnctxXXlog{}}

% defns Sty_wfT
%% defn sq_wfT
\newcommand{\ottdrulesQTXXTC}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }'  } } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } = \source {  {\source { \Gamma_C } }_{{\mathrm{1}}}  }, \source {  {\source m}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  {\source \sigma}  }, \source {  {\source { \Gamma_C } }_{{\mathrm{2}}}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }_{{\mathrm{1}}}  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }  \source {  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \target {  [  {\target \sigma }'  /  {\target a }  ]  \ottsym{\{}  {\target m}  \ottsym{:}  {\target \sigma }  \ottsym{\}}  } }{%
{\ottdrulename{sQT\_TC}}{}%
}}

\newcommand{\ottdefnsqXXwfT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}  }  \rightsquigarrow  \target {  {\target \sigma }  } $}{}
\ottusedrule{\ottdrulesQTXXTC{}}
\end{ottdefnblock}}

%% defn sc_wfT
\newcommand{\ottdrulesCTXXabs}[1]{\ottdrule[#1]{%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}_{\ottmv{i}}  }  \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}  }  \rightsquigarrow  \target {  {\target \sigma }  } }%
\ottpremise{ \source {  {\overline {\source a} }_{\ottmv{j}}  }  \notin  \source {  {\source \Gamma}  } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {C} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source Q}  }  \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }  } }{%
{\ottdrulename{sCT\_abs}}{}%
}}

\newcommand{\ottdefnscXXwfT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {C} }  \source {  {\source C}  }  \rightsquigarrow  \target {  {\target \sigma }  } $}{}
\ottusedrule{\ottdrulesCTXXabs{}}
\end{ottdefnblock}}

%% defn sty_wfT
\newcommand{\ottdrulesTyTXXbool}[1]{\ottdrule[#1]{%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  \mathit{\source {Bool} }  }\,{ \stoi{ \rightsquigarrow  \target {  \mathit{\target {Bool} }  } } } }{%
{\ottdrulename{sTyT\_bool}}{}%
}}


\newcommand{\ottdrulesTyTXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source a }  }  \in  \source {  {\source \Gamma}  } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source a }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target a }  } } } }{%
{\ottdrulename{sTyT\_var}}{}%
}}


\newcommand{\ottdrulesTyTXXarrow}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{{\mathrm{2}}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } } } }{%
{\ottdrulename{sTyT\_arrow}}{}%
}}


\newcommand{\ottdrulesTyTXXqual}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}  }  \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \rho}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{2}}}  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source Q}  \Rightarrow  {\source \rho}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{{\mathrm{1}}}  \rightarrow  {\target \sigma }_{{\mathrm{2}}}  } } } }{%
{\ottdrulename{sTyT\_qual}}{}%
}}


\newcommand{\ottdrulesTyTXXscheme}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source a }  }  \notin  \source {  {\source \Gamma}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source a }  }  \vdash_{ty}  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  \forall  {\source a }  \ottsym{.}  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\target a }  \ottsym{.}  {\target \sigma }  } } } }{%
{\ottdrulename{sTyT\_scheme}}{}%
}}

\newcommand{\ottdefnstyXXwfT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } $}{}
\ottusedrule{\ottdrulesTyTXXbool{}}
\ottusedrule{\ottdrulesTyTXXvar{}}
\ottusedrule{\ottdrulesTyTXXarrow{}}
\ottusedrule{\ottdrulesTyTXXqual{}}
\ottusedrule{\ottdrulesTyTXXscheme{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsStyXXwfT}{
\ottdefnsqXXwfT{}\ottdefnscXXwfT{}\ottdefnstyXXwfT{}}

% defns Sty_wf
%% defn sq_wf
\newcommand{\ottdrulesQXXTC}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } = \source {  {\source { \Gamma_C } }_{{\mathrm{1}}}  }, \source {  {\source m}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  {\source \sigma}  }, \source {  {\source { \Gamma_C } }_{{\mathrm{2}}}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }_{{\mathrm{1}}}  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}'  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \intermed {  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } }{%
{\ottdrulename{sQ\_TC}}{}%
}}

\newcommand{\ottdefnsqXXwf}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source Q}  }  \rightsquigarrow  \intermed {  {\intermed Q}  } $}{}
\ottusedrule{\ottdrulesQXXTC{}}
\end{ottdefnblock}}

%% defn sc_wf
\newcommand{\ottdrulesCXXabs}[1]{\ottdrule[#1]{%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source Q}_{\ottmv{i}}  }  \rightsquigarrow  \intermed {  {\intermed Q}_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source Q}  }  \rightsquigarrow  \intermed {  {\intermed Q}  } }%
\ottpremise{ \source {  {\overline {\source a} }_{\ottmv{j}}  }  \notin  \source {  {\source \Gamma}  } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {C} }^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source Q}  }  \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed Q}  } }{%
{\ottdrulename{sC\_abs}}{}%
}}

\newcommand{\ottdefnscXXwf}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {C} }^{\intermed {M} }  \source {  {\source C}  }  \rightsquigarrow  \intermed {  {\intermed C}  } $}{}
\ottusedrule{\ottdrulesCXXabs{}}
\end{ottdefnblock}}

%% defn sty_wf
\newcommand{\ottdrulesTyXXbool}[1]{\ottdrule[#1]{%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  \mathit{\source {Bool} }  }\,{ \stoi{ \rightsquigarrow  \intermed {  \mathit{\intermed {Bool} }  } } } }{%
{\ottdrulename{sTy\_bool}}{}%
}}


\newcommand{\ottdrulesTyXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source a }  }  \in  \source {  {\source \Gamma}  } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source a }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed a }  } } } }{%
{\ottdrulename{sTy\_var}}{}%
}}


\newcommand{\ottdrulesTyXXarrow}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  } } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{{\mathrm{2}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}_{{\mathrm{2}}}  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}_{{\mathrm{1}}}  \rightarrow  {\intermed \sigma}_{{\mathrm{2}}}  } } } }{%
{\ottdrulename{sTy\_arrow}}{}%
}}


\newcommand{\ottdrulesTyXXqual}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source Q}  }  \rightsquigarrow  \intermed {  {\intermed Q}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \rho}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source Q}  \Rightarrow  {\source \rho}  }\,{ \stoi{ \rightsquigarrow  \intermed {   {\intermed Q}  \Rightarrow  {\intermed \sigma}   } } } }{%
{\ottdrulename{sTy\_qual}}{}%
}}


\newcommand{\ottdrulesTyXXscheme}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source a }  }  \notin  \source {  {\source \Gamma}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source a }  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
}{
 \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\source a }  \ottsym{.}  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\intermed a }  \ottsym{.}  {\intermed \sigma}  } } } }{%
{\ottdrulename{sTy\_scheme}}{}%
}}

\newcommand{\ottdefnstyXXwf}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } $}{}
\ottusedrule{\ottdrulesTyXXbool{}}
\ottusedrule{\ottdrulesTyXXvar{}}
\ottusedrule{\ottdrulesTyXXarrow{}}
\ottusedrule{\ottdrulesTyXXqual{}}
\ottusedrule{\ottdrulesTyXXscheme{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsStyXXwf}{
\ottdefnsqXXwf{}\ottdefnscXXwf{}\ottdefnstyXXwf{}}

% defns Sctx_wfT
%% defn sctx_wfT
\newcommand{\ottdrulesCtxTXXempty}[1]{\ottdrule[#1]{%
}{
 \vdash_{ctx}  \source {  \bullet  } ; \source {  \bullet  } ; \source {  \bullet  }  \rightsquigarrow  \target {  \target {\bullet}  } }{%
{\ottdrulename{sCtxT\_empty}}{}%
}}


\newcommand{\ottdrulesCtxTXXtyEnvTm}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  {\source \sigma}  }  \rightsquigarrow  \target {  {\target \Gamma }  \ottsym{,}  {\target x}  \ottsym{:}  {\target \sigma }  } }{%
{\ottdrulename{sCtxT\_tyEnvTm}}{}%
}}


\newcommand{\ottdrulesCtxTXXtyEnvTy}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source a }  }  \notin  \source {  {\source \Gamma}  } }%
\ottpremise{ \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source a }  }  \rightsquigarrow  \target {  {\target \Gamma }  \ottsym{,}  {\target a }  } }{%
{\ottdrulename{sCtxT\_tyEnvTy}}{}%
}}


\newcommand{\ottdrulesCtxTXXtyEnvD}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }  \source {  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \target {  {\target \sigma }  } }%
\ottpremise{ \source {  {\source \delta }  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source \delta }  \ottsym{:}  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \target {  {\target \Gamma }  \ottsym{,}  {\target \delta }  \ottsym{:}  {\target \sigma }  } }{%
{\ottdrulename{sCtxT\_tyEnvD}}{}%
}}


\newcommand{\ottdrulesCtxTXXclsEnv}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  \ottcomp{{\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }}{\ottmv{i}}  \Rightarrow  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
\ottpremise{ \source {  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  } =  \textbf {fv}  ( \source {  {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{\mathit {Q} }  \source {  {\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }  }  \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{ \source {  {\source m}  }  \notin   \textbf {dom}  ( \source {  {\source { \Gamma_C } }  } ) }%
\ottpremise{ \source {  {\source {\mathit{TC} } } \, {\source b }  }  \notin   \textbf {dom}  ( \source {  {\source { \Gamma_C } }  } ) }%
\ottpremise{ \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  }  \rightsquigarrow  \target {  \target {\bullet}  } }%
}{
 \vdash_{ctx}  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  \ottsym{,}  {\source m}  \ottsym{:}  \overline {\source {\mathit{TC}_i~a } }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  \ottcomp{{\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }}{\ottmv{i}}  \Rightarrow  {\source \tau }  } ; \source {  \bullet  }  \rightsquigarrow  \target {  \target {\bullet}  } }{%
{\ottdrulename{sCtxT\_clsEnv}}{}%
}}


\newcommand{\ottdrulesCtxTXXpgmInst}[1]{\ottdrule[#1]{%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  }  \vdash_{\mathit {C} }  \source {  \forall  {\overline {\source b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \target {  \forall  {\overline {\target b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  [  {\target \sigma }  /  {\target a }  ]  \ottsym{\{}  {\target m}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{k}}  \ottsym{.}  {\overline {\target \sigma} }'_{\ottmv{h}}  \rightarrow  {\target \sigma }'  \ottsym{\}}  } }%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{h}}  \Rightarrow  {\source \tau }'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{h}}  \Rightarrow  {\source \tau }'  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{k}}  \ottsym{.}  {\overline {\target \sigma} }'_{\ottmv{h}}  \rightarrow  {\target \sigma }'  } } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{j}}  }  \vdash_{ty}  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }'  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \source {  {\source D }  }  \notin   \textbf {dom}  ( \source {  { \source P }  } ) }%
\ottpremise{ ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }''_{\ottmv{h}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }''  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  } }%
\ottpremise{ \textbf {where}  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source b} }_{\ottmv{j}}  ]  {\source \tau }  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }'_{\ottmv{k}}  ]  {\source \tau }''  } }%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \vdash_{ctx}  \source {  { \source P }  \ottsym{,}  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  \ottsym{:}  {\source e}  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }{%
{\ottdrulename{sCtxT\_pgmInst}}{}%
}}

\newcommand{\ottdefnsctxXXwfT}[1]{\begin{ottdefnblock}[#1]{$ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } $}{}
\ottusedrule{\ottdrulesCtxTXXempty{}}
\ottusedrule{\ottdrulesCtxTXXtyEnvTm{}}
\ottusedrule{\ottdrulesCtxTXXtyEnvTy{}}
\ottusedrule{\ottdrulesCtxTXXtyEnvD{}}
\ottusedrule{\ottdrulesCtxTXXclsEnv{}}
\ottusedrule{\ottdrulesCtxTXXpgmInst{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSctxXXwfT}{
\ottdefnsctxXXwfT{}}

% defns Sctx_wf
%% defn sctx_wf
\newcommand{\ottdrulesCtxXXempty}[1]{\ottdrule[#1]{%
}{
 \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  \bullet  } ; \source {  \bullet  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  \bullet  } ; \intermed {  \bullet  } }{%
{\ottdrulename{sCtx\_empty}}{}%
}}


\newcommand{\ottdrulesCtxXXtyEnvTm}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \sigma}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  {\source \sigma}  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed x}  \ottsym{:}  {\intermed \sigma}  } }{%
{\ottdrulename{sCtx\_tyEnvTm}}{}%
}}


\newcommand{\ottdrulesCtxXXtyEnvTy}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source a }  }  \notin  \source {  {\source \Gamma}  } }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source a }  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed a }  } }{%
{\ottdrulename{sCtx\_tyEnvTy}}{}%
}}


\newcommand{\ottdrulesCtxXXtyEnvD}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \intermed {  {\intermed Q}  } }%
\ottpremise{ \source {  {\source \delta }  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source \delta }  \ottsym{:}  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  \ottsym{,}  {\intermed \delta }  \ottsym{:}  {\intermed Q}  } }{%
{\ottdrulename{sCtx\_tyEnvD}}{}%
}}


\newcommand{\ottdrulesCtxXXclsEnv}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  \ottcomp{{\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }}{\ottmv{i}}  \Rightarrow  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
\ottpremise{ \source {  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  } =  \textbf {fv}  ( \source {  {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }  }  \rightsquigarrow  \intermed {  {\intermed Q}_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{ \source {  {\source m}  }  \notin   \textbf {dom}  ( \source {  {\source { \Gamma_C } }  } ) }%
\ottpremise{ \source {  {\source {\mathit{TC} } } \, {\source b }  }  \notin   \textbf {dom}  ( \source {  {\source { \Gamma_C } }  } ) }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  \bullet  } }%
}{
 \vdash_{ctx}^{\intermed {M} }  \source {  \bullet  } ; \source {  {\source { \Gamma_C } }  \ottsym{,}  {\source m}  \ottsym{:}  \overline {\source {\mathit{TC}_i~a } }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  \ottcomp{{\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }}{\ottmv{i}}  \Rightarrow  {\source \tau }  } ; \source {  \bullet  }  \rightsquigarrow  \intermed {  \bullet  } ; \intermed {  {\intermed { \Gamma_C } }  \ottsym{,}  {\intermed m}  \ottsym{:}  {\intermed {\mathit{TC} } } \, {\intermed a }  \ottsym{:}  {\intermed \sigma}  } ; \intermed {  \bullet  } }{%
{\ottdrulename{sCtx\_clsEnv}}{}%
}}


\newcommand{\ottdrulesCtxXXpgmInst}[1]{\ottdrule[#1]{%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  }  \vdash_{\mathit {C} }^{\intermed {M} }  \source {  \forall  {\overline {\source b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  }  \rightsquigarrow  \intermed {  \forall  {\overline {\intermed b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  } }%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{h}}  \Rightarrow  {\source \tau }'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }_{\ottmv{h}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }'  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{h}}  \Rightarrow  {\source \tau }'  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{k}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{h}}  \Rightarrow  {\intermed \sigma}'   } } } }%
\ottpremise{ \source {  {\source D }  }  \notin   \textbf {dom}  ( \source {  { \source P }  } ) }%
\ottpremise{ ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }''_{\ottmv{h}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }''  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  } }%
\ottpremise{ \textbf {where}  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source b} }_{\ottmv{j}}  ]  {\source \tau }  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }'_{\ottmv{k}}  ]  {\source \tau }''  } }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
\ottpremise{ \intermed {  {\intermed \Sigma}'  } = \intermed {  {\intermed \Sigma}  \ottsym{,}  \ottsym{(}  {\intermed D }  \ottsym{:}  \forall  {\overline {\intermed b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed {\mathit{TC} } } \, {\intermed \sigma}  \ottsym{)}  \ottsym{.}  {\intermed m}  \mapsto  \Lambda  {\overline {\intermed b} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  \ottsym{.}  \Lambda  {\overline {\intermed a} }_{\ottmv{k}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\intermed \sigma}  /  {\intermed a }  ]  {\overline {\intermed Q} }_{\ottmv{h}}  \ottsym{.}  {\intermed e}  } }%
}{
 \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  \ottsym{,}  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }_{\ottmv{h}}  \ottsym{:}  {\source e}  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}'  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }{%
{\ottdrulename{sCtx\_pgmInst}}{}%
}}

\newcommand{\ottdefnsctxXXwf}[1]{\begin{ottdefnblock}[#1]{$ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } $}{}
\ottusedrule{\ottdrulesCtxXXempty{}}
\ottusedrule{\ottdrulesCtxXXtyEnvTm{}}
\ottusedrule{\ottdrulesCtxXXtyEnvTy{}}
\ottusedrule{\ottdrulesCtxXXtyEnvD{}}
\ottusedrule{\ottdrulesCtxXXclsEnv{}}
\ottusedrule{\ottdrulesCtxXXpgmInst{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSctxXXwf}{
\ottdefnsctxXXwf{}}

% defns Stm_typingT
%% defn stm_inf_typingT
\newcommand{\ottdrulesTmXXinfTXXtrue}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  \mathit{\source {True} }  } \Rightarrow \source {  \mathit{\source {Bool} }  } \stot{ \rightsquigarrow  \target {  \mathit{\target {True} }  } } }{%
{\ottdrulename{sTm\_infT\_true}}{}%
}}


\newcommand{\ottdrulesTmXXinfTXXfalse}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  \mathit{\source {False} }  } \Rightarrow \source {  \mathit{\source {Bool} }  } \stot{ \rightsquigarrow  \target {  \mathit{\target {False} }  } } }{%
{\ottdrulename{sTm\_infT\_false}}{}%
}}


\newcommand{\ottdrulesTmXXinfTXXlet}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{k}}  } }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}_{\ottmv{k}}  }  \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{k}}  } }{\ottmv{k}}}%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{k}}  \rightarrow  {\target \sigma }  } } } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{k}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{k}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{k}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
\ottpremise{ \target {  {\target e }  } = \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{k}}  \rightarrow  {\target \sigma }  \ottsym{=}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{k}}  \ottsym{:}  {\target \sigma }_{\ottmv{k}}}{\ottmv{k}} \, \ottsym{.}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }{%
{\ottdrulename{sTm\_infT\_let}}{}%
}}


\newcommand{\ottdrulesTmXXinfTXXletXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{k}}  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{k}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{k}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
\ottpremise{ \target {  {\target e }  } = \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{k}}  \rightarrow  {\target \sigma }  \ottsym{=}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{k}}  \ottsym{:}  {\target \sigma }_{\ottmv{k}}}{\ottmv{k}} \, \ottsym{.}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }{%
{\ottdrulename{sTm\_infT\_let\_simp}}{}%
}}


\newcommand{\ottdrulesTmXXinfTXXArrE}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}} \, {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}} \, {\target e }_{{\mathrm{2}}}  } } }{%
{\ottdrulename{sTm\_infT\_ArrE}}{}%
}}


\newcommand{\ottdrulesTmXXinfTXXAnn}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}  ::  {\source \tau }  } \Rightarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }{%
{\ottdrulename{sTm\_infT\_Ann}}{}%
}}

\newcommand{\ottdefnstmXXinfXXtypingT}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } $}{}
\ottusedrule{\ottdrulesTmXXinfTXXtrue{}}
\ottusedrule{\ottdrulesTmXXinfTXXfalse{}}
\ottusedrule{\ottdrulesTmXXinfTXXlet{}}
\ottusedrule{\ottdrulesTmXXinfTXXletXXsimp{}}
\ottusedrule{\ottdrulesTmXXinfTXXArrE{}}
\ottusedrule{\ottdrulesTmXXinfTXXAnn{}}
\end{ottdefnblock}}

%% defn stm_check_typingT
\newcommand{\ottdrulesTmXXcheckTXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source x}  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }  } )  \in  \source {  {\source \Gamma}  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source Q}_{\ottmv{i}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{\ottmv{j}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{j}}  } } } }{\ottmv{j}}}%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source x}  } \Leftarrow \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target x} \, {\overline {\target \sigma} }_{\ottmv{j}} \, {\overline {\target e} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sTm\_checkT\_var}}{}%
}}


\newcommand{\ottdrulesTmXXcheckTXXmeth}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{k}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  {\source {\mathit{TC} } } \, {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source Q}_{\ottmv{i}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{\ottmv{j}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{j}}  } } } }{\ottmv{j}}}%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source m}  } \Leftarrow \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source \tau }'  } \stot{ \rightsquigarrow  \target {  {\target e }  \ottsym{.}  {\target m} \, {\overline {\target \sigma} }_{\ottmv{j}} \, {\overline {\target e} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sTm\_checkT\_meth}}{}%
}}


\newcommand{\ottdrulesTmXXcheckTXXmethXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{k}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  {\source {\mathit{TC} } } \, {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source Q}_{\ottmv{i}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source m}  } \Leftarrow \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source \tau }'  } \stot{ \rightsquigarrow  \target {  {\target e }  \ottsym{.}  {\target m} \, {\overline {\target \sigma} }_{\ottmv{j}} \, {\overline {\target e} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sTm\_checkT\_meth\_simp}}{}%
}}


\newcommand{\ottdrulesTmXXcheckTXXArrI}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  \lambda  {\source x}  \ottsym{.}  {\source e}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target e }  } } }{%
{\ottdrulename{sTm\_checkT\_ArrI}}{}%
}}


\newcommand{\ottdrulesTmXXcheckTXXInf}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }{%
{\ottdrulename{sTm\_checkT\_Inf}}{}%
}}

\newcommand{\ottdefnstmXXcheckXXtypingT}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } $}{}
\ottusedrule{\ottdrulesTmXXcheckTXXvar{}}
\ottusedrule{\ottdrulesTmXXcheckTXXmeth{}}
\ottusedrule{\ottdrulesTmXXcheckTXXmethXXsimp{}}
\ottusedrule{\ottdrulesTmXXcheckTXXArrI{}}
\ottusedrule{\ottdrulesTmXXcheckTXXInf{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsStmXXtypingT}{
\ottdefnstmXXinfXXtypingT{}\ottdefnstmXXcheckXXtypingT{}}

% defns Stm_typing
%% defn stm_inf_typing
\newcommand{\ottdrulesTmXXinfXXtrue}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  \mathit{\source {True} }  } \Rightarrow \source {  \mathit{\source {Bool} }  } \stoi{ \rightsquigarrow  \intermed {  \mathit{\intermed {True} }  } } }{%
{\ottdrulename{sTm\_inf\_true}}{}%
}}


\newcommand{\ottdrulesTmXXinfXXfalse}[1]{\ottdrule[#1]{%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  \mathit{\source {False} }  } \Rightarrow \source {  \mathit{\source {Bool} }  } \stoi{ \rightsquigarrow  \intermed {  \mathit{\intermed {False} }  } } }{%
{\ottdrulename{sTm\_inf\_false}}{}%
}}


\newcommand{\ottdrulesTmXXinfXXlet}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{k}}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{k}}  \Rightarrow  {\intermed \sigma}   } } } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{k}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{k}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{k}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
\ottpremise{ \intermed {  {\intermed e}  } = \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{k}}  \Rightarrow  {\intermed \sigma}   \ottsym{=}  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{k}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{k}}  \ottsym{.}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }{%
{\ottdrulename{sTm\_inf\_let}}{}%
}}


\newcommand{\ottdrulesTmXXinfXXletXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{k}}  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{k}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{k}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
\ottpremise{ \intermed {  {\intermed e}  } = \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{k}}  \Rightarrow  {\intermed \sigma}   \ottsym{=}  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{k}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{k}}  \ottsym{.}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }{%
{\ottdrulename{sTm\_inf\_let\_simp}}{}%
}}


\newcommand{\ottdrulesTmXXinfXXArrE}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}} \, {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}} \, {\intermed e}_{{\mathrm{2}}}  } } }{%
{\ottdrulename{sTm\_inf\_ArrE}}{}%
}}


\newcommand{\ottdrulesTmXXinfXXAnn}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  ::  {\source \tau }  } \Rightarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }{%
{\ottdrulename{sTm\_inf\_Ann}}{}%
}}

\newcommand{\ottdefnstmXXinfXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } $}{}
\ottusedrule{\ottdrulesTmXXinfXXtrue{}}
\ottusedrule{\ottdrulesTmXXinfXXfalse{}}
\ottusedrule{\ottdrulesTmXXinfXXlet{}}
\ottusedrule{\ottdrulesTmXXinfXXletXXsimp{}}
\ottusedrule{\ottdrulesTmXXinfXXArrE{}}
\ottusedrule{\ottdrulesTmXXinfXXAnn{}}
\end{ottdefnblock}}

%% defn stm_check_typing
\newcommand{\ottdrulesTmXXcheckXXvar}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source x}  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }  } )  \in  \source {  {\source \Gamma}  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source Q}_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{\ottmv{j}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}_{\ottmv{j}}  } } } }{\ottmv{j}}}%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source x}  } \Leftarrow \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed x} \, \overline {\intermed \sigma}_{\ottmv{j}} \, {\overline {\intermed d} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sTm\_check\_var}}{}%
}}


\newcommand{\ottdrulesTmXXcheckXXmeth}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{k}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  {\source {\mathit{TC} } } \, {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source Q}_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{\ottmv{j}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}_{\ottmv{j}}  } } } }{\ottmv{j}}}%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source m}  } \Leftarrow \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source \tau }'  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}  \ottsym{.}  {\intermed m} \, \overline {\intermed \sigma}_{\ottmv{j}} \, {\overline {\intermed d} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sTm\_check\_meth}}{}%
}}


\newcommand{\ottdrulesTmXXcheckXXmethXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{k}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  {\source {\mathit{TC} } } \, {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}  } } }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source Q}_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}_{\ottmv{i}}  } } }{\ottmv{i}}}%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source m}  } \Leftarrow \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  [  {\source \tau }  /  {\source a }  ]  {\source \tau }'  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}  \ottsym{.}  {\intermed m} \, \overline {\intermed \tau}_{\ottmv{j}} \, {\overline {\intermed d} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sTm\_check\_meth\_simp}}{}%
}}


\newcommand{\ottdrulesTmXXcheckXXArrI}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  \ottsym{,}  {\source x}  \ottsym{:}  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  \lambda  {\source x}  \ottsym{.}  {\source e}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  \lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed e}  } } }{%
{\ottdrulename{sTm\_check\_ArrI}}{}%
}}


\newcommand{\ottdrulesTmXXcheckXXInf}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }{%
{\ottdrulename{sTm\_check\_Inf}}{}%
}}

\newcommand{\ottdefnstmXXcheckXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } $}{}
\ottusedrule{\ottdrulesTmXXcheckXXvar{}}
\ottusedrule{\ottdrulesTmXXcheckXXmeth{}}
\ottusedrule{\ottdrulesTmXXcheckXXmethXXsimp{}}
\ottusedrule{\ottdrulesTmXXcheckXXArrI{}}
\ottusedrule{\ottdrulesTmXXcheckXXInf{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsStmXXtyping}{
\ottdefnstmXXinfXXtyping{}\ottdefnstmXXcheckXXtyping{}}

% defns Spgm_typingT
%% defn scls_typingT
\newcommand{\ottdrulesClsTXXcls}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source m}  }  \notin   \textbf {dom}  ( \source {  {\source { \Gamma_C } }  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{k}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{p}}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{\mathit {Q} }  \source {  {\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }  }  \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{ \nexists  \source {  {\source {\mathit{TC} } }'  } : ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }'  }~\source {  {\source b }  } : \source {  {\source \sigma}'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \nexists  \source {  {\source m}'  } : ( \source {  {\source m}'  } : \source {  {\overline {\source Q} }'_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  {\source \sigma}'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
}{
 \source {  {\source { \Gamma_C } }  }  \vdash_{cls}  \source {  \textbf{\source {class} } \, \overline {\source {\mathit{TC}_i~a } }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }  \ottsym{\}}  } : \source {  \bullet  \ottsym{,}  {\source m}  \ottsym{:}  \overline {\source {\mathit{TC}_i~a } }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source \tau }  } }{%
{\ottdrulename{sClsT\_cls}}{}%
}}

\newcommand{\ottdefnsclsXXtypingT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  }  \vdash_{cls}  \source {  {\source {cls} }  } : \source {  {\source { \Gamma_C } }'  } $}{}
\ottusedrule{\ottdrulesClsTXXcls{}}
\end{ottdefnblock}}

%% defn sinst_typingT
\newcommand{\ottdrulesInstTXXinst}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{i}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{h}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \source {  {\overline {\source b} }_{\ottmv{k}}  } =  \textbf {fv}  ( \source {  {\source \tau }  } ) }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  }  \vdash_{ty}  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{p}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{q}}  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}_{\ottmv{q}}  }  \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{q}}  } }{\ottmv{q}}}%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  }  \vDash  \source {  [  {\source \tau }  /  {\source a }  ]  {\source Q}'_{\ottmv{i}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }'_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \source {  {\source D }  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{q}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\overline {\source \delta} }'_{\ottmv{h}}  }~ \textbf {fresh} }%
\ottpremise{ ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{s}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{n}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }_{{\mathrm{2}}}  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  }~\textit{where}~\source {  [  {\overline {\source \tau} }'_{\ottmv{s}}  /  {\overline {\source b} }'_{\ottmv{s}}  ]  {\source \tau }_{{\mathrm{2}}}  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }_{\ottmv{k}}  ]  {\source \tau }  } }%
\ottpremise{ \source {  { \source P }'  } = \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }'_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  \ottsym{:}  {\source e}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}  \source {  \textbf{\source {instance} } \, {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{=}  {\source e}  \ottsym{\}}  } : \source {  { \source P }'  } }{%
{\ottdrulename{sInstT\_inst}}{}%
}}


\newcommand{\ottdrulesInstTXXinstXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{i}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{h}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \source {  {\overline {\source b} }_{\ottmv{k}}  } =  \textbf {fv}  ( \source {  {\source \tau }  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{p}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{q}}  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }%
\ottpremise{ \source {  {\source D }  }~ \textbf {fresh} }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  }  \vDash  \source {  [  {\source \tau }  /  {\source a }  ]  {\source Q}'_{\ottmv{i}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }'_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  }  \vdash_{tm}  \source {  {\source e}  } \Leftarrow \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{s}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{n}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }_{{\mathrm{2}}}  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  }~\textit{where}~\source {  [  {\overline {\source \tau} }'_{\ottmv{s}}  /  {\overline {\source b} }'_{\ottmv{s}}  ]  {\source \tau }_{{\mathrm{2}}}  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }_{\ottmv{k}}  ]  {\source \tau }  } }%
\ottpremise{ \source {  { \source P }'  } = \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }'_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  \ottsym{:}  {\source e}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}  \source {  \textbf{\source {instance} } \, {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{=}  {\source e}  \ottsym{\}}  } : \source {  { \source P }'  } }{%
{\ottdrulename{sInstT\_inst\_simp}}{}%
}}

\newcommand{\ottdefnsinstXXtypingT}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}  \source {  {\source {inst} }  } : \source {  { \source P }'  } $}{}
\ottusedrule{\ottdrulesInstTXXinst{}}
\ottusedrule{\ottdrulesInstTXXinstXXsimp{}}
\end{ottdefnblock}}

%% defn spgm_typingT
\newcommand{\ottdrulesPgmTXXcls}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  }  \vdash_{cls}  \source {  {\source {cls} }  } : \source {  {\source { \Gamma_C } }'  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  \ottsym{,}  {\source { \Gamma_C } }'  }  \vdash_{pgm}  \source {  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }''  }  \rightsquigarrow  \target {  {\target e }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}  \source {  {\source {cls} }  \ottsym{;}  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  \ottsym{,}  {\source { \Gamma_C } }''  }  \rightsquigarrow  \target {  {\target e }  } }{%
{\ottdrulename{sPgmT\_cls}}{}%
}}


\newcommand{\ottdrulesPgmTXXinst}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}  \source {  {\source {inst} }  } : \source {  { \source P }'  } }%
\ottpremise{ \source {  { \source P }  \ottsym{,}  { \source P }'  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}  \source {  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }''  } ; \source {  {\source { \Gamma_C } }'  }  \rightsquigarrow  \target {  {\target e }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}  \source {  {\source {inst} }  \ottsym{;}  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  \ottsym{,}  { \source P }''  } ; \source {  {\source { \Gamma_C } }'  }  \rightsquigarrow  \target {  {\target e }  } }{%
{\ottdrulename{sPgmT\_inst}}{}%
}}


\newcommand{\ottdrulesPgmTXXexpr}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  }  \vdash_{tm}  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}  \source {  {\source e}  } : \source {  {\source \tau }  } ; \source {  \bullet  } ; \source {  \bullet  }  \rightsquigarrow  \target {  {\target e }  } }{%
{\ottdrulename{sPgmT\_expr}}{}%
}}

\newcommand{\ottdefnspgmXXtypingT}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}  \source {  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  }  \rightsquigarrow  \target {  {\target e }  } $}{}
\ottusedrule{\ottdrulesPgmTXXcls{}}
\ottusedrule{\ottdrulesPgmTXXinst{}}
\ottusedrule{\ottdrulesPgmTXXexpr{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSpgmXXtypingT}{
\ottdefnsclsXXtypingT{}\ottdefnsinstXXtypingT{}\ottdefnspgmXXtypingT{}}

% defns Spgm_typing
%% defn scls_typing
\newcommand{\ottdrulesClsXXcls}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source m}  }  \notin   \textbf {dom}  ( \source {  {\source { \Gamma_C } }  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{k}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{p}}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\source a }  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\source a }  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source {\mathit{TC} } }_{\ottmv{i}} \, {\source a }  }  \rightsquigarrow  \intermed {  {\intermed Q}_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{ \nexists  \source {  {\source {\mathit{TC} } }'  } : ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }'  }~\source {  {\source b }  } : \source {  {\source \sigma}'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \nexists  \source {  {\source m}'  } : ( \source {  {\source m}'  } : \source {  {\overline {\source Q} }'_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  {\source \sigma}'  } )  \in  \source {  {\source { \Gamma_C } }  } }%
}{
 \source {  {\source { \Gamma_C } }  }  \vdash_{cls}^{\intermed {M} }  \source {  \textbf{\source {class} } \, \overline {\source {\mathit{TC}_i~a } }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{k}}  \Rightarrow  {\source \tau }  \ottsym{\}}  } : \source {  \bullet  \ottsym{,}  {\source m}  \ottsym{:}  \overline {\source {\mathit{TC}_i~a } }  \Rightarrow  {\source {\mathit{TC} } } \, {\source a }  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source \tau }  } }{%
{\ottdrulename{sCls\_cls}}{}%
}}

\newcommand{\ottdefnsclsXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source { \Gamma_C } }  }  \vdash_{cls}^{\intermed {M} }  \source {  {\source {cls} }  } : \source {  {\source { \Gamma_C } }'  } $}{}
\ottusedrule{\ottdrulesClsXXcls{}}
\end{ottdefnblock}}

%% defn sinst_typing
\newcommand{\ottdrulesInstXXinst}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{i}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{h}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \source {  {\overline {\source b} }_{\ottmv{k}}  } =  \textbf {fv}  ( \source {  {\source \tau }  } ) }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{p}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{q}}  } }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  }  \vdash_{\mathit {Q} }^{\intermed {M} }  \source {  {\source Q}_{\ottmv{q}}  }  \rightsquigarrow  \intermed {  {\intermed Q}_{\ottmv{q}}  } }{\ottmv{q}}}%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  }  \vDash^{\intermed {M} }  \source {  [  {\source \tau }  /  {\source a }  ]  {\source Q}'_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }_{\ottmv{h}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
\ottpremise{ \source {  {\source D }  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{h}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{q}}  }~ \textbf {fresh} }%
\ottpremise{ ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{m}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{n}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }_{{\mathrm{2}}}  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  }~\textit{where}~\source {  [  {\overline {\source \tau} }'_{\ottmv{m}}  /  {\overline {\source b} }'_{\ottmv{m}}  ]  {\source \tau }_{{\mathrm{2}}}  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }_{\ottmv{k}}  ]  {\source \tau }  } }%
\ottpremise{ \source {  { \source P }'  } = \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }_{\ottmv{h}}  \ottsym{:}  {\source e}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}^{\intermed {M} }  \source {  \textbf{\source {instance} } \, {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{=}  {\source e}  \ottsym{\}}  } : \source {  { \source P }'  } }{%
{\ottdrulename{sInst\_inst}}{}%
}}


\newcommand{\ottdrulesInstXXinstXXsimp}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{i}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{h}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \source {  {\overline {\source b} }_{\ottmv{k}}  } =  \textbf {fv}  ( \source {  {\source \tau }  } ) }%
\ottpremise{ \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{p}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{q}}  } }%
\ottpremise{ \source {  {\source D }  }~ \textbf {fresh} }%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  }  \vDash^{\intermed {M} }  \source {  [  {\source \tau }  /  {\source a }  ]  {\source Q}'_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}_{\ottmv{i}}  } } }{\ottmv{i}}}%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }_{\ottmv{h}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Leftarrow \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
\ottpremise{ ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{m}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{n}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }_{{\mathrm{2}}}  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  }~\textit{where}~\source {  [  {\overline {\source \tau} }'_{\ottmv{m}}  /  {\overline {\source b} }'_{\ottmv{m}}  ]  {\source \tau }_{{\mathrm{2}}}  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }_{\ottmv{k}}  ]  {\source \tau }  } }%
\ottpremise{ \source {  { \source P }'  } = \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }_{\ottmv{h}}  \ottsym{:}  {\source e}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}^{\intermed {M} }  \source {  \textbf{\source {instance} } \, {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{=}  {\source e}  \ottsym{\}}  } : \source {  { \source P }'  } }{%
{\ottdrulename{sInst\_inst\_simp}}{}%
}}

\newcommand{\ottdefnsinstXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}^{\intermed {M} }  \source {  {\source {inst} }  } : \source {  { \source P }'  } $}{}
\ottusedrule{\ottdrulesInstXXinst{}}
\ottusedrule{\ottdrulesInstXXinstXXsimp{}}
\end{ottdefnblock}}

%% defn spgm_typing
\newcommand{\ottdrulesPgmXXcls}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source { \Gamma_C } }  }  \vdash_{cls}^{\intermed {M} }  \source {  {\source {cls} }  } : \source {  {\source { \Gamma_C } }'  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  \ottsym{,}  {\source { \Gamma_C } }'  }  \vdash_{pgm}^{\intermed {M} }  \source {  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }''  }  \rightsquigarrow  \intermed {  {\intermed e}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}^{\intermed {M} }  \source {  {\source {cls} }  \ottsym{;}  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  \ottsym{,}  {\source { \Gamma_C } }''  }  \rightsquigarrow  \intermed {  {\intermed e}  } }{%
{\ottdrulename{sPgm\_cls}}{}%
}}


\newcommand{\ottdrulesPgmXXinst}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}^{\intermed {M} }  \source {  {\source {inst} }  } : \source {  { \source P }'  } }%
\ottpremise{ \source {  { \source P }  \ottsym{,}  { \source P }'  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}^{\intermed {M} }  \source {  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }''  } ; \source {  {\source { \Gamma_C } }'  }  \rightsquigarrow  \intermed {  {\intermed e}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}^{\intermed {M} }  \source {  {\source {inst} }  \ottsym{;}  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  \ottsym{,}  { \source P }''  } ; \source {  {\source { \Gamma_C } }'  }  \rightsquigarrow  \intermed {  {\intermed e}  } }{%
{\ottdrulename{sPgm\_inst}}{}%
}}


\newcommand{\ottdrulesPgmXXexpr}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}  } } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}^{\intermed {M} }  \source {  {\source e}  } : \source {  {\source \tau }  } ; \source {  \bullet  } ; \source {  \bullet  }  \rightsquigarrow  \intermed {  {\intermed e}  } }{%
{\ottdrulename{sPgm\_expr}}{}%
}}

\newcommand{\ottdefnspgmXXtyping}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{pgm}^{\intermed {M} }  \source {  {\source {pgm} }  } : \source {  {\source \tau }  } ; \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  }  \rightsquigarrow  \intermed {  {\intermed e}  } $}{}
\ottusedrule{\ottdrulesPgmXXcls{}}
\ottusedrule{\ottdrulesPgmXXinst{}}
\ottusedrule{\ottdrulesPgmXXexpr{}}
\end{ottdefnblock}}

%% defn sclosure
\newcommand{\ottdrulesClosureXXempty}[1]{\ottdrule[#1]{%
}{
 \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  } ) = \source {  \bullet  } }{%
{\ottdrulename{sClosure\_empty}}{}%
}}


\newcommand{\ottdrulesClosureXXTC}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source m}  } : \source {  {\overline {\source Q} }_{\ottmv{m}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  }~\source {  {\source a }  } : \source {  {\source \sigma}  } )  \in  \source {  {\source { \Gamma_C } }  } }%
\ottpremise{ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\overline {\source Q} }_{\ottmv{m}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{j}}  } }%
}{
 \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\source {\mathit{TC} } } \, {\source a }  } ) = \source {  {\overline {\source Q} }_{\ottmv{j}}  \ottsym{,}  {\source {\mathit{TC} } } \, {\source a }  } }{%
{\ottdrulename{sClosure\_TC}}{}%
}}

\newcommand{\ottdefnsclosure}[1]{\begin{ottdefnblock}[#1]{$ \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{i}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{j}}  } $}{}
\ottusedrule{\ottdrulesClosureXXempty{}}
\ottusedrule{\ottdrulesClosureXXTC{}}
\end{ottdefnblock}}

%% defn sunambig
\newcommand{\ottdrulesUnambigXXscheme}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\overline {\source a} }_{\ottmv{j}}  }  \in   \textbf {fv}  ( \source {  {\source \tau }  } ) }%
}{
 \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }  } ) }{%
{\ottdrulename{sUnambig\_scheme}}{}%
}}

\newcommand{\ottdefnsunambig}[1]{\begin{ottdefnblock}[#1]{$ \textbf {unambig}  ( \source {  {\source \sigma}  } ) $}{}
\ottusedrule{\ottdrulesUnambigXXscheme{}}
\end{ottdefnblock}}

%% defn sunambigC
\newcommand{\ottdrulesUnambigXXconstraint}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\overline {\source a} }_{\ottmv{j}}  }  \in   \textbf {fv}  ( \source {  {\source \tau }  } ) }%
}{
 \textbf {unambig}  ( \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } ) }{%
{\ottdrulename{sUnambig\_constraint}}{}%
}}

\newcommand{\ottdefnsunambigC}[1]{\begin{ottdefnblock}[#1]{$ \textbf {unambig}  ( \source {  {\source C}  } ) $}{}
\ottusedrule{\ottdrulesUnambigXXconstraint{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSpgmXXtyping}{
\ottdefnsclsXXtyping{}\ottdefnsinstXXtyping{}\ottdefnspgmXXtyping{}\ottdefnsclosure{}\ottdefnsunambig{}\ottdefnsunambigC{}}

% defns Sctr_provingT
%% defn sctr_provingT
\newcommand{\ottdrulesEntailTXXinst}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } = \source {  { \source P }_{{\mathrm{1}}}  }, \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{i}}  \Rightarrow  {\source Q}'  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }'_{\ottmv{i}}  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{h}}  \ottsym{:}  {\source e}  }, \source {  { \source P }_{{\mathrm{2}}}  } }%
\ottpremise{ \source {  {\source Q}  } = \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source Q}'  } }%
\ottpremise{ \source {  { \source P }_{{\mathrm{1}}}  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }'_{\ottmv{i}}  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{h}}  }  \vdash_{tm}  \source {  {\source e}  } \Rightarrow \source {  {\source \tau }  } \stot{ \rightsquigarrow  \target {  {\target e }  } } }%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}  \source {  {\source \tau }_{\ottmv{j}}  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }_{\ottmv{j}}  } } } }{\ottmv{j}}}%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}'_{\ottmv{i}}  }  \rightsquigarrow  \target {  {\target \sigma }'_{\ottmv{i}}  } }{\ottmv{i}}}%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  }  \vdash_{\mathit {Q} }  \source {  {\source Q}_{\ottmv{h}}  }  \rightsquigarrow  \target {  {\target \sigma }''_{\ottmv{h}}  } }{\ottmv{h}}}%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source Q}'_{\ottmv{i}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}}}%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  {\source Q}  } \stot{ \rightsquigarrow  \target {  \ottsym{(}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }'_{\ottmv{i}}  \ottsym{:}  {\target \sigma }'_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  \ottsym{\{}  {\target m}  \ottsym{=}  \Lambda  {\overline {\target b} }_{\ottmv{k}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{h}}  \ottsym{:}  {\target \sigma }''_{\ottmv{h}}}{\ottmv{h}} \, \ottsym{.}  {\target e }  \ottsym{\}}  \ottsym{)} \, {\overline {\target \sigma} }_{\ottmv{j}} \, {\overline {\target e} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sEntailT\_inst}}{}%
}}


\newcommand{\ottdrulesEntailTXXlocal}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source \delta }  } : \source {  {\source Q}  } )  \in  \source {  {\source \Gamma}  } }%
\ottpremise{ \vdash_{ctx}  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \target {  {\target \Gamma }  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  {\source Q}  } \stot{ \rightsquigarrow  \target {  {\target \delta }  } } }{%
{\ottdrulename{sEntailT\_local}}{}%
}}

\newcommand{\ottdefnsctrXXprovingT}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash  \source {  {\source Q}  } \stot{ \rightsquigarrow  \target {  {\target e }  } } $}{}
\ottusedrule{\ottdrulesEntailTXXinst{}}
\ottusedrule{\ottdrulesEntailTXXlocal{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSctrXXprovingT}{
\ottdefnsctrXXprovingT{}}

% defns Sctr_proving
%% defn sctr_proving
\newcommand{\ottdrulesEntailXXinst}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  { \source P }  } = \source {  { \source P }_{{\mathrm{1}}}  }, \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source Q}'  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{h}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{h}}  \ottsym{:}  {\source e}  }, \source {  { \source P }_{{\mathrm{2}}}  } }%
\ottpremise{ \source {  {\source Q}  } = \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source Q}'  } }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
\ottpremise{\ottcomp{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }_{\ottmv{j}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}_{\ottmv{j}}  } } } }{\ottmv{j}}}%
\ottpremise{\ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  [  {\overline {\source \tau} }_{\ottmv{j}}  /  {\overline {\source a} }_{\ottmv{j}}  ]  {\source Q}_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}_{\ottmv{i}}  } } }{\ottmv{i}}}%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  {\source Q}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed D } \, \overline {\intermed \sigma}_{\ottmv{j}} \, {\overline {\intermed d} }_{\ottmv{i}}  } } }{%
{\ottdrulename{sEntail\_inst}}{}%
}}


\newcommand{\ottdrulesEntailXXlocal}[1]{\ottdrule[#1]{%
\ottpremise{ ( \source {  {\source \delta }  } : \source {  {\source Q}  } )  \in  \source {  {\source \Gamma}  } }%
\ottpremise{ \vdash_{ctx}^{\intermed {M} }  \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \rightsquigarrow  \intermed {  {\intermed \Sigma}  } ; \intermed {  {\intermed { \Gamma_C } }  } ; \intermed {  {\intermed \Gamma}  } }%
}{
 \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  {\source Q}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed \delta }  } } }{%
{\ottdrulename{sEntail\_local}}{}%
}}

\newcommand{\ottdefnsctrXXproving}[1]{\begin{ottdefnblock}[#1]{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \vDash^{\intermed {M} }  \source {  {\source Q}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed d}  } } $}{}
\ottusedrule{\ottdrulesEntailXXinst{}}
\ottusedrule{\ottdrulesEntailXXlocal{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSctrXXproving}{
\ottdefnsctrXXproving{}}

% defns Sctx_typingT
%% defn sctx_typing_inf_infT
\newcommand{\ottdrulesMXXinfXXinfTXXempty}[1]{\ottdrule[#1]{%
}{
 \source {  \ottsym{[} \, \bullet \, \ottsym{]}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \rightsquigarrow  \target {  \ottsym{[} \, \bullet \, \ottsym{]}  } }{%
{\ottdrulename{sM\_inf\_infT\_empty}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfTXXappL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
}{
 \source {  {\source M} \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M } \, {\target e }_{{\mathrm{2}}}  } }{%
{\ottdrulename{sM\_inf\_infT\_appL}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfTXXappR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
}{
 \source {  {\source e}_{{\mathrm{1}}} \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}} \, {\target M }  } }{%
{\ottdrulename{sM\_inf\_infT\_appR}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfTXXletL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  } } } }%
\ottpremise{ \target {  {\target M }'  } = \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  {\target M } \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source M} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }'  } }{%
{\ottdrulename{sM\_inf\_infT\_letL}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfTXXletR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  } } } }%
\ottpremise{ \target {  {\target M }'  } = \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target M }  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }'  } }{%
{\ottdrulename{sM\_inf\_infT\_letR}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfTXXann}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }%
}{
 \source {  {\source M}  ::  {\source \tau }'  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }{%
{\ottdrulename{sM\_inf\_infT\_ann}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXinfXXinfT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } $}{}
\ottusedrule{\ottdrulesMXXinfXXinfTXXempty{}}
\ottusedrule{\ottdrulesMXXinfXXinfTXXappL{}}
\ottusedrule{\ottdrulesMXXinfXXinfTXXappR{}}
\ottusedrule{\ottdrulesMXXinfXXinfTXXletL{}}
\ottusedrule{\ottdrulesMXXinfXXinfTXXletR{}}
\ottusedrule{\ottdrulesMXXinfXXinfTXXann{}}
\end{ottdefnblock}}

%% defn sctx_typing_inf_checkT
\newcommand{\ottdrulesMXXinfXXcheckTXXabs}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  {\source \tau }  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
}{
 \source {  \lambda  {\source x}  \ottsym{.}  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target M }  } }{%
{\ottdrulename{sM\_inf\_checkT\_abs}}{}%
}}


\newcommand{\ottdrulesMXXinfXXcheckTXXinf}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }%
}{
 \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }{%
{\ottdrulename{sM\_inf\_checkT\_inf}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXinfXXcheckT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } $}{}
\ottusedrule{\ottdrulesMXXinfXXcheckTXXabs{}}
\ottusedrule{\ottdrulesMXXinfXXcheckTXXinf{}}
\end{ottdefnblock}}

%% defn sctx_typing_check_infT
\newcommand{\ottdrulesMXXcheckXXinfTXXappL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
}{
 \source {  {\source M} \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M } \, {\target e }_{{\mathrm{2}}}  } }{%
{\ottdrulename{sM\_check\_infT\_appL}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfTXXappR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
}{
 \source {  {\source e}_{{\mathrm{1}}} \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}} \, {\target M }  } }{%
{\ottdrulename{sM\_check\_infT\_appR}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfTXXletL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{2}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  } } } }%
\ottpremise{ \target {  {\target M }'  } = \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  {\target M } \, \textbf{\target {in} } \, {\target e }_{{\mathrm{2}}}  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source M} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }'  } }{%
{\ottdrulename{sM\_check\_infT\_letL}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfTXXletR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \vdash_{tm}  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stot{ \rightsquigarrow  \target {  {\target e }_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \target {  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  } } } }%
\ottpremise{ \target {  {\target M }'  } = \target {  \textbf{\target {let} } \, {\target x}  \ottsym{:}  \forall  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\target \sigma} }_{\ottmv{i}}  \rightarrow  {\target \sigma }_{{\mathrm{1}}}  \ottsym{=}  \Lambda  {\overline {\target a} }_{\ottmv{j}}  \ottsym{.}  \lambda \, \ottcomp{{\target \delta }_{\ottmv{i}}  \ottsym{:}  {\target \sigma }_{\ottmv{i}}}{\ottmv{i}} \, \ottsym{.}  {\target e }_{{\mathrm{1}}} \, \textbf{\target {in} } \, {\target M }  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }'  } }{%
{\ottdrulename{sM\_check\_infT\_letR}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfTXXann}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }%
}{
 \source {  {\source M}  ::  {\source \tau }'  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }{%
{\ottdrulename{sM\_check\_infT\_ann}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXcheckXXinfT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } $}{}
\ottusedrule{\ottdrulesMXXcheckXXinfTXXappL{}}
\ottusedrule{\ottdrulesMXXcheckXXinfTXXappR{}}
\ottusedrule{\ottdrulesMXXcheckXXinfTXXletL{}}
\ottusedrule{\ottdrulesMXXcheckXXinfTXXletR{}}
\ottusedrule{\ottdrulesMXXcheckXXinfTXXann{}}
\end{ottdefnblock}}

%% defn sctx_typing_check_checkT
\newcommand{\ottdrulesMXXcheckXXcheckTXXempty}[1]{\ottdrule[#1]{%
}{
 \source {  \ottsym{[} \, \bullet \, \ottsym{]}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \rightsquigarrow  \target {  \ottsym{[} \, \bullet \, \ottsym{]}  } }{%
{\ottdrulename{sM\_check\_checkT\_empty}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXcheckTXXabs}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  {\source \tau }  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  {\target M }  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \target {  {\target \sigma }  } } } }%
}{
 \source {  \lambda  {\source x}  \ottsym{.}  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \target {  \lambda  {\target x}  \ottsym{:}  {\target \sigma }  \ottsym{.}  {\target M }  } }{%
{\ottdrulename{sM\_check\_checkT\_abs}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXcheckTXXinf}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }%
}{
 \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } }{%
{\ottdrulename{sM\_check\_checkT\_inf}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXcheckXXcheckT}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \target {  {\target M }  } $}{}
\ottusedrule{\ottdrulesMXXcheckXXcheckTXXempty{}}
\ottusedrule{\ottdrulesMXXcheckXXcheckTXXabs{}}
\ottusedrule{\ottdrulesMXXcheckXXcheckTXXinf{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSctxXXtypingT}{
\ottdefnsctxXXtypingXXinfXXinfT{}\ottdefnsctxXXtypingXXinfXXcheckT{}\ottdefnsctxXXtypingXXcheckXXinfT{}\ottdefnsctxXXtypingXXcheckXXcheckT{}}

% defns Sctx_typing
%% defn sctx_typing_inf_inf
\newcommand{\ottdrulesMXXinfXXinfXXempty}[1]{\ottdrule[#1]{%
}{
 \source {  \ottsym{[} \, \bullet \, \ottsym{]}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \rightsquigarrow  \intermed {  \ottsym{[} \, \bullet \, \ottsym{]}  } }{%
{\ottdrulename{sM\_inf\_inf\_empty}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfXXappL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
}{
 \source {  {\source M} \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M} \, {\intermed e}_{{\mathrm{2}}}  } }{%
{\ottdrulename{sM\_inf\_inf\_appL}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfXXappR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
}{
 \source {  {\source e}_{{\mathrm{1}}} \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}} \, {\intermed M}  } }{%
{\ottdrulename{sM\_inf\_inf\_appR}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfXXletL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   } } } }%
\ottpremise{ \intermed {  {\intermed M}'  } = \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   \ottsym{=}  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  \ottsym{.}  {\intermed M} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source M} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}'  } }{%
{\ottdrulename{sM\_inf\_inf\_letL}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfXXletR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   } } } }%
\ottpremise{ \intermed {  {\intermed M}'  } = \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   \ottsym{=}  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  \ottsym{.}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed M}  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}'  } }{%
{\ottdrulename{sM\_inf\_inf\_letR}}{}%
}}


\newcommand{\ottdrulesMXXinfXXinfXXann}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
}{
 \source {  {\source M}  ::  {\source \tau }'  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }{%
{\ottdrulename{sM\_inf\_inf\_ann}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXinfXXinf}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } $}{}
\ottusedrule{\ottdrulesMXXinfXXinfXXempty{}}
\ottusedrule{\ottdrulesMXXinfXXinfXXappL{}}
\ottusedrule{\ottdrulesMXXinfXXinfXXappR{}}
\ottusedrule{\ottdrulesMXXinfXXinfXXletL{}}
\ottusedrule{\ottdrulesMXXinfXXinfXXletR{}}
\ottusedrule{\ottdrulesMXXinfXXinfXXann{}}
\end{ottdefnblock}}

%% defn sctx_typing_inf_check
\newcommand{\ottdrulesMXXinfXXcheckXXabs}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  {\source \tau }  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
}{
 \source {  \lambda  {\source x}  \ottsym{.}  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  \lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed M}  } }{%
{\ottdrulename{sM\_inf\_check\_abs}}{}%
}}


\newcommand{\ottdrulesMXXinfXXcheckXXinf}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
}{
 \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }{%
{\ottdrulename{sM\_inf\_check\_inf}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXinfXXcheck}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Rightarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } $}{}
\ottusedrule{\ottdrulesMXXinfXXcheckXXabs{}}
\ottusedrule{\ottdrulesMXXinfXXcheckXXinf{}}
\end{ottdefnblock}}

%% defn sctx_typing_check_inf
\newcommand{\ottdrulesMXXcheckXXinfXXappL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
}{
 \source {  {\source M} \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M} \, {\intermed e}_{{\mathrm{2}}}  } }{%
{\ottdrulename{sM\_check\_inf\_appL}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfXXappR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{1}}}  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
}{
 \source {  {\source e}_{{\mathrm{1}}} \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}} \, {\intermed M}  } }{%
{\ottdrulename{sM\_check\_inf\_appR}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfXXletL}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{2}}}  } \Rightarrow \source {  {\source \tau }_{{\mathrm{2}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{2}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   } } } }%
\ottpremise{ \intermed {  {\intermed M}'  } = \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   \ottsym{=}  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  \ottsym{.}  {\intermed M} \, \textbf{\intermed {in} } \, {\intermed e}_{{\mathrm{2}}}  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  \ottsym{=}  {\source M} \, \textbf{\source {in} } \, {\source e}_{{\mathrm{2}}}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}'  } }{%
{\ottdrulename{sM\_check\_inf\_letL}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfXXletR}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  {\overline {\source \delta} }_{\ottmv{i}}  }~ \textbf {fresh} }%
\ottpremise{ \source {  {\source x}  }  \notin   \textbf {dom}  ( \source {  {\source \Gamma}'  } ) }%
\ottpremise{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{i}}  }  \vdash_{tm}^{\intermed {M} }  \source {  {\source e}_{{\mathrm{1}}}  } \Leftarrow \source {  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \intermed {  {\intermed e}_{{\mathrm{1}}}  } } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}^{\intermed {M} }  \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{i}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  }\,{ \stoi{ \rightsquigarrow  \intermed {  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   } } } }%
\ottpremise{ \intermed {  {\intermed M}'  } = \intermed {  \textbf{\intermed {let} } \, {\intermed x}  \ottsym{:}  \forall  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}   {\overline {\intermed Q} }_{\ottmv{i}}  \Rightarrow  {\intermed \sigma}_{{\mathrm{1}}}   \ottsym{=}  \Lambda  {\overline {\intermed a} }_{\ottmv{j}}  \ottsym{.}  \lambda  {\overline {\intermed \delta} }_{\ottmv{i}}  \ottsym{:}  {\overline {\intermed Q} }_{\ottmv{i}}  \ottsym{.}  {\intermed e}_{{\mathrm{1}}} \, \textbf{\intermed {in} } \, {\intermed M}  } }%
}{
 \source {  \textbf{\source {let} } \, {\source x}  \ottsym{:}  {\source \sigma}_{{\mathrm{1}}}  \ottsym{=}  {\source e}_{{\mathrm{1}}} \, \textbf{\source {in} } \, {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}'  } }{%
{\ottdrulename{sM\_check\_inf\_letR}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXinfXXann}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
}{
 \source {  {\source M}  ::  {\source \tau }'  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }{%
{\ottdrulename{sM\_check\_inf\_ann}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXcheckXXinf}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } $}{}
\ottusedrule{\ottdrulesMXXcheckXXinfXXappL{}}
\ottusedrule{\ottdrulesMXXcheckXXinfXXappR{}}
\ottusedrule{\ottdrulesMXXcheckXXinfXXletL{}}
\ottusedrule{\ottdrulesMXXcheckXXinfXXletR{}}
\ottusedrule{\ottdrulesMXXcheckXXinfXXann{}}
\end{ottdefnblock}}

%% defn sctx_typing_check_check
\newcommand{\ottdrulesMXXcheckXXcheckXXempty}[1]{\ottdrule[#1]{%
}{
 \source {  \ottsym{[} \, \bullet \, \ottsym{]}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \rightsquigarrow  \intermed {  \ottsym{[} \, \bullet \, \ottsym{]}  } }{%
{\ottdrulename{sM\_check\_check\_empty}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXcheckXXabs}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  \ottsym{,}  {\source x}  \ottsym{:}  {\source \tau }  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
\ottpremise{ \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \vdash_{ty}^{\intermed {M} }  \source {  {\source \tau }  }\,{ \stoi{ \rightsquigarrow  \intermed {  {\intermed \sigma}  } } } }%
}{
 \source {  \lambda  {\source x}  \ottsym{.}  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }_{{\mathrm{1}}}  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }  \rightarrow  {\source \tau }_{{\mathrm{2}}}  } )  \rightsquigarrow  \intermed {  \lambda  {\intermed x}  \ottsym{:}  {\intermed \sigma}  \ottsym{.}  {\intermed M}  } }{%
{\ottdrulename{sM\_check\_check\_abs}}{}%
}}


\newcommand{\ottdrulesMXXcheckXXcheckXXinf}[1]{\ottdrule[#1]{%
\ottpremise{ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Rightarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }%
}{
 \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } }{%
{\ottdrulename{sM\_check\_check\_inf}}{}%
}}

\newcommand{\ottdefnsctxXXtypingXXcheckXXcheck}[1]{\begin{ottdefnblock}[#1]{$ \source {  {\source M}  } : ( \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  {\source \Gamma}  }  \Leftarrow  \source {  {\source \tau }  } )  \mapsto  ( \source {  { \source P }'  } ; \source {  {\source { \Gamma_C } }'  } ; \source {  {\source \Gamma}'  }  \Leftarrow  \source {  {\source \tau }'  } )  \rightsquigarrow  \intermed {  {\intermed M}  } $}{}
\ottusedrule{\ottdrulesMXXcheckXXcheckXXempty{}}
\ottusedrule{\ottdrulesMXXcheckXXcheckXXabs{}}
\ottusedrule{\ottdrulesMXXcheckXXcheckXXinf{}}
\end{ottdefnblock}}


\newcommand{\ottdefnsSctxXXtyping}{
\ottdefnsctxXXtypingXXinfXXinf{}\ottdefnsctxXXtypingXXinfXXcheck{}\ottdefnsctxXXtypingXXcheckXXinf{}\ottdefnsctxXXtypingXXcheckXXcheck{}}

\newcommand{\ottdefnss}{
\ottdefnsGTXXwf
\ottdefnsTtyXXscope
\ottdefnsTtmXXty
\ottdefnsTeval
\ottdefnsGTelab
\ottdefnsTctxXXtyping
\ottdefnsItyXXwf
\ottdefnsIctxXXwf
\ottdefnsItmXXty
\ottdefnsDXXty
\ottdefnsIctxXXtyping
\ottdefnsIevaluate
\ottdefnsCtxLog
\ottdefnsStyXXwfT
\ottdefnsStyXXwf
\ottdefnsSctxXXwfT
\ottdefnsSctxXXwf
\ottdefnsStmXXtypingT
\ottdefnsStmXXtyping
\ottdefnsSpgmXXtypingT
\ottdefnsSpgmXXtyping
\ottdefnsSctrXXprovingT
\ottdefnsSctrXXproving
\ottdefnsSctxXXtypingT
\ottdefnsSctxXXtyping
}

\newcommand{\ottall}{\ottmetavars\\[0pt]
\ottgrammar\\[5.0mm]
\newcommnad{target}{ \color{Red} }

\newcommand{intermed}{ \color{ForestGreen} }

\newcommand{source}{ \color{NavyBlue} }

\ottdefnss}



==> doc/sections/lemmas.tex <==
\newpage
% this whole section has nothing to do with target language

\renewcommand\itot[1]{}

% =================================================================================
% SOURCE Theorems
% =================================================================================
\section{\srcL{} Theorems}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% SOURCE Conjectures
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Conjectures}
\label{app:src_conj}

We are confident that the following lemmas can be proven using well-known proof
techniques. 

\begin{lemmaB}[Type Variable Substitution in \srcL{} Constraint Typing]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:tvar_subst_ctr}
  If \([[ GC ; GG1 , a , GG2 |-q sq ~> iq ]]\)
  and \([[ GC ; GG1 |-ty st ~> is ]]\)
  then \([[ GC ; GG1 , [| st / a |] GG2 |-q [| st / a |] sq ~> [| is / c |] iq ]]\).
\end{lemmaB}

\begin{lemmaB}[Type Well-Formedness Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:type_weakening}
  If \([[GC1 ; GG1 |-ty ss ~> is]]\)
  and \([[|-ctx empty; GC1, GC2 ; GG1, GG2 ~> empty ; TC ; TT ]]\)
  then \([[GC1, GC2 ; GG1, GG2 |-ty ss ~> is]]\).
\end{lemmaB}

\begin{lemmaB}[Class Constraint Well-Formedness Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:class_constraint_weakening}
  If \([[ GC1 ; GG1 |-q sq ~> iq' ]]\)
  and \([[|-ctx empty; GC1, GC2 ; GG1, GG2 ~> empty ; TC ; TT ]]\)
  then \([[GC1, GC2 ; GG1, GG2 |-q sq ~> iq']]\).
\end{lemmaB}

\begin{lemmaB}[Constraint Well-Formedness Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:constraint_weakening}
  If \([[ GC1 ; GG1 |-c sc ~> ic' ]]\)
  and \([[|-ctx empty; GC1, GC2 ; GG1, GG2 ~> empty ; TC ; TT ]]\)
  then \([[GC1, GC2 ; GG1, GG2 |-c sc ~> ic']]\).
\end{lemmaB}

\begin{lemmaB}[Context Well-Formedness Class Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:ctx_weakening_class}
  If \([[|-ctx P ; GC1 ; GG ~> SS ; TC1 ; TT ]]\)
  and \([[|-ctx empty; GC1, GC2 ; GG ~> empty ; TC1, TC2 ; TT ]]\)
  then \([[|-ctx P ; GC1, GC2 ; GG ~> SS ; TC1, TC2 ; TT]]\).
\end{lemmaB}

\begin{lemmaB}[Context Well-Formedness Typing Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:ctx_weakening_typing}
  If \([[|-ctx P ; GC ; GG1 ~> SS ; TC ; TT1 ]]\)
  and \([[|-ctx empty; GC ; GG1, GG2 ~> empty ; TC ; TT1, TT2 ]]\)
  then \([[|-ctx P ; GC ; GG1, GG2 ~> SS ; TC ; TT1, TT2]]\).
\end{lemmaB}


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% SOURCE Lemmas
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Lemmas}

\begin{lemmaB}[Determinism of Context Typing]\leavevmode
  \label{lemma:ctx_type_unique}
  \begin{itemize}
  \item If \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st1 ) ~~> iM1 ]]\)
       and \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> iM2 ]]\) \\
       then \([[ st1 = st2 ]]\).
  \item If \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st1 ) ~~> iM1 ]]\)
       and \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st2 ) ~~> iM2 ]]\) \\
       then \([[ st1 = st2 ]]\).
  \item If \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' ==> st1 ) ~~> iM1 ]]\)
       and \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> iM2 ]]\) \\
       then \([[ st1 = st2 ]]\).
  \item If \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' <== st1 ) ~~> iM1 ]]\)
       and \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' <== st2 ) ~~> iM2 ]]\) \\
       then \([[ st1 = st2 ]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the first typing derivation, in combination with
case analysis on the second derivation. \\
\qed

\begin{lemmaB}[Class Constraint Elaboration to \interL{} Uniqueness]\ \\
  \label{lemma:q_elab_unique}
  If \([[ GC ; GG |-q sq ~> iq1 ]]\) and \([[ GC ; GG |-q sq ~> iq2 ]]\),
  then \([[ iq1 = iq2 ]]\).
\end{lemmaB}

\proof
By mutual induction on both well-formedness derivations, together with
Lemma~\ref{lemma:ty_elab_unique}. \\
\qed

\begin{lemmaB}[Type Elaboration to \interL{} Uniqueness]\ \\
  \label{lemma:ty_elab_unique}
  If \([[ GC ; GG |-ty ss ~> is1 ]]\) and \([[ GC ; GG |-ty ss~> is2 ]]\),
  then \([[ is1 = is2 ]]\).
\end{lemmaB}

\proof
By mutual induction on both well-formedness derivations, together with
Lemma~\ref{lemma:q_elab_unique}. \\
\qed

\begin{lemmaB}[Constraint Elaboration to \interL{} Uniqueness]\ \\
  \label{lemma:c_elab_unique}
  If \([[ GC ; GG |-c sc ~> ic1 ]]\) and \([[ GC ; GG |-c sc~> ic2 ]]\),
  then \([[ ic1 = ic2 ]]\).
\end{lemmaB}

\proof
By straightforward induction on both well-formedness derivations, in combination
with Lemma~\ref{lemma:q_elab_unique}. \\
\qed

\begin{lemmaB}[Environment Elaboration to \interL{} Uniqueness]\ \\
  \label{lemma:env_elab_unique}
  If \([[ |-ctx P ; GC ; GG ~> SS1 ; TC1 ; TT2 ]]\)
  and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC2 ; TT2 ]]\),
  then \([[ TC1 = TC2 ]]\) and \([[ TT1 = TT2 ]]\).
\end{lemmaB}

\proof
By straightforward induction on both well-formedness derivations, in combination
with Lemmas~\ref{lemma:q_elab_unique}, \ref{lemma:ty_elab_unique} and~\ref{lemma:c_elab_unique}. \\
\qed

\begin{lemmaB}[Environment Well-Formedness of \srcL{} Typing]\leavevmode
  \label{lemma:ctx_well_source_typing}
  \begin{itemize}
  \item If \([[ PT ; GC ; GG |-tm se => st ~> te ]]\) then \([[|-ctx PT ; GC ; GG
    ~> GT]]\).
  \item If \([[ PT ; GC ; GG |-tm se <= st ~> te ]]\) then \([[|-ctx PT ; GC ; GG
    ~> GT]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\begin{lemmaB}[Environment Well-Formedness of \srcL{} Typing through \interL{}]\leavevmode
  \label{lemma:ctx_well_source_mid_typing}
  \begin{itemize}
  \item If \([[ P ; GC ; GG |-tm se => st ~> ie ]]\) then \([[|-ctx P ; GC ; GG
    ~> SS ; TC ; TT]]\).
  \item If \([[ P ; GC ; GG |-tm se <= st ~> ie ]]\) then \([[|-ctx P ; GC ; GG
    ~> SS ; TC ; TT]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\begin{lemmaB}[Well-Formedness of \srcL{} Typing Result] \leavevmode
  \label{lemma:type_well_source_typing}
  \begin{itemize}
  \item If \([[ P ; GC ; GG |-tm se => st ~> ie ]]\)
    then \([[GC ; GG |-ty st ~> is]]\).
  \item If \([[ P ; GC ; GG |-tm se <= st ~> ie ]]\)
    then \([[GC ; GG |-ty st ~> is]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\begin{lemmaB}[Preservation of Environment Term Variables from \srcL{} to \interL{}]\leavevmode
  \label{lemma:pres_env_tm}
  \begin{itemize}
  \item If \([[ ( sx : ss ) in GG ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    then \([[ ( ix : is ) in TT ]]\)
    where \([[ GC ; GG |-ty ss ~> is ]]\).
  \item If \([[ sx notin dom ( GG ) ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    then \([[ ix notin dom ( TT ) ]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the environment elaboration derivation. \\
\qed

\begin{lemmaB}[Preservation of Environment Type Variables from \srcL{} to \interL{}]\leavevmode
  \label{lemma:pres_env_ty}
  \begin{itemize}
  \item If \([[ a in GG ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    then \([[ c in TT ]]\).
  \item If \([[ a notin GG ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    then \([[ c notin TT ]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the environment elaboration derivation. \\
\qed

\begin{lemmaB}[Preservation of Environment Dictionary Variables from \srcL{} to \interL{}]\leavevmode
  \label{lemma:pres_env_d}
  \begin{itemize}
  \item If \([[ ( sdvar : sq ) in GG ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    then \([[ ( idvar : iq ) in TT ]]\)
    where \([[ GC ; GG |-q sq ~> iq ]]\).
  \item If \([[ sdvar notin dom ( GG ) ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    then \([[ idvar notin dom ( TT ) ]]\).
  \end{itemize}
\end{lemmaB}

\proof
By straightforward induction on the environment elaboration derivation. \\
\qed

\begin{lemmaB}[Environment Well-Formedness Strengthening]\ \\
  \label{lemma:env_strengthening}
  If \([[ |-ctx P ; GC ; GG ~> GT ]]\)
  then \([[ |-ctx P ; GC ; empty ~> tempty ]]\).
\end{lemmaB}

\proof
By case analysis on the hypothesis,
the last rules used to construct it must be (possibly zero)
consecutive applications of \textsc{sCtxT-pgmInst}. Revert those rules, to obtain
\([[ |-ctx empty ; GC ; GG ~> GT ]]\).
By further case analysis (\textsc{sCtxT-tyEnvTm}, \textsc{sCtxT-tyEnvTy} and
\textsc{sCtxT-tyEnvD}), we get \([[ |-ctx empty ; GC ; empty ~> tempty ]]\).
The goal follows by consecutively
re-applying rule \textsc{sCtxT-pgmInst} with the appropriate premises. \\
\qed

\begin{lemmaB}[Environment Well-Formedness with \interL{} Elaboration
    Strengthening]\ \\
  \label{lemma:env_mid_strengthening}
  If \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
  then \([[ |-ctx P ; GC ; empty ~> SS ; TC ; empty ]]\).
\end{lemmaB}

\proof
By case analysis on the hypothesis,
the last rules used to construct it must be (possibly zero)
consecutive applications of \textsc{sCtx-pgmInst}. Revert those rules, to obtain
\([[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]]\).
By further case analysis (\textsc{sCtx-tyEnvTm}, \textsc{sCtx-tyEnvTy} and
\textsc{sCtx-tyEnvD}), we get \([[ |-ctx empty ; GC ; empty ~> empty ; TC ; empty ]]\).
The goal follows by consecutively
re-applying rule \textsc{sCtx-pgmInst} with the appropriate premises. \\
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Typing Preservation
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Typing Preservation}
\label{app:type_pres}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Typing Preservation - Expressions]\leavevmode
\label{thmA:typing_pres_expr}
  \begin{itemize}
  \item If $[[P ; GC ; GG |-tm se => st ~> ie]]$,
    and $[[GC ; GG |-ty st ~> is]]$,
    then $[[|-ctx P ; GC ; GG ~> SS ; TC ; TT]]$,
    and $[[SS ; TC ; TT |-tm ie : is ~> te]]$.
  \item If $[[P ; GC ; GG |-tm se <= st ~> ie]]$,
    and $[[GC ; GG |-ty st ~> is]]$,
    then $[[|-ctx P ; GC ; GG ~> SS ; TC ; TT]]$,
    and $[[SS ; TC ; TT |-tm ie : is ~> te]]$.
  \end{itemize}
\end{theoremB}

\begin{figure}[htp]
  \centering

  \def\svgscale{0.75}
  \input{mut_dep_graph_pres.pdf_tex}

  %% \includegraphics[height=5cm]{mut_dep_graph_pres.png}
  \caption{Dependency graph for Theorems~\ref{thmA:typing_pres_expr},
    \ref{thmA:typing_pres_constraint} and
    \ref{thmA:typing_pres_env}}
  \label{fig:dep_graph_pres}
\end{figure}

\proof
This theorem is mutually proven with Theorems~\ref{thmA:typing_pres_constraint}
and~\ref{thmA:typing_pres_env}. This mutual dependency is illustrated in
Figure~\ref{fig:dep_graph_pres}, where an arrow from A to B denotes A being
dependent on B. Note that at the dependency from
Theorem~\ref{thmA:typing_pres_env} to \ref{thmA:typing_pres_expr}, the size of
\([[P]]\) is strictly decreasing, whereas \([[P]]\) remains constant at every
other dependency. Consequently, the size of \([[P]]\) is strictly decreasing in
every possible cycle. The induction thus remains well-founded.

By applying Lemma~\ref{lemma:ctx_well_source_mid_typing} to the first
hypothesis, we get:
\begin{equation}
  [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
  \label{eq:typing_pres_expr0}
\end{equation}
We continue by induction on the lexicographic order of the tuple (size of the
expression, typing mode). Regarding typing mode, we define type checking to be
larger than type inference. In each mutual dependency, we know that the
tuple size decreases, meaning that the induction is well-founded.

\begin{description}
  \item[Part 1]~\\
\proofStep{\textsc{sTm-inf-true}}
  {
    \drule{sTm-inf-true}
  }
  {
    By \textsc{sTy-bool}, we know that:
    \begin{equation*}
      [[GC ; GG |-ty sbool ~> ibool]]
    \end{equation*}
    The goal to be proven is the following:
    \begin{equation*}
      [[SS ; TC ; TT |-tm itrue : ibool ~> ttrue]]
    \end{equation*}
    From Theorem~\ref{thmA:typing_pres_env}, we know that:
    \begin{equation*}
      [[ |-ctx SS ; TC ; TT ]]
    \end{equation*}
    The goal follows from \textsc{iTm-true}. \\
  }
\proofStep{\textsc{sTm-inf-false}}
  {
    \drule{sTm-inf-false}
  }
  { Similar to the \textsc{sTm-inf-true} case. \\
  }
\proofStep{\textsc{sTm-inf-let}}
  {}
  {
 \drule{sTm-inf-let}

    Given
    \begin{equation*}
    [[GC ; GG |-ty st2 ~> is2]]
    \end{equation*}
    The goal to be proven is the following:
    \begin{equation*}
      [[SS ; TC ; TT |-tm
 ilet ix : \/ clj . iqlk -> is = /\ clj . \ idvarlk : iqlk . ie1 iin ie2 : is2 ~> tlet tx : tt = te1 tin te2]]
    \end{equation*}
    By case analysis on Equation~\ref{eq:typing_pres_expr0} (\textsc{sCtx-pgmInst}), we know:
    \begin{equation}
      \label{eq:preserve:let1}
      [[|-ctx empty ; GC ; GG ~> empty ; TC ; TT]]
    \end{equation}
    From the rule premise we know that:
    \begin{equation}
      \label{eq:preserve:let2}
      [[GC ; GG |-ty \/ alj . sqlk => st1 ~> \/ clj . iqlk -> is]]
    \end{equation}
    Applying Theorem~\ref{thmA:typing_pres_types} to
    Equations~\ref{eq:preserve:let1} and \ref{eq:preserve:let2},
    we get that:
    \begin{equation}
      \label{eq:preserve:let3}
      [[TC ; TT |-ty \/ clj . iqlk -> is ~> tt]]
    \end{equation}
    By repeated case analysis on Equation~\ref{eq:preserve:let2} (\textsc{sTy-scheme} and \textsc{sTy-qual}), we get that:
    \begin{gather}
      [[ alj notin GG ]]
      \nonumber \\
      [[ </ GC ; GG, alj |-q sqk ~> iqk // k /> ]]
      \nonumber
    \end{gather}
    Applying these results, together with Equation~\ref{eq:preserve:let1},
    to \textsc{sCtx-tyEnvTy} and \textsc{sCtx-tyEnvD}, we get:
    \begin{equation}
      \label{eq:preserve:let100}
      [[|-ctx empty ; GC ; GG, alj, sdvarlk : sqlk ~> empty ; TC; TT, clj, idvarlk : iqlk]]
    \end{equation}
    By weakening (Lemma~\ref{lemma:ctx_weakening_typing}) on
    Equations~\ref{eq:typing_pres_expr0} and \ref{eq:preserve:let100}, we get:
    \begin{equation}
      \label{eq:preserve:let4}
      [[|-ctx P ; GC ; GG, alj, sdvarlk : sqlk ~> SS; TC; TT, clj, idvarlk : iqlk]]
    \end{equation}
    The rule premise also gives us that:
    \begin{equation}
      \label{eq:preserve:let5}
      [[P ; GC ; GG, alj, sdvarlk : sqlk |-tm se1 <= st1 ~> ie1]]
    \end{equation}
    By applying induction hypothesis with Equations~\ref{eq:preserve:let2} and
    \ref{eq:preserve:let5}, we get that:
    \begin{equation*}
      [[SS; TC; TT, clj, idvarlk : iqlk |-tm ie1 : is  ~> te1 ]]
    \end{equation*}
    Because of \textsc{iTm-constrI} and \textsc{iTm-forallI}, it is equivalent
    to say that:
    \begin{equation}
      \label{eq:preserve:let6}
      [[SS; TC; TT |-tm /\ clj . \ idvarlk : iqlk . ie1 :\/ clj . iqlk -> is  ~> te1 ]]
    \end{equation}
    Through a similar analysis, we get that:
    \begin{equation}
      \label{eq:preserve:let7}
      [[SS; TC; TT, ix : \/ clj . iqlk -> is |-tm ie2 : is2 ~> te2 ]]
    \end{equation}
    By \textsc{iTm-let}, in combination with Equations~\ref{eq:preserve:let3},
    \ref{eq:preserve:let6} and \ref{eq:preserve:let7}, the goal has been proven. \\
  }
\proofStep{\textsc{sTm-inf-ArrE}}
  {}
  { \drule{sTm-inf-ArrE}

    From the rule premise:
    \begin{gather}
      \label{eq:preserve:app1}
      [[P ; GC ; GG |-tm se1 => st1 -> st2 ~> ie1]]\\
      \label{eq:preserve:app2}
      [[P ; GC ; GG |-tm se2 <= st1 ~> ie2]]
    \end{gather}
    The goal to be proven is the following:
    \begin{equation*}
      [[SS ; TC ; TT |-tm ie1 ie2 : is2 ~> te1 te2]]
    \end{equation*}
    where $[[GC ; GG |-ty st2 ~> is2]]$.

    Because the typing result is well-formed
    (Lemma~\ref{lemma:type_well_source_typing}), we know:
    \begin{equation*}
      [[GC ; GG |-ty st1 -> st2 ~> is1 -> is2]]
    \end{equation*}

    By applying the induction hypothesis on Equations~\ref{eq:preserve:app1} and
    \ref{eq:preserve:app2}, we know respectively:
    \begin{gather*}
      [[SS ; TC ; TT |-tm ie1 : is1 -> is2 ~> te1]] \\
      [[SS ; TC ; TT |-tm ie2 : is1 ~> te2]]
    \end{gather*}
    The goal follows from \textsc{iTm-arrE}. \\
  }
\proofStep{\textsc{sTm-inf-Ann}}
  { \drule{sTm-inf-Ann}}
  {
    Follows directly from the induction hypothesis. \\
  }
  
  \item[Part 2]~\\
\proofStep{\textsc{sTm-check-var}}
  {
  }
  {
    \drule{sTm-check-var}

    From the rule premise:
    \begin{equation*}
      [[( sx : \/ alj . sqli => st ) in GG]]
    \end{equation*}
    By repeated case analysis on Equation~\ref{eq:typing_pres_expr0} (\textsc{sCtx-pgmInst}), we get that:
    \begin{equation}
      \label{eq:preserve_exp:var1b}
      [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]]
    \end{equation}
    By case analysis on Equation~\ref{eq:preserve_exp:var1b} (\textsc{sCtx-tyEnvTm}), we know:
    \begin{gather}
      \label{eq:preserve_exp:var1a}
      [[( sx : \/ alj . sqli => st ) in GG]]\\ 
      [[ GC ; GG1 |-ty \/ alj . sqli => st ~> \/clj . iqli -> is]]
      \label{eq:preserve_exp:var1c}
    \end{gather}
    where \([[ GG = GG1, sx : \/ alj . sqli => st , GG2 ]]\).

    By applying Lemma~\ref{lemma:pres_env_tm} to Equation~\ref{eq:preserve_exp:var1a}, we get:
    \begin{equation}
      \label{eq:preserve_exp:var1}
      [[( ix : \/ clj . iqli -> is ) in TT]]
    \end{equation}
    Furthermore, from the rule premise, we know that:
    \begin{equation}
      [[</ GC ; GG |-ty stj ~> isj // j />]]
      \label{eq:preserve_exp:var2e}
    \end{equation}
    By Typing Preservation - Types (Theorem~\ref{thmA:typing_pres_types}),
    together with Equation~\ref{eq:preserve_exp:var1b}, we have:
    \begin{equation}
      \label{eq:preserve_exp:var2}
      [[</ TC ; TT |-ty isj ~> ttj // j />]]
    \end{equation}
    Similarly, the rule premise tells us that:
    \begin{equation}
      \label{eq:preserve_exp:var2b}
      [[</ P ; GC ; GG |= [| stlj / alj |] sqi ~> idi // i />]]
    \end{equation}
    By applying weakening (Lemma~\ref{lemma:type_weakening}) to Equation~\ref{eq:preserve_exp:var1c}, we get:
    \begin{equation}
      \label{eq:preserve_exp:var2d}
      [[ GC ; GG |-ty \/ alj . sqli => st ~> \/clj . iqli -> is]]
    \end{equation}
    By repeated case analysis on Equation~\ref{eq:preserve_exp:var2d} (sTy-qual), we get that:
    \begin{equation}
      \label{eq:preserve_exp:var2c}
      [[ </ GC ; GG, alj |-q sqi ~> iqi // i /> ]]
    \end{equation}
    By applying Lemma~\ref{lemma:tvar_subst_ctr} on Equations~\ref{eq:preserve_exp:var2c}
    and~\ref{eq:preserve_exp:var2e}, we get:
    \begin{equation}
      \label{eq:preserve_exp:var2f}
      [[ </ GC ; GG |-q [| stlj / alj |] sqi ~> [| islj / clj |] iqi // i /> ]]
    \end{equation}
    By Typing Preservation - Constraints Proving (Theorem~\ref{thmA:typing_pres_constraint}),
    applied to Equations~\ref{eq:preserve_exp:var2b}, \ref{eq:typing_pres_expr0}
    and~\ref{eq:preserve_exp:var2f}, we have:
    \begin{equation}
      \label{eq:preserve_exp:var3}
      [[</ SS ; TC ; TT |-d idi : [| islj / clj |]iqi ~> tei // i />]]
    \end{equation}
    
    The goal to be proven is the following:
    \begin{equation*}
      [[SS ; TC ; TT |-tm ix islj idli : [| islj / clj |] is ~> tx ttj tei]]
    \end{equation*}
    where $[[ GC ; GG |-ty [| stlj / alj |] st ~> [| islj / clj |] is ]]$.
    
    From Equation~\ref{eq:preserve_exp:var1}, by applying \textsc{iTm-var}, we get
    \begin{equation}
      \label{eq:preserve_exp:var4}
      [[SS ; TC ; TT |-tm ix : \/ clj . iqli -> is ~> tx]]
    \end{equation}
    By Equations~\ref{eq:preserve_exp:var2}, \ref{eq:preserve_exp:var4} and \textsc{iTm-forallE}, we get:
    \begin{equation}
      \label{eq:preserve_exp:var5}
      [[SS ; TC ; TT |-tm ix islj : [| islj / clj |] iqli -> [| islj /clj |]is ~> tx ttj]]
    \end{equation}
    By Equations~\ref{eq:preserve_exp:var3} and \ref{eq:preserve_exp:var5},
    in combination with rule \textsc{iTm-constrE}, we get
    \begin{equation}
      [[SS ; TC ; TT |-tm ix islj idli : [| islj / clj |] is ~> tx ttj tei]]
    \end{equation}
    which is exactly the goal. \\
  }
\proofStep{\textsc{sTm-check-meth}}
  {}
  {
    \drule{sTm-check-meth}

    The goal to be proven is the following:
    \begin{equation}
      [[ SS ; TC ; TT |-tm id . im islj idli : [| islj / clj |] [| is / c |] is' ~> te ]]
      \label{eqg:preserve_exp:meth}
    \end{equation}
    where \([[ GC ; empty, alj, a |-ty st' ~> is' ]]\).

    From the rule premise, we get that:
    \begin{gather}
      \label{eq:preserve_exp:m:1}
      [[P ; GC ; GG |= sTC st ~> id]]\\
      \label{eq:preserve_exp:m:2}
      [[GC ; GG |-ty st ~> is]]
    \end{gather}
    By repeated case analysis on Equation~\ref{eq:typing_pres_expr0} (\textsc{sCtx-clsEnv}),
    together with the first rule premise, we get:
    \begin{equation*}
      [[ GC1 ; empty, a |-ty \/ alj . sqli => st' ~> is'' ]]
    \end{equation*}
    where \([[ GC = GC1, sm : sqlk' => sTC a : \/ alj . sqli => st', GC2 ]]\).

    Following \textsc{sQ-TC}, in combination with this result,
    Equation~\ref{eq:preserve_exp:m:2} and the first rule premise, we have:
    \begin{align}
      \label{eq:preserve_exp:m:3}
      [[GC ; GG |-q sTC st ~> iTC is]]
    \end{align}
    Applying Typing Preservation - Constraints Proving
    (Theorem~\ref{thmA:typing_pres_constraint}) on
    Equations~\ref{eq:preserve_exp:m:1} and \ref{eq:preserve_exp:m:3}, we get:
    \begin{align}
      \label{eq:preserve_exp:m:4}
       [[SS ; TC ; TT |-d id : iTC is ~> te]]
    \end{align}
    Furthermore, we know from the rule premise that:
    \begin{align*}
      [[( sm : sqlk' => sTC a : \/ alj . sqli => st' ) in GC]]
    \end{align*}
    Consequently, by repeated case analysis on Equation~\ref{eq:typing_pres_expr0}
    (\textsc{sCtx-clsEnv}), we know that:
    \begin{align}
      \label{eq:preserve_exp:m:5}
      [[( im : iTC c : is'' ) in TC]]
    \end{align}
    By Equations~\ref{eq:preserve_exp:m:4} and \ref{eq:preserve_exp:m:5},
    in combination with rule \textsc{iTm-method}, we get:
    \begin{align*}
      [[SS ; TC ; TT |-tm id . im : [| is / c |] is'' ~> te . tl]]
    \end{align*}

    The rest of the proof is similar to case \textsc{sTm-check-var}. \\
  }
\proofStep{\textsc{sTm-check-ArrI}}
  {}
  { \drule{sTm-check-ArrI}

    The second hypothesis is:
    \begin{equation*}
      [[|-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
    \end{equation*}
    It is easy to verify that 
    \begin{equation*}
      [[|-ctx P ; GC ; GG, sx : st1 ~> SS ; TC ; TT, ix : is ]]
    \end{equation*}
    The goal follows directly by applying the induction hypothesis,
    in combination with rule \textsc{iTm-arrI}. \\
  }
\proofStep{\textsc{sTm-check-Inf}}
  { \drule{sTm-check-Inf}}
  {
    Follows directly from the induction hypothesis.
  }
\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Typing Preservation - Instance]\ \\
  If $[[ P ; GC |-instM sinst : P' ]]$,
  and $[[|-ctx P; GC ; empty ~> SS ; TC ; empty]]$
  then we have $[[|-ctx P, P'; GC ; empty ~> SS, SS' ; TC ; empty]]$.
\label{thmA:typing_pres_instance}
\end{theoremB}
\proof

We restate the rule for typing instance declarations  for reference:

\[\drule{sInst-inst}\]
By inversion of rule \textsc{sInst-inst}, we know that:
\begin{gather*}
  [[ P' = (sD : \/ blk . sqlq => sTC st) . sm |-> empty, blk, sdvarlq : sqlq,
  alj, sdvarlh : [| st / a |] sqlh : se ]]
\end{gather*}
Therefore our goal is
\begin{equation}
  \label{eq:pres_inst:1}
  [[|-ctx P, (sD : \/ blk . sqlq => sTC st) . sm |-> empty, blk, sdvarlq : sqlq,
  alj, sdvarlh : [| st / a |] sqlh : se ; GC ; empty ~> SS, SS' ; TC ; empty]]
\end{equation}
From the hypothesis, we know that:
\begin{align}
  \label{eq:pres_inst:2}
  [[|-ctx P; GC ; empty ~> SS ; TC ; empty]]
\end{align}
Goal~\ref{eq:pres_inst:1} follows directly from \textsc{sCtx-pgmInst} with
\([[ SS' = (iD : \/ iblk . iqlq => iTC is) . im |-> /\ iblk . \ idvarlq : iqlq .
/\ clj . \ idvarlh : [| is / c |] iqlh . ie ]]\), if we can show the following:
\begin{gather}
  \label{eq:pres_inst:3a}
  [[ unambig(\/ blk . sqlq => sTC st) ]] \\
  \label{eq:pres_inst:3}
  [[GC ; empty |-c \/ blk . sqlq => sTC st ~> \/ iblk . iqlq => iTC is]] \\
  \label{eq:pres_inst:4}
  [[( sm : sqli' => sTC a : \/ alj . sqlh => st1 ) in GC]]\\
  \label{eq:pres_inst:5}
  [[P ; GC ; empty, blk, sdvarlq : sqlq, alj, sdvarlh : [| st / a |] sqlh |-tm
  se <= [| st / a |] st1 ~> ie ]] \\
  \label{eq:pres_inst:6}
  [[GC ; empty, a |-ty \/ alj . sqlh => st1 ~> is']] \\
  \label{eq:pres_inst:7}
  [[sD notin dom (P)]] \\
  \label{eq:pres_inst:8}
  [[( sD' : \/ blk' . sqlh'' => sTC st'' ) . sm' |-> GG' : se' notin P]] \\
  \label{eq:pres_inst:9}
  [[where [| stlj / blj |] st = [| stlk' / blk' |] st'']] \\
  \label{eq:pres_inst:10}
  [[|-ctx P ; GC ; empty ~> SS ; TC ; empty]] 
\end{gather}
Goal~\ref{eq:pres_inst:10} is exactly Equation~\ref{eq:pres_inst:2}, which we
already have. Goals~\ref{eq:pres_inst:3a} and \ref{eq:pres_inst:4} follow
directly from the premise of \textsc{sInst-inst}. The premise also tells us that
$[[ sD ]]$ is freshly generated, which satisfies Goal~\ref{eq:pres_inst:7}. Similarly
Goals~\ref{eq:pres_inst:5}, \ref{eq:pres_inst:8} and \ref{eq:pres_inst:9} can be proven directly from
the rule premise. 

From the premise, we know:
\begin{gather}
  [[GC ; empty, blk |-ty st ~> is]] \\
  [[</ GC ; empty, blk |-q sqq ~> iqq // q />]]
\end{gather}
Goal~\ref{eq:pres_inst:3} follows directly from the definition of
well-formedness of constraints and types.
Goals~\ref{eq:pres_inst:5} and
\ref{eq:pres_inst:6} remain to be proven.

From the rule premise, we know that
\begin{equation}
[[( sm : sqli' => sTC a : \/ alj . sqlh => st1 ) in GC]]
\end{equation}
From the definition of well-formedness of the source context, we know that:
\begin{gather*}
[[GC1 ; empty, a |-ty \/ alj . sqlh => st1 ~> is']] \\
[[GC = GC1, GC2]]
\end{gather*}
By weakening of class environment (Lemma~\ref{lemma:type_weakening}), we
can prove Goal~\ref{eq:pres_inst:6}. \\
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Typing Preservation - Classes]\ \\
  If $[[GC |-clsM scls : GC']]$,
  and $[[|-ctx P ; GC ; empty ~> SS ; TC ; empty]]$,
  then we have $[[|-ctx P ; GC, GC' ; empty ~> SS ; TC, TC' ; empty]]$.
\label{thmA:typing_pres_class}
\end{theoremB}
\proof

We restate the rule for class declaration typing for reference:
\[\drule{sCls-cls}\]
By case analysis, we know that $\source{[[GC']]}$ is of the form
\begin{equation*}
\source{[[empty, sm : sTCl => sTC a : \/ alj . sqlp => st]]}
\end{equation*}
The goal to be proven is the following:
\begin{equation}
  \label{eq:pres_class:1}
[[|-ctx P ; GC, sm : sTCl => sTC a : \/ alj . sqlp => st ; empty ~> SS ; TC, im : iTC c : is ; empty]]
\end{equation}
We can derive from \textsc{sCtx-clsEnv} that
\begin{equation}
  \label{eq:pres_class:8}
[[|-ctx empty ; GC, sm : sTCl => sTC a : \/ alj . sqlp => st ; empty ~> empty ; TC, im : iTC c : is ; empty]]
\end{equation}
assuming we can show that:
\begin{gather}
  \label{eq:pres_class:2}
[[GC ; empty, a |-ty \/ alk . sqlp => st ~> is]] \\
  \label{eq:pres_class:3}
[[alj, a = fv (st)]] \\
  \label{eq:pres_class:4}
[[</ GC ; empty, a |-q sTCi a ~> iqi // i />]] \\
  \label{eq:pres_class:5}
[[sm notin dom (GC)]] \\
  \label{eq:pres_class:6}
[[sTC b notin dom (GC)]] \\
  \label{eq:pres_class:7}
[[|-ctx empty ; GC ; empty ~> empty ; TC ; empty]]
\end{gather}
Goals~\ref{eq:pres_class:2} till \ref{eq:pres_class:6} follow directly from the
premises and from the hypothesis. Goal~\ref{eq:pres_class:7} follows by repeated
inversion on the second hypothesis.
Finally, Goal~\ref{eq:pres_class:1} follows from Equation~\ref{eq:pres_class:8}
by the definition of environment well-formedness and the second hypothesis. \\
\qed

\begin{theoremB}[Typing Preservation - Programs]\ \\
  If $[[ P ; GC |-pgmM spgm : st ; P' ; GC' ~> ie ]]$,
  and $[[|-ctx P; GC ; empty ~> SS ; TC ; empty]]$,
  and $[[GC, GC' ; empty |-ty st ~> is]]$
  then we have $[[|-ctx P, P'; GC, GC' ; empty ~> SS, SS' ; TC, TC' ; empty]]$,
  and we have $[[SS, SS' ; TC, TC' ; empty |-tm ie : is ~> te]]$.
\label{thmA:typing_pres_pgm}
\end{theoremB}

\proof By structural induction on the typing derivation.\\
\proofStep{\textsc{sPgmCls}}
  {\drule{sPgm-cls}}
  {
    We know that
    \begin{equation*}
      [[|-ctx P; GC ; empty ~> SS ; TC ; empty]]
    \end{equation*}
    By inversion it follows that:
    \begin{equation*}
      [[|-ctx empty ; GC ; empty ~> empty ; TC ; empty]]
    \end{equation*}
    By Typing Preservation - Classes (Theorem~\ref{thmA:typing_pres_class}), we know
    \begin{equation*}
      [[|-ctx empty ; GC, GC' ; empty ~> empty ; TC, TC' ; empty]]
    \end{equation*}
    Through weakening (Lemma~\ref{lemma:ctx_weakening_class}), we know that
    \begin{equation*}
      [[|-ctx P ; GC, GC' ; empty ~> SS ; TC, TC' ; empty]]
    \end{equation*}
    The goal follows directly from the induction hypothesis. \\
    }
\proofStep{\textsc{sPgm-Inst}}
  { \drule{sPgm-inst}}
  {
    We know that
    \begin{equation*}
      [[|-ctx P; GC ; empty ~> SS ; TC ; empty]]
    \end{equation*}
    By Typing Preservation - Instance (Theorem~\ref{thmA:typing_pres_instance}),
    we know that 
    \begin{equation}
      \label{eq:pres_pgm:1}
      [[|-ctx P, P' ; GC ; empty ~> SS, SS' ; TC ; empty]]
    \end{equation}
    The goal follows directly from the induction hypothesis. \\
  }
\proofStep{\textsc{sPgm-expr}}
  {\drule{sPgm-expr}}
  {
    Follows directly from Typing Preservation - Expressions
    (Theorem~\ref{thmA:typing_pres_expr}). 
  }
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Typing Preservation - Types and Class Constraints]\leavevmode
  \begin{itemize}
    \item
      If \( [[ GC ; GG |-ty ss ~> is  ]]\),
      and \( [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]] \),
      then \( [[ TC ; TT |-ty is ~> tt]] \).
    \item 
      If \( [[ GC ; GG |-q sq ~> iq  ]]\),
      and \( [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]] \),
      then \( [[ TC ; TT |-q iq ~> tt]] \).
  \end{itemize}
  \label{thmA:typing_pres_types}
\end{theoremB}

\proof By induction on the lexicographic order of the tuple (size of
$[[GC]]$, the derivation height of type well-formedness and the constraint
well-formedness). In each mutual dependency, the size of the tuple is
decreasing, so we know that the induction is well-founded.

\begin{description}
  \item[Part 1]~\\
    \proofStep{\textsc{sTy-arrow}}
    { \drule{sTy-bool} }
    { Follows directly by \textsc{iTy-bool}.\\}
    \proofStep{\textsc{sTy-var}}
    { \drule{sTy-var} }
    { It is easy to verify that for any environment for which $[[|-ctx P ; GC ;
      GG ~> SS ; TC ; TT]]$ holds,
      \([[ a in GG ]]\) implies \([[ c in TT ]]\). Therefore, the goal follows
      from \textsc{iTy-var}. \\}
    \proofStep{\textsc{sTy-arrow}}
    { \drule{sTy-arrow} }
    { By induction hypothesis, we get
        \begin{gather*}
         [[ TC ; TT |-ty is1 ~> tt1  ]] \\
         [[ TC ; TT |-ty is2 ~> tt2  ]] 
        \end{gather*}
      The goal follows directly from \textsc{iTy-Arrow}.\\
    }
    \proofStep{\textsc{sTy-qual}}
    { \drule{sTy-qual} }
    { By induction hypothesis, we get
      \begin{align*}
         [[ TC ; TT |-ty is ~> tt  ]] 
      \end{align*}
      By Part 2 of this lemma, we get
      \begin{align*}
         [[ TC ; TT |-q iq ~> tt'  ]] 
      \end{align*}
      The goal follows directly from \textsc{iTy-Qual}.\\
    }
    \proofStep{\textsc{sTy-scheme}}
    { \drule{sTy-scheme} }
    {
      Given $[[  |-ctx empty ; GC ; GG ~> empty ; TC ; TT  ]]$, by \textsc{sCtx-EnvTy},
      we know that $[[  |-ctx empty ; GC ; GG, a ~> empty ; TC ; TT, c ]]$.
      By induction hypothesis, we get
      \begin{align*}
         [[ TC ; TT , c |-ty is ~> tt  ]] 
      \end{align*}
      The goal follows directly by \textsc{iTy-scheme}.
    }

  \item[Part 2]~\\
    \proofStep{\textsc{sQ-TC}}
    { \drule{sQ-TC}}
    {
      By Part 1 of this lemma, we know that
      \begin{align}
        \label{eq:preserve_type:1}
         [[ TC ; TT |-ty is ~> tt  ]] 
      \end{align}
      It is easy to verify that given any environment for which
      \begin{gather}
        [[|-ctx empty ; GC ; GG ~> empty ; TC ; TT]] 
        \nonumber \\
        [[ GC = GC1, sm : sqli => sTC a : ss , GC2 ]]
        \label{eq:preserve_type:2}
      \end{gather}
      then
      \begin{gather*}
      [[ TC = TC1, im : iTC c : is' , TC2 ]]\\
      [[ |-ctx empty ; GC1 ; empty ~> empty ; TC1 ; empty]]\\
      [[ GC1 ; empty , a |-ty ss ~> is' ]]
      \end{gather*}
      By \textsc{sCtx-TyEnvTy}, we get
      \begin{align*}
      [[ |-ctx empty ; GC1 ; empty, a ~> empty ; TC1 ; empty, c]]
      \end{align*}
      The size of $[[TC1]]$ is trivially smaller than $[[TC]]$. So by induction
      hypothesis, we have
      \begin{align}
        \label{eq:preserve_type:3}
         [[ TC ; empty , c |-ty is' ~> tt'  ]] 
      \end{align}
      The goal follows directly from \textsc{sQ-TC}, and Equations
      \ref{eq:preserve_type:1}, \ref{eq:preserve_type:2},
      \ref{eq:preserve_type:3}.
      
    }

\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Typing Preservation - Constraints Proving]\ \\
  If $[[ P ; GC ; GG |= sq ~> id ]]$,
  and $ [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]] $,
  and $ [[ GC ; GG |-q sq ~> iq ]]$,
  then $[[SS ; TC ; TT |-d id : iq ~> te]]$.
  \label{thmA:typing_pres_constraint}
\end{theoremB}

\proof By induction on the constraint resolution derivation tree.
This theorem is mutually proven with Theorems~\ref{thmA:typing_pres_expr}
and~\ref{thmA:typing_pres_env} (Figure~\ref{fig:dep_graph_pres}).
Note that at the dependency from
Theorem~\ref{thmA:typing_pres_env} to \ref{thmA:typing_pres_expr}, the size of
\([[P]]\) is strictly decreasing, whereas \([[P]]\) remains constant at every
other dependency. Consequently, the size of \([[P]]\) is strictly decreasing in
every possible cycle. The induction thus remains well-founded.\\
\proofStep{\textsc{sEntail-local}}{\drule{sEntail-local}}
{
  It is easy to verify that given
  \begin{gather*}
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]  \\
    [[ ( sdvar : sq ) in GG]]
  \end{gather*}
  we can derive
  \begin{gather*}
    [[( idvar : iq' ) in TT]]\\
    [[ GC ; GG1 |-q sq ~> iq' ]] \\
    [[GG = GG1, sdvar : sq , GG2]]
  \end{gather*}
  By weakening lemma (Lemma~\ref{lemma:class_constraint_weakening})
  \begin{align*}
  [[ GC ; GG |-q sq ~> iq' ]] 
  \end{align*}
  We already know from the hypothesis:
  \begin{align*}
  [[ GC ; GG |-q sq ~> iq ]]
  \end{align*}
  Since the elaboration of $[[|-q]]$ is deterministic (Lemma~\ref{lemma:q_elab_unique}), we know that $[[iq]] =
  [[iq']]$.
  The goal follows directly by \textsc{D-var}. \\
}
\proofStep{\textsc{sEntail-inst}}
          {}
{
  \drule{sEntail-inst}

  The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT |-d iD islj idli : iq ~> te ]]~
    \textit{where}~[[ iq = iTC isq ]]
  \end{equation*}
  Using \textsc{D-con}, proving this is equivalent to proving:
  \begin{gather}
    \label{eq:preserve_proof:1}
    [[( iD : \/ clj . iqli => iTC isq') . im |-> /\ clj . \ idvarli : iqli . ie in SS]] \\
    \textit{where}~[[ isq = [| islj / clj |] isq' ]] \nonumber \\
    \label{eq:preserve_proof:2}
    [[ |-ctx SS ; TC ; TT ]] \\
    \label{eq:preserve_proof:3}
    [[ </ TC ; empty, clj |-q iqi ~> tti' // i /> ]] \\
    \label{eq:preserve_proof:4}
    [[</ TC ; TT |-ty isj ~> ttj // j />]] \\
    \label{eq:preserve_proof:5}
    [[SS1 ; TC ; empty, clj, idvarli : iqli |-tm ie : [| isq' / c |] ism ~> te' ]] \\
    \textit{where}~[[SS = SS1, ( iD : \/ clj . iqli => iq) . im |-> ie, SS2]] \nonumber \\
    \label{eq:preserve_proof:6}
    [[</ SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei // i />]]
  \end{gather}
  The rule premise tells us, among other things, that:
  \begin{gather}
    \label{eq:preserve_proof:7}
    [[ P = P1, (sD : \/ alj . sqli => sq') . sm |-> empty, alj, sdvarli : sqli, blk,
    sdvarlh : sqlh : se, P2 ]] \\
    \label{eq:preserve_proof:8}
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]] \\
    \label{eq:preserve_proof:9}
    [[ </ GC ; GG |-ty stj ~> isj // j /> ]] \\
    \label{eq:preserve_proof:10}
    [[ </ P ; GC ; GG |= [| stlj / alj |] sqi ~> idi // i /> ]] 
  \end{gather}
  Goal~\ref{eq:preserve_proof:1} follows directly from
  Equations~\ref{eq:preserve_proof:7} and \ref{eq:preserve_proof:8}.
  Goal~\ref{eq:preserve_proof:2} follows by applying
  Equation~\ref{eq:preserve_proof:8} to preservation
  Theorem~\ref{thmA:typing_pres_env}.

  Consequently, from Equation~\ref{eq:preserve_proof:2}, in combination with
  rule \textsc{iCtx-MEnv}, we know that:
  \begin{equation}
    [[ TC ; empty |-c \/ clj . iqli => iTC isq' ]]
    \label{eq:preserve_proof:11}
  \end{equation}
  Goal~\ref{eq:preserve_proof:3} follows from rule \textsc{iC-abs}, in
  combination with Equation~\ref{eq:preserve_proof:11}.

  By inversion on Equation~\ref{eq:preserve_proof:8}, we know that:
  \begin{equation}
    [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]]
    \label{eq:preserve_proof:12}
  \end{equation}
  Goal~\ref{eq:preserve_proof:4} follows by applying
  Equations~\ref{eq:preserve_proof:9} and \ref{eq:preserve_proof:12} to
  Theorem~\ref{thmA:typing_pres_types}. 
  
  From rule \textsc{iCtx-MEnv}, in combination with
  Equations~\ref{eq:preserve_proof:1} and \ref{eq:preserve_proof:2}, we know
  that:
  \begin{equation}
    [[ SS1 ; TC ; empty |-tm /\ clj . \ idvarli : iqli . ie : \/ clj . iqli -> [| isq' / c |] ism ~> tem ]]
    \label{eq:preserve_proof:13}
  \end{equation}
  Goal~\ref{eq:preserve_proof:5} follows from inversion of rules
  \textsc{iTm-forallI} and \textsc{iTm-constrI}, on Equation~\ref{eq:preserve_proof:13}.

  Finally, Goal~\ref{eq:preserve_proof:6} follows by applying the induction
  hypothesis on Equation~\ref{eq:preserve_proof:10}, assuming we can show that:
  \begin{equation}
    [[ </ GC ; GG |-q [| stlj / alj |] sqi ~> [| islj / clj |] iqi // i /> ]]
    \label{eq:preserve_proof:14}
  \end{equation}
  From rule \textsc{sCtx-pgmInst}, in combination with
  Equation~\ref{eq:preserve_proof:7}, we know that:
  \begin{equation}
    [[ GC ; empty |-c \/ alj . sqli => sq' ~> \/ clj . iqli => iTC isq' ]]
    \label{eq:preserve_proof:15}
  \end{equation}
  From weakening Lemma~\ref{lemma:constraint_weakening}, we know that:
  \begin{equation}
    [[ GC ; GG |-c \/ alj . sqli => sq' ~> \/ clj . iqli => iTC isq' ]]
    \label{eq:preserve_proof:16}
  \end{equation}
  From rule \textsc{sQ-TC}, in combination with
  Equation~\ref{eq:preserve_proof:16}, we know that:
  \begin{equation}
    [[ </ GC ; GG , alj |-q sqi ~> iqi // i /> ]]
    \label{eq:preserve_proof:17}
  \end{equation}
  Goal~\ref{eq:preserve_proof:14} follows by applying type substitution
  Lemma~\ref{lemma:tvar_subst_ctr} on Equations~\ref{eq:preserve_proof:17} and
  \ref{eq:preserve_proof:9} (in combination with weakening
  Lemma~\ref{lemma:type_weakening}). 
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Typing Preservation - Environment Well-Formedness]\ \\
  If $ [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]] $,
  then $[[ |-ctx SS ; TC ; TT ]]$.
  \label{thmA:typing_pres_env}
\end{theoremB}

\proof By induction on the well-formedness derivation.
This theorem is mutually proven with Theorems~\ref{thmA:typing_pres_expr}
and~\ref{thmA:typing_pres_constraint} (Figure~\ref{fig:dep_graph_pres}).
Note that at the dependency from
Theorem~\ref{thmA:typing_pres_env} to \ref{thmA:typing_pres_expr}, the size of
\([[P]]\) is strictly decreasing, whereas \([[P]]\) remains constant at every
other dependency. Consequently, the size of \([[P]]\) is strictly decreasing in
every possible cycle. The induction thus remains well-founded.\\
\proofStep{\textsc{sCtx-empty}}{
  \drule{sCtx-empty}
}
{
Follows directly by \textsc{iCtx-empty}. \\
}
\proofStep{\textsc{sCtx-tyEnvTm}}{
  \drule{sCtx-tyEnvTm}
}
{
 By induction hypothesis, we know 
  \begin{equation*}
    [[ |-ctx empty; TC ; TT ]]
  \end{equation*}
  By Typing Preservation - Types and Class Constraints
  (Theorem~\ref{thmA:typing_pres_types}), we know
  \begin{equation*}
    [[ TC ; TT |-ty is ~> tt]]
  \end{equation*}
  Since $[[sx notin dom(GG)]]$, it is easy to verify that $[[ix notin dom (TT)]]$.
  Therefore the goal follows directly by \textsc{iCtx-tyEnvTm}. \\
}
\proofStep{\textsc{sCtx-tyEnvTy}}{
  \drule{sCtx-tyEnvTy}
}
{
  By induction hypothesis, we know
  \begin{equation*}
    [[ |-ctx empty; TC ; TT ]]
  \end{equation*}
  Since we know $[[a notin GG]]$, it is easy to verify that $[[c notin TT]]$.
  Therefore the goal follows directly by \textsc{iCtx-tyEnvTy}. \\
}
\proofStep{\textsc{sCtx-tyEnvD}}{
  \drule{sCtx-tyEnvD}
}
{
  By induction hypothesis, we know
  \begin{equation*}
    [[ |-ctx empty; TC ; TT ]]
  \end{equation*}
  By Typing Preservation - Types and Class Constraints
  (Theorem~\ref{thmA:typing_pres_types}), we know
  \begin{equation*}
    [[ TC ; TT |-q iq ~> tt]]
  \end{equation*}
  Since $[[sdvar notin dom(GG)]]$, it is easy to verify that $[[idvar notin dom (TT)]]$.
  Therefore the goal follows directly by \textsc{iCtx-tyEnvD}. \\  
}
\proofStep{\textsc{sCtx-clsEnv}}{
}
{
  \drule{sCtx-clsEnv}

  By induction hypothesis, we know
  \begin{equation*}
    [[ |-ctx empty; TC ; empty ]]
  \end{equation*}
  By \textsc{sCtx-tyEnvTy}, we know that 
  \begin{equation*}
    [[ |-ctx empty; GC ; empty, a ~> empty ; TC ; empty, c]]
  \end{equation*}
  Then by Typing Preservation - Types and Class Constraints
  (Theorem~\ref{thmA:typing_pres_types}), we know
  \begin{equation*}
    [[ TC ; empty, c |-ty is ~> tt]]
  \end{equation*}
  It is easy to verify that given $[[sm notin dom (GC)]], [[sTC b notin dom
  (GC)]]$, we can derive $[[im notin dom (TC)]], [[iTC ib notin dom (TC)]]$.

  The goal follows directly by \textsc{iCtx-ClsEnv}. \\
}
\proofStep{\textsc{sCtx-pgmInst}}{
}
{
  \drule{sCtx-pgmInst}

  By induction hypothesis, we know that
  \begin{equation}
    \label{eq:preserve_ctx:goal:0}
    [[ |-ctx SS ; TC ; TT ]]
  \end{equation}
  Also, since we know that
  \begin{equation*}
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
  \end{equation*}
  by applying inversion, we get:
  \begin{equation}
    \label{eq:preserve_ctx:1}
    [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]]
  \end{equation}
  From the premise, we already know
  \begin{align}
    \label{eq:preserve_ctx:2}
    [[GC ; empty |-c \/ blj . sqli => sTC st ~> \/ iblj . iqli => iTC is ]]
  \end{align}
  Then by Typing Preservation - Types and Class Constraints
  (Theorem~\ref{thmA:typing_pres_types}) on Equations~\ref{eq:preserve_ctx:1} and
  \ref{eq:preserve_ctx:2}, we know
  \begin{equation}
    \label{eq:preserve_ctx:goal:1}
    [[ TC ; empty |-c \/ iblj . iqli => iTC is ]]
  \end{equation}
  From the 3\textsuperscript{rd} rule premise, we know that
  \begin{equation}
    \label{eq:preserve_ctx:3}
    [[( sm : sqlm' => sTC a : \/ alk . sqlh => st' ) in GC]]
  \end{equation}
  By inversion on Equation~\ref{eq:preserve_ctx:1} (\textsc{sCtx-clsEnv}),
  together with Equation~\ref{eq:preserve_ctx:3}, we get
  \begin{gather}
    \label{eq:preserve_ctx:41}
    [[(im : iTC c : is1) in TC]] \\
    \label{eq:preserve_ctx:4}
    [[GC1 ; empty, a |-ty \/ alk . sqlh => st' ~> is1]] \\
    \label{eq:preserve_ctx:5}
    [[GC = GC1, GC2]]
  \end{gather}
  By applying weakening (Lemma~\ref{lemma:type_weakening}) on
  Equation~\ref{eq:preserve_ctx:4}, we have
  \begin{align}
    \label{eq:preserve_ctx:6}
    [[GC ; empty, a |-ty \/ alk . sqlh => st' ~> is1]] 
  \end{align}
  From the 5\textsuperscript{th} rule premise, we know that
  \begin{align}
    \label{eq:preserve_ctx:7}
    [[GC ; empty, a |-ty \/ alk . sqlh => st' ~> \/ clk . iqlh -> is' ]]
  \end{align}
  Because the elaboration of types is deterministic (Lemma~\ref{lemma:ty_elab_unique}), combining
  Equations~\ref{eq:preserve_ctx:6} and \ref{eq:preserve_ctx:7}, we know that
  $[[is1 = \/ clk . iqlh -> is']]$. By rewriting Equation~\ref{eq:preserve_ctx:41}, we get
  \begin{align}
    \label{eq:preserve_ctx:goal:2}
    [[(im : iTC c : \/ clk . iqlh -> is') in TC]] 
  \end{align}
  By applying Theorem~\ref{thmA:typing_pres_expr} to the 4\textsuperscript{th} rule premise, we get:
  \begin{equation}
    [[ SS ; TC ; empty, iblj, idvarli : iqli, clk, idvarlh : [| is / c |] iqlh |-tm ie : [| is / c |] is' ~> te ]] 
    \label{eq:preserve_ctx:8}
  \end{equation}
  Lemma~\ref{lemma:ctx_well_inter_typing}, applied to this result, gives us:
  \begin{equation}
    [[ |-ctx SS ; TC ; empty, iblj, idvarli : iqli, clk, idvarlh : [| is / c |] iqlh ]]
    \label{eq:preserve_ctx:9}
  \end{equation}
  Furthermore, by applying \textsc{iTm-constrI} and \textsc{iTm-forallI} to
  Equation~\ref{eq:preserve_ctx:8}, in combination with inversion on
  Equation~\ref{eq:preserve_ctx:9}, we get
  \begin{equation*}
    [[ SS ; TC ; empty |-tm /\ iblj . \ idvarli : iqli . /\ clk . \ idvarlh : [| is / c |] iqlh . ie : \/ iblj . iqli -> \/ clk . [| is / c |] iqlh -> [| is / c |] is' ~> te' ]] 
  \end{equation*}
  which is equivalent to
  \begin{equation}
    [[ SS ; TC ; empty |-tm /\ iblj . \ idvarli : iqli . /\ clk . \ idvarlh : [| is / c |] iqlh . ie : \/ iblj . iqli -> [| is / c |] ( \/ clk . iqlh -> is' ) ~> te' ]] 
    \label{eq:preserve_ctx:10}
  \end{equation}
  Given
  \begin{gather*}
    [[ unambig(\/ blj . sqli => sTC st) ]] \\
    [[sD notin dom (P)]] \\
    [[( sD' : \/ blk' . sqlh'' => sTC st'' ) . sm' |-> GG' : se' notin P]]\\
    [[ where [| stlj / blj |] st = [| stlk' / blk' |] st'']]
  \end{gather*}
  It is easy to verify that 
  \begin{gather}
    \label{eq:preserve_ctx:goal:7}
    [[ unambig(\/ iblj . iqli => iTC is) ]] \\
    \label{eq:preserve_ctx:goal:4}
    [[iD notin dom (SS)]] \\
    \label{eq:preserve_ctx:goal:5}
    [[( iD' : \/ clm' . iqln'' => iTC is'' ) . im' |-> ie' notin SS]] \\
    \label{eq:preserve_ctx:goal:6}
    [[where [| islj / clj |] is = [| islm' / clm' |] is'']] 
  \end{gather}
  The goal follows by
  combining Equations~\ref{eq:preserve_ctx:goal:0}, \ref{eq:preserve_ctx:goal:1},
  \ref{eq:preserve_ctx:goal:2}, \ref{eq:preserve_ctx:10},
  \ref{eq:preserve_ctx:goal:7}, 
  \ref{eq:preserve_ctx:goal:4}, \ref{eq:preserve_ctx:goal:5},
  \ref{eq:preserve_ctx:goal:6}, and the rule \textsc{iCtx-MEnv}.
}
\qed


% =================================================================================
% INTER Theorems
% =================================================================================
\newpage
\section{\interL{} Theorems}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% INTER Conjectures
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Conjectures}
\label{app:mid_conj}

We are confident that the following lemmas can be proven using well-known proof
techniques. 

\begin{lemmaB}[Type Variable Substitution in Types]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:tvar_tsubst}
  If \([[ TC ; TT1, c , TT2 |-ty is1 ~> tt1 ]]\)
  and \([[ TC ; TT1 |-ty is2 ~> tt2 ]]\)
  then \([[ TC ; TT1, [| is2 / c |] TT2 |-ty [| is2 / c |] is1 ~> [| tt2 / ta |] tt1 ]]\).
\end{lemmaB}

\begin{lemmaB}[Type Variable Substitution in Dictionaries]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:tvar_tsubst_iq}
  If \([[ TC ; TT1, c , TT2 |-q iq ~> tt ]]\)
  and \([[ TC ; TT1 |-ty is' ~> tt' ]]\)
  then \([[ TC ; TT1, [| is' / c |] TT2 |-q [| is' / c |] iq ~> [| tt' / ta |] tt ]]\).
\end{lemmaB}

\begin{lemmaB}[Variable Substitution]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:var_subst}
  If \([[ SS ; TC ; TT1, ix : is2, TT2 |-tm ie1 : is1 ~> te1 ]]\)
  and \([[ SS ; TC ; TT1, TT2 |-tm ie2 : is2 ~> te2 ]]\)
  then \([[ SS ; TC ; TT1, TT2 |-tm [| ie2 / ix |] ie1 : is1 ~> [| te2 / tx |] te1 ]]\).
\end{lemmaB}

\begin{lemmaB}[Reverse Variable Substitution]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:rev_var_subst}
  If \([[ SS ; TC ; TT |-tm [| ie2 / ix |] ie1 : is1 ~> te3]]\)
  and \([[ SS ; TC ; TT |-tm ie2 : is2 ~> te2 ]]\)
  then \([[ SS ; TC ; TT, ix : is2 |-tm ie1 : is1 ~> te1 ]]\).
\end{lemmaB}

\begin{lemmaB}[Dictionary Variable Substitution]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:dvar_subst}
  If \([[ SS ; TC ; TT1, idvar : iq, TT2 |-tm ie : is ~> te ]]\)
  and \([[ SS ; TC ; TT1, TT2 |-d id : iq ~> te' ]]\)
  then \([[ SS ; TC ; TT1, TT2 |-tm [| id / idvar |] ie : is ~> [| te' / txd |] te ]]\).
\end{lemmaB}

\begin{lemmaB}[Reverse Dictionary Variable Substitution]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:rev_dvar_subst}
  If \([[ SS ; TC ; TT |-tm [| id / idvar |] ie : is ~> te1 ]]\)
  and \([[ SS ; TC ; TT |-d id : iq ~> te2 ]]\)
  then \([[ SS ; TC ; TT, idvar : iq |-tm ie : is ~> te ]]\).
\end{lemmaB}

\begin{lemmaB}[Type Variable Substitution]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:tvar_subst}
  If \([[ SS ; TC ; TT1, c, TT2 |-tm ie : is ~> te ]]\)
  and \([[ TC ; TT1 |-ty is' ~> tt' ]]\)
  then \([[ SS ; TC ; TT1, [| is' / c |] TT2 |-tm [| is' / c |] ie : [| is' / c
  |] is ~> [| tt' / ta |] te ]]\).
\end{lemmaB}

\begin{lemmaB}[Reverse Type Variable Substitution]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:rev_tvar_subst}
  If \([[ SS ; TC ; TT |-tm [| is' / c |] ie : [| is' / c |] is ~> [| tt' / ta |] te ]]\)
  then \([[ SS ; TC ; TT, c |-tm ie : is ~> te ]]\).
\end{lemmaB}

\begin{lemmaB}[Dictionary Variable Substitution in Dictionaries]\ \\
  If \([[ SS ; TC ; TT1, idvar : iq', TT2 |-d iD islj idli : iq ~> te ]]\)
  and \([[ SS ; TC ; TT1, TT2 |-d id : iq' ~> te' ]]\)
  then \([[ SS ; TC ; TT1, TT2 |-d iD islj [| id / idvar |] idli : iq ~> [| te'
  / txd |] te ]]\).
  \label{lemma:dvar_subst_dict}
\end{lemmaB}

\begin{lemmaB}[Type Variable Substitution in Dictionaries]\ \\
  If \([[ SS ; TC ; TT1, c, TT2 |-d iD islj idli : iq ~> te ]]\)
  and \([[ TC ; TT1 |-ty is ~> tt ]]\)
  then \([[ SS ; TC ; TT1, [| is / c |] TT2 |-d iD [| is / c |] islj [| is / c |] idli : [| is / c |] iq ~> [| tt / ta |] te ]]\).
  \label{lemma:tvar_subst_dict}
\end{lemmaB}

\begin{lemmaB}[Expression Well-Typed Method Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:exp_weakening_method}
  If \([[SS1 ; TC ; TT |-tm ie : is ~> te]]\)
  and \([[|-ctx SS1, SS2; TC ; TT ]]\)
  then \([[SS1, SS2 ; TC ; TT |-tm ie : is ~> te]]\).
\end{lemmaB}

\begin{lemmaB}[Type Well-Formedness Dictionary Environment Weakening]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:ty_weakening}
  If \([[|-ctx SS ; TC1 ; TT1]]\)
  and \([[TC1 ; TT1 |-ty is ~> tt]]\)
  and \([[|-ctx SS ; TC1 , TC2 ; TT1 , TT2]]\),
  then \([[TC1 , TC2 ; TT1 , TT2 |-ty is ~> tt]]\).
\end{lemmaB}

\begin{lemmaB}[Class Constraint Well-Formedness Environment Weakening]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:q_weakening}
  If \([[ TC1 ; TT1 |-q iq ~> tt ]]\)
  and \([[ |-ctx SS ; TC1, TC2 ; TT1, TT2 ]]\)
  then \([[ TC1, TC2 ; TT1, TT2 |-q iq ~> tt ]]\).
\end{lemmaB}

\begin{lemmaB}[Logical Equivalence Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:log_weakening}
  If \([[ TC1 ; TT1 |- SS1 : ie1 =log SS2 : ie2 : is ]]\)
  and \([[ |-ctx SS1 , SS1' ; TC1 , TC2 ; TT1 , TT2 ]]\)
  and \([[ |-ctx SS2 , SS2' ; TC1 , TC2 ; TT1 , TT2 ]]\), \\
  then \([[ TC1 , TC2 ; TT1 , TT2 |- SS1 , SS1' : ie1 =log SS2 , SS2' : ie2 : is ]]\).
\end{lemmaB}

\begin{lemmaB}[Strong Normalization Relation Method Environment Weakening]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:sn_menv_weakening}
  If \([[ ie in SN (is) with SS1 ; TC ; RSN ]]\)
  and \([[ |-ctx SS1, SS2 ; TC ; TT ]]\)
  then \([[ ie in SN (is) with SS1, SS2 ; TC ; RSN ]]\).
\end{lemmaB}

\begin{lemmaB}[Dictionary Value Relation Preserved under Substitution]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:dict_Rsubst}
  \([[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R1, R2 ]]\)
  if and only if
  \([[ (SS1 : idv1 , SS2 : idv2) in V (R2 (iq)) with TC ; R1 ]]\).
\end{lemmaB}


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% INTER Lemmas
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Lemmas}

\begin{lemmaB}[Environment Well-Formedness Strengthening]\ \\
  \label{lemma:env_strengthening_mid}
  If \([[ |-ctx SS ; TC ; TT ]]\)
  then \([[ |-ctx SS ; TC ; empty ]]\).
\end{lemmaB}

\proof
By case analysis on the hypothesis,
the last rules used to construct it must be (possibly zero)
consecutive applications of \textsc{iCtx-MEnv}. Revert those rules, to obtain
\([[ |-ctx empty ; TC ; TT ]]\).
By further case analysis (with \textsc{iCtx-tyEnvTm}, \textsc{iCtx-tyEnvTy} and
\textsc{iCtx-tyEnvD}), we get \([[ |-ctx empty ; TC ; empty ]]\).
The goal follows by consecutively
re-applying rule \textsc{iCtx-MEnv} with the appropriate premises. \\
\qed

\begin{lemmaB}[Variable Strengthening in Dictionaries]\ \\
  If \([[ SS ; TC ; TT1, ix : is, TT2 |-d iD islj idli : iq ~> te ]]\)
  then \([[ SS ; TC ; TT1, TT2 |-d iD islj idli : iq ~> te ]]\).
  \label{lemma:var_subst_dict}
\end{lemmaB}

\proof
By straightforward induction on the well-formedness derivation. \\
\qed

\begin{lemmaB}[Variable Strengthening in Types]\ \\
  If\, \([[ TC ; TT1, ix : is, TT2 |-ty is'  ~> tt' ]]\)
  then\, \([[ TC ; TT1, TT2 |-ty is'  ~> tt' ]]\).
  \label{lemma:var_subst_types}
\end{lemmaB}

\proof
By straightforward induction on the well-formedness derivation. \\
\qed

\begin{lemmaB}[Method Type Well-Formedness]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:classmethodwty}
  If \([[ |-ctx SS ; TC ; TT]]\)
  and \([[TC = TC1 , im : iTC c : is , TC2 ]]\)
  then there is a \([[ tt ]]\) such,
  that \([[ TC1 ; empty , c |-ty is ~> tt ]]\).
\end{lemmaB}

\proof
By straightforward induction on the environment well-formedness derivation. \\
\qed

\begin{lemmaB}[Method Environment Well-Formedness]\ \\
  \renewcommand\itot[1]{#1}
  \label{lemma:inSS2C}
  If \([[ |-ctx SS ; TC ; TT]]\)
  and \([[ ( iD : \/ clj . iqli => iTC is ) . im |-> ie in SS ]]\), where $i = 1 \ldots n$,
  then there are unique $[[c]]$, $\intermed{[[ism]]}$, $\target{[[ttm]]}$ and \(\target{[[ ttli ]]}\), such
  that \([[ ( im : iTC c : ism ) in TC ]]\)
  and \([[ TC ; empty , c |-ty ism ~> ttm ]]\)
  and \([[ SS ; TC ; empty |-tm ie : \/ clj . iqli -> [| is / c |] ism ~> te ]]\)
  and \([[ </ TC ; empty , clj |-q iqi ~> tti // i /> ]]\).
  and \([[ TC ; empty , clj |-q iTC is ~> [| tt / ta |]{ tl : ttm } ]]\)
  and \([[ TC ; empty , clj |-ty is ~> tt ]]\).
\end{lemmaB}

\proof
By straightforward induction on the environment well-formedness derivation. \\
\qed

\begin{lemmaB}[Determinism of Evaluation]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:eval_unique}
  If \([[ SS |- ie --> ie1 ]]\)
  and \([[ SS |- ie --> ie2 ]]\)
  then \([[ ie1 = ie2 ]]\).
\end{lemmaB}

\proof
By straightforward induction on the evaluation derivation. \\
\qed

\begin{lemmaB}[Preservation of Environment Type Variables from \interL{} to \targetL{}]\leavevmode
  \begin{itemize}
  \item If \([[ c in TT ]]\)
    and \([[ TC ; TT ~> GT ]]\)
    then \([[ ta in GT ]]\).
  \item If \([[ c notin TT ]]\)
    and \([[ TC ; TT ~> GT ]]\)
    then \([[ ta notin GT ]]\).
  \end{itemize}
  \label{lemma:pres_env_tyT}
\end{lemmaB}

\proof
By straightforward induction on the environment elaboration derivation. \\
\qed

\begin{lemmaB}[Well-Formedness of \interL{} Typing Result]\ \\
  \renewcommand\itot[1]{{#1}}
  \label{lemma:type_well_inter_typing}
  If \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\)
  then \([[ TC ; TT |-ty is ~> tt ]]\).
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\begin{lemmaB}[Context Well-Formedness of \interL{} Typing]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:ctx_well_inter_typing}
  If \([[SS ; TC ; TT |-tm ie : is ~> te]]\)
  then \([[|-ctx SS ; TC ; TT]]\).
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\begin{lemmaB}[Context Well-Formedness of Dictionary Typing]\ \\
  \renewcommand\itot[1]{}
  \label{lemma:ctx_well_dict_typing}
  If \([[ SS ; TC ; TT |-d id : iq ~> te ]]\)
  then \([[|-ctx SS ; TC ; TT]]\).
\end{lemmaB}

\proof
By straightforward induction on the dictionary typing derivation. \\
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Type Safety
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Type Safety}


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Preservation]\ \\
  \label{thmA:intermediate_preservation}
  If $[[ SS ; TC ; TT |-tm ie : is ~> te ]]$,
  and $[[SS |- ie --> ie']]$,
  then $[[ SS ; TC ; TT |-tm ie' : is ~> te' ]]$.
\end{theoremB}

\proof
By induction on the typing derivation. \\
\proofStep{\textsc{iTm-true}}
{\drule{iTm-true}}
{ $[[itrue]]$ is already a value, so impossible case. \\
}
\proofStep{\textsc{iTm-false}}
{\drule{iTm-false}}
{ $[[ifalse]]$ is already a value, so impossible case. \\
}
\proofStep{\textsc{iTm-var}}
{\drule{iTm-var}}
{ $[[ix]]$ cannot be reduced, so impossible case. \\
}
\proofStep{\textsc{iTm-let}}
{\drule{iTm-let}}
{ By inversion on the evaluation (\textsc{iEval-let}), we get that
  \begin{equation*}
    [[ ie' = [| ie1 / ix |] ie2]]
  \end{equation*}
  Given
  \begin{gather*}
    [[SS ; TC ; TT |-tm ie1 : is1 ~> te1]]\\
    [[SS ; TC ; TT, ix : is1 |-tm ie2 : is2 ~> te2]]
  \end{gather*}
  The goal follows directly from Lemma~\ref{lemma:var_subst}. \\
}
\proofStep{\textsc{iTm-method}}
{\drule{iTm-method}}
{ By inversion on the evaluation (\textsc{iEval-method}), we get that 
  \begin{gather}
    \label{eq:pres:method:1}
    [[ie' =  ie islj idli ]] \\
    \label{eq:pres:method:2}
    [[id =  iD islj idli  ]] 
  \end{gather}
  The goal to be proven thus becomes:
  \begin{gather}
    \label{eq:pres:method:4}
    [[SS ; TC ; empty |-tm ie islj idli : [| is / c |] is' ~> te']]
  \end{gather}
  By substituting Equation~\ref{eq:pres:method:2} in the 1\textsuperscript{st} rule premise, we get that
  \begin{gather}
    \label{eq:pres:method:3}
    [[SS ; TC ; TT |-d  iD islj idli : iTC is ~> te]]
  \end{gather}
  By inversion on Equation~\ref{eq:pres:method:3} (\textsc{D-con}), we know that
  \begin{gather}
    \label{eq:pres:method:5}
    [[( iD : \/ clj . iqli => iTC is1) . im |-> /\ clj . \ idvarli : iqli . ie in SS]]\\
    \label{eq:pres:method:6}
    [[is =  [| islj / clj |] is1]] \\
    \label{eq:pres:method:7}
    [[</ SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei // i />]]\\
    \label{eq:pres:method:11}
    [[</ TC ; TT |-ty isj ~> ttj // j />]] \\
    \label{eq:pres:method:12}
    [[|-ctx SS; TC ; TT]]
  \end{gather}
  By combining this result with Equation~\ref{eq:pres:method:5}, through inversion
  (\textsc{iCtx-MEnv}), we know that
  \begin{gather}
    \label{eq:pres:method:8}
    [[SS1 ; TC ; empty |-tm /\ clj . \ idvarli : iqli . ie : \/ clj . iqli -> [| is1 / c |] is' ~> te1]]
  \end{gather}
  where \([[ SS = SS1 , ( iD : \/ clj . iqli => iTC is1) . im |-> /\ clj . \
  idvarli : iqli . ie , SS2 ]]\).
  By \textsc{iTm-forallE} and Equations~\ref{eq:pres:method:8} and
  \ref{eq:pres:method:11}, we have
  \begin{gather}
    \label{eq:pres:method:9}
    [[SS1 ; TC ; empty |-tm ie islj : [| islj / clj |] iqli -> [| islj / clj |]
    [| is1 / c |] is' ~> te1 ttlj]]
  \end{gather}
  By \textsc{iTm-constrE} and Equations~\ref{eq:pres:method:9} and \ref{eq:pres:method:7}, we have
  \begin{gather}
    \label{eq:pres:method:10}
    [[SS1 ; TC ; empty |-tm ie islj idli: [| islj / clj |]
    [| is1 / c |] is' ~> te1 ttlj teli]]
  \end{gather}
  From the 2\textsuperscript{nd} rule premise we know that
  \begin{gather}
    [[( im : iTC c : is' ) in TC]]
  \end{gather}
  Combining this result with Equation~\ref{eq:pres:method:12}, by inversion
  (\textsc{iCtx-clsEnv}), we know
  \begin{gather}
    [[TC1 ; empty, c |-ty is' ~> tt']] \\
    [[TC = TC1, TC2]]
  \end{gather}
  Therefore, $\intermed{[[islj]]}$ are not free variables in $\intermed{[[is']]}$.
  Equation~\ref{eq:pres:method:9} thus simplifies to
  \begin{gather}
    \label{eq:pres:method:13}
    [[SS1 ; TC ; empty |-tm ie islj idli: 
    [| [| islj / clj |]is1 / c |] is' ~> te1 ttlj teli]]
  \end{gather}
  By applying Equation~\ref{eq:pres:method:13} to
  Lemma~\ref{lemma:exp_weakening_method}, in combination with
  Equation~\ref{eq:pres:method:12}, we get
  \begin{gather*}
    [[SS ; TC ; empty |-tm ie islj idli: 
    [| [| islj / clj |]is1 / c |] is' ~> te1 ttlj teli]]
  \end{gather*}
  Goal~\ref{eq:pres:method:4} follows by combining this result with
  Equation~\ref{eq:pres:method:6}. \\
}
\proofStep{\textsc{iTm-arrI}}
{\drule{iTm-arrI}}
{$\intermed{[[\ ix : is1 . ie]]}$ is already a value, so impossible case. \\}
\proofStep{\textsc{iTm-arrE}}
{\drule{iTm-arrE}}
{
  By inversion on the evaluation, we have two possible cases:
    \begin{itemize}
    \item Case \textsc{iEval-app}.
      \drule{iEval-app}

      By induction hypothesis, we get
      \begin{gather*}
        [[ SS ; TC ; TT |-tm ie1' : is1 -> is2 ~> te']]
      \end{gather*}
      By \textsc{iTm-arrE} we get
      \begin{gather*}
        [[SS ; TC ; TT |-tm ie1' ie2 : is2 ~> te1 te2]]
      \end{gather*}
    \item Case \textsc{iEval-appAbs}.
      $\ottdruleiEvalXXappAbs{}$

      From premise, we know
      \begin{gather*}
        [[SS ; TC ; TT |-tm  \ ix : is . ie1 : is -> is2 ~> te1]]
      \end{gather*}
      By inversion (\textsc{iTm-arrI})
      \begin{gather*}
        [[SS ; TC ; TT, ix : is |-tm  ie1 : is2 ~> te1]]
      \end{gather*}
      By substitution (Lemma~\ref{lemma:var_subst}) we get
      \begin{gather*}
        [[SS ; TC ; TT |-tm [| ie2 / ix|] ie1 : is2 ~> [| te2 / tx |] te1]]
      \end{gather*}
    \end{itemize}
}
\proofStep{\textsc{iTm-constrI}}
{\drule{iTm-constrI}}
{$\intermed{[[\ idvar : iq . ie]]}$ is already a value, so impossible case. \\}
\proofStep{\textsc{iTm-constrE}}
{\drule{iTm-constrE}}
{Similar to case \textsc{iTm-arrE}. The only difference lies in applying
  Lemma~\ref{lemma:dvar_subst}. \\}
\proofStep{\textsc{iTm-forallI}}
{\drule{iTm-constrI}}
{$\intermed{[[/\ c . ie]]}$ is already a value, so impossible case. \\}
\proofStep{\textsc{iTm-forallE}}
{\drule{iTm-forallE}}
{Similar to case \textsc{iTm-arrE}. The only difference lies in applying Lemma~\ref{lemma:tvar_subst}.}

\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Progress]\ \\
  If $[[SS ; empty ; empty |-tm ie : is ~> te]]$,
  then either $[[ie]]$ is a value,
  or there exists $\intermed{[[ie']]}$ such that $[[SS |- ie --> ie']]$.
\label{thmA:progress_expressions}
\end{theoremB}

\proof By structural induction on the typing derivation. \\
\proofStep{\textsc{iTm-true}}
{ \drule{iTm-true}}
{
  with $[[TC = empty]]$, $[[TT = empty]]$.

  $[[itrue]]$ is a value. \\
}
\proofStep{\textsc{iTm-false}}
  { \drule{iTm-false} }
  { 
     with $[[TC = empty]]$, $[[TT = empty]]$.

     $[[ifalse]]$ is a value. \\
  }
\proofStep{\textsc{iTm-var}}
  { \drule{iTm-var} }
  {
     with $[[TC = empty]]$, $[[TT = empty]]$.

    $[[ix]]$ cannot be in an empty context. Impossible case. \\
  }
\proofStep{\textsc{iTm-let}}
  { \drule{iTm-let} }
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    By \textsc{iEval-let}:
    \begin{equation*}
      [[ie' =  [| ie1 / ix |] ie2]]
    \end{equation*}
  }
\proofStep{\textsc{iTm-method}}
  { \drule{iTm-method} }
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    $[[im]]$ cannot be in an empty context. Impossible case. \\
  }
\proofStep{\textsc{iTm-arrI}}
  { \drule{iTm-arrI} }
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    $\intermed{ [[\ ix : is1 . ie]] }$ is a value. \\
  }
\proofStep{\textsc{iTm-arrE}}
  {\drule{iTm-arrE} }
  {

    with $[[TC = empty]]$, $[[TT = empty]]$.

    From the 1\textsuperscript{st} rule premise:
    \begin{equation}
      [[SS ; TC ; TT |-tm ie1 : is1 -> is2 ~> te1]]
      \label{proofeq:progress_app1}
    \end{equation}
    By applying the induction hypothesis on Equation~\ref{proofeq:progress_app1},
    we know that either:
    \begin{itemize}
    \item \( \intermed{ [[ie1]] } \) is a value. Because it has an arrow type, we know:
      \begin{equation*}
        [[ie1 = ( \ ix : is . ie1 ) ie2]]
      \end{equation*}
      By \textsc{iEval-appAbs}:
      \begin{equation*}
        [[ie' =  [| ie2 / ix |] ie1]]
      \end{equation*}
    \item There exists an $ \intermed { [[ ie1' ]] } $ where \( [[SS |- ie1 --> ie1']] \).
      By \textsc{iEval-app}:
      \begin{equation*}
        [[ie' = ie1' ie2]]
      \end{equation*}
    \end{itemize}
  }
\proofStep{\textsc{iTm-constrI}}
  {\drule{iTm-constrI}}
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    \( \intermed{ [[\ idvar : iq . ie]] } \) is a value. \\
  }
\proofStep{\textsc{iTm-constrE}}
  {\drule{iTm-constrE}}
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    From the 1\textsuperscript{st} rule premise:
    \begin{equation}
      [[SS ; TC ; TT |-tm ie : iq -> is ~> te1]]
      \label{proofeq:progress_dapp1}
    \end{equation}
    By applying the induction hypothesis on
    Equation~\ref{proofeq:progress_dapp1}, we know that either:
    \begin{itemize}
    \item \( \intermed{ [[ie1]] } \) is a value. By case analysis, we know:
      \begin{equation*}
        [[ie1 = ( \ idvar : iq . ie )]]
      \end{equation*}
      By \textsc{iEval-DAppAbs}:
      \begin{equation*}
        [[ie' = [| id / idvar |] ie ]]
      \end{equation*}
    \item There exists an \( \intermed { [[ie']] } \) where $[[SS |- ie --> ie']]$
      By \textsc{iEval-DApp}:
      \begin{equation*}
        [[SS |- ie id --> ie' id]]
      \end{equation*}
    \end{itemize}
  }
\proofStep{\textsc{iTm-forallI}}
  {\drule{iTm-forallI}}
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    $ \intermed { [[/\ c . ie]] } $ is a value. \\
  }
\proofStep{\textsc{iTm-forallE}}
  {\drule{iTm-forallE}}
  {
    with $[[TC = empty]]$, $[[TT = empty]]$.

    From the 1\textsuperscript{st} rule premise:
    \begin{equation}
      [[SS ; TC ; TT |-tm ie : \/ c . is' ~> te]]
      \label{proofeq:progress_tyapp1}
    \end{equation}
    By applying the induction hypothesis on
    Equation~\ref{proofeq:progress_tyapp1}, we know that either:
    \begin{itemize}
    \item \( \intermed { [[ie1]] } \) is a value. By case analysis, we know:
      \begin{equation*}
        [[ie1 = ( /\ c . ie )]]
      \end{equation*}
      By \textsc{iEval-tyAppAbs}:
      \begin{equation*}
        [[ie' =  [| is / c |] ie]]
      \end{equation*}
    \item There exists an \( \intermed{ [[ie1']] } \) where \( [[SS |- ie --> ie']] \).
      By \textsc{iEval-tyApp}:
      \begin{equation*}
        [[ie' = ie1' is]]
      \end{equation*}
    \end{itemize}
  }
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Strong Normalization
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Strong Normalization}
\label{app:sn}
\renewcommand\itot[1]{}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Strong Normalization]\ \\
  If \([[ SS ; TC ; empty |-tm ie : is ~> te ]]\)
  then all possible evaluation derivations for \([[ie]]\) terminate :
  \( \exists [[iv]] : [[ SS |- ie -->> iv ]]\).
  \label{thmA:strong_norm}
\end{theoremB}
\proof By Theorem~\ref{thmA:sn:part:a} and \ref{thmA:sn:part:b}, with $[[RSN]] =
\intermed{[[empty]]}$, $[[phiSN = empty]]$, $[[gammaSN = empty]]$, since $[[TT = empty]]$,
it follows that:
\begin{equation*}
  \exists [[iv]] : [[ SS |- ie -->> iv ]]
\end{equation*}
Furthermore, since evaluation in \interL{} is deterministic
(Lemma~\ref{lemma:eval_unique}), there is exactly 1
possible evaluation derivation. Consequently, all derivations terminate. \\
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -

\begin{lemmaB}[Well Typedness from Strong Normalization]\ \\
  \label{lemma:sn_typing}
  $[[ ie in SN (is) with SS ; TC ; RSN]]$,
  then $[[ SS ; TC ; empty |-tm ie : RSN(is) ~> te ]]$
\end{lemmaB}
\proof The goal is baked into the relation. It follows by simple induction on
$[[is]]$. \\
\qed

\begin{lemmaB}[Strong Normalization preserved by forward/backward reduction]\ \\
  \label{lemma:sn_pres}
  Suppose $[[SS ; TC ; empty |-tm ie1 : RSN (is) ~> te1]]$,
  and $[[SS |- ie1 --> ie2 ]]$, then
  \begin{itemize}
    \item If $[[ ie1 in SN (is) with SS ; TC ; RSN]]$,
      then $[[ ie2 in SN (is) with SS ; TC ; RSN]]$.
    \item If $[[ ie2 in SN (is) with SS ; TC ; RSN]]$,
      then $[[ ie1 in SN (is) with SS ; TC ; RSN]]$.
  \end{itemize}
\end{lemmaB}
\proof

\begin{description}
  \item[Part 1]
    By induction on $[[is]]$. \\
    \proofStep{Bool}
    {
      \begin{aligned}
    [[ ie1 in SN ( ibool ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie1 : ibool ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie1 -->> iv ]] \\
      \end{aligned}
    }
    {
      By Preservation (Theorem~\ref{thmA:intermediate_preservation}), we know
      that $[[ SS ; TC ; empty |-tm ie2 : ibool ~> te ]]$.
      Because the evaluation in \interL{} is deterministic (Lemma~\ref{lemma:eval_unique}), given $[[SS |- ie1 -->> iv]]$,
      we have $[[SS |- ie2 -->> iv]]$. \\
    }
    \proofStep{Type variable}
    {
      \begin{aligned}
    [[ ie1 in SN ( c ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie1 : RSN1 ( c ) ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie1 -->> iv ]] \\
    & \land [[ iv in RSN2 ( c ) ]] \\
      \end{aligned}
    }
    {
      Similar to Bool case. \\}
    \proofStep{Function}
    {
      \begin{aligned}
    [[ ie1 in SN ( is1 -> is2 ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie1 : RSN1 ( is1 -> is2 ) ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie1 -->> iv ]] \\
    & \land \forall [[ ie' ]] : [[ ie' in SN ( is1 ) with SS ; TC ; RSN ]]
      \Rightarrow [[ ie1 ie' in SN ( is2 ) with SS ; TC ; RSN ]] \\
      \end{aligned}
    }
    {
      By Preservation (Theorem~\ref{thmA:intermediate_preservation}), we know
      that $[[ SS ; TC ; empty |-tm ie2 : RSN1 ( is1 -> is2 ) ~> te ]]$. Because
      the evaluation
      in \interL{} is deterministic (Lemma~\ref{lemma:eval_unique}), given $[[SS |- ie1 -->> iv]]$, we have $[[SS |-
      ie2 -->> iv]]$. Given any $[[ ie' ]] : [[ ie' in SN ( is1 ) with SS ; TC ;
      RSN ]]$, we know that $[[SS |- ie1 --> ie2]]$, so $[[SS |- ie1 ie' --> ie2
      ie']]$. By induction hypothesis, we get $ [[ ie2 ie' in SN ( is2 ) with SS
      ; TC ; RSN ]] $. \\
    }
    \proofStep{Function over constraint}
    {[[ ie in SN ( iq -> is ) with SS ; TC ; RSN ]]}
    {
      Similar to Function case. \\
    }
    \proofStep{Polymorphic type}
    {[[ ie in SN ( \/ c . is ) with SS ; TC ; RSN ]]}
    {
      Similar to Function case.
    }

    \item[Part 2]
      Similar to Part 1.
\end{description}
\qed

\begin{lemmaB}[Substitution for Context Interpretation]\leavevmode
  \label{lemma:sn_ctx_inter}
  \begin{itemize}
    \item
  If \([[ SS ; TC ; TT |-tm ie : is ~> te1 ]]\)
  then \( \forall [[ RSN in FSN (TT) with SS; TC ]]\),
  \([[ phiSN in GSN (TT) with SS ; TC ; RSN ]]\) and
  \([[ gammaSN in HSN (TT) with SS ; TC ; RSN ]]\), \\
  we have $[[SS ; TC ; empty |-tm ie with RSN ; phiSN ; gammaSN : RSN (is) ~> te2]]$.
    \item
  If \([[ SS ; TC ; TT |-d id : iq ~> te1 ]]\)
  then \( \forall [[ RSN in FSN (TT) with SS; TC ]]\),
  \([[ phiSN in GSN (TT) with SS ; TC ; RSN ]]\) and
  \([[ gammaSN in HSN (TT) with SS ; TC ; RSN ]]\), \\
  we have $[[SS ; TC ; empty |-d id with RSN ; phiSN ; gammaSN : RSN (iq) ~> te2]]$.
    \item
  If \([[ TC ; TT |-ty is ~> tt ]]\)
  then \( \forall [[ RSN in FSN (TT) with SS; TC ]]\),
  \([[ phiSN in GSN (TT) with SS ; TC ; RSN ]]\) and
  \([[ gammaSN in HSN (TT) with SS ; TC ; RSN ]]\), \\
  we have $[[TC ; empty |-ty RSN (is) ~> tt2]]$.
  \item
  If \([[ TC ; TT |-q iq ~> tt ]]\)
  then \( \forall [[ RSN in FSN (TT) with SS; TC ]]\),
  \([[ phiSN in GSN (TT) with SS ; TC ; RSN ]]\) and
  \([[ gammaSN in HSN (TT) with SS ; TC ; RSN ]]\), \\
  we have $[[TC ; empty |-q RSN (iq) ~> tt2]]$.
  \end{itemize}
\end{lemmaB}

\proof

By induction on $[[ie]]$, $[[id]]$ $[[is]]$, and $[[iq]]$
respectively. The goal follows from Definitions~\ref{def:inter_ty},
\ref{def:inter_tm} and \ref{def:inter_d}.

\qed


\begin{lemmaB}[Compositionality for Strong Normalization]\ \\
  \label{lemma:comp_sn}
  Let $[[r]]$ = $[[SN(is2) with SS ; TC ; RSN]]$,
  then $[[ ie in SN (is1) with SS ; TC ; RSN , c |-> (RSN(is2), r) ]]$
  if and only if $[[ ie in SN ([|is2 / c |]is1) with SS ; TC ; RSN ]]$.
\end{lemmaB}

\proof

By induction on $[[is1]]$. \\
\proofStep{Bool}
{[[is1 = ibool]]}
{
  Since $[[ [|is2/c|] ibool  = ibool]]$, the goal follows directly. \\
}
\proofStep{Type variable}
{[[is1 = ib]]}
{
  Depending on whether $[[ib]]$ is the same variable as $[[c]]$, we have two cases:
  \begin{itemize}
    \item If $[[ib = c]]$, then $[[ [|is2/c|] c   = is2]]$.
      \begin{description}
        \item[Part 1: From left to right.]
      If $[[  ie in SN (c) with SS ; TC ; RSN , c |-> (RSN(is2), r)  ]]$, it
      means that:
      \begin{gather}
        \label{eq:comp:var:1}
        \exists [[ iv ]] : [[ SS |- ie -->> iv ]]  \\
        \label{eq:comp:var:2}
        [[iv in SN ( is2 ) with SS ; TC ; RSN ]]
      \end{gather}
      Combining with Strong Normalization preserved by forward/backward
      reduction (Lemma~\ref{lemma:sn_pres}), the goal is proven by
      Equations~\ref{eq:comp:var:1} and \ref{eq:comp:var:2}:
      \begin{gather}
        [[ie in SN ( is2 ) with SS ; TC ; RSN ]]
      \end{gather}
        \item[Part 2: From right to left.]
          From the hypothesis, we know that:
          \begin{gather}
            \label{eq:comp:var:3}
            [[ie in SN ( is2 ) with SS ; TC ; RSN ]]
          \end{gather}
          We want to
          prove that $[[  ie in SN (c) with SS ; TC ; RSN , c |-> (RSN(is2),
          r)  ]]$. By the definition, this goal is equivalent to:
          \begin{gather}
            \label{eq:comp:var:4}
            [[ SS ; TC ; empty |-tm ie : (RSN, c |-> (RSN(is2), r)) ( c ) ~> te ]] \\
            \label{eq:comp:var:5}
            \exists [[ iv ]] : [[ SS |- ie -->> iv ]]  \\
            \label{eq:comp:var:6}
            [[ iv in (RSN, c|-> (RSN(is2), r)) ]]_2~[[ ( c ) ]]
          \end{gather}
        Equation~\ref{eq:comp:var:4} simplifies to:
          \begin{gather}
            \label{eq:comp:var:7}
            [[ SS ; TC ; empty |-tm ie : RSN(is2) ~> te ]] 
          \end{gather}
        By Well-Typedness from Strong Normalization
        (Lemma~\ref{lemma:sn_typing}), Equation~\ref{eq:comp:var:3} proves
        \ref{eq:comp:var:7}.
        By  Strong Normalization - Part B (Theorem~\ref{thmA:sn:part:b}),
        Equation~\ref{eq:comp:var:3} proves \ref{eq:comp:var:5}.

        We already know that $[[ (RSN, c|-> (RSN(is2), r)) ]]_2~[[ ( c ) ]] = [[ r]] =
        [[SN(is2) with SS ; TC ; RSN]]$, so we simplify
        Equation~\ref{eq:comp:var:6} to get
          \begin{gather}
            \label{eq:comp:var:8}
            [[ iv in SN(is2) with SS ; TC ; RSN ]]
          \end{gather}
          From Equation~\ref{eq:comp:var:3} and Strong Normalization preserved
          by forward/backward reduction (Lemma~\ref{lemma:sn_pres}), we can
          prove Goal~\ref{eq:comp:var:8}.
        \end{description}
        
    \item If $[[ib]] \neq [[c]]$, since $[[ [|is2/c|] ib  = ib]]$, the goal
      follows directly.
  \end{itemize}
}
\proofStep{Function}
{[[is1 = is11 -> is12]]}
{
  \begin{description}
    \item[Part 1: From left to right.]

  From the hypothesis, we get:
  \begin{equation*}
    [[ ie in SN (is11 -> is12) with SS ; TC ; RSN , c |-> (RSN(is2), r) ]]
  \end{equation*}
  We thus know that:
  \begin{gather}
    \label{eq:comp:arr:1}
    [[ SS ; TC ; empty |-tm ie : (RSN, c |-> (RSN(is2), r)) ( is11 -> is12 ) ~> te ]] \\
    \label{eq:comp:arr:2}
     \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    \label{eq:comp:arr:3}
     \forall [[ ie' ]] : [[ ie' in SN ( is11 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]]
      \Rightarrow [[ ie ie' in SN ( is12 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]] 
  \end{gather}
  Our goal is to prove that $[[ ie in SN ( [|is2 / c|] is11 -> [|is2 / c|] is12) with SS ; TC ; RSN
  ]]$. This is equivalent to proving:
  \begin{gather}
    \label{eq:comp:arr:4}
    [[ SS ; TC ; empty |-tm ie : RSN ( [|is2/ c|] is11 -> [|is2/ c|] is12)  ~> te ]] \\
    \label{eq:comp:arr:5}
     \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    \label{eq:comp:arr:6}
     \forall [[ ie' ]] : [[ ie' in SN ( [|is2/ c|]is11 ) with SS ; TC ; RSN ]]
      \Rightarrow [[ ie ie' in SN ( [|is2/ c|]is12) with SS ; TC ; RSN ]] 
  \end{gather}
  Goal~\ref{eq:comp:arr:4} and \ref{eq:comp:arr:5} are proven directly by
  Equations~\ref{eq:comp:arr:1} and \ref{eq:comp:arr:2}. Only
  Goal~\ref{eq:comp:arr:6} remains to be proven.
  
  Given  $[[ ie' in SN ( [|is2/ c|]is11 ) with SS ; TC ; RSN ]]$, the induction
  hypothesis tells us that $[[ ie' in SN (is11 ) with SS ; TC ; RSN, c |-> (RSN(is2), r)
  ]]$. In combination with equation Equation~\ref{eq:comp:arr:3}, we get
  \begin{align}
      [[ ie ie' in SN ( is12 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]] 
  \end{align}
  By induction hypothesis, we get:
  \begin{align}
      [[ ie ie' in SN ( [|is2/ c|]is12) with SS ; TC ; RSN ]] 
  \end{align}
  The goal has been proven.
    \item[Part 2: From right to left.] Similar to Part 1. \\
      \end{description} 
}
\proofStep{Function over constraints}
{[[is1 = iq -> is12]]}
{
  \begin{description}
    \item[Part 1: From left to right.]

  We know from the hypothesis that:
  \begin{equation*}
    [[ ie in SN (iq -> is12) with SS ; TC ; RSN , c |-> (RSN(is2), r) ]]
  \end{equation*}
  It follows that:
  \begin{gather}
    \label{eq:comp:arrc:1}
    [[ SS ; TC ; empty |-tm ie : (RSN, c |-> (RSN(is2), r)) ( iq -> is12 ) ~> te ]] \\
    \label{eq:comp:arrc:2}
     \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    \label{eq:comp:arrc:3}
      \forall [[ id ]] : [[ SS ; TC ; empty |-d id :  (RSN, c |-> (RSN(is2), r))(iq) ~> te ]]
      \Rightarrow [[ ie id in SN ( is12 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]] 
  \end{gather}
  Our goal is to prove that $[[ ie in SN ( [|is2 / c|] iq -> [|is2 / c|] is12) with SS ; TC ; RSN
  ]]$. This is equivalent to proving:
  \begin{gather}
    \label{eq:comp:arrc:4}
    [[ SS ; TC ; empty |-tm ie : RSN ( [|is2/ c|] iq -> [|is2/ c|] is12)  ~> te ]] \\
    \label{eq:comp:arrc:5}
     \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    \label{eq:comp:arrc:6}
     \forall [[ id' ]] : [[ SS ; TC ; empty |-d id' : RSN1 ( [|is2/ c|]iq) ~> te ]]
      \Rightarrow [[ ie id' in SN ( [|is2/ c|] is12) with SS ; TC ; RSN ]] 
  \end{gather}
  Goals~\ref{eq:comp:arrc:4} and \ref{eq:comp:arrc:5} are proven directly by
  Equations~\ref{eq:comp:arrc:1} and \ref{eq:comp:arrc:2}.
  Only Goal~\ref{eq:comp:arrc:6} remains to be proven.
  Given  $[[ SS ; TC ; empty |-d id' : RSN1 ( [|is2/ c|]iq) ~> te ]]$,
  in combination with Equation~\ref{eq:comp:arrc:3}, we get that:
  \begin{gather}
      [[ ie id' in SN ( is12 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]] 
  \end{gather}
  By induction hypothesis, we get:
  \begin{gather}
      [[ ie id' in SN ( [|is2/ c|]is12) with SS ; TC ; RSN ]] 
  \end{gather}
  The goal has been proven.
    \item[Part 2: From right to left.] Similar to Part 1. \\
      \end{description}
}
\proofStep{Polymorphic types}
{ [[is1 = \/ ib. is12]] }
{
  \begin{description}
    \item[Part 1: From left to right.]

  We know from the hypothesis that:
  \begin{equation*}
    [[ ie in SN (\/ ib. is12) with SS ; TC ; RSN , c |-> (RSN(is2), r) ]]
  \end{equation*}
  This implies that:
  \begin{gather}
    \label{eq:comp:all:1}
    [[ SS ; TC ; empty |-tm ie : (RSN, c |-> (RSN(is2), r)) ( \/ ib. is12 ) ~> te ]] \\
    \label{eq:comp:all:2}
     \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    \label{eq:comp:all:3}
      \forall [[ is' ]] , [[ r = SN ( is' ) with SS ; TC ; RSN ]] :
      [[ ie is' in SN ( is12 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]] 
  \end{gather}
  Our goal is to prove that $[[ ie in SN ( \/ ib. [|is2 / c|] is12) with SS ; TC ; RSN
  ]]$. This is equivalent to proving:
  \begin{gather}
    \label{eq:comp:all:4}
    [[ SS ; TC ; empty |-tm ie : RSN (\/ ib. [|is2/ c|] is12)  ~> te ]] \\
    \label{eq:comp:all:5}
     \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    \label{eq:comp:all:6}
     \forall [[ is' ]] , [[ r = SN ( is' ) with SS ; TC ; RSN ]]
      \Rightarrow [[ ie is' in SN ( [|is2/ c|] is12) with SS ; TC ; RSN ]] 
  \end{gather}
  Goals~\ref{eq:comp:all:4} and \ref{eq:comp:all:5} are directly proven by
  Equations~\ref{eq:comp:all:1} and \ref{eq:comp:all:2}.
  Only Goal~\ref{eq:comp:all:6} remains to be proven.
  Given  $[[is']]$ and $[[ r = SN ( is' ) with SS ; TC ; RSN ]]$,
  by feeding it to Equation~\ref{eq:comp:all:3}, we get that:
  \begin{gather}
      [[ ie is' in SN ( is12 ) with SS ; TC ; RSN, c |-> (RSN(is2), r) ]] 
  \end{gather}
  By induction hypothesis, we get:
  \begin{gather}
      [[ ie is' in SN ( [|is2/ c|]is12) with SS ; TC ; RSN ]] 
  \end{gather}
  The goal has been proven.
    \item[Part 2: From right to left.] Similar to Part 1.
      \end{description}
}
\qed

\begin{corollaryB}[Compositionality for Strong Normalization (Context Interpretation)]
  \label{cor:comp_sn_ctx}
  Suppose $[[RSN in FSN (TT) with SS;TC]]$,
  then $[[ ie in SN (is) with SS ; TC ; RSN ]]$
  if and only if $[[ ie in SN (RSN (is)) with SS ; TC ; empty ]]$.
\end{corollaryB}

\proof

The choices from $[[RSN in FSN(TT) with SS; TC]]$ always satisfy the
precondition of Compositionality for Strong Normalization
(Lemma~\ref{lemma:comp_sn}). Therefore,
we can do
induction on $[[TT]]$ and apply Compositionality for Strong Normalization
(Lemma~\ref{lemma:comp_sn}), in combination with the induction hypothesis,
to prove the goal.

\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Strong Normalization - Part A]\ \\
  \label{thmA:sn:part:a}
  If \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\)
  then \( \forall [[ RSN in FSN (TT) with SS; TC ]]\),
  \([[ phiSN in GSN (TT) with SS ; TC ; RSN ]]\) and
  \([[ gammaSN in HSN (TT) with SS ; TC ; RSN ]]\), \\
  it holds that \([[ ie with RSN ; phiSN ; gammaSN in SN (is) with SS ; TC ; RSN ]]\).
\end{theoremB}

\proof By induction on the first hypothesis of the theorem.\\
\proofStep{\textsc{iTm-true}}
{\drule{iTm-true}}
{We know $[[itrue with RSN ; phiSN ; gammaSN = itrue]]$. So the goal is
  $[[itrue in SN(is) with SS; TC ; RSN]]$. The goal follows directly since
  $[[SS; TC; empty |-tm itrue : ibool ~> ttrue]]$ and $[[SS |- itrue -->> itrue
  ]]$. \\
}
\proofStep{\textsc{iTm-false}}
{\drule{iTm-false}}
{ Similar to the \textsc{iTm-true} case. \\
}
\proofStep{\textsc{iTm-var}}
{\drule{iTm-var}}
{
  We know that $[[  phiSN in GSN (TT) with SS ; TC ; RSN ]]$ and $[[(ix : is)
  in TT]]$, so we know that $[[ix |-> ie in phiSN]]$ for some $[[ie]]$ with $[[ie
   in SN(is) with SS;TC;RSN]]$. Since $[[ie
   in SN(is) with SS;TC;RSN]]$, we know from the definition of the relation that $[[ie]]$ does not
   contain any free variables in $[[TT]]$. Consequently, $\intermed{[[ie with RSN; phiSN ; gammaSN]]} =
   [[ie]]$. Therefore, $[[ix with RSN ; phiSN ; gammaSN = ie]]$. Now our goal
   becomes $[[ie in SN(is) with SS;TC;RSN]]$, which we already know. \\
}
\proofStep{\textsc{iTm-let}}
{\drule{iTm-let}}
{
  By induction hypothesis, we know
  \begin{gather}
    \label{eq:sn:let1}
    [[ie1 with RSN ; phiSN ; gammaSN in SN (is1) with SS; TC ; RSN]] \\
    \label{eq:sn:let1b}
    [[ie2 with RSN ; phiSN2 ; gammaSN in SN (is2) with SS; TC ; RSN]]
  \end{gather}
  Given Equation~\ref{eq:sn:let1}, we can choose $[[phiSN2 = phiSN, ix |->
  ie1 with RSN ; phiSN ; gammaSN]]$. Equation~\ref{eq:sn:let1b} thus reduces to:
  \begin{gather}
    \label{eq:sn:let2}
    [[ie2 with RSN ; phiSN, ix |-> ie1 with RSN ; phiSN ; gammaSN ; gammaSN in SN (is2) with SS; TC ; RSN]]
  \end{gather}
  Simplifying Equation~\ref{eq:sn:let2} results in:
  \begin{gather}
    \label{eq:sn:let3}
    [[ [| ie1 with RSN ; phiSN ; gammaSN / ix|] (ie2 with RSN ; phiSN ; gammaSN) in SN (is2) with SS; TC ; RSN]]
  \end{gather}
  Our goal is $[[ilet ix : is1 = ie1 iin ie2 with RSN; phiSN ; gammaSN in
  SN(is2) with SS; TC ; RSN]]$.

  We know that
  \begin{gather}
    \intermed{[[ilet ix : is1 = ie1 iin ie2 with RSN; phiSN ; gammaSN]]} \nonumber \\
    \label{eq:sn:let4}
    = \intermed{[[ilet ix : is1 = (ie1 with RSN; phiSN ; gammaSN) iin (ie2 with RSN ;
    phiSN ; gammaSN)]]} \\
    [[SS]] [[|-]] \intermed{[[ilet ix : is1 = (ie1 with RSN; phiSN ; gammaSN) iin (ie2
    with RSN ; phiSN ; gammaSN)]]} \nonumber \\
    \label{eq:sn:let5}
    [[-->]] \intermed{[[ [| ie1 with RSN ; phiSN ; gammaSN / ix|] (ie2 with RSN ; phiSN ; gammaSN) ]]}
  \end{gather}
  Consequently, by Substitution for Context Interpretation (Lemma~\ref{lemma:sn_ctx_inter}), we
  know that 
  \begin{gather}
    \label{eq:sn:let6}
    [[ SS ; TC ; empty |-tm 
    ilet ix : is1 = (ie1 with RSN; phiSN ; gammaSN) iin (ie2
    with RSN ; phiSN ; gammaSN)
    : RSN (is2) ~> te]]
  \end{gather}
  By Equations~\ref{eq:sn:let3}, \ref{eq:sn:let5} and \ref{eq:sn:let6}, in
  combination with Strong
  Normalization preserved by forward/backward reduction
  (Lemma~\ref{lemma:sn_pres}), we get that
  \begin{gather}
    \label{eq:sn:let7}
    [[
    ilet ix : is1 = (ie1 with RSN; phiSN ; gammaSN) iin (ie2
    with RSN ; phiSN ; gammaSN) 
    in SN (is2) with SS; TC ; RSN
    ]]
  \end{gather}
  The goal follows from Equations~\ref{eq:sn:let4} and \ref{eq:sn:let7}. \\
}
\proofStep{\textsc{iTm-method}}
{\drule{iTm-method}}
{
  By inversion on the dictionary typing, we have two cases:

  \begin{itemize}
    \item $\drule{D-var}$
      with $[[iq = iTC is]]$.
      
      Given $[[ gammaSN in HSN (TT) with SS ; TC ; RSN ]]$, we know that there
      exists a $[[idv]]$ in $[[gammaSN]]$ such that
      \begin{gather}
        \label{eq:sn:method1}
        [[ SS ; TC ; empty |-d idv : iTC RSN(is) ~> te]].
      \end{gather}
      Without loss of generality, suppose
      \begin{gather}
        \label{eq:sn:method3}
      [[idv = iD islj idvlj]].
      \end{gather}
      Therefore
      \begin{gather}
        \label{eq:sn:method2}
      [[id . im with RSN ; phiSN ; gammaSN = ( iD islj idvlj ) . im]].
      \end{gather}
      Now our goal is to prove that:
      \begin{gather}
        \label{eq:sn:method21}
      [[( iD islj idvlj ) . im in SN ([| is / c |] is') with SS ; TC ; RSN]].
      \end{gather}
      Substituting Equation~\ref{eq:sn:method3} in Equation~\ref{eq:sn:method1}
      results in:
      \begin{gather}
        \label{eq:sn:method4}
        [[ SS ; TC ; empty |-d iD islj idvlj : iTC RSN(is) ~> te]].
      \end{gather}
      By inversion, we have
      \begin{gather}
        \label{eq:sn:method5}
        [[( iD : \/ clj . iqli => iTC is1) . im |-> /\ clj . \ idvarli : iqli . ie in SS]]\\
        \label{eq:sn:method51}
        [[</ SS ; TC ; empty |-d idvi : [| islj / clj |] iqi ~> tei // i />]] \\
        \label{eq:sn:method52}
        [[RSN(is) =  [| islj / clj |] is1]] \\
        \label{eq:sn:method53}
        [[ |-ctx SS ; TC ; TT ]] \\
        \label{eq:sn:method53b}
        [[ </ TC ; empty, clj |-q iqi ~> tt // i /> ]] \\
        \label{eq:sn:method53d}
        [[ </ TC ; TT |-ty isj ~> ttj // j /> ]] \\
        \label{eq:sn:method54}
        [[ SS1 ; TC ; empty, clj, idvarli : iqli |-tm ie : [| is1 / c |] is' ~> te ]]
        \\
        \nonumber
        \textit{where}~[[ SS = SS1 , ( iD : \/ clj . iqli => iTC is1) . im |->
        /\ clj . \ idvarli : iqli . ie, SS2 ]]
      \end{gather}
      By evaluation rule (\textsc{iEval}), together with Equation~\ref{eq:sn:method5}, we
      know that:
      \begin{gather}
        \label{eq:sn:method10}
        [[SS |- ( iD islj idvlj ) . im --> (/\ clj . \ idvarli : iqli . ie) islj idvlj]]
      \end{gather}
      By Strong Normalization preserved by forward/backward reduction
      (Lemma~\ref{lemma:sn_pres}), Goal~\ref{eq:sn:method21} becomes:
      \begin{gather}
        \label{eq:sn:method11}
      [[ie islj idvlj in SN ([| is / c |] is') with SS ; TC ; RSN]].
      \end{gather}
      By applying weakening Lemma~\ref{lemma:q_weakening} on
      Equation~\ref{eq:sn:method53b}, we get:
      \begin{gather}
        [[ </ TC ; TT |-q iqi ~> tt // i /> ]] \\
        \label{eq:sn:method53c}
      \end{gather}
      By applying rules \textsc{iTm-forallI} and \textsc{iTm-constrI} (in
      combination with Equation~\ref{eq:sn:method53c}) on
      Equation~\ref{eq:sn:method54}, we get that:
      \begin{gather}
        \label{eq:sn:method55}
        [[ SS1 ; TC ; empty |-tm /\ clj . \ idvarl : iqli . ie : \/ clj . iqli
        -> [| is1 / c |] is' ~> te ]]
      \end{gather}
      By applying rules \textsc{iTm-forallE} (in combination with
      Equation~\ref{eq:sn:method53d}) and \textsc{iTm-constrE} (in combination
      with Equation~\ref{eq:sn:method51}) on Equation~\ref{eq:sn:method55}, we
      get that:
      \begin{gather}
        \label{eq:sn:method301}
        [[SS1 ; TC ; empty |-tm ie islj idvli :  [|islj / clj|] [| is1 / c |] is' ~> te]] 
      \end{gather}
      From \textsc{iCtx-clsEnv}, we know that $\intermed{[[is']]}$ only contains one free
      variable $[[c]]$. We can thus simplify Equation~\ref{eq:sn:method301} to:
      \begin{gather}
        \label{eq:sn:method303}
        [[SS1 ; TC ; empty |-tm ie islj idvli :  [| [|islj / clj|] is1 / c |] is' ~> te]] 
      \end{gather}
      And by substituting Equation~\ref{eq:sn:method52}:
      \begin{gather}
        \label{eq:sn:method304}
        [[SS1 ; TC ; empty |-tm ie islj idvli :  [| RSN(is) / c |] is' ~> te]] 
      \end{gather}
      Again, since $\intermed{[[is']]}$ contains only one free variable $[[c]]$, we can
      further rewrite this result to:
      \begin{gather}
        \label{eq:sn:method305}
        [[SS1 ; TC ; empty |-tm ie islj idvli :  RSN ([| is / c |] is') ~> te]] 
      \end{gather}
      By induction hypothesis on Equation~\ref{eq:sn:method305}, we get:
      \begin{gather}
        [[ ie islj idvli in SN (RSN ([| is / c |] is')) with SS' ; TC ; empty ]]
      \end{gather}
      By weakening over $\intermed{[[SS']]}$ (Lemma~\ref{lemma:sn_menv_weakening}), we get:
      \begin{gather}
        \label{eq:sn:method306}
        [[ ie islj idvli in SN (RSN ([| is / c |] is')) with SS ; TC ; empty ]]
      \end{gather}
      Because we know that $[[ RSN in FSN (TT) with SS; TC ]]$, by
      Compositionality for Strong Normalization (Context Interpretation)
      (Corollary~\ref{cor:comp_sn_ctx}), Equation~\ref{eq:sn:method306} proves
      our Goal~\ref{eq:sn:method11}.
      
    \item $\drule{D-con}$ \\
      The goal to be proven is the following:
      \begin{gather}
        \label{eq:sn:method:con:g1}
        [[ id . im with RSN ; phiSN ; gammaSN in SN ([| is / c |] is') with SS ;
        TC ; RSN]] \\
        \label{eq:sn:method:con:g2}
        \textit{where}~[[ is = [| islj / clj |] isq ]]
      \end{gather}
      From the rule premise, we know that:
      \begin{gather}
        \label{eq:sn:method:con:g6}
        [[ (iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli .
        ie in SS ]] \\
        \label{eq:sn:method:con:g5}
        [[ </ TC ; empty, clj |-q iqi ~> tti // i /> ]] \\
        \label{eq:sn:method:con:g7}
        [[ </ TC ; TT |-ty isj ~> ttj // j /> ]] \\
        \label{eq:sn:method:con:g3}
        [[SS1 ; TC ; empty, clj , idvarli : iqli |-tm ie : [| isq / c |] ism ~>
        te]] \\
        \nonumber
        \textit{where}~[[ SS = SS1, (iD : \/ clj . iqli => iTC isq) . im |-> /\
        clj . \ idvarli : iqli . ie, SS2 ]]
      \end{gather}

      By evaluation rule (\textsc{iEval}), we know that:
      \begin{gather}
        \label{eq:sn:method:con1}
        [[SS |- ( iD islj idli ) . im --> (/\ clj . \ idvarli : iqli . ie) islj idli]]
      \end{gather}
      By applying the substitutions, we can verify that:
      \begin{gather*}
        [[SS |- (iD islj idli ) . im with RSN ; phiSN ; gammaSN --> (/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli))]]
      \end{gather*}
      By Strong Normalization preserved by forward/backward reduction
      (Lemma~\ref{lemma:sn_pres}), our goal becomes:
      \begin{gather}
        \label{eq:sn:method:con2}
      [[(/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli)) in SN ([| is / c |] is') with SS ; TC ; RSN]].
      \end{gather}
      By applying rules \textsc{iTm-constrI} (in combination with
      Equation~\ref{eq:sn:method:con:g5}) and \textsc{iTm-forallI},
      Equation~\ref{eq:sn:method:con:g3} reduces to:
      \begin{gather}
        \label{eq:sn:method:con:g4}
        [[SS1 ; TC ; empty |-tm /\ clj . \ idvarli : iqli . ie : \/ clj . iqli
        -> [| isq / c |] ism ~> te]]
      \end{gather}
      By applying this to \textsc{iTm-forallE}, in combination with
      Equation~\ref{eq:sn:method:con:g7}, we get: 
      \begin{gather*}
        [[SS1 ; TC ; empty |-tm (/\ clj . \ idvarli : iqli . ie) RSN(islj): [| RSN(islj) / clj |] iqli -> [|
        RSN(islj) / clj |] [| isq / c |] ism ~> te1]]
      \end{gather*}
      Through weakening Lemma~\ref{lemma:exp_weakening_method}, we know this is
      equivalent to:
      \begin{gather}
        \label{eq:sn:method:con:g4p}
        [[SS ; TC ; empty |-tm (/\ clj . \ idvarli : iqli . ie) RSN(islj): [| RSN(islj) / clj |] iqli -> [|
        RSN(islj) / clj |] [| isq / c |] ism ~> te1]]
      \end{gather}
      The 6\textsuperscript{th} rule premise tells us that:
      \begin{gather*}
      [[</ SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei // i />]]
      \end{gather*}
      From Equation~\ref{eq:sn:method:con:g5}, we know that $\intermed{[[iqlj]]}$ only
      contains free variables $\intermed{[[clj]]}$. By applying the substition, we can thus
      verify that:
      \begin{gather*}
      [[</ SS ; TC ; empty |-d RSN(gammaSN(idi)) : [| RSN(islj) / clj |] iqi ~> tei' // i />]]
      \end{gather*}
      Therefore, by \textsc{iTm-constrE},
      Equation~\ref{eq:sn:method:con:g4p} is equivalent to:
      \begin{gather}
        \label{eq:sn:method:con:g4b}
        [[SS ; TC ; empty |-tm (/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli)): [|
        RSN(islj) / clj |] [| isq / c |] ism ~> te1]]
      \end{gather}
      From Lemma~\ref{lemma:type_well_inter_typing}, in combination with
      Equation~\ref{eq:sn:method:con:g3}, we know that $\intermed{[[ [| isq / c |] ism ]]}$
      only contains free variables $\intermed{[[clj]]}$. we can thus rewrite
      Equation~\ref{eq:sn:method:con:g4b} to:
      \begin{gather}
        \label{eq:sn:method:con3}
        [[SS ; TC ; empty |-tm (/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli)):
        RSN([| islj / clj |] [| isq / c |] ism) ~> te1]]
      \end{gather}
      From the environment well-formedness we know that \([[ is' = ism ]]\) and
      that $\intermed{[[is']]}$ only contains free variable $\intermed{[[c]]}$. We can thus rewrite
      Equation~\ref{eq:sn:method:con3} to:
      \begin{gather}
        \label{eq:sn:method:con5}
        [[SS ; TC ; empty |-tm (/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli)):
        RSN([| [| islj / clj |] is2 / c|] is' ) ~> te1]]
      \end{gather}
      By substituting Equation~\ref{eq:sn:method:con:g2}, we have:
      \begin{gather}
        \label{eq:sn:method:con6}
        [[SS ; TC ; empty |-tm (/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli)):
        RSN([| is / c|] is' ) ~> te1]]
      \end{gather}
      By induction hypothesis on Equation~\ref{eq:sn:method:con6}, we get:
      \begin{gather}
        \label{eq:sn:method:con7}
      [[(/\ clj . \ idvarli : iqli . ie) RSN(islj) RSN(gammaSN(idli)) in SN (RSN([| is / c|] is' )) with SS ; TC ; empty]].
      \end{gather}
      Because we know that $[[ RSN in FSN (TT) with SS; TC ]]$, by
      Compositionality for Strong Normalization (Context Interpretation)
      (Corollary~\ref{cor:comp_sn_ctx}), Equation~\ref{eq:sn:method:con7}
      proves our Goal~\ref{eq:sn:method:con2}.
  \end{itemize}
}
\proofStep{\textsc{iTm-arrI}}
{\drule{iTm-arrI}}
{
  Because $[[ (\ ix : is1 . ie) with RSN ; phiSN ; gammaSN = \ix : RSN (is1) .
  (ie with RSN; phiSN; gammaSN)]]$,
  our goal is to show that:
  \begin{gather}
    [[ \ix : RSN (is1) . (ie with RSN; phiSN; gammaSN) in SN (is1 -> is2) with SS ; TC ;
    RSN ]]
  \end{gather}
  By definition, we need to prove the following goals:
  \begin{gather}
        \label{eq:sn:arri:1}
    [[ SS ; TC ; empty |-tm \ix : RSN (is1) . (ie with RSN; phiSN; gammaSN): RSN1 ( is1 -> is2 ) ~> te ]]\\
        \label{eq:sn:arri:2}
    \exists [[ iv ]] : [[ SS |- \ix : RSN (is1) . (ie with RSN; phiSN; gammaSN)-->> iv ]] \\
        \label{eq:sn:arri:3}
        \forall \intermed{[[ ie' ]]} : [[ ie' in SN ( is1 ) with SS ; TC ; RSN ]]
      \Rightarrow [[ (\ix : RSN (is1) . (ie with RSN; phiSN; gammaSN)) ie' in SN ( is2 ) with SS ; TC ; RSN ]] 
  \end{gather}
  By Substitution for Context Interpretation (Lemma~\ref{lemma:sn_ctx_inter}),
  we can easily prove Equation~\ref{eq:sn:arri:1}.
  
  Furthermore,
  $\intermed{[[\ix : RSN (is1) . (ie with RSN; phiSN; gammaSN)]]}$ is already a value,
  which proves Equation~\ref{eq:sn:arri:2}. Now given
  \begin{gather}
        \label{eq:sn:arri:4}
        \forall \intermed{[[ ie' ]]} : [[ ie' in SN ( is1 ) with SS ; TC ; RSN ]]
  \end{gather}
  We need to show
  \begin{gather}
        \label{eq:sn:arri:5}
       [[ (\ix : RSN (is1) . (ie with RSN; phiSN; gammaSN)) ie' in SN ( is2 ) with SS ; TC ; RSN ]] 
  \end{gather}
  % From Equation~\ref{eq:sn:arri:4} and Lemma~\ref{thmA:sn:part:b} we know that
  % there exists $[[iv']]$ such that $[[SS |- ie' --> iv']]$.
  Let $[[phiSN' = phiSN, ix |-> ie']]$. By induction hypothesis, we have
  \begin{gather}
        \label{eq:sn:arri:6}
    [[ie with RSN ; phiSN, ix |-> ie' ; gammaSN in SN (is2) with SS ; TC ; RSN]]
  \end{gather}
  We know that:
  \begin{gather*}
    \intermed{[[(\ix : RSN (is1) . (ie with RSN; phiSN; gammaSN)) ie']]} \\
    [[-->]] \intermed{[[ [|ie' / ix|] (ie with RSN; phiSN; gammaSN) ]]} \\
    = \intermed{[[ie with RSN ; phiSN, ix |-> ie' ; gammaSN]]}
  \end{gather*}
  Consequently, by Strong Normalization preserved by forward/backward
  reduction(Lemma~\ref{lemma:sn_pres}), Equation~\ref{eq:sn:arri:6} proves
  \ref{eq:sn:arri:5}. \\
}
\proofStep{\textsc{iTm-arrE}}
{\drule{iTm-arrE}}
{
  By induction hypothesis, we have:
  \begin{gather}
    \label{eq:sn:arre:1}
    [[ ie1 with RSN ; phiSN ; gammaSN in SN (is1 -> is2) with SS ; TC ; RSN ]] \\
    \label{eq:sn:arre:2}
    [[ ie2 with RSN ; phiSN ; gammaSN in SN (is1) with SS ; TC ; RSN ]] 
  \end{gather}
  By the definition of Equation~\ref{eq:sn:arre:1}, applying
  Equation~\ref{eq:sn:arre:2} results in:
  \begin{gather*}
    [[ (ie1 with RSN ; phiSN ; gammaSN) (ie2 with RSN ; phiSN ; gammaSN) in SN (is2) with SS ; TC ; RSN ]]
  \end{gather*}
  which is exactly our goal since
  \begin{gather*}
  \intermed{[[ (ie1 ie2) with RSN ; phiSN ; gammaSN ]]}
  = \intermed{[[ (ie1 with RSN ; phiSN ; gammaSN) (ie2 with RSN ; phiSN ; gammaSN)]]}
  \end{gather*}
}
\proofStep{\textsc{iTm-constrI}}
{\drule{iTm-constrI}}
{
  Because $[[ (\ idvar : iq . ie) with RSN ; phiSN ; gammaSN = \idvar : RSN (iq) .
  (ie with RSN; phiSN; gammaSN)]]$,
  our goal is to show that:
  \begin{gather}
    [[ \idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN) in SN (iq -> is) with SS ; TC ;
    RSN ]]
  \end{gather}
  By definition, we need to prove the following goals:
  \begin{gather}
        \label{eq:sn:di:1}
    [[ SS ; TC ; empty |-tm \idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN): RSN1 ( iq -> is ) ~> te ]]\\
        \label{eq:sn:di:2}
    \exists [[ iv ]] : [[ SS |- \idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN)-->> iv ]] \\
        \label{eq:sn:di:3}
        \forall [[ id ]] : [[ SS ; TC ; empty |-d id : RSN1 (iq) ~> te ]]
      \Rightarrow [[ (\idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN)) id in SN ( is ) with SS ; TC ; RSN ]] 
  \end{gather}
  By Substitution for Context Interpretation (Lemma~\ref{lemma:sn_ctx_inter}),
  we can easily prove Equation~\ref{eq:sn:di:1}.

  Furthermore,
  $\intermed{[[\idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN)]]}$ is already a value,
  which proves Equation~\ref{eq:sn:di:2}. Now given
  \begin{gather}
        \label{eq:sn:di:4}
        \forall [[id]] : [[ SS ; TC ; empty |-d id : RSN1 (iq) ~> te ]]
  \end{gather}
  We need to show
  \begin{gather}
        \label{eq:sn:di:5}
       [[ (\idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN)) id in SN ( is ) with SS ; TC ; RSN ]] 
  \end{gather}
  % From Equation~\ref{eq:sn:arri:4} and Lemma~\ref{thmA:sn:part:b} we know that
  % there exists $[[iv']]$ such that $[[SS |- ie' --> iv']]$.
  Let $[[gammaSN' = gammaSN, idvar |-> id]]$. By induction hypothesis, we have
  \begin{gather}
    \label{eq:sn:di:6}
    [[ie with RSN ; phiSN; gammaSN, idvar |-> id in SN (is) with SS ; TC ; RSN]]
  \end{gather}
  We know that:
  \begin{gather*}
    \intermed{[[(\idvar : RSN (iq) . (ie with RSN; phiSN; gammaSN)) id]]} \\
    [[-->]] \intermed{[[ [|id / idvar|] (ie with RSN; phiSN; gammaSN) ]]} \\
    = \intermed{[[ie with RSN ; phiSN ; gammaSN, idvar |-> id]]}
  \end{gather*}
  Consequently, by Strong Normalization preserved by forward/backward
  reduction(Lemma~\ref{lemma:sn_pres}), Equation~\ref{eq:sn:di:6} proves
  \ref{eq:sn:di:5}. \\
}
\proofStep{\textsc{iTm-constrE}}
{\drule{iTm-constrE}}
{
  By induction hypothesis, we have
  \begin{gather}
    \label{eq:sn:de:1}
    [[ ie with RSN ; phiSN ; gammaSN in SN (iq -> is) with SS ; TC ; RSN ]] 
  \end{gather}
  By Substitution for Context Interpretation (Lemma~\ref{lemma:sn_ctx_inter}),
  we know that:
  \begin{gather}
    \label{eq:sn:de:2}
    [[SS ; TC ; empty |-d id with RSN ; phiSN ; gammaSN : RSN (iq) ~> te2]] 
  \end{gather}
  By the definition of Equation~\ref{eq:sn:de:1}, applying
  Equation~\ref{eq:sn:de:2} results in:
  \begin{gather*}
    [[ (ie with RSN ; phiSN ; gammaSN) (id with RSN ; phiSN ; gammaSN) in SN (is) with SS ; TC ; RSN ]]
  \end{gather*}
  which is exactly our goal since
  \begin{equation*}
  [[ (ie id) with RSN ; phiSN ; gammaSN
  = (ie with RSN ; phiSN ; gammaSN) (id with RSN ; phiSN ; gammaSN)]]
  \end{equation*}
}
\proofStep{\textsc{iTm-forallI}}
{\drule{iTm-forallI}}
{
  Because $[[ (/\ c . ie) with RSN ; phiSN ; gammaSN =  /\ c .
  (ie with RSN; phiSN; gammaSN)]]$,
  our goal is to show that:
  \begin{gather}
    [[ /\ c . (ie with RSN; phiSN; gammaSN) in SN (\/ c . is) with SS ; TC ;
    RSN ]]
  \end{gather}
  By definition, we need to prove the following goals:
  \begin{gather}
        \label{eq:sn:alli:1}
    [[ SS ; TC ; empty |-tm /\ c . (ie with RSN; phiSN; gammaSN): RSN1 ( \/ c. is ) ~> te ]]\\
        \label{eq:sn:alli:2}
    \exists [[ iv ]] : [[ SS |- /\ c . (ie with RSN; phiSN; gammaSN)-->> iv ]] \\
        \label{eq:sn:alli:3}
        \forall \intermed{[[ is' ]]} , [[ r = SN ( is' ) with SS ; TC ; RSN ]]
      \Rightarrow [[ (/\ c . (ie with RSN; phiSN; gammaSN)) is' in SN ( is )
      with SS ; TC ; RSN, c |-> (is', r) ]] 
  \end{gather}
  By Substitution for Context Interpretation (Lemma~\ref{lemma:sn_ctx_inter}),
  we can easily prove Equation~\ref{eq:sn:alli:1}.

  Furthermore,
  $[[ SS |- /\ c . (ie with RSN; phiSN; gammaSN)-->> iv ]]$ is already a value,
  which proves Equation~\ref{eq:sn:alli:2}. Now given
  \begin{gather}
        \label{eq:sn:alli:4}
        \forall \intermed{[[ is' ]]} , [[ r = SN ( is' ) with SS ; TC ; RSN ]]
  \end{gather}
  We need to show
  \begin{gather}
        \label{eq:sn:alli:5}
      [[ (/\ c . (ie with RSN; phiSN; gammaSN)) is' in SN ( is )
      with SS ; TC ; RSN, c |-> (is', r) ]] 
  \end{gather}
  Let $[[RSN' = RSN, c |-> (is', r)]]$. By induction hypothesis, we have:
  \begin{gather}
        \label{eq:sn:alli:6}
    [[ie with RSN, c |-> (is', r) ; phiSN; gammaSN in SN (is) with SS ; TC ;
    RSN, c |-> (is', r)]]
  \end{gather}
  We know that:
  \begin{gather*}
    \intermed{[[(/\ c . (ie with RSN; phiSN; gammaSN)) is']]} \\
    [[-->]] \intermed{[[ [|is' / c|] (ie with RSN; phiSN; gammaSN) ]]} \\
    = \intermed{[[ie with RSN, c |-> (is', r) ; phiSN ; gammaSN]]}
  \end{gather*}
  Consequently, by Strong Normalization preserved by forward/backward
  reduction(Lemma~\ref{lemma:sn_pres}), Equation~\ref{eq:sn:alli:6} proves
  \ref{eq:sn:alli:5}. \\
}
\proofStep{\textsc{iTm-forallE}}
{\drule{iTm-forallE}}
{
  By induction hypothesis, we have:
  \begin{gather}
    \label{eq:sn:alle:1}
    [[ ie with RSN ; phiSN ; gammaSN in SN (\/ c. is') with SS ; TC ; RSN ]] 
  \end{gather}
  By Substitution for Context Interpretation (Lemma~\ref{lemma:sn_ctx_inter}),
  we know:
  \begin{gather}
    \label{eq:sn:alle:2}
    [[TC ; empty |-ty RSN (is) ~> tt ]] 
  \end{gather}
  Choose $[[r = SN (is) with SS ; TC ; RSN]]$.
  By the definition of Equation~\ref{eq:sn:alle:1}, applying
  Equation~\ref{eq:sn:alle:2} results in:
  \begin{gather*}
    [[ (ie with RSN ; phiSN ; gammaSN) (RSN (is)) in SN (is') with SS ; TC ;
    RSN, c |-> (RSN (is), r) ]]
  \end{gather*}
  By Compositionality for Strong Normalization (Lemma~\ref{lemma:comp_sn}), we get:
  \begin{gather*}
    [[ (ie with RSN ; phiSN ; gammaSN) (RSN (is)) in SN ([| is/ c|]is') with SS ; TC ;
    RSN, c |-> (is, r) ]]
  \end{gather*}
  which is exactly our goal since
  \begin{gather*}
  [[ (ie is) with RSN ; phiSN ; gammaSN 
  = (ie with RSN ; phiSN ; gammaSN) (RSN (is))]]
  \end{gather*}
}
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Strong Normalization - Part B]\ \\
  \label{thmA:sn:part:b}
  If \([[ ie in SN (is) with SS ; TC ; RSN ]]\)
  then \( \exists [[ iv ]] : [[ SS |- ie -->> iv ]]\).
\end{theoremB}

\proof

This goal is baked into the relation. It follows by straightforward induction on
$[[is]]$. \\
\qed


% =================================================================================
% Equivalence Theorems
% =================================================================================
\newpage
\section{Elaboration Equivalence Theorems}
\label{app:equiv}
\renewcommand\itot[1]{#1}


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Equivalence - Environments]\leavevmode
  If \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
  then \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
  and \([[ TC ; TT ~> GT ]]\).
  \label{thmA:equiv_env}
\end{theoremB}

\begin{figure}[htp]
  \centering

  \def\svgscale{0.75}
  \input{mut_dep_graph_equiv.pdf_tex}

  %% \includegraphics[height=5cm]{mut_dep_graph_equiv.png}
  \caption{Dependency graph for Theorems~\ref{thmA:equiv_env},
    \ref{thmA:equiv_dict} and
    \ref{thmA:equiv_expr}}
  \label{fig:dep_graph_equiv}
\end{figure}

\proof
By induction on the environment well-formedness relation.
This theorem is mutually proven with Theorems~\ref{thmA:equiv_dict}
and~\ref{thmA:equiv_expr} (Figure~\ref{fig:dep_graph_equiv}).
Note that at the dependencies between Theorem~\ref{thmA:equiv_env}
and~\ref{thmA:equiv_expr} and between Theorem~\ref{thmA:equiv_dict}
and~\ref{thmA:equiv_expr}, the size of \([[P]]\) is strictly decreasing, whereas
\([[P]]\) remains constant at every other dependency. Consequenty, the size of
\([[P]]\) is strictly decreasing at every cycle and the induction remains well-founded.\\
\proofStep{\textsc{sCtxT-empty}}
{
  [[ |-ctx empty ; empty ; empty ~> tempty ]]
}
{
  The goal follows directly from \textsc{sCtx-empty} and \textsc{Ctx-Empty}. \\
}
\proofStep{\textsc{sCtxT-clsEnv}}
{
  [[ |-ctx empty ; GC , sm : sTCl => sTC a : \/ alj . </ sTCi a // i /> => st ; empty ~> tempty ]]
}
{
  The goal to be proven is the following:
  \begin{gather}
    [[ |-ctx empty ; GC , sm : sTCl => sTC a : \/ alj . </ sTCi a // i /> => st ; empty ~> SS ; TC ; TT ]]
    \label{eqg:eq_env1} \\
    [[ TC ; TT ~> tempty ]]
    \label{eqg:eq_env2}
  \end{gather}
  From the rule premise we get that:
  \begin{gather}
    [[ GC ; empty, a |-ty \/ alj . </ sTCi a // i /> => st ~> tt ]]
    \label{eq:eq_env1} \\
    [[ </ GC ; empty, a |-q sTCi a ~> tti // i /> ]]
    \label{eq:eq_env2} \\
    [[ |-ctx empty ; GC ; empty ~> tempty ]]
    \label{eq:eq_env3}
  \end{gather}
  By applying the induction hypothesis to Equation~\ref{eq:eq_env3}, we get:
  \begin{gather}
    [[ |-ctx empty ; GC ; empty ~> empty ; TC' ; empty ]]
    \label{eq:eq_env4} \\
    [[ TC' ; empty ~> tempty ]]
    \label{eq:eq_env5} 
  \end{gather}
  From \textsc{sCtxT-tyEnvTy}, \textsc{sCtx-tyEnvTy} and \textsc{Ctx-TVar}, in combination with
  Equation~\ref{eq:eq_env3}, \ref{eq:eq_env4} and~\ref{eq:eq_env5}, respectively, we get:
  \begin{gather}
    [[ |-ctx empty ; GC ; empty, a ~> tempty, ta ]]
    \nonumber \\
    [[ |-ctx empty ; GC ; empty, a ~> empty ; TC' ; empty, c ]]
    \nonumber \\
    [[ TC' ; empty, c ~> tempty, ta ]]
    \nonumber 
  \end{gather}
  Applying type and constraint equivalence (Theorem~\ref{thmA:equiv_ty}) to
  Equations~\ref{eq:eq_env1} and~\ref{eq:eq_env2}, together with these results, gives us:
  \begin{gather}
    [[ GC ; empty, a |-ty \/ alj . </ sTCi a // i /> => st ~> is ]]
    \label{eq:eq_env6} \\
    [[ TC' ; empty, c |-ty is ~> tt ]]
    \label{eq:eq_env7} \\
    [[ </ GC ; empty, a |-q sTCi a ~> iqi // i /> ]]
    \label{eq:eq_env8} \\
    [[ </ TC' ; empty, c |-q iqi ~> tti // i /> ]]
    \label{eq:eq_env9} 
  \end{gather}
  Goal~\ref{eqg:eq_env1} follows from \textsc{sCtx-clsEnv}, in combination with
  Equations~\ref{eq:eq_env4}, \ref{eq:eq_env6} and~\ref{eq:eq_env8}, with
  \([[ SS = empty ]]\), \([[ TC = TC', im : iTC c : is ]]\) and \([[ TT = empty ]]\).
  Consequently, Goal~\ref{eqg:eq_env2} follows from \textsc{Ctx-Empty}. \\
}
\proofStep{\textsc{sCtxT-tyEnvTm}}
{
  [[ |-ctx empty ; GC ; GG , sx : ss ~> GT, tx : tt ]]
}
{
  The goal to be proven is the following:
  \begin{gather}
    [[ |-ctx empty ; GC ; GG , sx : ss ~> SS ; TC ; TT ]]
    \label{eqg:eq_env3} \\
    [[ TC ; TT ~> GT, tx : tt ]]
    \label{eqg:eq_env4}
  \end{gather}
  From the rule premise we get that:
  \begin{gather}
    [[ GC ; GG |-ty ss ~> tt ]]
    \label{eq:eq_env12} \\
    [[ sx notin dom (GG) ]]
    \label{eq:eq_env13} \\
    [[ |-ctx empty ; GC ; GG ~> GT ]]
    \label{eq:eq_env14}
  \end{gather}
  By applying the induction hypothesis to Equation~\ref{eq:eq_env14}, we get:
  \begin{gather}
    [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT' ]]
    \label{eq:eq_env15} \\
    [[ TC ; TT' ~> GT' ]]
    \label{eq:eq_env16}
  \end{gather}
  We know from type equivalence (Theorem~\ref{thmA:equiv_ty}), in combination with
  Equations~\ref{eq:eq_env12}, \ref{eq:eq_env15} and~\ref{eq:eq_env16}, that:
  \begin{gather}
    [[ GC ; GG |-ty ss ~> is ]]
    \label{eq:eq_env17} \\
    [[ TC ; TT |-ty is ~> tt ]]
    \label{eq:eq_env18}
  \end{gather}
  Goal~\ref{eqg:eq_env3} follows from \textsc{sCtx-tyEnvTm}, in combination with
  Equations~\ref{eq:eq_env13}, \ref{eq:eq_env15} and~\ref{eq:eq_env17}, with
  \([[ SS = empty ]]\) and \([[ TT = TT', ix : is ]]\).
  Consequently, Goal~\ref{eqg:eq_env4} follows from \textsc{Ctx-Var}, in
  combination with Equations~\ref{eq:eq_env16} and~\ref{eq:eq_env18}, with
  \([[ GT = GT' ]]\). \\
}
\proofStep{\textsc{sCtxT-tyEnvTy}}
{
  [[ |-ctx empty ; GC ; GG , a ~> GT, ta ]]
}
{
  Similar to the \textsc{sCtxT-tyEnvTm} case. \\
}
\proofStep{\textsc{sCtxT-tyEnvD}}
{
  [[ |-ctx empty ; GC ; GG , sdvar : sTC st ~> GT, txd : tt ]]
}
{
  Similar to the \textsc{sCtxT-tyEnvTm} case. \\
}
\proofStep{\textsc{sCtxT-pgmInst}}
{
  [[ |-ctx PT, ( sD : \/ blj . sqli => sTC st ) . sm |-> empty, blj, sdvarli :
  sqli, alk, sdvarlh : [| st / a |] sqlh' : se ; GC ; GG ~> GT ]]
}
{
  The goal to be proven is the following:
  \begin{gather}
    [[ |-ctx P, ( sD : \/ blj . sqli => sTC st ) . sm |-> empty, blj, sdvarli :
    sqli, alk, sdvarlh : [| st / a |] sqlh' : se ; GC ; GG ~> SS ; TC ; TT ]]
    \label{eqg:eq_env5} \\
    [[ TC ; TT ~> GT ]]
    \label{eqg:eq_env6}
  \end{gather}
  From the rule premise we get that:
  \begin{gather}
    [[ unambig (\/ blj . sqli => sTC st) ]]
    \label{eq:eq_env19} \\
    [[ GC ; empty |-c \/ blj . sqli => sTC st ~> \/ tblj . ttli -> [| tt / ta |]
    { tl : \/ talk . ttlh' -> tt' } ]]
    \label{eq:eq_env20} \\
    [[ ( sm : sqlm' => sTC a : \/ alk . sqlh' => st' ) in GC ]]
    \label{eq:eq_env21} \\
    [[ GC ; empty, a |-ty \/ alk . sqlh' => st' ~> \/ talk . ttlh' -> tt' ]]
    \label{eq:eq_env22} \\
    [[ GC ; empty, blj |-ty st ~> tt ]]
    \label{eq:eq_env23} \\
    [[ PT ; GC ; empty, blj, sdvarli : sqli, alk, sdvarlh : [| st / a |] sqlh' |-tm se <= [|
    st / a |] st' ~> te ]]
    \label{eq:eq_env24} \\
    [[ sD notin dom (PT) ]]
    \label{eq:eq_env25} \\
    [[ ( sD' : \/ blk' . sqlh'' => sTC st'' ) . sm' |-> GG' : se' notin PT ]]
    [[ where [| stlj / blj |] st = [| stlk' / blk' |] st'' ]]
    \label{eq:eq_env26} \\
    [[ |-ctx PT ; GC ; GG ~> GT ]]
    \label{eq:eq_env27}
  \end{gather}
  By applying the induction hypothesis to Equation~\ref{eq:eq_env27}, we get: 
  \begin{gather}
    [[ |-ctx P ; GC ; GG ~> SS' ; TC ; TT ]]
    \label{eq:eq_env29} \\
    [[ TC ; TT ~> GT ]]
    \label{eq:eq_env30}
  \end{gather}
  Goal~\ref{eqg:eq_env6} follows directly from Equation~\ref{eq:eq_env30}. 
  From type and constraint equivalence (Theorem~\ref{thmA:equiv_ty}, the required
  assumptions follow straightforwardly from \textsc{sCtxT-tyEnvTy},
  \textsc{sCtx-tyEnvTy} and \textsc{Ctx-TVar}, in combination with
  Equations~\ref{eq:eq_env27}, \ref{eq:eq_env29} and~\ref{eq:eq_env30}),
  together with Equations~\ref{eq:eq_env20}, \ref{eq:eq_env22} and~\ref{eq:eq_env23},
  we know: 
  \begin{gather}
    [[ GC ; empty |-c \/ blj . sqli => sTC st ~> \/ iblj . iqli => iTC is ]]
    \label{eq:eq_env32} \\
    [[ GC ; empty, a |-ty \/ alk . sqlh' => st' ~> \/ clk . iqlh' -> is' ]]
    \label{eq:eq_env33} \\
    [[ TC ; empty, c |-ty \/ clk . iqlh' -> is' ~> \/ talk . ttlh' -> tt' ]]
    \label{eq:eq_env34} \\
    [[ GC ; empty, blj |-ty st ~> is ]]
    \label{eq:eq_env35} \\
    [[ TC ; empty, iblj |-ty is ~> tt ]]
    \label{eq:eq_env36}
  \end{gather}
  Similarly, from expression equivalence (Theorem~\ref{thmA:equiv_expr}, the
  environment well-formedness assumption is constructed straightforwardly),
  together with Equation~\ref{eq:eq_env24}, we get:
  \begin{equation}
    [[ PT ; GC ; empty, blj, sdvarli : sqli, alk, sdvarlh : [| st / a |] sqlh' |-tm se <= [|
    st / a |] st' ~> ie ]]
    \label{eq:eq_env37}
  \end{equation}
  Goal~\ref{eqg:eq_env5} follows from \textsc{sCtx-pgmInst}, in combination with
  Equations~\ref{eq:eq_env19}, \ref{eq:eq_env32}, \ref{eq:eq_env21},
  \ref{eq:eq_env37}, \ref{eq:eq_env33}, \ref{eq:eq_env25}, \ref{eq:eq_env26}
  and~\ref{eq:eq_env29}, and with \([[ SS = SS', ( iD : \/ iblj . iqli => iTC
  is' ) . im |-> /\ iblj . \ idvarli : iqli . /\ clk . \ idvarlh : [| is / c |]
  iqlh' . ie ]]\).
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Equivalence - Types and Constraints]\leavevmode
  \begin{itemize}
  \item
    If \([[ GC ; GG |-ty ss ~> tt ]]\)
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ TC ; TT ~> GT ]]\) \\
    then \([[ GC ; GG |-ty ss ~> is ]]\)
    and \([[ TC ; TT |-ty is ~> tt ]]\).
  \item
    If \([[ GC ; GG |-q sq ~> tt ]]\)
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ TC ; TT ~> GT ]]\) \\
    then \([[ GC ; GG |-q sq ~> iq ]]\)
    and \([[ TC ; TT |-q iq ~> tt ]]\).
  \item
    If \([[ GC ; GG |-c sc ~> tt ]]\)
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
    and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ TC ; TT ~> GT ]]\) \\
    then \([[ GC ; GG |-c sc ~> ic ]]\)
    and \([[ TC ; TT |-c ic ]]\).
  \end{itemize}
  \label{thmA:equiv_ty}
\end{theoremB}

\proof
By induction on the size of the type \([[ss]]\), class constraint
\([[sq]]\) or constraint \([[sc]]\).

\begin{description}
\item[Part 1] By case analysis on the type well-formedness derivation. \\
  \proofStep{\textsc{sTyT-bool}}
  {
    [[ GC ; GG |-ty sbool ~> tbool ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-ty sbool ~> is ]]
      \label{eqg:eq_ty1} \\
      [[ TC ; TT |-ty is ~> tbool ]]
      \label{eqg:eq_ty2} 
    \end{gather}
    Goals~\ref{eqg:eq_ty1} and~\ref{eqg:eq_ty2} follow directly from
    \textsc{sTy-bool} and \textsc{iTy-bool} respectively,
    with \([[ is = ibool ]]\). \\
  }
  \proofStep{\textsc{sTyT-var}}
  {
    [[ GC ; GG |-ty a ~> ta ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-ty a ~> is ]]
      \label{eqg:eq_ty3} \\
      [[ TC ; TT |-ty is ~> ta ]]
      \label{eqg:eq_ty4} 
    \end{gather}
    From the rule premise we get that:
    \begin{equation}
      [[ a in GG ]]
      \label{eq:eq_ty1}
    \end{equation}
    By applying Lemmas~\ref{lemma:pres_env_ty} and~\ref{lemma:pres_env_tyT} to
    Equation~\ref{eq:eq_ty1}, we get:
    \begin{gather}
      [[ c in TT ]]
      \label{eq:eq_ty1b} \\
      [[ ta in GT ]]
      \label{eq:eq_ty1c}
    \end{gather}
    Goal~\ref{eqg:eq_ty3} and~\ref{eqg:eq_ty4} follow directly from
    \textsc{sTy-var} and \textsc{iTy-var} respectively, in combination with
    Equations~\ref{eq:eq_ty1b} and~\ref{eq:eq_ty1c}, with \([[ is = c ]]\). \\
  }
  \proofStep{\textsc{sTyT-arrow}}
  {
    [[ GC ; GG |-ty st1 -> st2 ~> tt1 -> tt2 ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-ty st1 -> st2 ~> is ]]
      \label{eqg:eq_ty5} \\
      [[ TC ; TT |-ty is ~> tt1 -> tt2 ]]
      \label{eqg:eq_ty6} 
    \end{gather}
    From the rule premise we get that:
    \begin{gather}
      [[ GC ; GG |-ty st1 ~> tt1 ]]
      \label{eq:eq_ty2} \\
      [[ GC ; GG |-ty st2 ~> tt2 ]]
      \label{eq:eq_ty3}
    \end{gather}
    By applying the induction hypothesis on Equations~\ref{eq:eq_ty2}
    and~\ref{eq:eq_ty3}, we get:
    \begin{gather}
      [[ GC ; GG |-ty st1 ~> is1 ]]
      \label{eq:eq_ty4} \\
      [[ TC ; TT |-ty is1 ~> tt1 ]]
      \label{eq:eq_ty5} \\
      [[ GC ; GG |-ty st2 ~> is2 ]]
      \label{eq:eq_ty6} \\
      [[ TC ; TT |-ty is2 ~> tt2 ]]
      \label{eq:eq_ty7}
    \end{gather}
    Goals~\ref{eqg:eq_ty5} and~\ref{eqg:eq_ty6} follow directly from
    \textsc{sTy-arrow} and \textsc{iTy-arrow} respectively, in combination with
    Equations~\ref{eq:eq_ty4}, \ref{eq:eq_ty5}, \ref{eq:eq_ty6}
    and~\ref{eq:eq_ty7}, with \([[ is = is1 -> is2 ]]\). \\
  }
  \proofStep{\textsc{sTyT-qual}}
  {
    [[ GC ; GG |-ty sq => sp ~> tt1 -> tt2 ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-ty sq => sp ~> is ]]
      \label{eqg:eq_ty7} \\
      [[ TC ; TT |-ty is ~> tt1 -> tt2 ]]
      \label{eqg:eq_ty8} 
    \end{gather}
    From the rule premise we get that:
    \begin{gather}
      [[ GC ; GG |-q sq ~> tt1 ]]
      \label{eq:eq_ty8} \\
      [[ GC ; GG |-ty sp ~> tt2 ]]
      \label{eq:eq_ty9}
    \end{gather}
    By applying the induction hypothesis on Equation~\ref{eq:eq_ty9}, we get:
    \begin{gather}
      [[ GC ; GG |-ty sp ~> is2 ]]
      \label{eq:eq_ty10} \\
      [[ TC ; TT |-ty is2 ~> tt2 ]]
      \label{eq:eq_ty11}
    \end{gather}
    By applying Part 2 of this theorem on Equation~\ref{eq:eq_ty8}, we get:
    \begin{gather}
      [[ GC ; GG |-q sq ~> iq ]]
      \label{eq:eq_ty12} \\
      [[ TC ; TT |-q iq ~> tt1 ]]
      \label{eq:eq_ty13}
    \end{gather}
    Goals~\ref{eqg:eq_ty7} and~\ref{eqg:eq_ty8} follow directly from
    \textsc{sTy-qual} and \textsc{iTy-qual} respectively, in combination with
    Equations~\ref{eq:eq_ty10}, \ref{eq:eq_ty11}, \ref{eq:eq_ty12}
    and~\ref{eq:eq_ty13}, with \([[ is = iq -> is2 ]]\). \\
  }
  \proofStep{\textsc{sTyT-scheme}}
  {
    [[ GC ; GG |-ty \/ a . ss ~> \/ ta . tt ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-ty \/ a . ss ~> is ]]
      \label{eqg:eq_ty9} \\
      [[ TC ; TT |-ty is ~> \/ ta . tt ]]
      \label{eqg:eq_ty10} 
    \end{gather}
    From the rule premise we get that:
    \begin{gather}
      [[ a notin GG ]]
      \label{eq:eq_ty14} \\
      [[ GC ; GG, a |-ty ss ~> tt ]]
      \label{eq:eq_ty15}
    \end{gather}
    By repeated case analysis on the 2\textsuperscript{nd} hypothesis (\textsc{sCtxT-pgmInst}),
    we get:
    \begin{equation}
      [[ |-ctx empty ; GC ; GG ~> GT ]]
      \label{eq:eq_ty16a}
    \end{equation}
    From \textsc{sCtxT-tyEnvTy}, in combination with
    Equations~\ref{eq:eq_ty16a} and~\ref{eq:eq_ty14}, we know that:
    \begin{equation}
      [[ |-ctx empty ; GC ; GG, a ~> GT, ta ]]
      \label{eq:eq_ty16}
    \end{equation}
    Similarly, we get from \textsc{sCtx-tyEnvTy} and \textsc{ctx-TVar} that:
    \begin{gather}
      [[ |-ctx empty ; GC ; GG, a ~> empty ; TC ; TT, c ]]
      \label{eq:eq_ty16b} \\
      [[ TC ; TT, c ~> GT, ta ]]
      \label{eq:eq_ty16c}
    \end{gather}
    By applying the induction hypothesis on Equation~\ref{eq:eq_ty15}, together
    with Equations~\ref{eq:eq_ty16}, \ref{eq:eq_ty16b} and~\ref{eq:eq_ty16c}, we get:
    \begin{gather}
      [[ GC ; GG, a |-ty ss ~> is' ]]
      \label{eq:eq_ty17} \\
      [[ TC ; TT, c |-ty is' ~> tt ]]
      \label{eq:eq_ty18}
    \end{gather}
    Goals~\ref{eqg:eq_ty9} and~\ref{eqg:eq_ty10} follow directly from
    \textsc{sTy-scheme} and \textsc{iTy-scheme} respectively, in combination
    with Equations~\ref{eq:eq_ty14}, \ref{eq:eq_ty17} and~\ref{eq:eq_ty18}, 
    with \([[ is = \/ c . is' ]]\). \\
  }
\item[Part 2] By case analysis on the class constraint well-formedness
  derivation. \\
  \proofStep{\textsc{sQT-TC}}
  {
    [[ GC ; GG |-q sTC st ~> [| tt' / ta |] { tl : tt } ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-q sTC st ~> iq ]]
      \label{eqg:eq_ty11} \\
      [[ TC ; TT |-q iq ~> [| tt' / ta |] { tl : tt } ]]
      \label{eqg:eq_ty12} 
    \end{gather}
    From the rule premise we get that:
    \begin{gather}
      [[ GC ; GG |-ty st ~> tt' ]]
      \label{eq:eq_ty19} \\
      [[ GC = GC1,  sm : sqli => sTC a : ss , GC2  ]]
      \label{eq:eq_ty20} \\
      [[ GC1 ; empty , a |-ty ss ~> tt ]]
      \label{eq:eq_ty21} 
    \end{gather}
    By repeated case analysis on the 2\textsuperscript{nd} hypothesis (\textsc{sCtxT-pgmInst}),
    we get:
    \begin{equation}
      [[ |-ctx empty ; GC ; GG ~> GT ]]
      \label{eq:eq_ty21a}
    \end{equation}
    From \textsc{sCtxT-tyEnvTy}, together with Equation~\ref{eq:eq_ty21a}
    and the fact that \([[ a notin empty ]]\), we know that:
    \begin{equation}
      [[ |-ctx empty ; GC1 ; empty, a ~> tempty, ta ]]
      \label{eq:eq_ty34}
    \end{equation}
    Similarly, we get from \textsc{sCtx-tyEnvTy} and \textsc{ctx-TVar} that:
    \begin{gather}
      [[ |-ctx empty ; GC1 ; empty, a ~> empty ; TC1 ; empty, c ]]
      \label{eq:eq_ty34b} \\
      [[ TC1 ; empty, c ~> GT, ta ]]
      \label{eq:eq_ty34c}
    \end{gather}
    By applying Part 1 of this theorem to Equations~\ref{eq:eq_ty19}
    and~\ref{eq:eq_ty21}, together with Equations~\ref{eq:eq_ty34},
    \ref{eq:eq_ty34b} and~\ref{eq:eq_ty34c}, we get:
    \begin{gather}
      [[ GC ; GG |-ty st ~> is' ]]
      \label{eq:eq_ty24} \\
      [[ TC ; TT |-ty is' ~> tt' ]]
      \label{eq:eq_ty25} \\
      [[ GC1 ; empty , a |-ty ss ~> is ]]
      \label{eq:eq_ty26} \\
      [[ TC1 ; empty , c |-ty is ~> tt ]]
      \label{eq:eq_ty27}
    \end{gather}
    Goal~\ref{eqg:eq_ty11} follows from \textsc{sQ-TC}, together with
    Equations~\ref{eq:eq_ty24}, \ref{eq:eq_ty20} and~\ref{eq:eq_ty26},
    with \([[ iq = iTC is' ]]\). 
    Consequently, Goal~\ref{eqg:eq_ty12} follows from \textsc{iQ-TC}, together
    with Equations~\ref{eq:eq_ty25}, \ref{eq:eq_ty20} and~\ref{eq:eq_ty27}. \\
  }
\item[Part 3] By case analysis on the constraint well-formedness derivation. \\
  \proofStep{\textsc{sCT-abs}}
  {
    [[ GC ; GG |-c \/ alj . sqli => sq ~> \/ talj . ttli -> tt ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ GC ; GG |-c \/ alj . sqli => sq ~> ic]]
      \label{eqg:eq_ty13} \\
      [[ TC ; TT |-c ic ]]
      \label{eqg:eq_ty14}
    \end{gather}
    From the rule premise we get that:
    \begin{gather}
      [[ </ GC ; GG, alj |-q sqi ~> tti // i /> ]]
      \label{eq:eq_ty22} \\
      [[ GC ; GG, alj |-q sq ~> tt ]]
      \label{eq:eq_ty23} \\
      [[ alj notin GG ]]
      \label{eq:eq_ty28}
    \end{gather}
    By repeated case analysis on the 2\textsuperscript{nd} hypothesis (\textsc{sCtxT-pgmInst}),
    we get:
    \begin{equation}
      [[ |-ctx empty ; GC ; GG ~> GT ]]
      \label{eq:eq_ty28a}
    \end{equation}
    By \textsc{sCtxT-tyEnvTy}, it follows from Equations~\ref{eq:eq_ty28} and~\ref{eq:eq_ty28a} that:
    \begin{equation}
      [[ |-ctx empty ; GC ; GG, alj ~> GT, talj ]]
      \label{eq:eq_ty29}
    \end{equation}
    Similarly, we get from \textsc{sCtx-tyEnvTy} and \textsc{ctx-TVar} that:
    \begin{gather}
      [[ |-ctx empty ; GC ; GG, alj ~> empty ; TC ; TT, clj ]]
      \label{eq:eq_ty29b} \\
      [[ TC ; TT, clj ~> GT, talj ]]
      \label{eq:eq_ty29c}
    \end{gather}
    By applying Part 2 of this theorem to Equations~\ref{eq:eq_ty22}
    and~\ref{eq:eq_ty23}, together with Equations~\ref{eq:eq_ty29},
    \ref{eq:eq_ty29b} and~\ref{eq:eq_ty29c}, we get:
    \begin{gather}
      [[ </ GC ; GG, alj |-q sqi ~> iqi // i /> ]]
      \label{eq:eq_ty30} \\
      [[ </ TC ; TT, clj |-q iqi ~> tti // i /> ]]
      \label{eq:eq_ty31} \\
      [[ GC ; GG, alj |-q sq ~> iq ]]
      \label{eq:eq_ty32} \\
      [[ TC ; TT, clj |-q iq ~> tt ]]
      \label{eq:eq_ty33}
    \end{gather}
    Goal~\ref{eqg:eq_ty13} follows from \textsc{sC-abs}, together with
    Equations~\ref{eq:eq_ty30} and~\ref{eq:eq_ty32},
    with \([[ ic = \/ clj . iqli => iq ]]\).
    Consequently, Goal~\ref{eqg:eq_ty14} follows from \textsc{iC-abs}, together
    with Equations~\ref{eq:eq_ty31} and~\ref{eq:eq_ty33}. \\
  }
\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Equivalence - Dictionaries]\leavevmode
  If \([[ PT ; GC ; GG |= sq ~> te ]]\)
  and \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
  then \([[ P ; GC ; GG |= sq ~> id ]]\)
  and \([[ SS ; TC ; TT |-d id : iq ~> te ]]\) \\
  where \([[ GC ; GG |-q sq ~> iq ]]\)
  and \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
  and \([[ TC ; TT ~> GT ]]\).
  \label{thmA:equiv_dict}
\end{theoremB} 

\proof
By induction on the entailment derivation, and mutually proven with
Theorems~\ref{thmA:equiv_env}
and~\ref{thmA:equiv_expr} (Figure~\ref{fig:dep_graph_equiv}).
Note that at the dependencies between Theorem~\ref{thmA:equiv_env}
and~\ref{thmA:equiv_expr} and between Theorem~\ref{thmA:equiv_dict}
and~\ref{thmA:equiv_expr}, the size of \([[P]]\) is strictly decreasing, whereas
\([[P]]\) remains constant at every other dependency. Consequenty, the size of
\([[P]]\) is strictly decreasing at every cycle and the induction remains well-founded.

From environment equivalence (Theorem~\ref{thmA:equiv_env}), in combination with
the 2\textsuperscript{nd} hypothesis, we derive that:
\begin{gather}
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
    \label{eq:eq_d0a} \\
    [[ TC ; TT ~> GT ]]
    \label{eq:eq_d0b}
\end{gather}
\proofStep{\textsc{sEntailT-local}}
{
  [[ PT ; GC ; GG |= sq ~> txd ]]
}
{
  The goal to be proven is the following:
  \begin{gather}
    [[ P ; GC ; GG |= sq ~> id ]]
    \label{eqg:eq_d1} \\
    [[ SS ; TC ; TT |-d id : iq ~> txd ]]
    \label{eqg:eq_d2} \\
    [[ GC ; GG |-q sq ~> iq ]]
    \label{eqg:eq_d2b}
  \end{gather}
  We know from the rule premise that:
  \begin{equation*}
    [[ ( sdvar : sq ) in GG ]]
  \end{equation*} 
  Consequently, Goal~\ref{eqg:eq_d2b} follows by repeated case analysis on
  Equation~\ref{eq:eq_d0a} (\textsc{sCtx-tyEnvD}).
  Furthermore, we know from Lemma~\ref{lemma:pres_env_d} that:
  \begin{equation*}
    [[ ( idvar : iq ) in TT ]]
  \end{equation*}
  Goal~\ref{eqg:eq_d2} follows by \textsc{D-var}.
  Goal~\ref{eqg:eq_d1} follows by \textsc{sEntail-local}, with \([[ id = idvar ]]\). \\
}
\proofStep{\textsc{sEntailT-inst}}
{
  [[ PT ; GC ; GG |= sq ~> (/\ talj . \ </ txdi : tti' // i /> . {tl = /\ tblk .
  \ </ txdh' : tth'' // h /> . te}) ttlj
  teli ]]
}
{
  The goal to be proven is the following:
  \begin{gather}
    [[ P ; GC ; GG |= sq ~> id ]]
    \label{eqg:eq_d3} \\
    [[ SS ; TC ; TT |-d id : iq ~> (/\ talj . \ </ txdi : tti' // i /> . {tl = /\ tblk .
  \ </ txdh' : tth'' // h /> . te}) ttlj teli ]]
    \label{eqg:eq_d4} \\
    [[ GC ; GG |-q sq ~> iq ]]
    \label{eqg:eq_d4b}
  \end{gather}
  From the rule premise we get that:
  \begin{gather}
    [[ PT = PT1, (sD : \/ alj . sqli' => sq') . sm |-> empty, alj, sdvarli : sqli', blk,
    sdvarlh : sqlh : se, PT2 ]]
    \label{eq:eq_d1} \\
    [[ sq = [| stlj / alj |] sq' ]]
    \label{eq:eq_d2} \\
    [[ PT1 ; GC ; empty, alj, sdvarli : sqli', blk, sdvarlh : sqlh |-tm se => st
    ~> te ]]
    \label{eq:eq_d2b} \\
    [[ |-ctx PT ; GC ; GG ~> GT ]]
    \label{eq:eq_d3} \\
    [[ </ GC ; GG |-ty stj ~> ttj // j /> ]]
    \label{eq:eq_d4} \\
    [[ </ GC ; empty, alj |-q sqi' ~> tti' // i /> ]]
    \label{eq:eq_d5} \\
    [[ </ GC ; empty, alj, blk |-q sqh ~> tth'' // h /> ]]
    \label{eq:eq_d5b} \\
    [[ </ PT ; GC ; GG |= [| stlj / alj |] sqi' ~> tei // i /> ]]
    \label{eq:eq_d6} 
  \end{gather}
  By applying the induction hypothesis to Equation~\ref{eq:eq_d6}, we get:
  \begin{gather}
    [[ </ P ; GC ; GG |= [| stlj / alj |] sqi' ~> idi // i /> ]]
    \label{eq:eq_d7} \\
    [[ </ SS ; TC ; TT |-d idi : [| islj / clj |] iqi' ~> tei // i /> ]]
    \label{eq:eq_d8}
  \end{gather}
  By repeated case analysis on the 2\textsuperscript{nd} hypothesis, we know that:
  \begin{equation*}
    [[ |-ctx empty ; GC ; empty ~> tempty ]]
  \end{equation*}
  From \textsc{sCtxT-tyEnvTy}, we get that:
  \begin{equation*}
    [[ |-ctx empty ; GC ; empty, alj ~> tempty, talj ]]
  \end{equation*}
  Similarly, we can derive from Equations~\ref{eq:eq_d0a} and~\ref{eq:eq_d0b} that:
  \begin{gather}
    [[ |-ctx empty ; GC ; empty, alj ~> empty ; TC ; empty, clj ]]
    \nonumber \\
    [[ TC ; empty, clj ~> tempty, talj ]]
    \nonumber
  \end{gather}
  It follows from type and constraint equivalence (Theorem~\ref{thmA:equiv_ty}), in
  combination with Equations~\ref{eq:eq_d4}, \ref{eq:eq_d5}, \ref{eq:eq_d0a} and~\ref{eq:eq_d0b} that:
  \begin{gather}
    [[ </ GC ; GG |-ty stj ~> isj // j /> ]]
    \label{eq:eq_d11} \\
    [[ </ TC ; TT |-ty isj ~> ttj // j /> ]]
    \label{eq:eq_d12} \\
    [[ </ GC ; empty, alj |-q sqi' ~> iqi' // i /> ]]
    \label{eq:eq_d13} \\
    [[ </ TC ; empty, clj |-q iqi' ~> tti' // i /> ]]
    \label{eq:eq_d14}
  \end{gather}
  By repeated case analysis on Equation~\ref{eq:eq_d0a} (\textsc{sCtx-pgmInst}),
  together with Equation~\ref{eq:eq_d1}, we know that:
  \begin{gather}
    [[ GC ; empty |-c \/ alj . sqli' => sq' ~> \/ clj . iqli' => iq' ]]
    \label{eq:eq_d6b} \\
    [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]]
    \label{eq:eq_d6e}
  \end{gather}
  By applying Lemma~\ref{lemma:constraint_weakening} to Equations~\ref{eq:eq_d6b}
  and~\ref{eq:eq_d6e}, we get:
  \begin{equation}
    [[ GC ; GG |-c \/ alj . sqli' => sq' ~> \/ clj . iqli' => iq' ]]
    \label{eq:eq_d6f} 
  \end{equation}
  By case analysis on Equation~\ref{eq:eq_d6b} (\textsc{sC-abs}), we get that:
  \begin{equation}
    [[ GC ; GG, alj |-q sq' ~> iq' ]]
    \label{eq:eq_d6c} 
  \end{equation}
  It follows from Lemma~\ref{lemma:tvar_subst_ctr} and
  Equations~\ref{eq:eq_d6c} and~\ref{eq:eq_d11} that:
  \begin{equation}
    [[ GC ; GG |-q [| stlj / alj |] sq' ~> [| islj / clj |] iq' ]]
    \label{eq:eq_d6d} 
  \end{equation}
  Goal~\ref{eqg:eq_d4b} follows directly from Equation~\ref{eq:eq_d6d},
  since we know that \([[ sq = [| stlj / alj |] sq' ]]\) (Equation~\ref{eq:eq_d2}).

  By applying Lemma~\ref{lemma:ctx_well_source_typing} to
  Equation~\ref{eq:eq_d2b}, we get that:
  \begin{equation}
    [[ |-ctx PT1 ; GC ; empty, alj, sdvarli : sqli', blk, sdvarlh : sqlh ~> GT' ]]
    \label{eq:eq_d14a}
  \end{equation}
  From expression equivalence (Theorem~\ref{thmA:equiv_expr}), in combination
  with Equations~\ref{eq:eq_d2b} and~\ref{eq:eq_d14a}, we get:
  \begin{gather}
    [[ PT1 ; GC ; empty, alj, sdvarli : sqli', blk, sdvarlh : sqlh |-tm se => st
    ~> ie ]]
    \label{eq:eq_d14b} \\
    [[ SS1 ; TC ; empty, clj, idvarli : iqli', iblk, idvarlh : iqlh |-tm ie : is
    ~> te ]]
    \label{eq:eq_d14c}
  \end{gather}
  Goal~\ref{eqg:eq_d3} follows from \textsc{sEntail-inst}, in combination with
  Equations~\ref{eq:eq_d1}, \ref{eq:eq_d2}, \ref{eq:eq_d0a},
  \ref{eq:eq_d11} and~\ref{eq:eq_d7}, with \([[ id = iD islj idli]]\).

  By inversion on Equation~\ref{eq:eq_d0a}, in combination with
  Equation~\ref{eq:eq_d1}, we get:
  \begin{equation}
    [[ SS = SS1, (iD : \/ clj . iqli' => iq') . im |-> /\ clj . \ idvarli : iqli' . /\ iblk . \ idvarlh : iqlh . ie , SS2 ]]
    \label{eq:eq_d14d}
  \end{equation}
  By applying preservation Theorem~\ref{thmA:typing_pres_env} to
  Equation~\ref{eq:eq_d0a}, we get:
  \begin{equation}
    [[ |-ctx SS ; TC ; TT ]]
    \label{eq:eq_d14e}
  \end{equation}
  Finally, Goal~\ref{eqg:eq_d4} follows from \textsc{D-con}, in combination with
  Equations~\ref{eq:eq_d14}, \ref{eq:eq_d12}, \ref{eq:eq_d8}, \ref{eq:eq_d14c},
  \ref{eq:eq_d14d} and~\ref{eq:eq_d14e}. \\
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Equivalence - Expressions]\leavevmode
  \begin{itemize}
  \item If \([[ PT ; GC ; GG |-tm se => st ~> te ]]\)
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
    then \([[ P ; GC ; GG |-tm se => st ~> ie ]]\)
    and \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\) \\
    where \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ TC ; TT ~> GT ]]\)
    and \([[ GC ; GG |-ty st ~> is ]]\).
  \item If \([[ PT ; GC ; GG |-tm se <= st ~> te ]]\)
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
    then \([[ P ; GC ; GG |-tm se <= st ~> ie ]]\)
    and \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\) \\
    where \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ TC ; TT ~> GT ]]\)
    and \([[ GC ; GG |-ty st ~> is ]]\).
  \end{itemize}
  \label{thmA:equiv_expr}
\end{theoremB} 

\proof
By induction on the lexicographic order of the tuple (size of the expression
\([[se]]\), typing mode). Regarding typing mode, we define type checking to be
larger than type inference. In each mutual dependency, we know that the tuple
size decreases, meaning that the induction is well-founded. 

Furthermore, this theorem is mutually proven with
Theorems~\ref{thmA:equiv_env}
and~\ref{thmA:equiv_dict} (Figure~\ref{fig:dep_graph_equiv}).
Note that at the dependencies between Theorem~\ref{thmA:equiv_env}
and~\ref{thmA:equiv_expr} and between Theorem~\ref{thmA:equiv_dict}
and~\ref{thmA:equiv_expr}, the size of \([[P]]\) is strictly decreasing, whereas
\([[P]]\) remains constant at every other dependency. Consequenty, the size of
\([[P]]\) is strictly decreasing at every cycle and the induction remains well-founded.

From environment equivalence (Theorem~\ref{thmA:equiv_env}), in combination with
the 2\textsuperscript{nd} hypothesis, we derive that:
\begin{gather}
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
    \label{eq:eq_expr0a} \\
    [[ TC ; TT ~> GT ]]
    \label{eq:eq_expr0b}
\end{gather}
Consequently, by Theorem~\ref{thmA:typing_pres_env} we derive that
\begin{equation}
  [[ |-ctx SS ; TC ; TT ]]
  \label{eq:eq_expr0c}
\end{equation}

\begin{description}
\item[Part 1] 
  By case analysis on the typing derivation. \\
  \proofStep{\textsc{sTm-infT-true}}
  {
    [[ PT ; GC ; GG |-tm strue => sbool ~> ttrue ]]
  }
  {
    The goal follows by \textsc{sTm-inf-true}, \textsc{iTm-true}
    (in combination with Equation~\ref{eq:eq_expr0c})
    and \textsc{sTy-bool}, with \([[ ie = itrue ]]\). \\
  }
  \proofStep{\textsc{sTm-infT-false}}
  {
    [[ PT ; GC ; GG |-tm sfalse => sbool ~> tfalse ]]
  }
  {
    Similar to the \textsc{sTm-infT-true} case. \\
  }
  \proofStep{\textsc{sTm-infT-let}}
  {
    [[ PT ; GC ; GG |-tm slet sx : \/ alj . sqli => st1 = se1 sin se2 => st2 ~> tlet tx : \/ talj . ttlk -> tt = /\ talj . \ </ txdk : ttk // k /> . te1 tin te2 ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm slet sx : \/ alj . sqli => st1 = se1 sin se2 => st2
      ~> ie ]]
      \label{eqg:eq_expr1} \\
      [[ SS ; TC ; TT |-tm ie : is2 ~> tlet tx : \/ talj . ttlk -> tt = /\ talj . \ </ txdk : ttk // k /> . te1 tin te2 ]]
      \label{eqg:eq_expr2} \\
      [[ GC ; GG |-ty st2 ~> is2 ]]
      \label{eqg:eq_expr2b}
    \end{gather}
    From the rule premise we know that:
    \begin{gather}
      [[ sx notin dom ( GG ) ]]
      \label{eq:eq_expr1} \\
      [[ unambig ( \/ alj . sqli => st1 ) ]]
      \label{eq:eq_expr2} \\
      [[ closure ( GC ; sqli ) = sqlk ]]
      \label{eq:eq_expr3} \\
      [[ </ GC ; GG |-q sqk ~> ttk // k /> ]]
      \label{eq:eq_expr4} \\
      [[ GC ; GG |-ty \/ alj . sqlk => st1 ~> \/ talj . ttlk -> tt ]]
      \label{eq:eq_expr5} \\
      [[ sdvarlk fresh ]]
      \label{eq:eq_expr6} \\
      [[ PT ; GC ; GG, alj, sdvarlk : sqlk |-tm se1 <= st1 ~> te1 ]]
      \label{eq:eq_expr7} \\
      [[ PT ; GC ; GG, sx : \/ alj . sqlk => st1 |-tm se2 => st2 ~> te2 ]]
      \label{eq:eq_expr8} 
    \end{gather}
    By applying Lemma~\ref{lemma:type_well_source_typing} to Equation~\ref{eq:eq_expr8},
    we get that:
    \begin{equation}
      [[ GC ; GG, sx : \/ alj . sqlk => st1 |-ty st2 ~> is2 ]]
      \label{eq:eq_expr8b} 
    \end{equation}
    It is straightforward to see from the definition of type well-formedness,
    that Goal~\ref{eqg:eq_expr2b} follows from Equation~\ref{eq:eq_expr8b},
    since term variables in the environment are not relevant for type well-formedness.

    We know from the hypothesis that \([[ |-ctx PT ; GC ; GG ~> GT ]]\).
    By repeated case analysis on this result (\textsc{sCtxT-pgmInst}), we get that
    \([[ |-ctx empty ; GC ; GG ~> GT ]]\).
    From \textsc{sCtxT-tyEnvTm}, \textsc{sCtxT-tyEnvTy} and \textsc{sCtxT-tyEnvD}, in
    combination with Equations~\ref{eq:eq_expr1}, \ref{eq:eq_expr4},
    \ref{eq:eq_expr5} and~\ref{eq:eq_expr6}, we know that:
    \begin{gather}
      [[ |-ctx PT ; GC ; GG, alj, sdvarlk : sqlk ~> GT, talj, </ txdk : ttk // k
      /> ]]
      \label{eq:eq_expr9} \\
      [[ |-ctx PT ; GC ; GG, sx : \/ alj . sqlk => st1 ~> GT, tx : \/ talj .
      ttlk -> tt ]]
      \label{eq:eq_expr10} 
    \end{gather}
    Applying the induction hypothesis on Equations~\ref{eq:eq_expr7}
    and~\ref{eq:eq_expr8}, in combination with Equations~\ref{eq:eq_expr9}
    and~\ref{eq:eq_expr10}, results in:
    \begin{gather}
      [[ P ; GC ; GG, alj, sdvarlk : sqlk |-tm se1 <= st1 ~> ie1 ]]
      \label{eq:eq_expr11} \\
      [[ SS ; TC ; TT, clj, idvarlk : iqlk |-tm ie1 : is1 ~> te1 ]]
      \label{eq:eq_expr12} \\
      [[ P ; GC ; GG, sx : \/ alj . sqlk => st1 |-tm se2 => st2 ~> ie2 ]]
      \label{eq:eq_expr13} \\
      [[ SS ; TC ; TT, ix : \/ clj . iqlk -> is1 |-tm ie2 : is2 ~> te2 ]]
      \label{eq:eq_expr14} 
    \end{gather}
    From constraint equivalence (Theorem~\ref{thmA:equiv_ty}), in combination with
    Equation~\ref{eq:eq_expr4}, we get:
    \begin{equation}
      [[ </ TC ; TT |-q iqk ~> ttk // k /> ]]
      \label{eq:eq_expr15} 
    \end{equation}
    By applying \textsc{iTm-forallI} and \textsc{iTm-constrI} to
    Equation~\ref{eq:eq_expr12}, together with Equation~\ref{eq:eq_expr15}, we get:
    \begin{equation}
      [[ SS ; TC ; TT |-tm /\ clj . \ idvarlk : iqlk . ie1 : \/ clj . iqlk -> is1 ~> /\ talj . \ </ txdk : ttk // k /> . te1 ]]
      \label{eq:eq_expr16} 
    \end{equation}
    From Lemma~\ref{lemma:type_well_inter_typing}, in combination with
    Equation~\ref{eq:eq_expr16}, we know that:
    \begin{equation}
      [[ TC ; TT |-ty \/ clj . iqlk -> is1 ~> \/ talj . ttlk -> tt ]]
      \label{eq:eq_expr16b} 
    \end{equation}
    Goals~\ref{eqg:eq_expr1} and~\ref{eqg:eq_expr2} follow from
    \textsc{sTm-inf-let} and \textsc{iTm-let} respectively, with
    \begin{equation*}
    [[ ie = ilet ix : \/ clj . iqlk -> is1 = /\ clj . \ idvarlk : iqlk . ie1
        iin ie2 ]]
    \end{equation*}
  }
  \proofStep{\textsc{sTm-infT-ArrE}}
  {
    [[ PT ; GC ; GG |-tm se1 se2 => st2 ~> te1 te2 ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm se1 se2 => st2 ~> ie ]]
      \label{eqg:eq_expr3} \\
      [[ SS ; TC ; TT |-tm ie : is2 ~> te1 te2 ]]
      \label{eqg:eq_expr4} \\
      [[ GC ; GG |-ty st2 ~> is2 ]]
      \label{eqg:eq_expr4b}
    \end{gather}
    From the rule premise we know that:
    \begin{gather}
      [[ PT ; GC ; GG |-tm se1 => st1 -> st2 ~> te1 ]]
      \label{eq:eq_expr17} \\
      [[ PT ; GC ; GG |-tm se2 <= st1 ~> te2 ]]
      \label{eq:eq_expr18} 
    \end{gather}
    By applying the induction hypothesis to Equations~\ref{eq:eq_expr17}
    and~\ref{eq:eq_expr18}, we get:
    \begin{gather}
      [[ P ; GC ; GG |-tm se1 => st1 -> st2 ~> ie1 ]]
      \label{eq:eq_expr19} \\
      [[ SS ; TC ; TT |-tm ie1 : is1 -> is2 ~> te1 ]]
      \label{eq:eq_expr20} \\
      [[ P ; GC ; GG |-tm se2 <= st1 ~> ie2 ]]
      \label{eq:eq_expr21} \\
      [[ SS ; TC ; TT |-tm ie2 : is1 ~> te2 ]]
      \label{eq:eq_expr22} 
    \end{gather}
    Goals~\ref{eqg:eq_expr3} and~\ref{eqg:eq_expr4} follow from
    \textsc{sTm-inf-ArrE} and \textsc{iTm-arrE} respectively, in combination
    with Equations~\ref{eq:eq_expr19}, \ref{eq:eq_expr20}, \ref{eq:eq_expr21}
    and~\ref{eq:eq_expr22}. Goal~\ref{eqg:eq_expr4b} follows by applying
    Lemma~\ref{lemma:type_well_source_typing} to Equation~\ref{eqg:eq_expr3}. \\
  }
  \proofStep{\textsc{sTm-infT-Ann}}
  {
    [[ PT ; GC ; GG |-tm se <: st => st ~> te ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm se <: st => st ~> ie ]]
      \label{eqg:eq_expr5} \\
      [[ SS ; TC ; TT |-tm ie : is ~> te ]]
      \label{eqg:eq_expr6} \\
      [[ GC ; GG |-ty st ~> is ]]
      \label{eqg:eq_expr6b}
    \end{gather}
    From the rule premise we know that:
    \begin{equation}
      [[ PT ; GC ; GG |-tm se <= st ~> te ]]
      \label{eq:eq_expr23}
    \end{equation}
    Goals~\ref{eqg:eq_expr5}, \ref{eqg:eq_expr6} and~\ref{eqg:eq_expr6b} follow by applying Part
    2 of this theorem to Equation~\ref{eq:eq_expr23}. \\
  }
\item[Part 2] 
  By case analysis on the typing derivation. \\
  \proofStep{\textsc{sTm-checkT-var}}
  {
    [[ PT ; GC ; GG |-tm sx <= [| stlj / alj |] st ~> tx ttlj teli ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm sx <= [| stlj / alj |] st ~> ie ]]
      \label{eqg:eq_expr7} \\
      [[ SS ; TC ; TT |-tm ie : is' ~> tx ttlj teli ]]
      \label{eqg:eq_expr8} \\
      [[ GC ; GG |-ty [| stlj / alj |] st ~> is' ]]
      \label{eqg:eq_expr8b} 
    \end{gather}
    From the rule premise we know that:
    \begin{gather}
      [[ ( sx : \/ alj . sqli => st ) in GG ]]
      \label{eq:eq_expr24} \\
      [[ unambig ( \/ alj . sqli => st ) ]]
      \label{eq:eq_expr25} \\
      [[ </ PT ; GC ; GG |= [| stlj / alj |] sqi ~> tei // i /> ]]
      \label{eq:eq_expr26} \\
      [[ </ GC ; GG |-ty stj ~> ttj // j /> ]]
      \label{eq:eq_expr27} \\
      [[ |-ctx PT ; GC ; GG ~> GT ]]
      \label{eq:eq_expr28} 
    \end{gather}
    We know from Lemma~\ref{lemma:pres_env_tm}, in combination with Equations~\ref{eq:eq_expr24}
    and~\ref{eq:eq_expr0a}, that:
    \begin{equation}
      [[ ( ix : \/ clj . iqli -> is ) in TT ]]
      \label{eq:eq_expr24b}
    \end{equation}
    By applying type equivalence (Theorem~\ref{thmA:equiv_ty}) to
    Equation~\ref{eq:eq_expr27}, we get:
    \begin{gather}
      [[ </ GC ; GG |-ty stj ~> isj // j /> ]]
      \label{eq:eq_expr31} \\
      [[ </ TC ; TT |-ty isj ~> ttj // j /> ]]
      \label{eq:eq_expr32} 
    \end{gather}
    By applying dictionary equivalence (Theorem~\ref{thmA:equiv_dict}) to
    Equation~\ref{eq:eq_expr26}, we get:
    \begin{gather}
      [[ </ P ; GC ; GG |= [| stlj / alj |] sqi ~> idi // i /> ]]
      \label{eq:eq_expr29} \\
      [[ </ SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei // i /> ]]
      \label{eq:eq_expr30} \\
      [[ </ GC ; GG |-q [| stlj / alj |] sqi ~> [| islj / clj |] iqi // i /> ]]
      \label{eq:eq_expr30b} 
    \end{gather}
    Goal~\ref{eqg:eq_expr7} follows from \textsc{sTm-check-var}, in combination
    with Equations~\ref{eq:eq_expr24}, \ref{eq:eq_expr25}, \ref{eq:eq_expr29},
    \ref{eq:eq_expr31} and~\ref{eq:eq_expr0a}, with
    \([[ ie = ix islj idli ]]\).
    Goal~\ref{eqg:eq_expr8} follows from \textsc{iTm-var}, \textsc{iTm-forallE}
    and \textsc{iTm-constrE}, in combination with Equations~\ref{eq:eq_expr0c}, \ref{eq:eq_expr24b},
    \ref{eq:eq_expr32} and~\ref{eq:eq_expr30}, with \([[ is' = [| islj / clj |] is ]]\).
    Goal~\ref{eqg:eq_expr8b} follows
    by applying Lemma~\ref{lemma:type_well_source_typing} to Equation~\ref{eqg:eq_expr7}. \\
  }
  \proofStep{\textsc{sTm-checkT-meth}}
  {
    [[ PT ; GC ; GG |-tm sm <= [| stlj / alj |] [|st / a |] st' ~> te . tl ttlj
    teli ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm sm <= [| stlj / alj |] [| st / a |] st' ~> ie ]]
      \label{eqg:eq_expr9} \\
      [[ SS ; TC ; TT |-tm ie : is0 ~> te . tl ttlj teli ]]
      \label{eqg:eq_expr10} \\
      [[ GC ; GG |-ty [| stlj / alj |] [| st / a |] st' ~> is0 ]]
      \label{eqg:eq_expr10b} 
    \end{gather}
    From the rule premise we know that:
    \begin{gather}
      [[ ( sm : sqlk' => sTC a : \/ alj . sqli => st' ) in GC ]]
      \label{eq:eq_expr33} \\
      [[ unambig ( \/ alj, a . sqli => st' ) ]]
      \label{eq:eq_expr34} \\
      [[ PT ; GC ; GG |= sTC st ~> te ]]
      \label{eq:eq_expr35} \\
      [[ GC ; GG |-ty st ~> tt ]]
      \label{eq:eq_expr36} \\
      [[ </ PT ; GC ; GG |= [| stlj / alj |] [|st / a |] sqi ~> tei // i /> ]]
      \label{eq:eq_expr37} \\
      [[ </ GC ; GG |-ty stj ~> ttj // j /> ]]
      \label{eq:eq_expr38} \\
      [[ |-ctx PT ; GC ; GG ~> GT ]]
      \label{eq:eq_expr39}
    \end{gather}
    By repeated case analysis on Equation~\ref{eq:eq_expr0a} (\textsc{sCtx-clsEnv}),
    together with Equation~\ref{eq:eq_expr33}, we know that:
    \begin{equation}
      [[ ( im : iTC c : \/ clj . iqli -> is' ) in TC ]]
      \label{eq:eq_expr33b}
    \end{equation}
    By applying type equivalence (Theorem~\ref{thmA:equiv_ty}) to
    Equations~\ref{eq:eq_expr36} and~\ref{eq:eq_expr38}, we get:
    \begin{gather}
      [[ GC ; GG |-ty st ~> is ]]
      \label{eq:eq_expr44} \\
      [[ TC ; TT |-ty is ~> tt ]]
      \label{eq:eq_expr45} \\
      [[ </ GC ; GG |-ty stj ~> isj // j /> ]]
      \label{eq:eq_expr46} \\
      [[ </ TC ; TT |-ty isj ~> ttj // j /> ]]
      \label{eq:eq_expr47}
    \end{gather}
    By applying dictionary equivalence (Theorem~\ref{thmA:equiv_dict}) to
    Equations~\ref{eq:eq_expr35} and~\ref{eq:eq_expr37}, we get:
    \begin{gather}
      [[ P ; GC ; GG |= sTC st ~> id ]]
      \label{eq:eq_expr40} \\
      [[ SS ; TC ; TT |-d id : iTC is ~> te ]]
      \label{eq:eq_expr41} \\
      [[ </ P ; GC ; GG |= [| stlj / alj |] [|st / a |] sqi ~> idi // i /> ]]
      \label{eq:eq_expr42} \\
      [[ </ SS ; TC ; TT |-d idi : [| islj / clj |] [| is / c |] iqi ~> tei // i /> ]]
      \label{eq:eq_expr43}
    \end{gather}
    Goal~\ref{eqg:eq_expr9} follows from \textsc{sTm-check-meth}, in combination
    with Equations~\ref{eq:eq_expr33}, \ref{eq:eq_expr34}, \ref{eq:eq_expr40},
    \ref{eq:eq_expr44}, \ref{eq:eq_expr42}, \ref{eq:eq_expr46}
    and~\ref{eq:eq_expr0a},
    with \([[ ie = id . im islj idli ]]\).
    Consequently, Goal~\ref{eqg:eq_expr10} follows from \textsc{iTm-method},
    \textsc{iTm-forallE} and \textsc{iTm-constrE}, in combination with
    Equations~\ref{eq:eq_expr41}, \ref{eq:eq_expr33b}, \ref{eq:eq_expr47}
    and~\ref{eq:eq_expr43}, with \([[ is0 = [| islj / clj |] [| is / c |] is' ]]\).
    Goal~\ref{eqg:eq_expr10b} follows
    by applying Lemma~\ref{lemma:type_well_source_typing} to Equation~\ref{eqg:eq_expr9}. \\
  }
  \proofStep{\textsc{sTm-checkT-ArrI}}
  {
    [[ PT ; GC ; GG |-tm \ sx . se <= st1 -> st2 ~> \ tx : tt . te ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm \ sx . se <= st1 -> st2 ~> ie ]]
      \label{eqg:eq_expr11} \\
      [[ SS ; TC ; TT |-tm ie : is0 ~> \ tx : tt . te ]]
      \label{eqg:eq_expr12} \\
      [[ GC ; GG |-ty st1 -> st2 ~> is0 ]]
      \label{eqg:eq_expr12b}
    \end{gather}
    From the rule premise we know that:
    \begin{gather}
      [[ sx notin dom(GG) ]]
      \label{eq:eq_expr48} \\
      [[ PT ; GC ; GG , sx : st1 |-tm se <= st2 ~> te ]]
      \label{eq:eq_expr49} \\
      [[ GC ; GG |-ty st1 ~> tt ]]
      \label{eq:eq_expr50}
    \end{gather}
    By applying type equivalence (Theorem~\ref{thmA:equiv_ty}) to
    Equation~\ref{eq:eq_expr50}, we get:
    \begin{gather}
      [[ GC ; GG |-ty st1 ~> is ]]
      \label{eq:eq_expr52} \\
      [[ TC ; TT |-ty is ~> tt ]]
      \label{eq:eq_expr53}
    \end{gather}
    From \textsc{sCtxT-tyEnvTm}, together with the 2\textsuperscript{nd}
    hypothesis and Equation~\ref{eq:eq_expr50}, we know that:
    \begin{equation}
      [[ |-ctx PT ; GC ; GG , sx : st1 ~> GT, tx : tt ]]
      \label{eq:eq_expr54}
    \end{equation}
    By applying the induction hypothesis on Equation~\ref{eq:eq_expr49},
    together with Equation~\ref{eq:eq_expr54}, we get:
    \begin{gather}
      [[ P ; GC ; GG , sx : st1 |-tm se <= st2 ~> ie' ]]
      \label{eq:eq_expr55} \\
      [[ SS ; TC ; TT , ix : is |-tm ie' : is2 ~> te ]]
      \label{eq:eq_expr56} \\
      [[ GC ; GG, sx : st1 |-ty st2 ~> is2 ]]
      \label{eq:eq_expr56b} 
    \end{gather}
    Goal~\ref{eqg:eq_expr11} follows from \textsc{sTm-check-ArrI}, together with
    Equations~\ref{eq:eq_expr48}, \ref{eq:eq_expr55} and~\ref{eq:eq_expr52},
    with \([[ ie = \ ix : is . ie' ]]\).
    Consequently, Goal~\ref{eqg:eq_expr12} follows from \textsc{iTm-arrI},
    together with Equations~\ref{eq:eq_expr56} and~\ref{eq:eq_expr53}, with
    \([[ is0 = is -> is2 ]]\).
    Goal~\ref{eqg:eq_expr12b} follows
    by applying Lemma~\ref{lemma:type_well_source_typing} to Equation~\ref{eqg:eq_expr11}. \\
  }
  \proofStep{\textsc{sTm-checkT-Inf}}
  {
    [[ PT ; GC ; GG |-tm se <= st ~> te ]]
  }
  {
    The goal to be proven is the following:
    \begin{gather}
      [[ P ; GC ; GG |-tm se <= st ~> ie ]]
      \label{eqg:eq_expr13} \\
      [[ SS ; TC ; TT |-tm ie : is ~> te ]]
      \label{eqg:eq_expr14} \\
      [[ GC ; GG |-ty st ~> is ]]
      \label{eqg:eq_expr14b}
    \end{gather}
    From the rule premise we know that:
    \begin{gather}
      [[ PT ; GC ; GG |-tm se => st ~> te ]]
      \label{eq:eq_expr51}
    \end{gather}
    Goals~\ref{eqg:eq_expr13}, \ref{eqg:eq_expr14} and~\ref{eqg:eq_expr14b} follow directly by
    applying Part 1 of this theorem to Equation~\ref{eq:eq_expr51}. 
  }
\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Equivalence - Contexts]\leavevmode
  \begin{itemize}
  \item
    If \([[ sM : ( PT ; GC ; GG ==> st ) |--> ( PT ; GC ; GG' ==> st' ) ~~> tM ]]\) \\
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\)
    and \([[ |-ctx PT ; GC ; GG' ~> GT' ]]\) \\
    then \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM ]]\) \\
    and \([[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM ]]\) \\
    where \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ |-ctx P ; GC ; GG' ~> SS ; TC ; TT' ]]\) \\
    and \([[ GC ; GG |-ty st ~> is ]]\)
    and \([[ GC ; GG' |-ty st' ~> is' ]]\).
  \item
    If \([[ sM : ( PT ; GC ; GG ==> st ) |--> ( PT ; GC ; GG' <== st' ) ~~> tM ]]\) \\
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\)
    and \([[ |-ctx PT ; GC ; GG' ~> GT' ]]\) \\
    then \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM ]]\) \\
    and \([[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM ]]\) \\
    where \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ |-ctx P ; GC ; GG' ~> SS ; TC ; TT' ]]\) \\
    and \([[ GC ; GG |-ty st ~> is ]]\)
    and \([[ GC ; GG' |-ty st' ~> is' ]]\).
  \item
    If \([[ sM : ( PT ; GC ; GG <== st ) |--> ( PT ; GC ; GG' ==> st' ) ~~> tM ]]\) \\
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\)
    and \([[ |-ctx PT ; GC ; GG' ~> GT' ]]\) \\
    then \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM ]]\) \\
    and \([[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM ]]\) \\
    where \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ |-ctx P ; GC ; GG' ~> SS ; TC ; TT' ]]\) \\
    and \([[ GC ; GG |-ty st ~> is ]]\)
    and \([[ GC ; GG' |-ty st' ~> is' ]]\).
  \item
    If \([[ sM : ( PT ; GC ; GG <== st ) |--> ( PT ; GC ; GG' <== st' ) ~~> tM ]]\) \\
    and \([[ |-ctx PT ; GC ; GG ~> GT ]]\)
    and \([[ |-ctx PT ; GC ; GG' ~> GT' ]]\) \\
    then \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM ]]\) \\
    and \([[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM ]]\) \\
    where \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\)
    and \([[ |-ctx P ; GC ; GG' ~> SS ; TC ; TT' ]]\) \\
    and \([[ GC ; GG |-ty st ~> is ]]\)
    and \([[ GC ; GG' |-ty st' ~> is' ]]\).
  \end{itemize}
  \label{thmA:equiv_ctx}
\end{theoremB}

\proof
By straightforward induction on the typing derivation. \\
\qed


% =================================================================================
% Coherence Theorems
% =================================================================================
\newpage
\section{Coherence Theorems}
\label{app:coh}
\renewcommand\itot[1]{}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Compatibility Lemmas
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Compatibility Lemmas}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{lemmaB}[Compatibility - Term Abstraction]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT, ix : is1 |- SS1 : ie1 =log SS2 : ie2 : is2 ]]
    }
    { [[ TC ; TT |- SS1 : \ ix : is1 . ie1 =log SS2 : \ ix : is1 . ie2 : is1 -> is2 ]] }
    \label{lemma:compat_abs}
  \end{mathpar}
\end{lemmaB}

\proof
By the definition of logical equivalence, suppose we have:
\begin{gather}
  \label{eq:compat_absR}
  [[ R in F ( TT ) with TC ]]\\
  \nonumber
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  \label{eq:compat_absH}
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gather}
The goal to be proven is the following:
\begin{equation*}
  [[ (SS1 : \ ix : is1 . ie1 with R ; phi1 ; gamma1 , SS2 : (? \ ix : is1 . ie2 ?) with R ; phi2 ; gamma2) in E (is1 -> is2) with TC ; R ]]
\end{equation*}
By the definition of the \( \mathcal{E} \) relation and the fact that term abstractions
are values, the goal reduces to:
\begin{gather*}
  [[ SS1 ; TC ; empty |-tm \ ix : is1 . ie1 with R ; phi1 ; gamma1 : R (is1 -> is2) ~> te ]]\\
  [[ SS2 ; TC ; empty |-tm \ ix : is1 . ie2 with R ; phi2 ; gamma2 : R (is1 -> is2) ~> te' ]]\\
  [[ (SS1 : \ ix : is1 . ie1 with R ; phi1 ; gamma1 , SS2 : \ ix : is1 . ie2 with R ; phi2 ; gamma2) in V (is1 -> is2) with TC ; R ]]
\end{gather*}
By applying the substitutions, the goal simplifies to:
\begin{gather}
  \label{eq:compat_abs1}
  [[ SS1 ; TC ; empty |-tm \ ix : R (is1) . (ie1 with R ; phi1 ; gamma1) : R (is1 -> is2) ~> te ]]\\
  \label{eq:compat_abs2}
  [[ SS2 ; TC ; empty |-tm \ ix : R (is1) . (ie2 with R ; phi2 ; gamma2) : R (is1 -> is2) ~> te' ]]\\
  \label{eq:compat_abs3}
  [[ (SS1 : \ ix : R (is1) . (ie1 with R ; phi1 ; gamma1) , SS2 : \ ix : R (is1) . (ie2 with R ; phi2 ; gamma2) ) in V (is1 -> is2) with TC ; R ]]
\end{gather}
By unfolding the definition of logical equivalence in the hypothesis of the theorem, we get:
\begin{equation}
  [[ (SS1 : ie1 with R' ; phi1' ; gamma1' , SS2 : ie2 with R' ; phi2' ; gamma2') in E (is2) with TC ; R' ]]
  \label{eq:compat_abs4}
\end{equation}
for any \([[ R' in F ( TT, ix : is1 ) with TC ]]\),
\([[ phi' in G ( TT, ix : is1 ) with SS1 ; SS2 ; TC ; R' ]]\) and
\([[ gamma' in H ( TT, ix : is1 ) with SS1 ; SS2 ; TC ; R' ]]\).

%% By the definition of \( \mathcal{F} \), \( \mathcal{G} \) and \( \mathcal{H} \),
%% we know that \([[ R' = R'' ]]\),
%% \([[ phi' = phi'', ix |-> (ie3 , ie4) ]]\) and
%% \([[ gamma' = gamma'' ]]\)
%% with \([[ R'' in F ( TT ) with TC ]]\),
%% \([[ phi'' in G ( TT ) with SS1 ; SS2 ; TC ; R'' ]]\),
%% \([[ gamma'' in H ( TT ) with SS1 ; SS2 ; TC ; R'' ]]\),
%% \([[ (SS1 : ie3 , SS2 : ie4) in E (is1) with TC ; R'' ]]\).

%We choose \([[ R'' = R ]]\), \([[ phi'' = phi ]]\) and \([[ gamma'' = gamma ]]\).

By the definition of the \( \mathcal{F} \)-relation and from Equation~\ref{eq:compat_absR},
we have that \([[R in F ( TT, ix : is1 ) with TC]]\) and we choose \([[ R' = R]]\).
By case analysis on \(\intermed{[[phi']]}\), we know that
\([[ phi' = phi'', ix |-> (ie3 , ie4) ]]\) for some
\([[phi'' in G (TT) with SS1 ; SS2 ; TC ; R]]\)
and expressions \(\intermed{[[ie3]]}\) and \(\intermed{[[ie4]]}\) such that
\begin{equation}
  \label{eq:compat_abs_ie34}
  [[ (SS1 : ie3 , SS2 : ie4) in E (is1) with TC ; R ]]
\end{equation}
We choose \([[ phi'' = phi ]]\).
Lastly, by the definition of the \( \mathcal{H} \)-relation and from
Equation~\ref{eq:compat_absH}, we have that
\([[ gamma in H ( TT, ix : is1 ) with SS1 ; SS2 ; TC ; R ]]\) and we choose
\([[ gamma' = gamma]]\).

With the above mentioned choices for \(\intermed{[[gamma']]}\), \(\intermed{[[phi']]}\) and
\(\intermed{[[R']]}\), unfolding the definition of the \( \mathcal{E} \)-relation in
Equation~\ref{eq:compat_abs4}, gives us:
\begin{gather}
  \label{eq:compat_abs5}
        [[ SS1 ; TC ; empty |-tm ie1 with R ; ( phi1, ix |-> ie3 ) ; gamma1 : R (is2) ~> te1 ]]\\
  \label{eq:compat_abs6}
        [[ SS2 ; TC ; empty |-tm ie2 with R ; ( phi2, ix |-> ie4 ) ; gamma2 : R (is2) ~> te2 ]]\\
        \label{eq:compat_abs7a}
\begin{split}    
  \exists \intermed{[[iv3]]}, \intermed{[[iv4]]} & :
    [[ SS1 |- ie1 with R ; (phi1, ix |-> ie3) ; gamma1 -->> iv3 ]]\\
%      \label{eq:compat_abs7b} 
    & \band [[ SS2 |- ie2 with R ; (phi2, ix |-> ie4) ; gamma2 -->> iv4 ]]\\
%      \label{eq:compat_abs7c}
      & \band [[ (SS1 : iv3 , SS2 : iv4) in V (is2) with TC ; R ]]
\end{split}
\end{gather}
By unfolding the definition of the \( \mathcal{E} \)-relation in
Equation~\ref{eq:compat_abs_ie34},
we know that:
%the given that \([[ (SS1 : ie3 , SS2 : ie4) in E (is1) with TC ; R ]]\), we know that:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm ie3 : is1 ~> te3 ]]
  \label{eq:compat_abs5c} \\
  [[ SS2 ; TC ; empty |-tm ie4 : is1 ~> te4 ]]
  \label{eq:compat_abs6c}
\end{gather}
Note that neither \(\intermed{[[ie3]]}\) nor \(\intermed{[[ie4]]}\) contain any free
variables, thus \([[ ie3 with R ; phi1 ; gamma1 = ie3 ]]\) and
\([[ ie4 with R ; phi2 ; gamma2 = ie4 ]]\). Taking these equations into account, from the
definition of substitution, Equations~\ref{eq:compat_abs5} and \ref{eq:compat_abs6} are rewritten to:
\begin{gather}
  \label{eq:compat_abs5b}
  [[ SS1 ; TC ; empty |-tm [| ie3 / ix |] ( ie1 with R ; phi1 ; gamma1 ) : R (is2) ~> te1 ]]\\
  \label{eq:compat_abs6b}
  [[ SS2 ; TC ; empty |-tm [| ie4 / ix |] ( ie2 with R ; phi2 ; gamma2 ) : R (is2) ~> te2 ]]
\end{gather}
By applying the substitution Lemma~\ref{lemma:rev_var_subst} on
Equations~\ref{eq:compat_abs5b} and \ref{eq:compat_abs6b} respectively, in
combination with Equations~\ref{eq:compat_abs5c} and \ref{eq:compat_abs6c}, we get:
\begin{gather}
  \label{eq:compat_abs13}
  [[ SS1 ; TC ; empty, ix : is1 |-tm ie1 with R ; phi1 ; gamma1 : R (is2) ~> te1' ]]\\
  \label{eq:compat_abs14}
  [[ SS2 ; TC ; empty, ix : is1 |-tm ie2 with R ; phi2 ; gamma2 : R (is2) ~> te2' ]]
\end{gather}
By Lemma~\ref{lemma:ctx_well_inter_typing}, it follows from
Equation~\ref{eq:compat_abs13} that \([[ |-ctx SS1 ; TC ; empty , ix : is1 ]]\).
By case analysis on this result, rule \textsc{iCtx-tyEnvTm} (the rule with which variable
\([[ix]]\) wad inserted in the environment) tells us that:
\begin{equation}
  \label{eq:compat_abs13b}
  [[ TC ; empty |-ty is1 ~> tt1 ]]
\end{equation}
Goals~\ref{eq:compat_abs1} and \ref{eq:compat_abs2} follow from applying the typing rule
\textsc{iTm-arrI} on Equations~\ref{eq:compat_abs13} and \ref{eq:compat_abs14} respectively,
together with Equation~\ref{eq:compat_abs13b}.

It remains to show Goal~\ref{eq:compat_abs3}. By unfolding the definition of the
\( \mathcal{V} \) relation, the goal simplifies to
\begin{align}
  \label{eq:compat_abs10}
  &\forall \intermed{[[ie5]]}\,\intermed{[[ie6]]},~\text{if}~
    [[ (SS1 : ie5 , SS2 : ie6) in E (is1) with TC ; R ]],\\
  \label{eq:compat_absglast}
  &\text{then}~[[ ( SS1 : (? \ ix : R (is1) . ( ie1 with R ; phi1 ; gamma1 ) ?) ie5 , SS2 : (? \ ix : R (is1) . ( ie2 with R ; phi2 ; gamma2 ) ?) ie6 ) in E (is2) with TC ; R ]]
\end{align}
Then, suppose expressions \(\intermed{[[ie5]]}\) and \(\intermed{[[ie6]]}\), such that
Equation~\ref{eq:compat_abs10} holds. By unfolding the definition of the \(\mathcal{E}\)
relation in Equation~\ref{eq:compat_abs10}, we have
\begin{gather}
  \label{eq:compat_abs15}
  [[ SS1 ; TC ; empty |-tm ie5 : is1 ~> te5' ]]\\
  \label{eq:compat_abs16}
  [[ SS2 ; TC ; empty |-tm ie6 : is1 ~> te6' ]]
\end{gather}
We also unfold the definition of the \( \mathcal{E} \) relation in
Goal~\ref{eq:compat_absglast},
to get:
\begin{gather}
  \label{eq:compat_abs8}
  [[ SS1 ; TC ; empty |-tm ( \ ix : R (is1) . ( ie1 with R ; phi1 ; gamma1 ) ) ie5 : is2 ~> te5 ]]\\
  \label{eq:compat_abs9}
  [[ SS2 ; TC ; empty |-tm ( \ ix : R (is1) . ( ie2 with R ; phi2 ; gamma2 ) ) ie6 : is2 ~> te6 ]]\\
\begin{split}
  \label{eq:compat_abs11}
  \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} & :
    [[ SS1 |- ( \ ix : R (is1) . ( ie1 with R ; phi1 ; gamma1 ) ) ie5 -->> iv5 ]] \\
    & \band [[ SS2 |- ( \ ix : R (is1) . ( ie2 with R ; phi2 ; gamma2 ) ) ie6 -->> iv6 ]] \\
    & \band [[ (SS1 : iv5 , SS2 : iv6) in V (is2) with TC ; R ]]
  \end{split}
\end{gather}
Goals~\ref{eq:compat_abs8} and \ref{eq:compat_abs9} follow by applying the \textsc{iTm-arrE}
typing rule once on Equations~\ref{eq:compat_abs13} and~\ref{eq:compat_abs15} and once more
on Equations~\ref{eq:compat_abs14} and~\ref{eq:compat_abs16}. Note that
Equations~\ref{eq:compat_abs13} and~\ref{eq:compat_abs14} have been already proven above.

%% By case analysis, the last rule used to build the derivations in
%% Equations~\ref{eq:compat_abs8} and~\ref{eq:compat_abs9} must be the \textsc{iTm-arrE}
%% typing rule. Therefore, it suffices to show the premises of the two \textsc{iTm-arrE}
%% instantiated rules. Goals~\ref{eq:compat_abs1}
%% and \ref{eq:compat_abs2} respectively (both of which have already been proven above)

%% By instantiating the \textsc{iTm-arrE} typing rule with the Goals~\ref{eq:compat_abs1}
%% and \ref{eq:compat_abs2} respectively (both of which have already been proven above),
%% Goals~\ref{eq:compat_abs8} and \ref{eq:compat_abs9} reduce to:
%% \begin{gather*}
%%   [[ SS1 ; TC ; empty |-tm ie5 : is1 ~> te5' ]]\\
%%   [[ SS2 ; TC ; empty |-tm ie6 : is1 ~> te6' ]]
%% \end{gather*}
%% both of which follow by unfolding the definition of \( \mathcal{E} \) in Equation~\ref{eq:compat_abs10}.

By case analysis, it is easy to see that the first step of the evaluations in
Goal~\ref{eq:compat_abs11} is \textsc{iEval-appAbs}, reducing the goal to:
\begin{equation*}
  \begin{split}
  \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} & :
    [[ SS1 |- [| ie5 / ix |] ie1 with R ; phi1 ; gamma1 -->> iv5 ]] \\
    & \band [[ SS2 |- [| ie6 / ix |] ie2 with R ; phi2 ; gamma2 -->> iv6 ]]\\
    & \band [[ (SS1 : iv5 , SS2 : iv6) in V (is2) with TC ; R ]]
  \end{split}
\end{equation*}
We choose \([[ ie3 = ie5 ]]\) and \([[ ie4 = ie6 ]]\) in Equation~\ref{eq:compat_abs_ie34}.
The goal follows by choosing \([[ iv5 = iv3 ]]\) and \([[ iv6 = iv4 ]]\) from
Equation~\ref{eq:compat_abs7a}. \\
\qed

\begin{lemmaB}[Compatibility - Term Application]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT |- SS1 : ie1 =log SS2 : ie1' : is1 -> is2 ]]
      \\ [[ TC ; TT |- SS1 : ie2 =log SS2 : ie2' : is1 ]]
    }
    { [[ TC ; TT |- SS1 : ie1 ie2 =log SS2 : ie1' ie2' : is2 ]] }
    \label{lemma:compat_app}
  \end{mathpar}
\end{lemmaB}

\proof By inlining the definition of logical equivalence, suppose we have:
\begin{gather*}
  [[ R in F ( TT ) with TC ]]\\
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gather*}
The goal to be proven is the following:
\begin{equation*}
  [[ (SS1 : ie1 ie2 with R ; phi1 ; gamma1 , SS2 : (? ie1' ie2' ?) with R ; phi2 ; gamma2) in E (is2) with TC ; R ]]
\end{equation*}
By applying the definition of the \( \mathcal{E} \) relation, the goal reduces
to:
\begin{gather}
  \label{eq:compat_app1}
  [[ SS1 ; TC ; empty |-tm ie1 ie2 with R ; phi1 ; gamma1 : R (is2) ~> te ]]\\
  \label{eq:compat_app2}
  [[ SS2 ; TC ; empty |-tm ie1' ie2' with R ; phi2 ; gamma2 : R (is2) ~> te' ]]\\
  \label{eq:compat_app3}
\begin{split}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- ie1 ie2 with R ; phi1 ; gamma1 -->> iv1 ]] \\ %\nonumber \\
    & \band [[ SS2 |- ie1' ie2' with R ; phi2 ; gamma2 -->> iv2 ]]\\ % \nonumber \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is2) with TC ; R ]]
\end{split}
\end{gather}
By applying the substitutions in Goals~\ref{eq:compat_app1} and
\ref{eq:compat_app2}, they reduce to:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm (ie1 with R ; phi1 ; gamma1) (ie2 with R ; phi1 ; gamma1) : R (is2) ~> te ]]
  \label{eq:compat_app10}\\
  [[ SS2 ; TC ; empty |-tm (ie1' with R ; phi2 ; gamma2) (ie2' with R ; phi2 ; gamma2) : R (is2) ~> te' ]]
  \label{eq:compat_app11}
\end{gather}
By inlining the definition of logical equivalence in the premise of the rule, we
get:
\begin{align}
  [[ SS1 ; TC ; empty |-tm ie1 with R ; phi1 ; gamma1 : R (is1 -> is2) ~> te1 ]]
  \label{eq:compat_app4} \\
  [[ SS2 ; TC ; empty |-tm ie1' with R ; phi2 ; gamma2 : R (is1 -> is2) ~> te1' ]]
  \label{eq:compat_app5}
\end{align}
\begin{align}
  \exists \intermed{[[iv3]]}, \intermed{[[iv4]]} & :
    [[ SS1 |- ie1 with R ; phi1 ; gamma1 -->> iv3 ]]
    \label{eq:compat_app6a} \\
    & \band [[ SS2 |- ie1' with R ; phi2 ; gamma2 -->> iv4 ]]
    \label{eq:compat_app6b} \\
    & \band [[ (SS1 : iv3 , SS2 : iv4) in V (is1 -> is2) with TC ; R ]]
  \label{eq:compat_app6c}
\end{align}
and
\begin{gather}
  [[ SS1 ; TC ; empty |-tm ie2 with R ; phi1 ; gamma1 : R (is1) ~> te2 ]]
  \label{eq:compat_app7} \\
  [[ SS2 ; TC ; empty |-tm ie2' with R ; phi2 ; gamma2 : R (is1) ~> te2' ]]
  \label{eq:compat_app8}\\
%\end{align}
  %\begin{align}
\begin{split}\nonumber
  \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} & :
    [[ SS1 |- ie2 with R ; phi1 ; gamma1 -->> iv5 ]]\\
%    \label{eq:compat_app9a} \\
    & \band [[ SS2 |- ie2' with R ; phi2 ; gamma2 -->> iv6 ]]\\
%    \label{eq:compat_app9b} \\
    & \band [[ (SS1 : iv5 , SS2 : iv6) in V (is1) with TC ; R ]]
%  \label{eq:compat_app9c}
\end{split}
\end{gather}
By applying both Equation~\ref{eq:compat_app4} and \ref{eq:compat_app7} and both
Equation~\ref{eq:compat_app5} and \ref{eq:compat_app8} respectively to \textsc{iTm-arrE},
Goal~\ref{eq:compat_app10} and \ref{eq:compat_app11} are proven.

By applying the substitution, Goal~\ref{eq:compat_app3} reduces to:
\begin{align*}
  \begin{split}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- (ie1 with R ; phi1 ; gamma1) (ie2 with R ; phi1 ; gamma1) -->> iv1 ]] \\
    & \band [[ SS2 |- (ie1' with R ; phi2 ; gamma2) (ie2' with R ; phi2 ; gamma2) -->> iv2 ]]\\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is2) with TC ; R ]]
  \end{split}
%  \label{eq:compat_app12}
\end{align*}
Through case analysis, we see that we should first (repeatedly) apply
\textsc{iEval-app} and Equation~\ref{eq:compat_app6a} and \ref{eq:compat_app6b}
respectively. The goal reduces to:
\begin{align}
  \begin{split}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- iv3 (ie2 with R ; phi1 ; gamma1) -->> iv1 ]] \\
    & \band [[ SS2 |- iv4 (ie2' with R ; phi2 ; gamma2) -->> iv2 ]] \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is2) with TC ; R ]]
  \end{split}
  \label{eq:compat_app13}
\end{align}
By the definition of the \( \mathcal{V} \)-relation in Equation~\ref{eq:compat_app6c}, we
know that:
\begin{gather}
%  \nonumber
%  \exists \intermed{[[ie3]]} : [[ iv3 = \ ix : is1 . ie3 ]]\\
  %  \label{eq:compat_app14} \\
%  \nonumber
%  \exists \intermed{[[ie4]]} : [[ iv4 = \ ix : is1 . ie4 ]]\\
  %  \label{eq:compat_app15}
  \nonumber
  [[ SS1 ; TC ; empty |-tm iv3 : R (is1 -> is2) ~> te3 ]]\\
  %  \label{eq:compat_app16}
  \nonumber
  [[ SS2 ; TC ; empty |-tm iv4 : R (is1 -> is2) ~> te4 ]]\\
%  \label{eq:compat_app17}
  \forall [[ (SS1 : ie5 , SS2 : ie6) in E (is1) with TC ; R ]] :
  [[ (SS1 : iv3 ie5 , SS2 : iv4 ie6) in E (is2) with TC ; R ]]
  \label{eq:compat_app18}
\end{gather}
We choose \([[ ie5 = ie2 with R ; phi1 ; gamma1 ]]\) and
\([[ ie6 = ie2' with R; phi2 ; gamma2 ]]\). Goal~\ref{eq:compat_app13} now follows from
the definition of the \( \mathcal{E} \)-relation in Equation~\ref{eq:compat_app18}. \\
\qed

\begin{lemmaB}[Compatibility - Dictionary Abstraction]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT, idvar : iq |- SS1 : ie1 =log SS2 : ie2 : is ]]
    }
    { [[ TC ; TT |- SS1 : \ idvar : iq . ie1 =log SS2 : \ idvar : iq . ie2 : iq -> is ]] }
    \label{lemma:compat_dabs}
  \end{mathpar}
\end{lemmaB}

\proof
By unfolding the definition of logical equivalence in the conclusion of the lemma,
suppose we have:
\begin{gather}
  \label{eq:compat_dabsR}
  [[ R in F ( TT ) with TC ]]\\
  \label{eq:compat_dabsG}
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  \nonumber
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gather}
The goal to be proven is the following:
\begin{equation*}
  [[ (SS1 : \ idvar : iq . ie1 with R ; phi1 ; gamma1 , SS2 : (? \idvar : iq . ie2 ?) with R ; phi2 ; gamma2) in E (iq -> is) with TC ; R ]]
\end{equation*}
By applying the definition of the \( \mathcal{E} \) relation (taking into
account that \(\intermed{[[ \ idvar : iq . ie ]]}\) is a value) and partially applying
the substitutions, the goal reduces to:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm \ idvar : R (iq) . (ie1 with R ; phi1 ; gamma1) : R (iq -> is) ~> te ]]
  \label{eq:compat_dabs1} \\
  [[ SS2 ; TC ; empty |-tm \ idvar : R (iq) . (ie2 with R ; phi2 ; gamma2) : R (iq -> is) ~> te' ]]
  \label{eq:compat_dabs2} \\
  [[ ( SS1 : \ idvar : R (iq) . (ie1 with R ; phi1 ; gamma1) , SS2 : \ idvar : R (iq) . (ie2 with R ; phi2 ; gamma2) ) in V ( iq -> is ) with TC ; R ]]
  \label{eq:compat_dabs3}
\end{gather}
By unfolding the definition of logical equivalence in the premise of this lemma, we get:
\begin{equation}
  [[ ( SS1 : ie1 with R' ; phi1' ; gamma1' , SS2 : ie2 with R' ; phi2' ; gamma2' ) in E (is) with TC ; R' ]]
  \label{eq:compat_dabs4}
\end{equation}
for any \([[ R' in F (TT, idvar : iq) with TC ]]\), \([[ phi' in G (TT, idvar :
iq) with SS1 ; SS2 ; TC ; R' ]]\) and \([[ gamma' in H (TT, idvar : iq) with SS1
; SS2 ; TC ; R' ]]\).

By the definition of the \( \mathcal{F} \) and the \( \mathcal{G} \) relations and from
Equations~\ref{eq:compat_dabsR} and~\ref{eq:compat_dabsG}, we have that
\([[ R in F (TT, idvar : iq) with TC ]]\) and
\([[ phi in G (TT, idvar : iq) with SS1 ; SS2 ; TC ; R' ]]\). We choose \([[ R' = R ]]\)
and \([[ phi' = phi ]]\). By case analysis on \(\intermed{[[gamma']]}\), we know that
\([[gamma' = gamma'', idvar |-> (idv1 , idv2)]]\) for some
\([[ gamma'' in H (TT) with SS1 ; SS2 ; TC ; R ]]\) and some dictionaries
\(\intermed{[[idv1]]}\) and \(\intermed{[[idv2]]}\) such that
\begin{equation}
  \label{eq:compat_dabs_dv12}
  [[(SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R]]
\end{equation}
We choose \([[gamma'' = gamma]]\).
%% By the definition of \( \mathcal{F} \), \( \mathcal{G} \) and \( \mathcal{H} \),
%% we know that \([[ R' = R'' ]]\), 
%% \([[ phi' = phi'' ]]\) and 
%% \([[ gamma' = gamma'', idvar |-> (idv1 , idv2) ]]\)
%% with \([[ R'' in F (TT) with TC ]]\), 
%% \([[ phi'' in G (TT) with SS1 ; SS2 ; TC ; R'' ]]\), 
%% \([[ gamma'' in H (TT) with SS1 ; SS2 ; TC ; R'' ]]\) and 
%% \([[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R'' ]]\).
%% We pick \([[ R'' = R ]]\), \([[ phi'' = phi ]]\) and \([[ gamma'' = gamma ]]\).
Then, unfolding the definition of the \( \mathcal{E} \) relation in Equation~\ref{eq:compat_dabs4}
results in:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm ie1 with R ; phi1 ; (gamma1, idvar |-> idv1) : R ( is ) ~> te1 ]]
  \label{eq:compat_dabs4b} \\
  [[ SS2 ; TC ; empty |-tm ie2 with R ; phi2 ; (gamma2, idvar |-> idv2) : R ( is ) ~> te2 ]]
  \label{eq:compat_dabs5} \\
\begin{split}
\label{eq:compat_dabs6}
  \exists \intermed{[[ iv1 ]]}, \intermed{[[ iv2 ]]} & :
    [[ SS1 |- ie1 with R ; phi1 ; (gamma1, idvar |-> idv1) -->> iv1 ]]\\
%      \nonumber \\
    & \band [[ SS2 |- ie2 with R ; phi2 ; (gamma2, idvar |-> idv2) -->> iv2 ]]\\
%      \nonumber \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is) with TC ; R ]]
\end{split}
\end{gather}
From the definition of the \( \mathcal{V} \) relation in Equation~\ref{eq:compat_dabs_dv12},
it follows that:
\begin{gather}
  [[ SS1 ; TC ; empty |-d idv1 : iq ~> te3 ]]
  \label{eq:compat_dabs4be} \\
  [[ SS2 ; TC ; empty |-d idv2 : iq ~> te4 ]]
  \label{eq:compat_dabs5be}
\end{gather}
Since neither \(\intermed{[[idv1]]}\) nor \(\intermed{[[idv2]]}\) contain any free variables, we know
that \([[ gamma1 (idv1) = idv1 ]]\) and \([[ gamma2 (idv2) = idv2 ]]\).
Consequently, Equations~\ref{eq:compat_dabs4b} and \ref{eq:compat_dabs5} are
equivalent to:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm [| idv1 / idvar |] ( ie1 with R ; phi1 ; gamma1 ) : R ( is ) ~> te1 ]]
  \label{eq:compat_dabs4ce} \\
  [[ SS2 ; TC ; empty |-tm [| idv2 / idvar |] ( ie2 with R ; phi2 ; gamma2 ) : R ( is ) ~> te2 ]]
  \label{eq:compat_dabs5ce}
\end{gather}
By applying the substitution Lemma~\ref{lemma:rev_dvar_subst} on
Equations~\ref{eq:compat_dabs4ce} and \ref{eq:compat_dabs5ce} respectively, in
combination with Equations~\ref{eq:compat_dabs4be} and \ref{eq:compat_dabs5be}, we
find:
\begin{gather}
  [[ SS1 ; TC ; empty, idvar : iq |-tm ie1 with R ; phi1 ; gamma1 : R ( is ) ~> te1' ]]
  \label{eq:compat_dabs7} \\
  [[ SS2 ; TC ; empty, idvar : iq |-tm ie2 with R ; phi2 ; gamma2 : R ( is ) ~> te2' ]]
  \label{eq:compat_dabs8}
\end{gather}
By Lemma~\ref{lemma:ctx_well_inter_typing}, it follows from
Equation~\ref{eq:compat_dabs7} that \([[ |-ctx SS1 ; TC ; empty , idvar : iq
]]\).
Consequently, we know from \textsc{iCtx-tyEnvD} that:
\begin{equation}
  \label{eq:compat_dabs7b}
  [[ TC ; empty |-q iq ~> ttq ]]
\end{equation}
Since \([[ iq ]]\) does not contain any free variables, it is straightforward to
see that \([[ R (iq) = iq ]]\).

Consequently, goals~\ref{eq:compat_dabs1} and \ref{eq:compat_dabs2} follow by applying
Equation~\ref{eq:compat_dabs7} and \ref{eq:compat_dabs8} respectively, in
combination with Equation~\ref{eq:compat_dabs7b}, to \textsc{iTm-constrI}.

By unfolding the definition of \( \mathcal{V} \),
Goal~\ref{eq:compat_dabs3} reduces to:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm \ idvar : R (iq) . (ie1 with R ; phi1 ; gamma1) : R (iq -> is) ~> te ]]
  \label{eq:compat_dabs9} \\
  [[ SS2 ; TC ; empty |-tm \ idvar : R (iq) . (ie2 with R ; phi2 ; gamma2) : R (iq -> is) ~> te' ]]
  \label{eq:compat_dabs10} \\
%  \begin{gathered}
  \forall \intermed{[[idv3]]}\,\intermed{[[idv4]]},~\text{if}~[[ (SS1 : idv3 , SS2 : idv4) in V (iq) with TC ; R ]] :
  \label{eq:compat_dabs11'} \\
  \text{then}~[[ ( SS1 : ( \ idvar : R (iq) . (ie1 with R ; phi1 ; gamma1) ) idv3 , SS2 : (\ idvar : R (iq) . (ie2 with R ; phi2 ; gamma2)) idv4 ) in E (is) with TC ; R ]]
  \label{eq:compat_dabs11}
%  \end{gathered}
\end{gather}
Goals~\ref{eq:compat_dabs9} and \ref{eq:compat_dabs10} are identical to
Goals~\ref{eq:compat_dabs1} and~\ref{eq:compat_dabs2}, which have been proven above.
For the final goal, suppose dictionaries \(\intermed{[[idv3]]}\) and
\(\intermed{[[idv4]]}\) such that Equation~\ref{eq:compat_dabs11'} holds. By the definition
of the \(\mathcal{V}\) relation in Equation~\ref{eq:compat_dabs11'}, we obtain:
\begin{gather}
  \label{eq:compat_dabs15}
  [[ SS1 ; TC ; empty |-d idv3 : iq ~> te3' ]]\\
  \label{eq:compat_dabs16}
  [[ SS2 ; TC ; empty |-d idv4 : iq ~> te4' ]]
\end{gather}
We unfold
the definition of the \( \mathcal{E} \) relation in Goal~\ref{eq:compat_dabs11},
reducing it to:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm (\ idvar : R (iq) . (ie1 with R ; phi1 ; gamma1)) idv3 : R (is) ~> te5 ]]
  \label{eq:compat_dabs12}\\
  [[ SS2 ; TC ; empty |-tm (\ idvar : R (iq) . (ie2 with R ; phi2 ; gamma2)) idv4 : R (is) ~> te6 ]]
  \label{eq:compat_dabs13}\\
\begin{split}
    \label{eq:compat_dabs14}
  \exists \intermed{[[ iv3 ]]}, \intermed{[[ iv4 ]]} & :
  [[ SS1 |- (\ idvar : R (iq) . (ie1 with R ; phi1 ; gamma1)) idv3 -->> iv3 ]]\\
  & \band [[ SS2 |- (\ idvar : R (iq) . (ie2 with R ; phi2 ; gamma2)) idv4 -->> iv4 ]]\\
  & \band [[ (SS1 : iv3 , SS2 : iv4) in V (is) with TC ; R ]]
\end{split}
\end{gather}
Goals~\ref{eq:compat_dabs12} and \ref{eq:compat_dabs13} follow by applying the
\textsc{iTm-constrE} typing rule once on Equations~\ref{eq:compat_dabs9}
and~\ref{eq:compat_dabs15} and once on Equations~\ref{eq:compat_dabs10}
and~\ref{eq:compat_dabs16}.
%% By applying Equation~\ref{eq:compat_dabs9} and \ref{eq:compat_dabs10} to \textsc{iTm-constrE}, Goals~\ref{eq:compat_dabs12} and
%% \ref{eq:compat_dabs13} respectively reduce to:
%% \begin{gather*}
%%   [[ SS1 ; TC ; empty |-d idv3 : iq ~> te3' ]]\\
%%   [[ SS2 ; TC ; empty |-d idv4 : iq ~> te4' ]]
%% \end{gather*}
%% Both of which follow immediately from the definition of the \( \mathcal{V} \)
%% relation in Equation~\ref{eq:compat_dabs11}.

Through case analysis, it is straightforward to note that the first step of
the evaluation paths in Equation~\ref{eq:compat_dabs14} should be by rule
\textsc{iEval-DAppAbs}. The goal reduces to:
\begin{align*}
  \exists \intermed{[[ iv3 ]]}, \intermed{[[ iv4 ]]} & :
  [[ SS1 |- [| idv3 / idvar |] (ie1 with R ; phi1 ; gamma1) -->> iv3 ]]\\
  & \band [[ SS2 |- [| idv4 / idvar |] (ie2 with R ; phi2 ; gamma2) -->> iv4 ]]\\
  & \band [[ (SS1 : iv3 , SS2 : iv4) in V (is) with TC ; R ]]
\end{align*}
The above goal follows directly from Equation~\ref{eq:compat_dabs6}, by choosing \([[ idv1 = idv3 ]]\), \([[ idv2 = idv4 ]]\), \([[ iv3 = iv1 ]]\) and \([[ iv4 = iv2 ]]\). \\
\qed

\begin{lemmaB}[Compatibility - Dictionary Application]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : iq -> is ]]
      \\ [[ TC ; TT |- SS1 : id1 =log SS2 : id2 : iq ]]
    }
    { [[ TC ; TT |- SS1 : ie1 id1 =log SS2 : ie2 id2 : is ]] }
    \label{lemma:compat_dapp}
  \end{mathpar}
\end{lemmaB}

\proof
By inlining the definition of logical equivalence, suppose we have:
\begin{gather*}
  [[ R in F ( TT ) with TC ]]\\
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gather*}
The goal to be proven is the following:
\begin{equation*}
  [[ ( SS1 : (? ie1 id1 ?) with R ; phi1 ; gamma1 , SS2 : (? ie2 id2 ?) with R ; phi2 ; gamma2) in E (is) with TC ; R ]]
\end{equation*}
By unfolding the definition of the \( \mathcal{E} \) relation in the goal above, and by
simplifying the substitutions, the goal reduces to:
%% \begin{gather*}
%%   [[ SS1 ; TC ; empty |-tm (? ie1 id1 ?) with R ; phi1 ; gamma1 : R (is) ~> te ]]\\
%%   [[ SS2 ; TC ; empty |-tm (? ie2 id2 ?) with R ; phi2 ; gamma2 : R (is) ~> te' ]]\\
%% \begin{split}
%%   \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
%%     [[ SS1 |- (? ie1 id1 ?) with R ; phi1 ; gamma1 -->> iv1 ]]\\ %\nonumber \\
%%     & \band [[ SS2 |- (? ie2 id2 ?) with R ; phi2 ; gamma2 -->> iv2 ]]\\ % \nonumber \\
%%     & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is) with TC ; R ]]
%% \end{split}
%% %\label{eq:compat_dapp3}
%% \end{gather*}
%% By simplifying the substitutions in the goal, it reduces to:
\begin{gather}
  \label{eq:compat_dapp4}
  [[ SS1 ; TC ; empty |-tm (ie1 with R ; phi1 ; gamma1) (id1 with R ; phi1 ; gamma1) : R ( is ) ~> te ]]\\
  \label{eq:compat_dapp5}
  [[ SS2 ; TC ; empty |-tm (ie2 with R ; phi2 ; gamma2) (id2 with R ; phi2 ; gamma2) : R ( is ) ~> te' ]]\\
  \label{eq:compat_dapp17}
\begin{split}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- (ie1 with R ; phi1 ; gamma1) (id1 with R ; phi1 ; gamma1) -->> iv1 ]]\\ %\nonumber \\
    & \band [[ SS2 |- (ie2 with R ; phi2 ; gamma2) (id2 with R ; phi2 ; gamma2) -->> iv2 ]]\\ %\nonumber \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is) with TC ; R ]]
\end{split}
\end{gather}
By inlining the definitions of logical equivalence and the \(\mathcal{E}\)
relation in the first premise of this lemma, we get:
\begin{gather}
  \label{eq:compat_dapp6}
  [[ SS1 ; TC ; empty |-tm ie1 with R ; phi1 ; gamma1 : R (iq -> is) ~> te1 ]]\\
  \label{eq:compat_dapp7}
  [[ SS2 ; TC ; empty |-tm ie2 with R ; phi2 ; gamma2 : R (iq -> is) ~> te2 ]]\\
  \label{eq:compat_dapp8}
  \begin{split}
  \exists \intermed{[[iv3]]}, \intermed{[[iv4]]} & :
    [[ SS1 |- ie1 with R ; phi1 ; gamma1 -->> iv3 ]]\\
%    \label{eq:compat_dapp8a} \\
    & \band [[ SS2 |- ie2 with R ; phi2 ; gamma2 -->> iv4 ]]\\
%    \label{eq:compat_dapp8b} \\
    & \band [[ (SS1 : iv3 , SS2 : iv4) in V (iq -> is) with TC ; R ]]
%    \label{eq:compat_dapp8c}
  \end{split}
\end{gather}
Similarly, by unfolding the definition of logical equivalence 
in the second premise of the rule, we get:
\begin{equation}
  [[ (SS1 : id1 with R ; phi1 ; gamma1 , SS2 : id2 with R ; phi2 ; gamma2) in V (iq) with TC ; R ]]
  \label{eq:compat_dapp16}
\end{equation}
From the definition of the \(\mathcal{V}\) relation in
Equation~\ref{eq:compat_dapp16} we have:
\begin{gather}
  \label{eq:compat_dapp11}
  [[ SS1 ; TC ; empty |-d id1 with R ; phi1 ; gamma1 : R (iq) ~> te3 ]]\\
  \label{eq:compat_dapp12}
  [[ SS2 ; TC ; empty |-d id2 with R ; phi2 ; gamma2 : R (iq) ~> te4 ]]
\end{gather}
Note that, by the definition of substitution, we have
\([[ R (iq -> is) = R (iq) -> R(is) ]]\). This allows the application of
the typing rule \textsc{iTm-constrE} once on
Equations~\ref{eq:compat_dapp6} and \ref{eq:compat_dapp11} and once more on
Equations~\ref{eq:compat_dapp7} and \ref{eq:compat_dapp12}, therefore proving
Goals~\ref{eq:compat_dapp4} and \ref{eq:compat_dapp5}.

Through application of the \textsc{iEval-DApp} evaluation rule on each step of the two
evaluation paths in Equation~\ref{eq:compat_dapp8},
Goal~\ref{eq:compat_dapp17} reduces to:
\begin{align}
\label{eq:compat_dapp18}
\begin{split}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- iv3 (id1 with R ; phi1 ; gamma1) -->> iv1 ]]\\  % \nonumber \\
    & \band [[ SS2 |- iv4 (id2 with R ; phi2 ; gamma2) -->> iv2 ]]\\ % \nonumber \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is) with TC ; R ]]
\end{split}
\end{align}
Unfolding the definition of the \(\mathcal{V}\) relation in
Equation~\ref{eq:compat_dapp8} results in:
\begin{gather}
%  \nonumber
%  [[ iv3 = \ idvar : iq . ie3 ]]\\
%  \nonumber
%  [[ iv4 = \ idvar : iq . ie4 ]]\\
%  \label{eq:compat_dapp13}
  \nonumber
  [[ SS1 ; TC ; empty |-tm iv3 : R (iq -> is) ~> te5 ]]\\
%  \label{eq:compat_dapp14}
  \nonumber
  [[ SS2 ; TC ; empty |-tm iv4 : R (iq -> is) ~> te6 ]]\\
  \label{eq:compat_dapp15}
  \forall [[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R ]] :
          [[ (SS1 : iv3 idv1 , SS2 : iv4 idv2) in E (is) with TC ; R ]]  
\end{gather}
%For some \([[idvar]]\), \([[ie3]]\) and \([[ie4]]\).
We take \([[ idv1 = id1 with R ; phi1 ; gamma1 ]]\) and
\([[ idv2 = id2 with R ; phi2 ; gamma2 ]]\).
%(given by Equation~\ref{eq:compat_dapp16}).
Goal~\ref{eq:compat_dapp18} follows from the definition of the \(\mathcal{E}\)
relation in Equation~\ref{eq:compat_dapp15}. \\
\qed

\begin{lemmaB}[Compatibility - Type Abstraction]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT, c |- SS1 : ie1 =log SS2 : ie2 : is ]]
    }
    { [[ TC ; TT |- SS1 : /\ c. ie1 =log SS2 : /\ c . ie2 : \/ c . is ]] }
    \label{lemma:compat_tyabs}
  \end{mathpar}
\end{lemmaB}

\proof
By unfolding the definition of logical equivalence, suppose we have:
\begin{gather}
  \label{eq:comat_tyabsR}
  [[ R in F ( TT ) with TC ]]\\
  \label{eq:comat_tyabsG}
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  \label{eq:comat_tyabsH}
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gather}
The goal to be proven is the following:
\begin{equation*}
  [[ (SS1 : /\ c . ie1 with R ; phi1 ; gamma1 , SS2 : (? /\ c. ie2 ?) with R ; phi2 ; gamma2) in E (\/ c . is) with TC ; R ]]
\end{equation*}
Because \([[c notin TT]]\), from Equation~\ref{eq:comat_tyabsR} it follows that
\([[c]]\) is not in the domain of \([[R]]\). Furthermore, from
Equations~\ref{eq:comat_tyabsG} and~\ref{eq:comat_tyabsH} it follows that for every mapping
\([[ix |-> ( ie1' , ie2' ) in phi]]\) and for every
mapping \([[idvar |-> ( idv1' , idv2' ) in gamma]]\), we have
\([[c]] \notin [[fv]](\intermed{[[iei']]})\) and
\([[c]] \notin [[fv]](\intermed{[[idvi']]})\), where \(\intermed{[[i]]}\in\{1,2\}\).
Therefore, we obtain
\([[(?/\ c. iei ?) with R ; phii ; gammai = /\ c . (? iei with R ; phii ; gammai ?)]]\),
for \(\intermed{[[i]]}\in\{1,2\}\). With these equations, the goal above reduces to
\begin{equation*}
  [[ (SS1 : /\ c . (? ie1 with R ; phi1 ; gamma1 ?) , SS2 : /\ c. (? ie2 with R ; phi2 ; gamma2 ?)) in E (\/ c . is) with TC ; R ]]
\end{equation*}
By applying the definition of the \( \mathcal{E} \) relation, taking into
account that expressions of the form \(\intermed{[[/\ c . ie]]}\) are values, the goal
reduces to:
\begin{gather}
  \label{eq:compat_tyabs1}
  [[ SS1 ; TC ; empty |-tm /\ c. (? ie1 with R ; phi1 ; gamma1 ?) : R (\/ c . is) ~> te ]]\\
  \label{eq:compat_tyabs2}
  [[ SS2 ; TC ; empty |-tm /\ c. (? ie2 with R ; phi2 ; gamma2 ?) : R (\/ c . is) ~> te' ]]\\
  \label{eq:compat_tyabs3}
  [[ (SS1 : /\ c . (? ie1 with R ; phi1 ; gamma1 ?) , SS2 : /\ c . (? ie2 with R ; phi2 ; gamma2 ?)) in V (\/ c . is) with TC ; R ]]
\end{gather}
Suppose any \(\intermed{[[is']]}\) such that 
\begin{equation}
  \label{eq:compat_tyabs20}
  [[TC ; empty |-ty is' ~> tt']]
\end{equation}
and any \([[r in Rel ( is' )]]\). Then, inlining the
definition of the \(\mathcal{V}\) relation in
Goal~\ref{eq:compat_tyabs3}, reduces it to:
\begin{equation}
  \label{eq:compat_tyabs8}
 [[ (SS1 : (/\ c . (? ie1 with R ; phi1 ; gamma1 ?)) is' , SS2 : (/\ c . (? ie2 with R ; phi2 ; gamma2 ?)) is') in E (is) with TC ; R, c |-> (is' , r) ]]
\end{equation}

Unfolding the definition of logical equivalence in the premise of this lemma, gives us:
\begin{equation}
  [[ (SS1 : ie1 with R' ; phi'1 ; gamma'1 , SS2 : ie2 with R' ; phi'2 ; gamma'2) in E (is) with TC ; R' ]]
  \label{eq:compat_tyabs4}
\end{equation}
for any \([[ R' in F ( TT, c ) with TC ]]\),
\([[ phi' in G ( TT, c ) with SS1 ; SS2 ; TC ; R' ]]\) and
\([[ gamma' in H ( TT, c ) with SS1 ; SS2 ; TC ; R' ]]\).

By the definition of the \( \mathcal{F} \) relation, we know that
\([[ R' = R'', c |-> (is'' , r') ]]\) for some \([[ R'' in F ( TT ) with TC ]]\) and
\(\intermed{[[is'']]}\) such that
\([[ TC ; empty |-ty is'' ~> tt' ]]\) and \([[ r' in Rel (is'') ]]\).
We choose \([[ R'' = R ]]\), \([[is'' = is']]\) and \([[r' = r]]\).
By the definition of the \( \mathcal{G} \) and \( \mathcal{H} \) relations and from
Equations~\ref{eq:comat_tyabsG} and~\ref{eq:comat_tyabsH}, we have that
\([[ phi in G ( TT, c ) with SS1 ; SS2 ; TC ; R ]]\) and \([[ gamma in H ( TT, c ) with SS1 ; SS2 ; TC ; R ]]\). Then, we choose \([[ phi' = phi ]]\) and
\([[ gamma' = gamma ]]\).

%% By the definition of \( \mathcal{F} \), \( \mathcal{G} \) and \( \mathcal{H} \),
%% we know that \([[ R' = R'', c |-> (is'' , r') ]]\),
%% \([[ phi' = phi'' ]]\) and
%% \([[ gamma' = gamma'' ]]\)
%% with \([[ R'' in F ( TT ) with TC ]]\),
%% \([[ phi'' in G ( TT ) with SS1 ; SS2 ; TC ; R'' ]]\),
%% \([[ gamma'' in H ( TT ) with SS1 ; SS2 ; TC ; R'' ]]\) 
%% for any \(\intermed{[[is'']]}\) such that: 
%% \([[ TC ; empty |-ty is'' ~> tt' ]]\)
%% and \([[ r' in Rel (is'') ]]\).

%% We choose \([[is'' = is']]\), \([[r' = r]]\), \([[ R'' = R ]]\), \([[ phi'' = phi ]]\) and \([[ gamma'' = gamma ]]\).

Unfolding the definition of the \(\mathcal{E}\) relation in
Equation~\ref{eq:compat_tyabs4}, results in:
\begin{gather}
  \label{eq:compat_tyabs5}
  [[ SS1 ; TC ; empty |-tm ie1 with R, c |-> (is' , r) ; phi1 ; gamma1 : (R, c |-> (is' , r)) (is) ~> te1 ]]\\
  \label{eq:compat_tyabs6}
  [[ SS2 ; TC ; empty |-tm ie2 with R, c |-> (is' , r) ; phi2 ; gamma2 : (R, c |-> (is' , r)) (is) ~> te2 ]]\\
  \label{eq:compat_tyabs7}
\begin{split}
  \exists \intermed{[[iv3]]}, \intermed{[[iv4]]} & :
  [[ SS1 |- ie1 with R, c |-> (is' , r) ; phi1 ; gamma1 -->> iv3 ]]\\
%    \nonumber \\
  & \band [[ SS2 |- ie2 with R, c |-> (is' , r) ; phi2 ; gamma2 -->> iv4 ]]\\
%    \nonumber \\
  & \band [[ (SS1 : iv1 , SS2 : iv2) in V (is) with TC ; (R, c |-> (is' , r)) ]]
\end{split}
\end{gather}
By the definition of substitution, and because \(\intermed{[[is']]}\) has no free
variables, it follows that \([[(R, c |-> (is' , r)) (is) = [| is' / c |] (R (is))]]\).
Furthermode, because \([[c notin TT]]\), from Equations~\ref{eq:comat_tyabsG}
and~\ref{eq:comat_tyabsH} it follows that \([[ie with (R, c |-> (is' , r)) ; phii ; gammai = [| is' / c |] (ie with R ; phii ; gammai)]]\),
for any expression \(\intermed{[[ie]]}\) and \(\intermed{[[i]]}\in\{1,2\}\). Taking these equalities into account, by
applying Equations~\ref{eq:compat_tyabs5} and \ref{eq:compat_tyabs6} to reverse
substitution Lemma~\ref{lemma:rev_tvar_subst} gives us:
\begin{align}
  \label{eq:compat_tyabs9}
  [[ SS1 ; TC ; empty, c |-tm ie1 with R ; phi1 ; gamma1 : R (is) ~> te1' ]]\\
  \label{eq:compat_tyabs10}
  [[ SS2 ; TC ; empty, c |-tm ie2 with R ; phi2 ; gamma2 : R (is) ~> te2' ]]
\end{align}
Because \([[c]]\) is not in the domain of \([[R]]\), we have
\([[R (\/ c . is) = \/ c . R ( is )]]\). %Similarly, we have
%\([[(/\ c. iei) with R ; phii ; gammai = /\ c . (iei with R ; phii ; gammai)]]\),
%for \(\intermed{[[i]]}\in\{1,2\}\).
Hence, Goals~\ref{eq:compat_tyabs1} and \ref{eq:compat_tyabs2} follow by passing
Equations~\ref{eq:compat_tyabs9} and \ref{eq:compat_tyabs10} to
\textsc{iTm-forallI}, respectively.

Unfolding the definition of the \(\mathcal{E}\) relation in
Goal~\ref{eq:compat_tyabs8} and since \([[(R, c |-> (is' , r)) (is) = [| is' / c |] (R (is))]]\), the goal
reduces to:
\begin{gather}
    \label{eq:compat_tyabs11a}
  [[ SS1 ; TC ; empty |-tm (/\ c . (? ie1 with R ; phi1 ; gamma1 ?)) is' : [| is' / c |] (R (is)) ~> te3 ]]\\
    \label{eq:compat_tyabs11b}
  [[ SS2 ; TC ; empty |-tm (/\ c . (? ie2 with R ; phi2 ; gamma2 ?)) is' : [| is' / c |] (R (is)) ~> te4 ]]\\
  \label{eq:compat_tyabs11c}
  \begin{split}
  \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} :\, & [[ SS1 |- (/\ c . (? ie1 with R ; phi1 ; gamma1 ?)) is' -->> iv5 ]]\\
%    \nonumber \\
   \band\, & [[ SS2 |- (/\ c . (? ie2 with R ; phi2 ; gamma2 ?)) is' -->> iv6 ]]\\
%    \nonumber \\
   \band\, & [[ (SS1 : iv5 , SS2 : iv6) in V (is) with TC ; R, c |-> (is' , r) ]]
  \end{split}
\end{gather}
Goals~\ref{eq:compat_tyabs11a} and \ref{eq:compat_tyabs11b} follow by applying
Goals~\ref{eq:compat_tyabs1} and \ref{eq:compat_tyabs2} (which have previously
been proven) to \textsc{iTm-forallE}, respectively, together with
Equation~\ref{eq:compat_tyabs20}.
%% Since \([[R]]\) does not contain any substitution for type variable \([[c]]\), Goal~\ref{eq:compat_tyabs11c} can be simplified to:
%% \begin{align}
%%   \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} & : [[ SS1 |- /\ c . (ie1 with R ; phi1 ; gamma1) is' -->> iv5 ]]
%%     \nonumber \\
%%   & \band [[ SS2 |- /\ c . (ie2 with R ; phi2 ; gamma2) is' -->> iv6 ]]
%%     \label{eq:compat_tyabs12}\\
%%   & \band [[ (SS1 : iv5 , SS2 : iv6) in V (is) with TC ; R, c |-> (is' , r) ]]
%%   \nonumber
%% \end{align}
The first step of both evaluation paths in Equation \ref{eq:compat_tyabs11c} can only be taken by appropriate instantiations of rule \textsc{iEval-tyAppAbs}. With this,
Goal~\ref{eq:compat_tyabs11c} can be further reduced to
\begin{align*}
  \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} & : [[ SS1 |- [| is' / c |] (ie1 with R ; phi1 ; gamma1) -->> iv5 ]]\\
  & \band [[ SS2 |- [| is' / c |] (ie2 with R ; phi2 ; gamma2) -->> iv6 ]]\\
  & \band [[ (SS1 : iv5 , SS2 : iv6) in V (is) with TC ; R, c |-> (is' , r) ]]
\end{align*}
which follows from Equation~\ref{eq:compat_tyabs7} by choosing \([[iv5 = iv3]]\)
and \([[iv6 = iv4]]\). \\
\qed

\begin{lemmaB}[Compatibility - Type Application]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : \/ c . is' ]]
      \\ [[ TC ; TT |-ty is ~> tt ]]
    }
    { [[ TC ; TT |- SS1 : ie1 is =log SS2 : ie2 is : [| is / c |] is' ]] }
    \label{lemma:compat_tyapp}
  \end{mathpar}
\end{lemmaB}

\proof
By inlining the definition of logical equivalence, suppose we have:
\begin{gather*}
  [[ R in F ( TT ) with TC ]]\\
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gather*}
Note that, by the definition of the \( \mathcal{F} \) relation, \([[c]]\) is not in the domain of \([[R]]\), since \([[c notin TT ]]\).
The goal to be proven is the following:
\begin{equation}
  \label{eq:compat_tyapp21}
  [[ (SS1 : ie1 is with R ; phi1 ; gamma1 , SS2 : ie2 is with R ; phi2 ; gamma2) in E ([| is / c |] is') with TC ; R ]]
\end{equation}
From the definition of substitution we have that
\begin{gather*}
  [[iei is with R ; phii ; gammai = (? iei with R ; phii ; gammai ?) R (is)]],~
  \text{for}~ \intermed{i}\in\{1,2\}\\
  \text{and}~~[[R ([| is / c |] is') = [| R(is) / c |] R(is')]]
\end{gather*}
Taking into account these equalities and
by unfolding the definition of the \( \mathcal{E} \) relation,
Goal~\ref{eq:compat_tyapp21} reduces to:
%% \begin{gather*}
%% %  \label{eq:compat_tyapp1}
%%   [[ SS1 ; TC ; empty |-tm ie1 is with R ; phi1 ; gamma1 : R ([| is / c |] is') ~> te ]]\\
%% %  \label{eq:compat_tyapp2}
%%   [[ SS2 ; TC ; empty |-tm ie2 is with R ; phi2 ; gamma2 : R ([| is / c |] is') ~> te' ]]\\
%% \begin{split} %\nonumber
%%   \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
%%     [[ SS1 |- ie1 is with R ; phi1 ; gamma1 -->> iv1 ]] \\
%%     & \band [[ SS2 |- ie2 is with R ; phi2 ; gamma2 -->> iv2 ]]\\
%%     & \band [[ (SS1 : iv1 , SS2 : iv2) in V ([| is / c |] is') with TC ; R ]]
%% %  \label{eq:compat_tyapp3}
%% \end{split}
%% \end{gather*}
%% and by applying the substitutions, the goal further reduces to:
\begin{gather}
  \label{eq:compat_tyapp4}
  [[ SS1 ; TC ; empty |-tm (? ie1 with R ; phi1 ; gamma1 ?) R (is) : [| R(is) / c |] R(is') ~> te ]]\\
  \label{eq:compat_tyapp5}
  [[ SS2 ; TC ; empty |-tm (? ie2 with R ; phi2 ; gamma2 ?) R (is) : [| R(is) / c |] R(is') ~> te' ]]\\
\begin{split}\label{eq:compat_tyapp6}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- (ie1 with R ; phi1 ; gamma1) R (is) -->> iv1 ]] \\
    & \band [[ SS2 |- (ie2 with R ; phi2 ; gamma2) R (is) -->> iv2 ]] \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V ([| is / c |] is') with TC ; R ]]
\end{split}
\end{gather}

By inlining the definition of logical equivalence in the first premise of this lemma, we
get
\[
  [[ (SS1 : ie1 with R ; phi1 ; gamma1 , SS2 : ie2 with R ; phi2 ; gamma2) in E (\/ c . is') with TC ; R ]]
\]
Unfolding the definition of the \(\mathcal{E}\) relation results in:
\begin{gather}
  \label{eq:compat_tyapp8}
  [[ SS1 ; TC ; empty |-tm ie1 with R ; phi1 ; gamma1 : R (\/ c . is') ~> te1 ]]\\
  \label{eq:compat_tyapp9}
  [[ SS2 ; TC ; empty |-tm ie2 with R ; phi2 ; gamma2 : R (\/ c . is') ~> te2 ]]\\
\begin{split}\label{eq:compat_tyapp10}
  \exists \intermed{[[iv3]]}, \intermed{[[iv4]]} & :
  [[ SS1 |- ie1 with R ; phi1 ; gamma1 -->> iv3 ]]\\
  & \band [[ SS2 |- ie2 with R ; phi2 ; gamma2 -->> iv4 ]]\\
  & \band [[ (SS1 : iv3 , SS2 : iv4) in V (\/ c . is') with TC ; R ]]
\end{split}
\end{gather}
Starting from the second premise of this lemma, by sequentially applying
Lemma~\ref{lemma:tvar_tsubst} with the substitutions of \([[R]]\) on \(\intermed{[[is]]}\),
it follows that \([[TC ; TT' |-ty R (is) ~> tt]]\), where \(\intermed{[[TT']]}\) only
contains term variables. Then, starting from this result, by sequentually applying
Lemma~\ref{lemma:var_subst_types}, we obtain
\begin{equation}
  \label{eq:compat_tyapp20}
  [[TC ; empty |-ty R (is) ~> tt]]
\end{equation}
Since \([[c]]\) is not in the domain of \([[R]]\), we have
\([[R (\/ c . is) = \/ c . R (is)]]\). Consequently, Goals~\ref{eq:compat_tyapp4} and
\ref{eq:compat_tyapp5} follow by instantiating rule \textsc{iTm-forallE} with
Equations~\ref{eq:compat_tyapp8} and \ref{eq:compat_tyapp9}, respectively, together
with Equation~\ref{eq:compat_tyapp20}.

The definition of the \(\mathcal{V}\) relation in Equation~\ref{eq:compat_tyapp10}
tells us that:
%\begin{equation*}
%  [[ iv3 = /\ c . ie3 ]]
%\end{equation*}
%\begin{equation*}
%  [[ iv4 = /\ c . ie4 ]]
%\end{equation*}
\begin{equation}\label{eq:compat_tyapp11}
\begin{aligned}
  \forall \intermed{[[is'']]}, [[r in Rel (is'')]] & :
  [[ TC ; empty |-ty is'' ~> tt'' ]]\\
%    \nonumber \\
  & \Rightarrow [[ (SS1 : iv3 is'' , SS2 : iv4 is'') in E (is') with TC ; R, c |-> (is'' , r) ]]
\end{aligned}
\end{equation}
%For some \([[ie3]]\) and \([[ie4]]\).

By repeatedly applying \textsc{iEval-tyApp} on each step of both evaluation paths in
Equation~\ref{eq:compat_tyapp10}, Goal~\ref{eq:compat_tyapp6} reduces to:
\begin{align*}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} & :
    [[ SS1 |- iv3 R (is) -->> iv1 ]]\\ %\nonumber \\
    & \band [[ SS2 |- iv4 R (is) -->> iv2 ]]\\ % \nonumber \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V ([| is / c |] is') with TC ; R ]]
%  \label{eq:compat_tyapp13}
\end{align*}
which follows directly from~\ref{eq:compat_tyapp11} by choosing \([[is'' = is]]\)
and unfolding the definition of the \(\mathcal{E}\) relation. \\
\qed

\begin{lemmaB}[Compatibility - Let Binding]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is1 ]]
      \\ [[ TC ; TT, ix : is1 |- SS1 : ie1 =log SS2 : ie2 : is2 ]]
    }
    { [[ TC ; TT |- SS1 : ilet ix : is1 = ie1' iin ie1 =log SS2 : ilet ix : is1 = ie2'
      iin ie2 : is2 ]] }
    \label{lemma:compat_let}
  \end{mathpar}
\end{lemmaB}

\proof
By inlining the definition of logical equivalence, suppose we have:
\begin{equation}
  \label{eq:compat_let1}
  \begin{gathered}
    [[ R in F ( TT ) with TC ]]\\
    [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
    [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
  \end{gathered}
\end{equation}
The goal to be proven is the following:
\begin{equation}
  \label{eq:compat_let20}
  [[ ( SS1 : (? ilet ix : is1 = ie1' iin ie1 ?) with R ; phi1 ; gamma1 , SS2 : (? ilet ix : is1 = ie2' iin ie2 ?) with R ; phi2 ; gamma2) in E (is2) with TC ; R ]]
\end{equation}
From the definition of substitution, it follows that
\[
  [[(? ilet ix : is1 = iei' iin iei ?) with R ; phii ; gammai =
      ilet ix : R (is1) = (iei' with R ; phii ; gammai) iin (iei with R ; phii ; gammai)]],
  ~\text{for}~\intermed{i}\in\{1,2\}
\]
Taking into account this equality, by applying the definition of the
\( \mathcal{E} \) relation, Goal~\ref{eq:compat_let20} reduces
to:
%% \begin{gather*}
%% %  \label{eq:compat_let1}
%%   [[ SS1 ; TC ; empty |-tm ilet ix : is1 = ie1 iin ie2 with R ; phi1 ; gamma1 : R (is2) ~> te ]]\\
%% %  \label{eq:compat_let2}
%%   [[ SS2 ; TC ; empty |-tm ilet ix : is1 = ie1' iin ie2' with R ; phi2 ; gamma2 : R (is2) ~> te' ]]\\
%%   %  \label{eq:compat_let3}
%% %  \vspace{1.2cm}
%%   \begin{split}
%%   \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} : \, &
%%     [[ SS1 |- ilet ix : is1 = ie1 iin ie2 with R ; phi1 ; gamma1 -->> iv1 ]] \\
%%     \band\, & [[ SS2 |- ilet ix : is1 = ie1' iin ie2' with R ; phi2 ; gamma2 -->> iv2 ]] \\
%%     \band\, & [[ (SS1 : iv1 , SS2 : iv2) in V (is2) with TC ; R ]]
%% \end{split}
%% \end{gather*}
%% By applying the substitutions, the goal reduces to:
\begin{gather}
  \label{eq:compat_let4}
  [[ SS1 ; TC ; empty |-tm ilet ix : R (is1) = (ie1' with R ; phi1 ; gamma1) iin (ie1 with R ; phi1 ; gamma1) : R (is2) ~> te ]]\\
  \label{eq:compat_let5}
  [[ SS2 ; TC ; empty |-tm ilet ix : R (is1) = (ie2' with R ; phi2 ; gamma2) iin (ie2 with R ; phi2 ; gamma2) : R (is2) ~> te' ]]\\
\begin{split}\label{eq:compat_let6}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} :\, &
    [[ SS1 |- ilet ix : R (is1) = (ie1' with R ; phi1 ; gamma1) iin (ie1 with R ; phi1 ; gamma1) -->> iv1 ]] \\
    \band\, & [[ SS2 |- ilet ix : R (is1) = (ie2' with R ; phi2 ; gamma2) iin (ie2 with R ; phi2 ; gamma2) -->> iv2 ]]\\
    \band\, & [[ (SS1 : iv1 , SS2 : iv2) in V (is2) with TC ; R ]]
\end{split}
\end{gather}
By inlining the definition of logical equivalence in the two hypotheses of this lemma, we
get:
\begin{gather}
  \label{eq:compat_let7}
  [[ ( SS1 : ie1' with R ; phi1 ; gamma1 , SS2 : ie2' with R ; phi2 ; gamma2 ) in E (is1) with TC ; R ]]\\
  \label{eq:compat_let8}
  [[ ( SS1 : ie1 with R' ; phi'1 ; gamma'1 , SS2 : ie2 with R' ; phi'2 ; gamma'2 ) in E (is2) with TC ; R' ]]
\end{gather}
for any \([[ R' in F ( TT, ix : is1 ) with TC ]]\),
\([[ phi' in G ( TT, ix : is1 ) with SS1 ; SS2 ; TC ; R' ]]\) and
\([[ gamma' in H ( TT, ix : is1 ) with SS1 ; SS2 ; TC ; R' ]]\).
Note that in Equation~\ref{eq:compat_let7} we have already chosen the substitutions
\([[R]]\), \([[phi]]\) and \([[gamma]]\) from Equation~\ref{eq:compat_let1}.
By the definition of \( \mathcal{F} \), we obtain \([[R in F ( TT, ix : is1 ) with TC]]\).
Therefore, a valid choice for \(\intermed{[[R']]}\) is \([[R]]\). From the definitions of
\( \mathcal{G} \) and \( \mathcal{H} \), it must hold that
\([[ phi' = phi'', ix |-> (ie3 , ie4) ]]\) and
\([[ gamma' = gamma'' ]]\)
where
\([[ phi'' in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\),
\([[ gamma'' in H ( TT ) with SS1 ; SS2 ; TC ; R ]]\) and
\([[ (SS1 : ie3 , SS2 : ie4) in E (is1) with TC ; R ]]\).
We choose \([[ phi'' = phi ]]\) and \([[ gamma'' = gamma ]]\). It remains to
instantiate \(\intermed{[[ie3]]}\) and \(\intermed{[[ie4]]}\) with concrete choices.
For reasons of presentation, we defer this choice to the end of the proof.

From the definition of the \(\mathcal{E}\) relation in
Equations~\ref{eq:compat_let8}, we get:
\begin{gather}
  \label{eq:compat_let12}
  [[ SS1 ; TC ; empty |-tm ie1 with R ; (phi1, ix |-> ie3) ; gamma1 : R (is2) ~> te2 ]]\\
  \label{eq:compat_let13}
  [[ SS2 ; TC ; empty |-tm ie2 with R ; (phi2, ix |-> ie4) ; gamma2 : R (is2) ~> te2' ]]\\
\begin{split}\label{eq:compat_let14}
  \exists \intermed{[[iv5]]}, \intermed{[[iv6]]} :\, &
  [[ SS1 |- ie1 with R ; (phi1, ix |-> ie3) ; gamma1 -->> iv5 ]]\\
  \band\, & [[ SS2 |- ie2 with R ; (phi2, ix |-> ie4) ; gamma2 -->> iv6 ]]\\
  \band\, & [[ (SS1 : iv5 , SS2 : iv6) in V (is2) with TC ; R ]]
\end{split}
\end{gather}
Similarly, from Equation~\ref{eq:compat_let7} and from 
\([[ (SS1 : ie3 , SS2 : ie4) in E (is1) with TC ; R ]]\), we get:
\begin{gather}
  \label{eq:compat_let9}
  [[ SS1 ; TC ; empty |-tm ie1' with R ; phi1 ; gamma1 : R (is1) ~> te1 ]]\\
  \label{eq:compat_let10}
  [[ SS2 ; TC ; empty |-tm ie2' with R ; phi2 ; gamma2 : R (is1) ~> te1' ]]
\end{gather}
and
\begin{gather}
  [[ SS1 ; TC ; empty |-tm ie3 : R (is1) ~> te3 ]]
  \label{eq:compat_lete1} \\
  [[ SS1 ; TC ; empty |-tm ie4 : R (is1) ~> te4 ]]
  \label{eq:compat_lete2}
\end{gather}
Note that from Equations~\ref{eq:compat_lete1} and~\ref{eq:compat_lete2} it is
evident that expressions \(\intermed{[[ie3]]}\) and \(\intermed{[[ie4]]}\)
contain no free variables. Therefore,
\begin{align*}
  &\intermed{[[ie1 with R ; (phi1, ix |-> ie3) ; gamma1]]}\\
  &~~~~= \intermed{[[gamma1 ( [| ie3 / ix |] (phi1 (R(ie1))))]]} && \text{(by definition)} \\
&~~~~= \intermed{[[ [| gamma1 (ie3) / ix |] ( ie1 with R ; phi1 ; gamma1 ) ]]} && \text{(distributivity property)}\\
&~~~~= \intermed{[[ [| ie3 / ix |] ( ie1 with R ; phi1 ; gamma1 ) ]]} && \text{(no free variables in \(\intermed{[[ie3]]}\))}
\end{align*}
and similarly, \([[ie2 with R ; (phi2, ix |-> ie4) ; gamma2 = [| ie4 / ix |] (? ie2 with R ; phi2 ; gamma2 ?)]]\). Taking these equalities into account, we can apply the reverse
substitution Lemma~\ref{lemma:rev_var_subst} on
Equations~\ref{eq:compat_let12} and~\ref{eq:compat_let13}, in combination with
Equations~\ref{eq:compat_lete1} and~\ref{eq:compat_lete2}, respectively, to obtain:
\begin{gather}
  \label{eq:compat_let12b}
  [[ SS1 ; TC ; empty, ix : R (is1) |-tm ie1 with R ; phi1 ; gamma1 : R (is2) ~> te2 ]]\\
  \label{eq:compat_let13b}
  [[ SS2 ; TC ; empty, ix : R (is1) |-tm ie2 with R ; phi2 ; gamma2 : R (is2) ~> te2' ]]
\end{gather}
Combining Lemma~\ref{lemma:ctx_well_inter_typing} with
Equation~\ref{eq:compat_let12b}, yields
\([[ |-ctx SS1 ; TC ; empty, ix : R (is1) ]]\) and, by case analysis
on this environment well-formedness judgment, it follows that
\([[ TC ; empty |-ty R (is1) ~> tt1 ]]\).
Using this, Goals~\ref{eq:compat_let4} and \ref{eq:compat_let5} follow by
applying both Equations~\ref{eq:compat_let9} and \ref{eq:compat_let12b} and both
Equations~\ref{eq:compat_let10} and \ref{eq:compat_let13b} to \textsc{iTm-let},
respectively.

By case analysis, the first step of both evaluation paths in Equation~\ref{eq:compat_let6}
must be appropriate instantiations of rule \textsc{iEval-let}, according to which,
\begin{equation*}
  [[ SSi |- ilet ix : R (is1) = (iei' with R ; phii ; gammai) iin (iei with R ; phii ; gammai) --> [| iei' with R ; phii ; gammai / ix |] (iei with R ; phii ; gammai) ]]
%  [[ SS2 |- ilet ix : R (is1) = (ie1' with R ; phi2 ; gamma2) iin (ie2' with R ; phi2 ; gamma2) --> [| ie1' with R ; phi2 ; gamma2 / ix |] (ie2' with R ; phi2 ; gamma2) ]]
\end{equation*}
for each \(\intermed{i}\in\{1,2\}\).
This simplifies Goal~\ref{eq:compat_let6} to:
\begin{equation*}%\label{eq:compat_let15}
\begin{aligned}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} :\, &
    [[ SS1 |- [| ie1' with R ; phi1 ; gamma1 / ix |] (ie1 with R ; phi1 ; gamma1) -->> iv1 ]] \\
    \band\,& [[ SS2 |- [| ie2' with R ; phi2 ; gamma2 / ix |] (ie2 with R ; phi2 ; gamma2) -->> iv2 ]] \\
    \band\,& [[ (SS1 : iv1 , SS2 : iv2) in V (is2) with TC ; R ]]
\end{aligned}
\end{equation*}

The goal follows from Equation~\ref{eq:compat_let14}. Because of
Equation~\ref{eq:compat_let7}, we can choose
\([[ ie3 = ie1' with R ; phi1 ; gamma1 ]]\)
and \([[ ie4 = ie2' with R ; phi2 ; gamma2 ]]\). \\
\qed

\begin{lemmaB}[Compatibility - Method]\ \\
  \begin{mathpar}
    \ottaltinferrule{}{}
    {
      [[ TC ; TT |- SS1 : id1 =log SS2 : id2 : iTC is ]]
      \\ [[ ( im : iTC c : is' ) in TC ]]
      \\ [[ TC |- SS1 =log SS2 ]]
    }
    { [[ TC ; TT |- SS1 : id1 . im =log SS2 : id2 . im : [| is / c |] is' ]] }
    \label{lemma:compat_method}
  \end{mathpar}
\end{lemmaB}

\proof
By inlining the definition of logical equivalence, suppose we have:
\begin{equation}\label{eq:compat_method1}
\begin{gathered}
  [[ R in F ( TT ) with TC ]]\\
  [[ phi in G ( TT ) with SS1 ; SS2 ; TC ; R ]]\\
  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]]
\end{gathered}
\end{equation}
The goal to be proven is the following:
\begin{equation*}
  [[ (SS1 : id1 . im with R ; phi1 ; gamma1 , SS2 : id2 . im with R ; phi2 ; gamma2) in E ([| is / c |] is' ) with TC ; R ]]
\end{equation*}
By applying the definition of the \( \mathcal{E} \) relation, it reduces
to:
\begin{gather*}
  [[ SS1 ; TC ; empty |-tm id1 . im with R ; phi1 ; gamma1 : R ([| is / c |] is') ~> te ]]\\
  [[ SS2 ; TC ; empty |-tm id2 . im with R ; phi2 ; gamma2 : R ([| is / c |] is') ~> te' ]]\\
\begin{split}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} :\, &
    [[ SS1 |- id1 . im with R ; phi1 ; gamma1 -->> iv1 ]] \\
    \band\, & [[ SS2 |- id2 . im with R ; phi2 ; gamma2 -->> iv2 ]] \\
    \band\, & [[ (SS1 : iv1 , SS2 : iv2) in V ([| is / c |] is') with TC ; R ]]
\end{split}
\end{gather*}
By applying the substitutions,
and because \([[R ([| is / c |] is') =  [| R (is) / c |] R (is') ]]\),
the goal further reduces to:
\begin{gather}
  \label{eq:compat_method4}
  [[ SS1 ; TC ; empty |-tm (id1 with R ; phi1 ; gamma1) . im : [| R (is) / c |] R (is') ~> te ]]\\
  \label{eq:compat_method5}
  [[ SS2 ; TC ; empty |-tm (id2 with R ; phi2 ; gamma2) . im : [| R (is) / c |] R (is') ~> te' ]]\\
\begin{split}\label{eq:compat_method6}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} :\ &
    [[ SS1 |- (id1 with R ; phi1 ; gamma1) . im -->> iv1 ]] \\
    \band\, & [[ SS2 |- (id2 with R ; phi2 ; gamma2) . im -->> iv2 ]] \\
    \band\, & [[ (SS1 : iv1 , SS2 : iv2) in V ([| is / c |] is') with TC ; R ]]
\end{split}
\end{gather}
By inlining the definition of logical equivalence in the first hypothesis of this lemma
and choosing \([[R]]\), \([[phi]]\) and \([[gamma]]\) from Equation~\ref{eq:compat_method1}, we
get:
\begin{equation*}
  [[ (SS1 : id1 with R ; phi1 ; gamma1 , SS2 : id2 with R ; phi2 ; gamma2) in V (iTC is) with TC ; R ]]
  \label{eq:compat_method7}
\end{equation*}
Then, from the definition of \(\mathcal{V}\), we get:
\begin{gather}
  \nonumber
  [[ id1 with R ; phi1 ; gamma1 = iD islj idvl1i ]]\\
  \nonumber
  [[ id2 with R ; phi2 ; gamma2 = iD islj idvl2i ]]\\
  \label{eq:compat_method8}
  [[ (iD : \/ clj . iqli => iTC isq) . im |-> ie1' in SS1 ]]\\
 % \textit{where}~[[iTC is = [| islj / clj |] iq' ]]\\
  \label{eq:compat_method9}
  [[ SS1 ; TC ; empty |-d iD islj idvl1i : iTC R (is) ~> te1 ]]\\
  \label{eq:compat_method10}
  [[ SS2 ; TC ; empty |-d iD islj idvl2i : iTC R (is) ~> te2 ]]\\
  \label{eq:compat_method11}
  [[ </ (SS1 : idv1i , SS2 : idv2i) in V ([| islj / clj |] iqi) with TC ; R // i /> ]]
\end{gather}
for some \(\intermed{[[ islj ]]}\), \(\intermed{[[ idvl1i ]]}\), \(\intermed{[[ idvl2i ]]}\), \(\intermed{[[iqli]]}\),
\(\intermed{[[ie']]}\) and \(\intermed{[[isq]]}\) such that \(\intermed{[[is =  [| islj / clj |] isq ]]}\).

Lemma~\ref{lemma:ctx_well_dict_typing}, applied on
Equations~\ref{eq:compat_method9} and~\ref{eq:compat_method10}, yields:
\begin{gather}
  [[ |-ctx SS1 ; TC ; empty ]]
  \label{eq:compat_method9b} \\
  [[ |-ctx SS2 ; TC ; empty ]]
  \label{eq:compat_method10b} 
\end{gather}
Also, from the second premise of this lemma's rule, there are
\(\intermed{[[TC1]]}\) and \(\intermed{[[TC2]]}\) such that
\([[TC = TC1 , im : iTC c : is' , TC2]]\). Then, from
Lemma~\ref{lemma:classmethodwty}, we get \([[TC1 ; empty , c |-ty is' ~> tt']]\),
which means that the only free variable appearing in \(\intermed{[[is']]}\) is the
fresh variable \([[c]]\). Then,
\begin{equation}\label{eq:compat_method2}
  [[R ( is') =  is' ]]
\end{equation}
Also, since the dictionary \(\intermed{[[iD islj idvl1i]]}\) is closed
(it is the result of applying the closing substitutions \([[R]]\),
\(\intermed{[[phi1]]}\) and \(\intermed{[[gamma1]]}\) on dictionary \(\intermed{[[id1]]}\)),
types \(\intermed{[[islj]]}\) can not contain any free variables. Hence,
\([[R (islj) = islj]]\).
In addition, from the last conclusion of Lemma~\ref{lemma:inSS2C},
supplied with \([[ |-ctx SS1 ; TC ; empty ]]\) and Equation~\ref{eq:compat_method8},
we have that \([[TC ; empty , clj |-ty isq ~> tt]]\).
Because the type variables
\(\intermed{[[clj]]}\) are not in \([[TT]]\), they are not in the domain of \([[R]]\), thus \([[R (isq) = isq]]\).
Then,
\begin{equation}\label{eq:compat_method2'}
\begin{aligned}
  \intermed{[[R (is)]]} & = \intermed{[[R ([| islj / clj |] isq)]]}\\
  & = \intermed{[[ [| R (islj) / clj |] R (isq) ]]}\\
  & = [[ [| islj / clj |] isq  = is]]
\end{aligned}
\end{equation}
Equations~\ref{eq:compat_method9} and \ref{eq:compat_method10} can only stand
as conclusions of dictionary typing rule \textsc{D-con}. After rewriting them with
Equation~\ref{eq:compat_method2'} we can invert them and get their premises. 
Also because environment \(\intermed{[[SS1]]}\) can only contain a unique entry
for each dictionary type (in this case, the one shown in Equation~\ref{eq:compat_method8}),
we finally conclude
\begin{gather}
  \label{eq:compat_method12}
  [[ </ TC ; empty |-ty isj ~> ttj // j /> ]]\\
  \label{eq:compat_method13}
  [[ </ SS1 ; TC ; empty |-d idv1i : [| islj / clj |] iqi ~> te1i // i /> ]]\\
  \label{eq:compat_method14}
  [[ </ SS2 ; TC ; empty |-d idv2i : [| islj / clj |] iqi ~> te2i // i /> ]]\\
  \label{eq:compat_method15}
  [[ SS1' ; TC ; empty , clj , idvarli : iqli |-tm ie1 :  [| isq / c |] is' ~> te3 ]]\\
  \label{eq:compat_method15b}
  [[ SS2' ; TC ; empty , clj , idvarli : iqli |-tm ie2 :  [| isq / c |] is' ~> te4 ]]\\
  \label{eq:compat_method3c}
  \textit{where}~[[ SS1 = SS1' , (iD : \/ clj . iqli => iTC isq) . im |-> ie1', SS1'' ]]\\
  \label{eq:compat_method3}
  \textit{and}~[[ie1' = /\ clj . \ idvarli : iqli . ie1]] \\
  \label{eq:compat_method3d}
  \textit{and}~[[ SS2 = SS2' , (iD : \/ clj . iqli => iTC isq) . im |-> ie2', SS2'' ]]\\
  \label{eq:compat_method3b}
  \textit{and}~[[ie2' = /\ clj . \ idvarli : iqli . ie2]]
\end{gather}
With Equations~\ref{eq:compat_method2} and \ref{eq:compat_method2'},
Goals~\ref{eq:compat_method4} and \ref{eq:compat_method5} follow by using the
second premise of the theorem's rule and Equations~\ref{eq:compat_method9} and
\ref{eq:compat_method10}, respectively, in \textsc{iTm-method}.

Using Equations~\ref{eq:compat_method3c} and~\ref{eq:compat_method3d} in
\textsc{iEval-method}, results in:
\begin{gather*}
  [[ SS1 |- (iD islj idvl1i) . im --> ie1' islj idvl1i ]]\\
  [[ SS2 |- (iD islj idvl2i) . im --> ie2' islj idvl2i ]]
\end{gather*}
This reduces Goal~\ref{eq:compat_method6} to:
\begin{equation}
\begin{aligned}\label{eq:compat_method16}
  \exists \intermed{[[iv1]]}, \intermed{[[iv2]]} :\, &
    [[ SS1 |- ie1' islj idvl1i -->> iv1 ]]\\
    \band\, & [[ SS2 |- ie2' islj idvl2i -->> iv2 ]] \\
    \band\, & [[ (SS1 : iv1 , SS2 : iv2) in V ([| is / c |] is') with TC ; R ]]
\end{aligned}
\end{equation}
From the definition of logical equivalence in the theorem's third hypothesis,
together with Equations~\ref{eq:compat_method3c} and~\ref{eq:compat_method3d},
we get that:
\begin{equation}
  [[ TC ; empty |- SS1' : ie1' =log SS2' : ie2' : \/ clj . [| isq / c |] is' ]]
  \label{eq:compat_method17}
\end{equation}
% where we have also used Equation~\ref{eq:compat_method3}.
Repeatedly applying compatibility
Lemma~\ref{lemma:compat_tyapp} to Equations~\ref{eq:compat_method17} and
\ref{eq:compat_method12}, results in:
\begin{equation}
  [[ TC ; empty |- SS1' : ie1' islj =log SS2' : ie2' islj : [| islj / clj |] iqli -> [| islj / clj |] [| isq / c |] is' ]]
  \label{eq:compat_method18}
\end{equation}
By applying weakening Lemma~\ref{lemma:log_weakening} on this result, in combination with
Equations~\ref{eq:compat_method9b} and~\ref{eq:compat_method10b}, we get:
\begin{equation}
  [[ TC ; empty |- SS1 : ie1' islj =log SS2 : ie2' islj : [| islj / clj |] iqli -> [| islj / clj |] [| isq / c |] is' ]]
  \label{eq:compat_method18b}
\end{equation}
From the definition of logical equivalence and
Equation~\ref{eq:compat_method11},
we can derive that:
\begin{equation*}
  [[ </ TC ; empty |- SS1 : idv1i =log SS2 : idv2i : [| islj / clj |] iqi // i /> ]]
  %\label{eq:compat_method20}
\end{equation*}
Repeatedly applying compatibility Lemma~\ref{lemma:compat_dapp} on
Equations~\ref{eq:compat_method18b}, together with
the above equation,
results in:
\begin{equation*}
  %\label{eq:compat_method21}
  [[ TC ; empty |- SS1 : ie1' islj idvl1i =log SS2 : ie2' islj idvl2i : [| islj / clj |] [| isq / c |] is' ]]
\end{equation*}
%% and by weakening Lemma~\ref{lemma:log_weakening}, we have
%% \begin{equation}
%%   [[ TC ; TT |- SS1 : ie' islj idvl1i =log SS2 : ie islj idvl2i : [| islj / clj |] [| isq / c |] is' ]]
%%   \label{eq:compat_method21}
%% \end{equation}
%% However,
Since expressions \(\intermed{[[ie1' islj idvl1i]]}\) and \(\intermed{[[ie2' islj idvl2i]]}\) are closed, by the definition of the logical relation, applying
any substitutions
\([[R in F (empty) with TC]]\), \([[phi in G (empty) with SS1; SS2; TC; R]]\)
and \([[gamma in H (empty) with SS1; SS2; TC; R]]\) on both expressions should result in two terms that are related by the \(\mathcal{E}\) relation. By case analysis on \([[R]]\), \([[phi]]\) and \([[gamma]]\), only the empty substitutions are valid choices, returning exactly the same
expressions. Taking this into account, we have:
\begin{equation*}
  [[ ( SS1 : ie1' islj idvl1i , SS2 : ie2' islj idvl2i) in E ([| islj / clj |] [| isq / c |] is') with TC ; R ]]
%  \label{eq:compat_method22}
\end{equation*}
In turn, unfolding the definition of the \(\mathcal{E}\) relation
results in:
\begin{equation}\label{eq:compat_method23}
\begin{aligned}
  \exists \intermed{[[iv3]]}, \intermed{[[iv4]]} :\, &
    [[ SS1 |- ie1' islj idvl1i -->> iv3 ]] \\
    \band\, & [[ SS2 |- ie2' islj idvl2i -->> iv4 ]]\\
    \band\, & [[ (SS1 : iv3 , SS2 : iv4) in V ([| islj / clj |] [| is / c |] is') with TC ; R ]]
\end{aligned}
\end{equation}
%The type \([[is']]\) originates from the static \([[TC]]\) environment,
%meaning it can only have been constructed in the \textsc{sCls-cls} rule.
%This rule tells us that:
%\begin{equation}
%  [[ TC' ; empty, c |-ty is' ~> tt' ]]
%  \label{eq:compat_method24}
%\end{equation}
%Meaning that \([[c]]\) is the only free type variable contained in \([[is']]\).
%Furthermore, Equation~\ref{eq:compat_method8}, in combination with
%Equation~\ref{eq:compat_method12}, tells us that the type variables \(\intermed{[[clj]]}\)
%are not free in \([[is]]\).
%Combining these results implies that:
%\begin{equation*}
%  [[ [| islj / clj |] [| is / c |] is' = [| is / c |] is' ]]
%\end{equation*}
%Finally, Equations~\ref{eq:compat_method12}, \ref{eq:compat_method13},
%\ref{eq:compat_method14} and \ref{eq:compat_method15}, tell us that neither
%\([[ie]]\), \([[islj]]\), \([[idvl1i]]\) nor \([[idvl2i]]\) contain any free
%type variables. This means that:
%\begin{equation*}
%  [[ R (ie islj idvl1i) = ie islj idvl1i ]]
%\end{equation*}
%\begin{equation*}
%  [[ R (ie islj idvl2i) = ie islj idvl2i ]]
%\end{equation*}
Goal~\ref{eq:compat_method16} follows from Equation~\ref{eq:compat_method23} by
noting that \([[ [| islj / clj |] [| is / c |] is'  =  [| [| islj / clj |] is / c |] [| islj / clj |] is'  =  [| [| islj / clj |] is / c |] is' ]] \) and
taking \([[ iv3 = iv1 ]]\) and \([[ iv4 = iv2 ]]\). \\
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Helper Theorems
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Helper Theorems}

\renewcommand\itot[1]{}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Congruence - Expressions]\ \\
  If \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\) \\
  and \( [[iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; TT' ==> is') ~> tM1]]\)
  and \( [[iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; TT' ==> is') ~> tM2]]\) \\
  and \([[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; TT' ==> is')
  ]]\) \\
  then \([[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]\).
  \label{thmA:congruence_expr}
\end{theoremB}

\proof
The goal follows directly from the definition of logical equivalence for
contexts. \\
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\renewcommand\itot[1]{#1}

\begin{theoremB}[\targetL{} Context Preserved by Elaboration]\ \\
  If \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\)
  and \([[ iM : (SS ; TC ; TT ==> is) |--> (SS ; TC ; TT' ==> is') ~> tM ]]\)
  then \([[ SS ; TC ; TT' |-tm iM (ie) : is' ~> tM (te) ]]\).
  \label{thmA:tgt_ctx_compat}
\end{theoremB}
\proof By structural induction on the typing derivation of \([[iM]]\).\\
\proofStep{\textsc{iM-empty}}
{
  [[ [empty] : (SS ; TC ; TT ==> is) |--> (SS ; TC ; TT ==> is) ~> [empty] ]]
}
{
  We need to show that:
  \begin{equation*}
    [[ SS ; TC ; TT |-tm ie : is ~> te ]]
  \end{equation*}
  which follows immediately from the first hypothesis of the theorem. \\
}
\proofStep{\textsc{iM-abs}}
{
  [[ \ ix : is1 . iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is1 ->
  is' ) ~> \ tx : tt1 . tM' ]]
}
{
  We need to show the following.
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm \ ix : is1 . iM' (ie) : is1 -> is' ~> \ tx : tt1 . tM' (te) ]]
  \end{equation*}
  From the premises of rule \textsc{iM-abs}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT', ix : is1 ==> is' ) ~> tM' ]]
    \label{eq:tctx_abs1} \\
    [[ TC ; TT' |-ty is1 ~> tt1 ]]
    \label{eq:tctx_abs2}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_abs1}, it follows that:
  \begin{equation}
    [[ SS ; TC ; TT', ix : is1 |-tm iM' (ie) : is' ~> tM' (te) ]]
    \label{eq:tctx_abs3}
  \end{equation}
  The goal follows from \textsc{iTm-arrI}, in combination with
  Equations~\ref{eq:tctx_abs2} and \ref{eq:tctx_abs3}. \\
}
\proofStep{\textsc{iM-appL}}
{
  [[ iM' ie2 : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM' te2 ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm iM' (ie) ie2 : is' ~> tM' (te) te2 ]]
  \end{equation*}
  From the premises of rule \textsc{iM-appL}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is1 -> is' ) ~> tM' ]]
    \label{eq:tctx_appL1} \\
    [[ SS ; TC ; TT' |-tm ie2 : is1 ~> te2 ]]
    \label{eq:tctx_appL2}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_appL1}, it follows
  that:
  \begin{equation}
    [[ SS ; TC ; TT' |-tm iM' (ie) : is1 -> is' ~> tM' (te) ]]
    \label{eq:tctx_appL3}
  \end{equation}
  The goal follows from \textsc{iTm-arrE}, in combination with
  Equations~\ref{eq:tctx_appL2} and \ref{eq:tctx_appL3}. \\
}
\proofStep{\textsc{iM-appR}}
{
  [[ ie1 iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> te1 tM' ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm ie1 iM' (ie) : is' ~> te1 tM' (te) ]]
  \end{equation*}
  From the premises of rule \textsc{iM-appR}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is1 ) ~> tM' ]]
    \label{eq:tctx_appR1} \\
    [[ SS ; TC ; TT' |-tm ie1 : is1 -> is' ~> te1 ]]
    \label{eq:tctx_appR2}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_appR1}, it follows
  that:
  \begin{equation}
    [[ SS ; TC ; TT' |-tm iM' (ie) : is1 ~> tM' (te) ]]
    \label{eq:tctx_appR3}
  \end{equation}
  The goal follows from \textsc{iTm-arrE}, in combination with
  Equations~\ref{eq:tctx_appR2} and \ref{eq:tctx_appR3}. \\
}
\proofStep{\textsc{iM-dictAbs}}
{
  [[ \ idvar : iq . iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> iq ->
  is' ) ~> \ txd : tt . tM' ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm \ idvar : iq . iM' (ie) : iq -> is' ~> \ txd : tt . tM' (te) ]]
  \end{equation*}
  %  From the rule premise:
  From the premises of rule \textsc{iM-dictAbs}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT', idvar : iq ==> is') ~> tM' ]]
    \label{eq:tctx_dabs1} \\
    [[ TC ; TT' |-q iq ~> tt ]]
    \label{eq:tctx_dabs2}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_dabs1}, it follows
  that:
  \begin{equation}
    [[ SS ; TC ; TT', idvar : iq |-tm iM' (ie) : is' ~> tM' (te) ]]
    \label{eq:tctx_dabs3}
  \end{equation}
  The goal follows from \textsc{iTm-constrI}, in combination with
  Equations~\ref{eq:tctx_dabs2} and \ref{eq:tctx_dabs3}. \\
}
\proofStep{\textsc{iM-dictApp}}
{
  [[ iM' id : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM' te ]]
}
{
    The goal to be proven is the following.
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm iM' (ie) id : is' ~> tM' (te) te' ]]
  \end{equation*}
  From the premises of rule \textsc{iM-dictApp}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> iq -> is' ) ~> tM' ]]
    \label{eq:tctx_dapp1} \\
    [[ SS ; TC ; TT' |-d id : iq ~> te' ]]
    \label{eq:tctx_dapp2}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_dapp1}, it follows
  that:
  \begin{equation}
    [[ SS ; TC ; TT' |-tm iM' (ie) : iq -> is' ~> tM' (te) ]]
    \label{eq:tctx_dapp3}
  \end{equation}
  The goal follows from \textsc{iTm-constrE}, in combination with
  Equations~\ref{eq:tctx_dapp2} and \ref{eq:tctx_dapp3}. \\
}
\proofStep{\textsc{iM-tyAbs}}
{
  [[ /\ c . iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> \/ c . is' ) ~>
  /\ ta . tM' ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm /\ c . iM' (ie) : \/ c . is' ~> /\ ta . tM' (te) ]]
  \end{equation*}
  From the premises of rule \textsc{iM-tyAbs}, we obtain:
  \begin{gather*}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT', c ==> is' ) ~> tM' ]]
    \label{eq:tctx_tabs1}
  \end{gather*}
  Applying the induction hypothesis on the above context typing, yields:
  \begin{equation*}
    [[ SS ; TC ; TT', c |-tm iM' (ie) : is' ~> tM' (te) ]]
    \label{eq:tctx_tabs2}
  \end{equation*}
  Using this result with rule \textsc{iTm-forallI}, we reach the goal.\\
%  Equation~\ref{eq:tctx_tabs2}. \\
}
\proofStep{\textsc{iM-tyApp}}
{
  [[ iM' is'' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> [| is'' / c |]
  is' ) ~> tM' tt'' ]]
}
{
  The goal to be proven is the following.
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm iM' (ie) is'' : [| is'' / c |] is' ~> tM' (te) tt'' ]]
  \end{equation*}
  From the premises of rule \textsc{iM-tyApp}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> \/ c. is' ) ~> tM' ]]
    \label{eq:tctx_tapp1} \\
    [[ TC ; TT' |-ty is'' ~> tt'' ]]
    \label{eq:tctx_tapp2}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_tapp1}, we have
  that:
  \begin{equation}
    [[ SS ; TC ; TT' |-tm iM' (ie) : \/ c . is' ~> tM' (te) ]]
    \label{eq:tctx_tapp3}
  \end{equation}
  The goal follows from \textsc{iTm-forallE}, in combination with
  Equations~\ref{eq:tctx_tapp2} and \ref{eq:tctx_tapp3}. \\
}
\proofStep{\textsc{iM-letL}}
{
  [[ ilet ix : is1 = iM' iin ie2 : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT'
  ==> is') ~> tlet tx : tt1 = tM' tin te2 ]]
}
{
    The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm ilet ix : is1 = iM' (ie) iin ie2 : is' ~> tlet tx : tt1 = tM' (te) tin te2 ]]
  \end{equation*}
  From the premises of rule \textsc{iM-letL}, we obtain:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is1 ) ~> tM' ]]
    \label{eq:tctx_letL1} \\
    [[ SS ; TC ; TT', ix : is1 |-tm ie2 : is' ~> te2 ]]
    \label{eq:tctx_letL2} \\
    [[ TC ; TT' |-ty is1 ~> tt1 ]]
    \label{eq:tctx_letL3}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_letL1}, we have
  that:
  \begin{equation}
    [[ SS ; TC ; TT' |-tm iM' (ie) : is1 ~> tM' (te) ]]
    \label{eq:tctx_letL4}
  \end{equation}
  The goal follows from \textsc{iTm-let}, in combination with
  Equations~\ref{eq:tctx_letL2}, \ref{eq:tctx_letL3} and \ref{eq:tctx_letL4}. \\
}
\proofStep{\textsc{iM-letR}}
{
  [[ ilet ix : is1 = ie1 iin iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT'
  ==> is') ~> tlet tx : tt1 = te1 tin tM' ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ SS ; TC ; TT' |-tm ilet ix : is1 = ie1 iin iM' (ie) : is' ~> tlet tx : tt1 = te1 tin tM' (te) ]]
  \end{equation*}
  From the rule premise:
  \begin{gather}
    [[ iM' : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT', ix : is1 ==> is' ) ~> tM' ]]
    \label{eq:tctx_letR1} \\
    [[ SS ; TC ; TT' |-tm ie1 : is1 ~> te1 ]]
    \label{eq:tctx_letR2} \\
    [[ TC ; TT' |-ty is1 ~> tt1 ]]
    \label{eq:tctx_letR3}
  \end{gather}
  From the induction hypothesis applied on Equation~\ref{eq:tctx_letR1}, we have
  that:
  \begin{equation}
    [[ SS ; TC ; TT', ix : is1 |-tm iM' (ie) : is' ~> tM' (te) ]]
    \label{eq:tctx_letR4}
  \end{equation}
  The goal follows from \textsc{iTm-let}, in combination with
  Equations~\ref{eq:tctx_letR2}, \ref{eq:tctx_letR3} and \ref{eq:tctx_letR4}.
}
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\renewcommand\itot[1]{}
\begin{theoremB}[Logical Equivalence Preserved by Forward/Backward Reduction]\ \\
  Given \([[ SS1 |- ie1 --> ie1' ]]\) and \([[ SS2 |- ie2 --> ie2' ]]\),
  \begin{itemize}
    \item If \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\), then \([[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]\).
    \item If \([[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]\)
      and \([[ SS1 ; TC ; TT |-tm ie1 : is ~> te1 ]]\)
      and \([[ SS2 ; TC ; TT |-tm ie2 : is ~> te2 ]]\), \\
      then \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\).
  \end{itemize}
  \label{thmA:log_eq_pres}
\end{theoremB}

\proof

\begin{description}
  \item[Part 1]
    By unfolding the definition of logical relation, we get:
    \begin{gather}
    [[R in F ( TT ) with TC]] \\
    [[phi in G ( TT ) with SS1 ; SS2 ; TC ; R]] \\
    [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]] \\
    \label{eq:logical:forward:1}
    [[ (SS1 : ie1 with R ; phi1 ; gamma1, SS2 : ie2 with R ; phi2 ; gamma2) in E (is) with TC ; R]]
    \end{gather}
    Unfolding the definition of the closed expression relation in
    \ref{eq:logical:forward:1} results in:
    \begin{gather}
      [[ SS1 ; TC ; empty |-tm  ie1 with R ; phi1 ; gamma1 : R (is) ~> te1 ]] \\
      [[ SS2 ; TC ; empty |-tm  ie2 with R ; phi2 ; gamma2: R (is) ~> te2 ]] \\
      \exists [[iv1]], [[iv2]], 
        [[SS1 |- ie1 with R ; phi1 ; gamma1 -->> iv1]],\\
        [[SS2 |- ie2 with R ; phi2 ; gamma2-->> iv2]],\\
        [[ (SS1 : iv1, SS2 : iv2) in V (is) with TC ; R]]
    \end{gather}
    By induction on $[[ie1]]$, it is easy to verify that
    \begin{gather}
        [[SS1 |- ie1 with R ; phi1 ; gamma1 --> ie1' with R ; phi1; gamma1]]
    \end{gather}
    By preservation (Theorem~\ref{thmA:intermediate_preservation}) we have:
    \begin{gather}
      [[ SS1 ; TC ; empty |-tm  ie1' with R ; phi1 ; gamma1 : R (is) ~> te3 ]] 
    \end{gather}
    Because the evaluation in \interL{} is deterministic (Lemma~\ref{lemma:eval_unique}), we know that:
    \begin{gather}
        [[SS1 |- ie1' with R ; phi1 ; gamma1 -->> iv1]]
    \end{gather}
    Similarly:
    \begin{gather}
      [[ SS2 ; TC ; empty |-tm  ie2' with R ; phi2 ; gamma2 : R (is) ~> te4 ]] \\
      [[SS2 |- ie2' with R ; phi2 ; gamma2 -->> iv2]]
    \end{gather}
    Combining those equations, results in:
    \begin{gather}
    [[ (SS1 : ie1' with R ; phi1 ; gamma1, SS2 : ie2' with R ; phi2 ; gamma2) in E (is) with TC ; R]]
    \end{gather}
    The goal follows from the definition of logical equivalence.
  \item[Part 2]
    Similar to Part 1.
\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Dictionary Reflexivity]\ \\
  If \([[ SS1 ; TC ; TT |-d id : iq ~> te ]]\)
  and \([[ SS2 ; TC ; TT |-d id : iq ~> te ]]\)
  and \([[ TC |- SS1 =log SS2 ]]\),
  then \([[ TC ; TT |- SS1 : id =log SS2 : id : iq ]]\).
  \label{thmA:dict_reflex}
\end{theoremB}

\proof
Proof by structural induction on the dictionary \([[id]]\) and consequently,
since \interL{} dictionary typing is syntax directed, on both typing derivations. \\
\proofStep{\([[ id = idvar ]]\) (\textsc{D-var})}
{
  [[ SS1 ; TC ; TT |-d idvar : iq ~> txd ]] \band
  [[ SS2 ; TC ; TT |-d idvar : iq ~> txd ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : idvar =log SS2 : idvar : iq ]]
    \label{eq:drefl_var1}
  \end{equation*}
  By unfolding the definition of logical equivalence, the goal reduces to:
  \begin{equation*}
    [[ ( SS1 : idvar with R ; phi1 ; gamma1 , SS2 : idvar with R ; phi2 ; gamma2 ) in V (iq) with TC ; R ]]
%    \label{eq:drefl_var2}
  \end{equation*}
  where \([[ R in F (TT) with TC ]]\), \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\)
  and \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\).

  From the given we know that \([[ (idvar : iq) in TT ]]\).
  Because of this, it follows from the definition of \(\mathcal{H}\) that:
  \begin{gather*}
    [[ idvar with R ; phi1 ; gamma1 = idv1 ]] \\
    [[ idvar with R ; phi2 ; gamma2 = idv2 ]] \\
    [[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R ]]
  \end{gather*}
}
\proofStep{\([[ id = iD islj idli ]]\) (\textsc{D-con})}
{
  [[ SS1 ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> te ]] \band
  [[ SS2 ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> te ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : iD islj idli =log SS2 : iD islj idli : iTC [| islj / clj |] isq ]]
%    \label{eq:drefl_con1}
  \end{equation*}
  Unfolding the definition of logical equivalence in the goal results in:
  \begin{equation*}
    [[ ( SS1 : iD islj idli with R ; phi1 ; gamma1 , SS2 : iD islj idli with R ; phi2 ; gamma2 ) in V ( iTC [| islj / clj |] isq) with TC ; R ]]
%    \label{eq:drefl_con2}
  \end{equation*}
  where \([[ R in F (TT) with TC ]]\), \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\)
  and \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\).
  
  By the definition of the \(\mathcal{V}\) relation and by distributivity of substitution
  over application, it suffices to show that:
  \begin{gather}
%    [[ (iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli . ie1 in SS1 ]]
    [[ (iD : \/ clj . iqli => iTC isq) . im |-> ie in SS1 ]]
    \label{eq:drefl_con10} \\
    [[ </ (SS1 : idi with R ; phi1 ; gamma1 , SS2 : idi with R ; phi2 ; gamma2) in V ([| islj / clj|] iqi) with TC ; R // i /> ]]
    \label{eq:drefl_con11} \\
    [[ SS1 ; TC ; empty |-d iD islj idli with R ; phi1 ; gamma1 : R (iTC [| islj / clj |] isq) ~> te1 ]]
    \label{eq:drefl_con12} \\
    [[ SS2 ; TC ; empty |-d iD islj idli with R ; phi2 ; gamma2 : R (iTC [| islj / clj |] isq) ~> te2 ]]
    \label{eq:drefl_con13}
  \end{gather}
  From the premises of the two \textsc{D-con} rules, we know that:
  \begin{gather}
%    [[ (iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli . ie1 in SS1 ]]
%    \label{eq:drefl_con3a} \\
%    [[ (iD : \/ clj . iqli' => iTC' isq') . im' |-> /\ clj . \ idvarli : iqli' . ie2 in SS2 ]]
%    \label{eq:drefl_con3ab} \\
    [[ |-ctx SS1 ; TC ; TT ]]
    \label{eq:drefl_con3b} \\
    [[ |-ctx SS2 ; TC ; TT ]]
    \label{eq:drefl_con3bb} \\
    [[ </ TC ; empty, clj |-q iqi ~> tti // i /> ]]
    \label{eq:drefl_con3c} \\
    [[ </ TC ; empty, clj |-q iqi' ~> tti // i /> ]]
    \label{eq:drefl_con3c'} \\
    [[ </ TC ; TT |-ty isj ~> ttj // j /> ]]
    \label{eq:drefl_con3d} \\
    [[ </ SS1 ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei // i /> ]]
    \label{eq:drefl_con3e} \\
    [[ </ SS2 ; TC ; TT |-d idi : [| islj / clj |] iqi' ~> tei // i /> ]]
    \label{eq:drefl_con3eb} \\
    [[ SS1' ; TC ; empty, clj, idvarli : iqli |-tm ie1 : [| islj / clj |] ism ~> te ]]
    \label{eq:drefl_con3f} \\
    [[ SS2' ; TC ; empty, clj, idvarli : iqli' |-tm ie2 : [| islj / clj |] ism ~> te ]]
    \label{eq:drefl_con3fb} \\
    \textit{where}~[[ SS1 = SS1', (iD : \/ clj . iqli => iTC isq) . im |-> /\ clj
    . \ idvarli : iqli . ie1, SS1'' ]]
    \label{eq:drefl_con3a} \\
    \textit{and}~\,[[ SS2 = SS2', (iD : \/ clj . iqli' => iTC' isq') . im' |-> /\ clj
    . \ idvarli : iqli' . ie2, SS2'' ]]
    \label{eq:drefl_con3ab}
  \end{gather}
  From the definition of logical equivalence in the third hypothesis of
  the theorem, we know that \([[ iqli = iqli' ]]\),
  \([[ iTC = iTC' ]]\), \([[ isq = isq' ]]\), \([[ im = im' ]]\).

  Goal~\ref{eq:drefl_con10} follows directly from Equation~\ref{eq:drefl_con3a} by
  setting \([[ie = /\ clj . \ idvarli : iqli' . ie2 ]]\).

  By applying the induction hypothesis on Equations~\ref{eq:drefl_con3e}
  and~\ref{eq:drefl_con3eb}, we obtain:
  \begin{equation*}
    [[ </ TC ; TT |- SS1 : idi =log SS2 : idi : [| islj / clj |] iqi // i /> ]]
%    \label{eq:drefl_cone1}
  \end{equation*}
  Unfolding the definition of logical equivalence in the above, we get:
  \begin{equation}
    [[ </ (SS1 : idvi1 , SS2 : idvi2) in V ([| islj / clj |] iqi) with TC ; R // i /> ]]
    \label{eq:drefl_cone2}
  \end{equation}
  where \([[ idvi1 = idi with R ; phi1 ; gamma1 ]]\) and
  \([[ idvi2 = idi with R ; phi2 ; gamma2 ]]\).
  This proves Goal~\ref{eq:drefl_con11}.

  By applying Lemma~\ref{lemma:tvar_tsubst} in Equation~\ref{eq:drefl_con3d},
  there is an environment \([[TT']]\) (the resulting environment
  after applying on \([[TT]]\) all type variable substitutions of \([[R]]\)) such that
  \begin{equation*}
    [[ </ TC ; TT' |-ty R (isj) ~> ttj // j /> ]]
  \end{equation*}
  From Lemma~\ref{lemma:tvar_tsubst} and since the domain of \([[R]]\) contains all type
  variables of \([[TT]]\), it is evident that all type variables are eliminated in
  \([[TT']]\). By consecutive applications of Lemma~\ref{lemma:var_subst_types} we have that
  \begin{equation}
    [[ </ TC ; empty |-ty R (isj) ~> ttj // j /> ]]
    \label{eq:drefl_con3d2}
  \end{equation}
  %% \begin{equation}
  %%   [[ </ TC ; TT |-ty R (isj) ~> ttj // j /> ]]
  %%   \label{eq:drefl_con3d2}
  %% \end{equation}
  Furthermore, from the definiton of the \(\mathcal{V}\) relation in
  Equation~\ref{eq:drefl_cone2}, we obtain:
  \begin{gather*}
    [[ </ SS1 ; TC ; empty |-d idvi1 : R ([| islj / clj |] iqi) ~> tei1 // i /> ]]\\
%    \label{eq:drefl_con5} \\
    [[ </ SS2 ; TC ; empty |-d idvi2 : R ([| islj / clj |] iqi) ~> tei2 // i /> ]]
%    \label{eq:drefl_con6}
  \end{gather*}
  From Equation~\ref{eq:drefl_con3c}, we know that \(\intermed{[[iqi]]}\) only contains
  free variables \(\intermed{[[clj]]}\). It follows that the above equations can be simplified to:
  \begin{gather}
    [[ </ SS1 ; TC ; empty |-d idvi1 : [| R (islj) / clj |] iqi ~> tei1 // i /> ]]
    \label{eq:drefl_con5b} \\
    [[ </ SS2 ; TC ; empty |-d idvi2 : [| R (islj) / clj |] iqi ~> tei2 // i /> ]]
    \label{eq:drefl_con6b}
  \end{gather}
  Applying the substitutions in Goals~\ref{eq:drefl_con12} and
  \ref{eq:drefl_con13},
  reduces them to:
  \begin{gather*}
    [[ SS1 ; TC ; empty |-d iD R (islj) idvli1 : iTC R ([| islj / clj |] isq) ~> te1 ]]\\
%    \label{eq:drefl_con14} \\
    [[ SS2 ; TC ; empty |-d iD R (islj) idvli2 : iTC R ([| islj / clj |] isq) ~> te2 ]]
%    \label{eq:drefl_con15}
  \end{gather*}
  Similarly to \(\intermed{[[iqi]]}\), it follows from \textsc{iCtx-MEnv} that
  \(\intermed{[[isq]]}\) only contains free variables \(\intermed{[[clj]]}\). The above goals thus
  simplify to:
  \begin{gather}
    [[ SS1 ; TC ; empty |-d iD R (islj) idvli1 : iTC [| R (islj) / clj |] isq ~> te1 ]]
    \label{eq:drefl_con14b} \\
    [[ SS2 ; TC ; empty |-d iD R (islj) idvli2 : iTC [| R (islj) / clj |] isq ~> te2 ]]
    \label{eq:drefl_con15b}
  \end{gather}
  Goal~\ref{eq:drefl_con14b} follows from \textsc{D-con}, in combination with
  Equations~\ref{eq:drefl_con3a}, \ref{eq:drefl_con3b}, \ref{eq:drefl_con3c},
  \ref{eq:drefl_con3d2}, \ref{eq:drefl_con3f} and \ref{eq:drefl_con5b}.
  Goal~\ref{eq:drefl_con15b} follows from from \textsc{D-con}, in combination with
  Equations~\ref{eq:drefl_con3ab}, \ref{eq:drefl_con3bb}, \ref{eq:drefl_con3c},
  \ref{eq:drefl_con3d2}, \ref{eq:drefl_con3fb} and \ref{eq:drefl_con6b}.
  
  %% These follow from \textsc{D-con}, in combination with
  %% Equation~\ref{eq:drefl_con3a}, \ref{eq:drefl_con3b}, \ref{eq:drefl_con3c},
  %% \ref{eq:drefl_con3d2}, \ref{eq:drefl_con3f}, \ref{eq:drefl_con3fb},
  %% \ref{eq:drefl_con5b} and \ref{eq:drefl_con6b}.
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Expression Reflexivity]\ \\
  If \([[ SS1 ; TC ; TT |-tm ie : is ~> te ]]\)
  and \([[ SS2 ; TC ; TT |-tm ie : is ~> te ]]\)
  and \([[ TC |- SS1 =log SS2 ]]\),
  then \([[ TC ; TT |- SS1 : ie =log SS2 : ie : is ]]\).
  \label{thmA:expr_reflex}
\end{theoremB}

\proof
%Proof by induction on the size of \([[SS1]]\) and \([[ie]]\).
The proof proceeds by induction on \([[ie]]\) and consequently, since \interL{} term typing
is syntax directed, on both typing derivations. \\
\proofStep{\([[ie = itrue]]\) (\textsc{iTm-true})}
{
  [[ SS1 ; TC ; TT |-tm itrue : ibool ~> ttrue ]] \band
  [[ SS2 ; TC ; TT |-tm itrue : ibool ~> ttrue ]]
}
{
  The goal to prove is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : itrue =log SS2 : itrue : ibool ]]
%    \label{eq:erefl_true1}
  \end{equation*}
  Unfolding the definition of logical equivalence in the above, 
  results in the following goal:
  \begin{equation}
    [[ (SS1 : itrue with R ; phi1 ; gamma1 , SS2 : itrue with R ; phi2 ; gamma2) in E (ibool) with TC ; R ]]
    \label{eq:erefl_true2}
  \end{equation}
  where \([[ R in F (TT) with TC ]]\), \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\)
  and \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\). However, since \([[itrue]]\)
  does not contain any free variables, we know that
  \([[ itrue with R ; phi1 ; gamma1 = itrue with R ; phi2 ; gamma2 = itrue
  ]]\). Similarly, it follows that
  \([[ R (ibool) = ibool ]]\).

  Unfolding the definition of the \(\mathcal{E}\) relation in
  Goal~\ref{eq:erefl_true2}, reduces the goal to:
  \begin{gather}
    [[ SS1 ; TC ; empty |-tm itrue : ibool ~> te ]]
    \label{eq:erefl_true3} \\
    [[ SS2 ; TC ; empty |-tm itrue : ibool ~> te ]]
    \label{eq:erefl_true3b} \\
    \begin{aligned}
      \exists [[iv1]], [[iv2]] :\, &
      [[ SS1 |- itrue -->> iv1 ]]  \\
      \band\, & [[ SS2 |- itrue -->> iv2 ]] \\
      \band\, & [[ (SS1 : iv1 , SS2 : iv2) in V (ibool) with TC ; R ]]
    \end{aligned}
    \nonumber %\label{eq:erefl_true4}
  \end{gather}
  Goals~\ref{eq:erefl_true3} and~\ref{eq:erefl_true3b} are satisified from the first and
  second hypotheses of the theorem.
  We set \([[ iv1 = iv2 = itrue ]]\) and since \([[itrue]]\) is a value, the term reductions
  above hold. Then, the last goal follows directly from the definition of the \(\mathcal{V}\)
  relation, according to which the following holds trivially.
  \begin{equation*}
    [[ (SS1 : itrue , SS2 : itrue) in V (ibool) with TC ; R ]]
  \end{equation*}
}
\proofStep{\([[ ie = ifalse ]]\) (\textsc{iTm-false})}
{
  [[ SS1 ; TC ; TT |-tm ifalse : ibool ~> tfalse ]] \band
  [[ SS2 ; TC ; TT |-tm ifalse : ibool ~> tfalse ]]
}
{
  The proof is similar to the \textsc{iTm-true} case. \\
}
\proofStep{\([[ ie = ix ]]\) (\textsc{iTm-var})}
{
  [[ SS1 ; TC ; TT |-tm ix : is ~> tx ]] \band
  [[ SS2 ; TC ; TT |-tm ix : is ~> tx ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : ix =log SS2 : ix : is ]]
%    \label{eq:erefl_var1}
  \end{equation*}
  By unfolding the definition of logical equivalence in the above, we have
  \begin{equation*}
    [[ (SS1 : ix with R ; phi1 ; gamma1 , SS2 : ix with R ; phi2 ; gamma2) in E (is) with TC ; R ]]
%    \label{eq:erefl_var2}
  \end{equation*}
  for any \([[ R in F (TT) with TC ]]\), \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\)
  and \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\). 
  From the definition of the \(\mathcal{G}\) relation, we know that:
  \begin{gather}
    [[ ix with R ; phi1 ; gamma1 = ie1 ]]
    \nonumber \\
    [[ ix with R ; phi2 ; gamma2 = ie2 ]]
    \nonumber \\
    [[ (SS1 : ie1 , SS2 : ie2) in E (is) with TC ; R ]]
    \label{eq:erefl_var3}
  \end{gather}
  The goal follows directly from Equation~\ref{eq:erefl_var3}. \\
}
\proofStep{\([[ ie = ilet ix : is1 = ie1 iin ie2 ]]\) (\textsc{iTm-let})}
{
  [[ SS1 ; TC ; TT |-tm ilet ix : is1 = ie1 iin ie2 : is2 ~> tlet tx : tt1 = te1
  tin te2 ]] \band
  [[ SS2 ; TC ; TT |-tm ilet ix : is1 = ie1 iin ie2 : is2 ~> tlet tx : tt1 = te1
  tin te2 ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : ilet ix : is1 = ie1 iin ie2 =log SS2 : ilet ix : is1 = ie1 iin ie2 : is2 ]]
%    \label{eq:erefl_let1}
  \end{equation*}
  By applying the induction hypothesis in the premises of the two \textsc{iTm-let} rules,
  we get:
  \begin{gather*}
    [[ TC ; TT |- SS1 : ie1 =log SS2 : ie1 : is1 ]]\\
%    \label{eq:erefl_let2} \\
    [[ TC ; TT, ix : is1 |- SS1 : ie2 =log SS2 : ie2 : is2 ]]
%    \label{eq:erefl_let3}
  \end{gather*}
  The goal follows directly by passing the above two Equations %Equations~\ref{eq:erefl_let2} and \ref{eq:erefl_let3}
  to compatibility Lemma~\ref{lemma:compat_let}. \\
}
\proofStep{\([[ ie = id . im ]]\) (\textsc{iTm-method})}
{
  [[ SS1 ; TC ; TT |-tm id . im : [| is / c |] is' ~> te . tl ]] \band
  [[ SS2 ; TC ; TT |-tm id . im : [| is / c |] is' ~> te . tl ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : id . im =log SS2 : id . im : [| is / c |] is' ]]
%    \label{eq:erefl_method1}
  \end{equation*}
  From the premises of rule \textsc{iTm-method} we have that
  \begin{gather}
    [[ SS1 ; TC ; TT |-d id : iTC is ~> te ]]
    \label{eq:erefl_method2} \\
    [[ SS2 ; TC ; TT |-d id : iTC is ~> te ]]
    \label{eq:erefl_method2b} \\
    [[ (im : iTC c : is') in TC ]]
    \label{eq:erefl_method3}
  \end{gather}
  Applying the Dictionary Reflexivity (Theorem~\ref{thmA:dict_reflex}) to
  Equations~\ref{eq:erefl_method2}~and~\ref{eq:erefl_method2b}, in combination
  with the theorem's third hypothesis, results in:
  \begin{equation}
    [[ TC ; TT |- SS1 : id =log SS2 : id : iTC is ]]
    \label{eq:erefl_method4}
  \end{equation}
  The goal follows directly from compatibility Lemma~\ref{lemma:compat_method}
  and Equations~\ref{eq:erefl_method3} and \ref{eq:erefl_method4}, in
  combination with the third hypothesis. \\
}
\proofStep{\([[ ie = \ ix : is1 . ie' ]]\) (\textsc{iTm-arrI})}
{
  [[ SS1 ; TC ; TT |-tm \ ix : is1 . ie' : is1 -> is2 ~> \ tx : tt1 . te ]] \band
  [[ SS2 ; TC ; TT |-tm \ ix : is1 . ie' : is1 -> is2 ~> \ tx : tt1 . te ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : \ ix : is1 . ie' =log SS2 : \ ix : is1 . ie' : is1 -> is2 ]]
%    \label{eq:erefl_arrI1}
  \end{equation*}
  By applying the induction hypothesis to the premises of the two \textsc{iTm-arrI} rules,
  we get:
  \begin{equation*}
    [[ TC ; TT, ix : is1 |- SS1 : ie' =log SS2 : ie' : is2 ]]
%    \label{eq:erefl_arrI2}
  \end{equation*}
  The goal follows by applying the above %Equation~\ref{eq:erefl_arrI2}
  to compatibility Lemma~\ref{lemma:compat_abs}. \\
}
\proofStep{\([[ ie = ie1 ie2 ]]\) (\textsc{iTm-arrE})}
{
  [[ SS1 ; TC ; TT |-tm ie1 ie2 : is2 ~> te1 te2 ]] \band
  [[ SS2 ; TC ; TT |-tm ie1 ie2 : is2 ~> te1 te2 ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : ie1 ie2 =log SS2 : ie1 ie2 : is2 ]]
%    \label{eq:erefl_arrE1}
  \end{equation*}
  By applying the induction hypothesis to the premises of the two \textsc{iTm-arrE} rules,
  we get:
  \begin{gather*}
    [[ TC ; TT |- SS1 : ie1 =log SS2 : ie1 : is1 -> is2 ]]\\
%    \label{eq:erefl_arrE2} \\
    [[ TC ; TT |- SS1 : ie2 =log SS2 : ie2 : is1 ]]
%    \label{eq:erefl_arrE3}
  \end{gather*}
  The goal follows by passing the above two equations to compatibility
  Lemma~\ref{lemma:compat_app}. \\
}
\proofStep{\([[ ie = \ idvar : iq . ie' ]]\) (\textsc{iTm-constrI})}
{
  [[ SS1 ; TC ; TT |-tm \ idvar : iq . ie' : iq -> is ~> \ txd : tt . te ]] \band
  [[ SS2 ; TC ; TT |-tm \ idvar : iq . ie' : iq -> is ~> \ txd : tt . te ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : \ idvar : iq . ie' =log SS2 : \ idvar : iq . ie' : iq -> is ]]
%    \label{eq:erefl_constrI1}
  \end{equation*}
  By applying the induction hypothesis to the premises of the two \textsc{iTm-constrI}
  rules, we get:
  \begin{equation*}
    [[ TC ; TT, idvar : iq |- SS1 : ie' =log SS2 : ie' : is ]]
%    \label{eq:erefl_constrI2}
  \end{equation*}
  The goal follows directly by passing the above equation %~\ref{eq:erefl_constrI2}
  to compatibility Lemma~\ref{lemma:compat_dabs}. \\
}
\proofStep{\([[ ie = ie' id ]]\) (\textsc{iTm-constrE})}
{
  [[ SS1 ; TC ; TT |-tm ie' id : is ~> te1 te2 ]] \band
  [[ SS2 ; TC ; TT |-tm ie' id : is ~> te1 te2 ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : ie' id =log SS2 : ie' id : is ]]
%    \label{eq:erefl_constrE1}
  \end{equation*}
  By applying the induction hypothesis to the premises of the two \textsc{iTm-constrE} rules,
  we get:
  \begin{equation}
    [[ TC ; TT |- SS1 : ie' =log SS2 : ie' : iq -> is ]]
    \label{eq:erefl_constrE2}
  \end{equation}
  Furthermore, applying Dictionary Reflexivity (Theorem~\ref{thmA:dict_reflex}) in the
  premises of the two \textsc{iTm-constrE} rules, in combination with the
  theorem's third
  hypothesis, results in:
  \begin{equation}
    [[ TC ; TT |- SS1 : id =log SS2 : id : iq ]]
    \label{eq:erefl_constrE3}
  \end{equation}
  The goal follows from compatibility Lemma~\ref{lemma:compat_dapp}
  and Equations~\ref{eq:erefl_constrE2} and \ref{eq:erefl_constrE3}. \\
}
\proofStep{\([[ ie = /\ c . ie' ]]\) (\textsc{iTm-forallI})}
{
  [[ SS1 ; TC ; TT |-tm /\ c . ie' : \/ c . is ~> /\ ta . te ]] \band
  [[ SS2 ; TC ; TT |-tm /\ c . ie' : \/ c . is ~> /\ ta . te ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : /\ c . ie' =log SS2 : /\ c . ie' : \/ c . is ]]
%    \label{eq:erefl_forallI1}
  \end{equation*}
  By applying the induction hypothesis to the premises of the two \textsc{iTm-forallI}
  rules, we get:
  \begin{equation*}
    [[ TC ; TT, c |- SS1 : ie' =log SS2 : ie' : is1 ]]
%    \label{eq:erefl_forallI2}
  \end{equation*}
  The goal follows directly by applying the above equation %Equation~\ref{eq:erefl_forallI2}
  to compatibility Lemma~\ref{lemma:compat_tyabs}. \\
}
\proofStep{\([[ ie = ie' is ]]\) (\textsc{iTm-forallE})}
{
  [[ SS1 ; TC ; TT |-tm ie' is : [| is / c |] is' ~> te tt ]] \band
  [[ SS2 ; TC ; TT |-tm ie' is : [| is / c |] is' ~> te tt ]]
}
{
  The goal to be proven is the following:
  \begin{equation*}
    [[ TC ; TT |- SS1 : ie' is =log SS2 : ie' is : [| is / c |] is' ]]
%    \label{eq:erefl_forallE1}
  \end{equation*}
  From the premises of \textsc{iTm-forallE}, we obtain
  \begin{equation}
    [[TC ; TT |-ty is ~> tt]]
    \label{eq:erefl_forallE_wt}
  \end{equation}
  By applying the induction hypothesis to the premises of the two \textsc{iTm-forallE}
  rules, we get:
  \begin{equation}
    [[ TC ; TT |- SS1 : ie'1 =log SS2 : ie'1 : is1 ]]
    \label{eq:erefl_forallE2}
  \end{equation}
  The goal follows from compatibility Lemma~\ref{lemma:compat_tyapp}
  and Equations~\ref{eq:erefl_forallE2} and~\ref{eq:erefl_forallE_wt}.
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Context Reflexivity]\ \\
  Suppose\, \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    and\, \([[ |-ctx P ; GC ; GG' ~> SS1 ; TC ; TT' ]]\) \\
    and\, \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\)
    and\, \([[ |-ctx P ; GC ; GG' ~> SS2 ; TC ; TT' ]]\) \\
    and\, \([[ GC ; GG |-ty st ~> is ]]\)
    and\, \([[ GC ; GG' |-ty st' ~> is' ]]\),
  \begin{itemize}
  \item If \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~>
    iM1 ]]\) \\
    and \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM2
    ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS1 ; TC ; TT' ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS2 ; TC ; TT' ]]\) \\
    %% and \([[ GC ; GG |-ty st ~> is ]]\)
    %% and \([[ GC ; GG' |-ty st' ~> is' ]]\) \\
    then \([[ SS1 : iM1 =log SS2 : iM2 : ( TC ; TT ==> is ) |--> ( TC ; TT' ==>
    is' ) ]]\).
  \item If \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~>
    iM1 ]]\) \\
    and \([[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM2
    ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS1 ; TC ; TT' ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS2 ; TC ; TT' ]]\) \\
    %% and \([[ GC ; GG |-ty st ~> is ]]\)
    %% and \([[ GC ; GG' |-ty st' ~> is' ]]\) \\
    then \([[ SS1 : iM1 =log SS2 : iM2 : ( TC ; TT ==> is ) |--> ( TC ; TT' ==>
    is' ) ]]\).
  \item If \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' ==> st' ) ~~>
    iM1 ]]\) \\
    and \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM2
    ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS1 ; TC ; TT' ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS2 ; TC ; TT' ]]\) \\
    %% and \([[ GC ; GG |-ty st ~> is ]]\)
    %% and \([[ GC ; GG' |-ty st' ~> is' ]]\) \\
    then \([[ SS1 : iM1 =log SS2 : iM2 : ( TC ; TT ==> is ) |--> ( TC ; TT' ==>
    is' ) ]]\).
  \item If \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' <== st' ) ~~>
    iM1 ]]\) \\
    and \([[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM2
    ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS1 ; TC ; TT' ]]\) \\
    %% and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\)
    %% and \([[ |-ctx P ; GC ; GG' ~> SS2 ; TC ; TT' ]]\) \\
    %% and \([[ GC ; GG |-ty st ~> is ]]\)
    %% and \([[ GC ; GG' |-ty st' ~> is' ]]\) \\
    then \([[ SS1 : iM1 =log SS2 : iM2 : ( TC ; TT ==> is ) |--> ( TC ; TT' ==>
    is' ) ]]\).
  \end{itemize}
  \label{thmA:ctx_reflex}
\end{theoremB}

\proof
The theorem is stated in a nested fashion, where all common hypotheses are introduced in the
outer statement. Each of the four inner statements extends the outer statement with two
context-typing hypotheses, and sets the conclusion of the theorem, which is identical for each of
the four cases.

Suppose expressions \(\intermed{[[ ie1 ]]}\) and \(\intermed{[[ ie2 ]]}\) such that
\begin{equation}
  \label{eq:ctx_refl0}
  [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]
\end{equation}
Then, by unfolding the defintion of logical equivalence in the goal of all four
sub-statements, it suffices to show
that
\begin{equation}
  \label{eqg:ctx_refl0}
  [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]
\end{equation}
We assume all hypotheses of the outer statement and we proceed by mutual induction on the
first hypothesis of the nested statements. Note that
context typing derivations are of finite size, thus mutual induction over them is safe.
%% By unfolding the definition of logical equivalence in the goal, the goal reduces
%% to:
%% \begin{gather}
%%   \forall [[ ie1 ]], [[ ie2 ]] : [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]
%%   \label{eq:ctx_refl0} \\
%%   \Rightarrow [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]
%%   \label{eqg:ctx_refl0}
%% \end{gather}
%% We continue by induction on the lexicographic order of the tuple (size of the
%% context \([[sM]]\), typing mode of the return type \([[TT']]\)). Regarding the typing mode,
%% we define type checking to be larger than type inference. In each mutual
%% dependency, we know that the type size decreases, therefore the induction is
%% well-founded. 

\begin{description}
\item[Part 1] ~ \\
  \proofStep{\textsc{sM-inf-inf-empty}}
  {
    [[ [empty] : (P ; GC ; GG ==> st) |--> (P ; GC ; GG ==> st) ~~> [ empty ] ]]
  }
  {
    By case analysis on the second hypothesis of the nested statement, its last context
    typing rule
    must be \textsc{sM-inf-inf-empty} as well. Therefore, the first and second hypotheses
    of the nested statement become
    \begin{gather*}
      [[ [empty] : (P ; GC ; GG ==> st) |--> (P ; GC ; GG ==> st) ~~> [ empty ] ]]\\
%      \label{eq:ctx_refl1} \\
      [[ [empty] : (P ; GC ; GG ==> st) |--> (P ; GC ; GG ==> st) ~~> [ empty ] ]]
%      \label{eq:ctx_refl2}
    \end{gather*}
    and we have \([[iM1 = iM2]] = \intermed{[[ [ empty ] ]]}\). Thus,
    Goal~\ref{eqg:ctx_refl0} becomes
    \begin{equation*}
      [[ TC ; TT' |- SS1 : ie1 =log SS2 : ie2 : is ]]
      \label{eqg:ctx_refl1}
    \end{equation*}
    The above logical equivalence follows directly from Equation~\ref{eq:ctx_refl0}. \\
  }
  \proofStep{\textsc{sM-inf-inf-appL}}
  {
    [[ sM' se2' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> iM1' ie21 ]]
  }
  {
    By case analysis on the second hypothesis of the nested statement, its last context
    typing rule
    must be \textsc{sM-inf-inf-appL} as well. Therefore, the first and second hypotheses
    of the nested statement become
    \begin{gather*}
      [[ sM' se2' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> iM1' ie21 ]]\\
%      \label{eq:ctx_refl3} \\
      [[ sM' se2' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> iM2' ie22 ]]
%      \label{eq:ctx_refl4}
    \end{gather*}
    and Goal~\ref{eqg:ctx_refl0} becomes
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1' (ie1) ie21 =log SS2 : iM2' (ie2) ie22 : is2 ]]
      \label{eqg:ctx_refl2}
    \end{equation}
    From the premises of the two \textsc{sM-inf-inf-appL} rules, we obtain:
    \begin{gather}
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st1 -> st2 ) ~~> iM1' ]]
      \label{eq:ctx_refl5} \\
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st1' -> st2 ) ~~> iM2' ]]
      \label{eq:ctx_refl6} \\
      [[ P ; GC ; GG' |-tm se2' <= st1 ~> ie21 ]]
      \label{eq:ctx_refl7} \\
      [[ P ; GC ; GG' |-tm se2' <= st1' ~> ie22 ]]
      \label{eq:ctx_refl8}
    \end{gather}
    By applying Lemma~\ref{lemma:ctx_type_unique} to
    Equations~\ref{eq:ctx_refl5} and~\ref{eq:ctx_refl6}, we know that
    \([[ st1' -> st2 = st1 -> st2 ]]\).

    Applying the induction hypothesis on Equations~\ref{eq:ctx_refl5}
    and~\ref{eq:ctx_refl6}, yields:
    \begin{equation*}
      [[ SS1 : iM1' =log SS2 : iM2' : ( TC ; TT ==> is ) |--> ( TC ; TT' ==> is1 -> is2 ) ]]
%      \label{eq:ctx_refl9}
    \end{equation*}
    By unfolding the definition of logical equivalence in the above equation
    and applying it on Equation~\ref{eq:ctx_refl0}, we get:
%    \begin{gather}
%      \forall [[ ie1' ]], [[ ie2' ]] : [[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]
%      \label{eq:ctx_refl10} \Rightarrow \\
%      [[ TC ; TT' |- SS1 : iM1' (ie1') =log SS2 : iM2' (ie2') : is1 -> is2 ]]
%      \label{eq:ctx_refl11}
%    \end{gather}
    %% This result, together with Equation~\ref{eq:ctx_refl0}, tells us that:
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1' (ie1) =log SS2 : iM2' (ie2) : is1 -> is2 ]]
      \label{eq:ctx_refl12}
    \end{equation}
    By applying Expression Coherence Theorem A (Theorem~\ref{thmA:coh_exprA}) on
    Equations~\ref{eq:ctx_refl7} and~\ref{eq:ctx_refl8} (and on the second and fourth
    hypotheses of the outer statement), we get:
    \begin{equation}
      [[ TC ; TT' |- SS1 : ie21 =log SS2 : ie22 : is1 ]]
      \label{eq:ctx_refl13}
    \end{equation}
    Goal~\ref{eqg:ctx_refl2} follows from compatibility of term applications
    (Lemma~\ref{lemma:compat_app}, together
    with Equations~\ref{eq:ctx_refl12} and~\ref{eq:ctx_refl13}). \\
  }
  \proofStep{\textsc{sM-inf-inf-appR}}
  {
    [[ se1' sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> ie11 iM1' ]]
  }
  {
    %% By case analysis, we know the final step in the second derivation has to be
    %% \textsc{sM-inf-inf-appR} as well. This means that:
    By case analysis on the second hypothesis of the nested statement, its last context
    typing rule
    must be \textsc{sM-inf-inf-appR} as well. Therefore, the first and second hypotheses
    of the nested statement become
    \begin{gather*}
      [[ se1' sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> ie11 iM1' ]]\\
%      \label{eq:ctx_refl14} \\
      [[ se1' sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st2 ) ~~> ie12 iM2' ]]
%      \label{eq:ctx_refl15}
    \end{gather*}
    and we need to show that
    \begin{equation}
      [[ TC ; TT' |- SS1 : ie11 iM1' (ie1) =log SS2 : ie12 iM2' (ie2) : is2 ]]
      \label{eqg:ctx_refl3}
    \end{equation}
    From the premises of the two \textsc{sM-inf-inf-appR} rules, we obtain:
    \begin{gather}
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st1 ) ~~> iM1' ]]
      \label{eq:ctx_refl16} \\
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st1' ) ~~> iM2' ]]
      \label{eq:ctx_refl17} \\
      [[ P ; GC ; GG' |-tm se1' => st1 -> st2 ~> ie11 ]]
      \label{eq:ctx_refl18} \\
      [[ P ; GC ; GG' |-tm se1' => st1' -> st2 ~> ie12 ]]
      \label{eq:ctx_refl19}
    \end{gather}
    By Lemma~\ref{lemma:ctx_type_unique}, we know that
    \([[ st1' = st1 ]]\).

    By applying Part 2 of this theorem to Equations~\ref{eq:ctx_refl16}
    and~\ref{eq:ctx_refl17}, we get:
    \begin{equation*}
      [[ SS1 : iM1' =log SS2 : iM2' : ( TC ; TT ==> is ) |--> ( TC ; TT' ==> is1 ) ]]
%      \label{eq:ctx_refl20}
    \end{equation*}
    By unfolding the definition of logical equivalence in the above and applying it on
    Equation~\ref{eq:ctx_refl0}, we get:
    %% Equation~\ref{eq:ctx_refl20}, we get:
    %% \begin{gather}
    %%   \forall [[ ie1' ]], [[ ie2' ]] : [[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]
    %%   \label{eq:ctx_refl21} \\
    %%   \Rightarrow [[ TC ; TT' |- SS1 : iM1' (ie1') =log SS2 : iM2' (ie2') : is1 ]]
    %%   \label{eq:ctx_refl22}
    %% \end{gather}
    %% This result, together with Equation~\ref{eq:ctx_refl0}, tells us that:
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1' (ie1) =log SS2 : iM2' (ie2) : is1 ]]
      \label{eq:ctx_refl23}
    \end{equation}
    By applying Expression Coherence Theorem A (Theorem~\ref{thmA:coh_exprA}) to
    Equations~\ref{eq:ctx_refl18} and~\ref{eq:ctx_refl19} (and on the second and fourth
    hypotheses of the outer statement), we get:
    \begin{equation}
      [[ TC ; TT' |- SS1 : ie11 =log SS2 : ie12 : is1 -> is2 ]]
      \label{eq:ctx_refl24}
    \end{equation}
    Goal~\ref{eqg:ctx_refl3} follows from compatibility of term applications
    (Lemma~\ref{lemma:compat_app}, together
    with Equations~\ref{eq:ctx_refl23} and~\ref{eq:ctx_refl24}). \\
  }
  \proofStep{\textsc{sM-inf-inf-letL}}
  {
    [[ slet sx : \/ alj . sqli => st1 = sM' sin se2' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ;
    GG' ==> st2) ~~> iM1 ]] 
  }
  {
    where \([[ iM1 = ilet ix : \/ clj . iqli -> is1 = /\ clj . \ idvarli : iqli . iM1' iin ie21 ]]\).

    By case analysis on the second hypothesis of the nested statement, its last context
    typing rule
    must be \textsc{sM-inf-inf-letL} as well. Therefore, the first and second hypotheses
    of the nested statement become
    %% By case analysis, we know the final step in the second derivation has to be
    %% \textsc{sM-inf-inf-letL} as well. This means that:
    \begin{gather*}
      [[ slet sx : \/ alj . sqli => st1 = sM' sin se2' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ;
      GG' ==> st2) ~~> iM1 ]] \\
%      \label{eq:ctx_refl25} \\
      [[ slet sx : \/ alj . sqli => st1 = sM' sin se2' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ;
      GG' ==> st2) ~~> iM2 ]] 
%      \label{eq:ctx_refl26}
    \end{gather*}
    where \([[ iM2 = ilet ix : \/ clj . iqli -> is1 = /\ clj . \ idvarli : iqli . iM2' iin ie22 ]]\).

    Goal~\ref{eqg:ctx_refl0} becomes
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is2 ]]
      \label{eqg:ctx_refl4}
    \end{equation}
    From the premises of the two \textsc{sM-inf-inf-letL} rules, we obtain:
    \begin{gather}
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG', alj, sdvarli : sqli <== st1 ) ~~> iM1' ]]
      \label{eq:ctx_refl27} \\
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG', alj, sdvarli : sqli <== st1 ) ~~> iM2' ]]
      \label{eq:ctx_refl28} \\
      [[ P ; GC ; GG', sx : \/ alj . sqli => st1 |-tm se2' => st2 ~> ie21 ]]
      \label{eq:ctx_refl29} \\
      [[ P ; GC ; GG', sx : \/ alj . sqli => st1 |-tm se2' => st2 ~> ie22 ]]
      \label{eq:ctx_refl30} \\
      [[ GC ; GG' |-ty \/ alj . sqli => st1 ~> \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl31} \\
      [[ sdvarli fresh ]]
      \label{eq:ctx_refl31b} \\
      [[ sx notin dom ( GG' ) ]]
      \label{eq:ctx_refl31g}
    \end{gather}
    Through repeated case analysis on Equation~\ref{eq:ctx_refl31}
    (\textsc{sTy-scheme} and \textsc{sTy-qual}), we know that
    \begin{gather}
      [[ alj notin GG' ]]
      \nonumber \\
      [[ </ GC ; GG', alj |-q sqi ~> iqi // i /> ]]
      \nonumber \\
      [[ GC ; GG' |-ty st1 ~> is1 ]]
      \label{eq:ctx_refl31e}
    \end{gather}
    By repeated case analysis on the second hypothesis, we get that
    \begin{equation}
      [[ |-ctx empty ; GC ; empty ~> empty ; TC ; empty ]]
      \label{eq:ctx_refl31f}
    \end{equation}
    By \textsc{sCtx-tyEnvTy} and \textsc{sCtx-tyEnvD}, in
    combination with these results and Equation~\ref{eq:ctx_refl31b}, we obtain
    \([[ |-ctx empty ; GC ; empty, alj, sdvarli : sqli ~> empty ; TC ; empty,
    clj, idvarli : iqli ]]\).
    Finally, Lemma~\ref{lemma:ctx_weakening_typing}, together with this
    result and the second and fourth hypothesis, teaches us that:
    \begin{gather}
      [[ |-ctx P ; GC ; GG', alj, sdvarli : sqli ~> SS1 ; TC ; TT',
      clj, idvarli : iqli ]]
      \label{eq:ctx_refl31c} \\
      [[ |-ctx P ; GC ; GG', alj, sdvarli : sqli ~> SS2 ; TC ; TT',
      clj, idvarli : iqli ]]
      \label{eq:ctx_refl31d}
    \end{gather}
    By applying Part 2 of this theorem to Equations~\ref{eq:ctx_refl27}
    and~\ref{eq:ctx_refl28}, in combination with Equations~\ref{eq:ctx_refl31e},
    \ref{eq:ctx_refl31c}
    and~\ref{eq:ctx_refl31d} and the first, third and fifth hypothesis, we get:
    \begin{equation*}
      [[ SS1 : iM1' =log SS2 : iM2' : ( TC ; TT ==> is ) |--> ( TC ; TT', clj, idvarli : iqli ==> is1 ) ]]
%      \label{eq:ctx_refl32}
    \end{equation*}
    By unfolding the definition of logical equivalence in the above and applying it on
    Equation~\ref{eq:ctx_refl0}, we get:
    %% Equation~\ref{eq:ctx_refl32}, we get:
    %% \begin{gather}
    %%   \forall [[ ie1' ]], [[ ie2' ]] : [[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]
    %%   \label{eq:ctx_refl33} \\
    %%   \Rightarrow [[ TC ; TT' |- SS1 : iM1' (ie1') =log SS2 : iM2' (ie2') : is1 ]]
    %%   \label{eq:ctx_refl34}
    %% \end{gather}
    %% This result, together with Equation~\ref{eq:ctx_refl0}, tells us that:
    \begin{equation}
      [[ TC ; TT', clj, idvarli : iqli |- SS1 : iM1' (ie1) =log SS2 : iM2' (ie2) : is1 ]]
      \label{eq:ctx_refl35}
    \end{equation}
    %% Lemma~\ref{lemma:ctx_well_source_mid_typing} applied twice on
    %% Equation~\ref{eq:ctx_refl29} concludes that
    %% \begin{gather*}
    %%   [[ |-ctx P ; GC ; GG', sx : ss1 ~> SS01 ; TC01 ; TT01' ]]
    %%   \label{eq:ctx_refl36} \\
    %%   [[ |-ctx P ; GC ; GG', sx : ss1 ~> SS02 ; TC02 ; TT02' ]]
    %%   \label{eq:ctx_refl37}
    %% \end{gather*}
    %% for some \(\intermed{[[SS01]]}\), \(\intermed{[[TC01]]}\), \(\intermed{[[TT01']]}\),
    %% \(\intermed{[[SS02]]}\), \(\intermed{[[TC02]]}\) and \(\intermed{[[TT02']]}\). By case
    %% analysis on both judgments and with the use of
    %% Equation~\ref{eq:ctx_refl31} and the first and third hypotheses of the outer
    %% statement, the above judgments are refined to:
    By repeatedly applying compatibility Lemmas~\ref{lemma:compat_dabs}
    and~\ref{lemma:compat_tyabs}, we get:
    \begin{equation}
      [[ TC ; TT' |- SS1 : /\ clj . \ idvarli : iqli . iM1' (ie1) =log SS2 : /\ clj . \ idvarli : iqli . iM2' (ie2) : \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl35b}
    \end{equation}
    It follows from \textsc{sCtx-tyEnvTm}, in combination with
    Equations~\ref{eq:ctx_refl31f}, \ref{eq:ctx_refl31g}
    and~\ref{eq:ctx_refl31}, that \\
    \([[ |-ctx empty ; GC ; empty, sx : \/ alj . sqli => st1 ~> empty ; TC ;
    empty, ix : \/ clj . iqli -> is1 ]]\).
    Similarly to before, by applying Lemma~\ref{lemma:ctx_weakening_typing} to
    this result, together with the second and fourth hypothesis, we get:
    \begin{gather}
      [[ |-ctx P ; GC ; GG', sx : \/ alj . sqli => st1 ~> SS1 ; TC ; TT', ix : \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl36} \\
      [[ |-ctx P ; GC ; GG', sx : \/ alj . sqli => st1 ~> SS2 ; TC ; TT', ix : \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl37}
    \end{gather}
    By applying Expression Coherence Theorem A (Theorem~\ref{thmA:coh_exprA}) to
    Equations~\ref{eq:ctx_refl29} and~\ref{eq:ctx_refl30}, together with
    Equations~\ref{eq:ctx_refl36} and~\ref{eq:ctx_refl37}, we get:
    \begin{equation}
      [[ TC ; TT', ix : \/ clj . iqli -> is1 |- SS1 : ie21 =log SS2 : ie22 : is2 ]]
      \label{eq:ctx_refl38}
    \end{equation}
    Goal~\ref{eqg:ctx_refl4} follows from compatibility of let expressions
    (Lemma~\ref{lemma:compat_let}, together
    with Equations~\ref{eq:ctx_refl35} and~\ref{eq:ctx_refl38}). \\
  }
  \proofStep{\textsc{sM-inf-inf-letR}}
  {
    [[ slet sx : \/ alj . sqli => st1 = se1' sin sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ;
    GG' ==> st2) ~~> iM1 ]]
  }
  {
    where \([[ iM1 = ilet ix : \/ clj . iqli -> is1 = /\ clj . \ idvarli : iqli
    . ie11 iin iM1' ]]\).

    %% By case analysis, we know the final step in the second derivation has to be
    %% \textsc{sM-inf-inf-letR} as well. This means that:
    By case analysis on the second hypothesis of the nested statement, its last context
    typing rule
    must be \textsc{sM-inf-inf-letR} as well. Therefore, the first and second hypotheses
    of the nested statement become
    \begin{gather*}
      [[ slet sx : \/ alj . sqli => st1 = se1' sin sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ;
      GG' ==> st2) ~~> iM1 ]]\\
%      \label{eq:ctx_refl39} \\
      [[ slet sx : \/ alj . sqli => st1 = se1' sin sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ;
      GG' ==> st2) ~~> iM2 ]]
%      \label{eq:ctx_refl40}
    \end{gather*}
    where \([[ iM2 = ilet ix : \/ clj . iqli -> is1 = /\ clj . \ idvarli : iqli
    . ie12 iin iM2' ]]\).
    
    Goal~\ref{eqg:ctx_refl0} becomes
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is2 ]]
      \label{eqg:ctx_refl5}
    \end{equation}
    From the premises of the two \textsc{sM-inf-inf-letR} rules, we obtain:
    \begin{gather}
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG', sx : \/ alj . sqli =>
      st1 ==> st2 ) ~~> iM1' ]]
      \label{eq:ctx_refl41} \\
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG', sx : \/ alj . sqli =>
      st1 ==> st2 ) ~~> iM2' ]]
      \label{eq:ctx_refl42} \\
      [[ P ; GC ; GG', alj, sdvarli : sqli |-tm se1 <= st1 ~> ie11 ]]
      \label{eq:ctx_refl43} \\
      [[ P ; GC ; GG', alj, sdvarli : sqli |-tm se1 <= st1 ~> ie12 ]]
      \label{eq:ctx_refl44} \\
      [[ GC ; GG' |-ty \/ alj . sqli => st1 ~> \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl45} \\
      [[ sdvarli fresh ]]
      \label{eq:ctx_refl45b} \\
      [[ sx notin dom (GG') ]]
      \label{eq:ctx_refl45c}
    \end{gather}
    By repeated case analysis on the second hypothesis, we get that
    \begin{equation}
      [[ |-ctx empty ; GC ; empty ~> empty ; TC ; empty ]]
      \label{eq:ctx_refl45d}
    \end{equation}
    By \textsc{sCtx-tyEnvTm}, in
    combination with this result and Equations~\ref{eq:ctx_refl45}
    and~\ref{eq:ctx_refl45c}, we obtain \\
    \([[ |-ctx empty ; GC ; empty, sx : \/ alj . sqli => st1 ~> empty ; TC ; empty,
    ix : \/ clj . iqli -> is1 ]]\).
    Lemma~\ref{lemma:ctx_weakening_typing}, together with this
    result and the second and fourth hypothesis, teaches us that:
    %% We know from \textsc{sCtx-tyEnvTm}, in combination with
    %% Equation~\ref{eq:ctx_refl45} and the 2\textsuperscript{nd} and
    %% 4\textsuperscript{th} hypothesis of the outer statement, that:
    \begin{gather}
      [[ |-ctx P ; GC ; GG', sx : \/ alj . sqli => st1 ~> SS1 ; TC ; TT', ix : \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl46} \\
      [[ |-ctx P ; GC ; GG', sx : \/ alj . sqli => st1 ~> SS2 ; TC ; TT', ix : \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl47}
    \end{gather}
    By applying the induction hypothesis to Equations~\ref{eq:ctx_refl41}
    and~\ref{eq:ctx_refl42}, in combination with Equations~\ref{eq:ctx_refl46}
    and~\ref{eq:ctx_refl47}, we get:
    \begin{equation*}
      [[ SS1 : iM1' =log SS2 : iM2' : ( TC ; TT ==> is ) |--> ( TC ; TT', ix : \/ clj . iqli -> is1 ==> is2 ) ]]
%      \label{eq:ctx_refl48}
    \end{equation*}
    By unfolding the definition of logical equivalence in the above and then applying it on
    Equation~\ref{eq:ctx_refl0}, we get:
    %% Equation~\ref{eq:ctx_refl48}, we get:
    %% \begin{gather}
    %%   \forall [[ ie1' ]], [[ ie2' ]] : [[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]
    %%   \label{eq:ctx_refl49} \\
    %%   \Rightarrow [[ TC ; TT', ix : is1 |- SS1 : iM1' (ie1') =log SS2 : iM2' (ie2') : is1 ]]
    %%   \label{eq:ctx_refl50}
    %% \end{gather}
    %% This result, together with Equation~\ref{eq:ctx_refl0}, tells us that:
    \begin{equation}
      [[ TC ; TT', ix : \/ clj . iqli -> is1 |- SS1 : iM1' (ie1) =log SS2 : iM2' (ie2) : is2 ]]
      \label{eq:ctx_refl51}
    \end{equation}
    Through repeated case analysis on Equation~\ref{eq:ctx_refl45}
    (\textsc{sTy-scheme} and \textsc{sTy-qual}), we know that
    \begin{gather}
      [[ alj notin GG' ]]
      \nonumber \\
      [[ </ GC ; GG', alj |-q sqi ~> iqi // i /> ]]
      \nonumber \\
      [[ GC ; GG' |-ty st1 ~> is1 ]]
      \label{eq:ctx_refl45e}
    \end{gather}
    By \textsc{sCtx-tyEnvTy} and \textsc{sCtx-tyEnvD}, in
    combination with these results and Equations~\ref{eq:ctx_refl45b}
    and~\ref{eq:ctx_refl45d}, we obtain
    \([[ |-ctx empty ; GC ; empty, alj, sdvarli : sqli ~> empty ; TC ; empty,
    clj, idvarli : iqli ]]\).
    Lemma~\ref{lemma:ctx_weakening_typing}, together with this
    result and the second and fourth hypothesis, teaches us that:
    \begin{gather}
      [[ |-ctx P ; GC ; GG', alj, sdvarli : sqli ~> SS1 ; TC ; TT',
      clj, idvarli : iqli ]]
      \label{eq:ctx_refl45f} \\
      [[ |-ctx P ; GC ; GG', alj, sdvarli : sqli ~> SS2 ; TC ; TT',
      clj, idvarli : iqli ]]
      \label{eq:ctx_refl45g}
    \end{gather}
    By applying Expression Coherence Theorem A (Theorem~\ref{thmA:coh_exprA}) to
    Equations~\ref{eq:ctx_refl43} and~\ref{eq:ctx_refl44}, in combination with
    Equations~\ref{eq:ctx_refl45f} and~\ref{eq:ctx_refl45g}, we get:
    \begin{equation}
      [[ TC ; TT', clj, idvarli : iqli |- SS1 : ie11 =log SS2 : ie12 : is1 ]]
      \label{eq:ctx_refl52}
    \end{equation}
    By repeatedly applying compatibility Lemmas~\ref{lemma:compat_dabs}
    and~\ref{lemma:compat_tyabs}, we get:
    \begin{equation}
      [[ TC ; TT' |- SS1 : /\ clj . \ idvarli : iqli . ie11 =log SS2 : /\ clj . \ idvarli : iqli . ie12 : \/ clj . iqli -> is1 ]]
      \label{eq:ctx_refl52b}
    \end{equation}
    Goal~\ref{eqg:ctx_refl5} follows from Lemma~\ref{lemma:compat_let}, together
    with Equations~\ref{eq:ctx_refl51} and~\ref{eq:ctx_refl52b}. \\
  }
  \proofStep{\textsc{sM-inf-inf-ann}}
  {
    [[ sM' <: st' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM1 ]]
  }
  {
    By case analysis, we know the final step in the second derivation has to be
    \textsc{sM-inf-inf-ann} as well. This means that:
    \begin{gather}
      [[ sM' <: st' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM1 ]]
      \label{eq:ctx_refl53} \\
      [[ sM' <: st' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM2 ]]
      \label{eq:ctx_refl54}
    \end{gather}
    The goal to be proven is the following:
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]
      \label{eqg:ctx_refl6}
    \end{equation}
    From the rule premise we know that:
    \begin{gather}
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM1 ]]
      \label{eq:ctx_refl55} \\
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM2 ]]
      \label{eq:ctx_refl56}
    \end{gather}
    Goal~\ref{eqg:ctx_refl6} follows directly from Part 2 of this theorem, in
    combination with Equations~\ref{eq:ctx_refl55} and~\ref{eq:ctx_refl56}. \\
  }
\item[Part 2] By case analysis on the first typing derivation. \\
  \proofStep{\textsc{sM-inf-check-abs}}
  {
    [[ \ sx . sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st1 -> st2 )
    ~~> \ ix : is1 . iM1' ]]
  }
  {
    By case analysis, we know that the final step in the second derivation has
    to be either \textsc{sM-inf-check-abs} or \textsc{sM-inf-check-inf}. Note
    however that no matching inference rules exist. The final step in the second
    derivation thus has to be \textsc{sM-inf-check-abs} as well. This means that:
    \begin{gather}
      [[ \ sx . sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st1 -> st2 )
      ~~> \ ix : is1 . iM1' ]]
      \label{eq:ctx_refl57} \\
      [[ \ sx . sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st1 -> st2 )
      ~~> \ ix : is1 . iM2' ]]
      \label{eq:ctx_refl58}
    \end{gather}
    The goal to be proven is the following:
    \begin{equation}
      [[ TC ; TT' |- SS1 : \ ix : is1 . iM1' (ie1) =log SS2 : \ ix : is1 . iM2' (ie2) : is1 -> is2 ]]
      \label{eqg:ctx_refl7}
    \end{equation}
    From the rule premise we know that:
    \begin{gather}
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG', sx : st1 <== st2 )
      ~~> iM1' ]]
      \label{eq:ctx_refl59} \\
      [[ sM' : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG', sx : st1 <== st2 )
      ~~> iM2' ]]
      \label{eq:ctx_refl60} \\
      [[ GC ; GG' |-ty st1 ~> is1 ]]
      \label{eq:ctx_refl61}
    \end{gather}
    We know from \textsc{sCtx-tyEnvTm}, in combination with
    Equation~\ref{eq:ctx_refl61} and the 4\textsuperscript{th} and
    6\textsuperscript{th} hypothesis that:
    \begin{gather}
      [[ |-ctx P ; GC ; GG', sx : st1 ~> SS1 ; TC ; TT', ix : is1 ]]
      \label{eq:ctx_refl62} \\
      [[ |-ctx P ; GC ; GG', sx : st1 ~> SS2 ; TC ; TT', ix : is1 ]]
      \label{eq:ctx_refl63}
    \end{gather}
    By applying the induction hypothesis to Equations~\ref{eq:ctx_refl59}
    and~\ref{eq:ctx_refl60}, in combination with Equations~\ref{eq:ctx_refl62}
    and~\ref{eq:ctx_refl63}, we get:
    \begin{equation}
      [[ SS1 : iM1' =log SS2 : iM2' : ( TC ; TT ==> is ) |--> ( TC ; TT', ix : is1 ==> is2 ) ]]
      \label{eq:ctx_refl64}
    \end{equation}
    By unfolding the definition of logical equivalence in
    Equation~\ref{eq:ctx_refl64}, we get:
    \begin{gather}
      \forall [[ ie1' ]], [[ ie2' ]] : [[ TC ; TT |- SS1 : ie1' =log SS2 : ie2' : is ]]
      \label{eq:ctx_refl65} \\
      \Rightarrow [[ TC ; TT', ix : is1 |- SS1 : iM1' (ie1') =log SS2 : iM2' (ie2') : is2 ]]
      \label{eq:ctx_refl66}
    \end{gather}
    This result, together with Equation~\ref{eq:ctx_refl0}, tells us that:
    \begin{equation}
      [[ TC ; TT', ix : is1 |- SS1 : iM1' (ie1) =log SS2 : iM2' (ie2) : is2 ]]
      \label{eq:ctx_refl67}
    \end{equation}
    Goal~\ref{eqg:ctx_refl7} follows from Lemma~\ref{lemma:compat_abs}, together
    with Equation~\ref{eq:ctx_refl67}. \\
  }
  \proofStep{\textsc{sM-inf-check-inf}}
  {
    [[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM1 ]]
  }
  {
    By case analysis, we know that the final step in the second derivation has
    to be either \textsc{sM-inf-check-abs} or \textsc{sM-inf-check-inf}. Note
    however that in the case of \textsc{sM-inf-check-abs}, \([[sM]]\) would have
    to be of the form \([[ sM = \ sx . sM' ]]\). In this case, no matching
    inference rules exist, meaning that this is an impossible case.
    Consequently, the final step in the second derivation can only be
    \textsc{sM-inf-check-inf}. This means that:
    \begin{gather}
      [[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM1 ]]
      \label{eq:ctx_refl68} \\
      [[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> iM2 ]]
      \label{eq:ctx_refl69}
    \end{gather}
    The goal to be proven is the following:
    \begin{equation}
      [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]
      \label{eqg:ctx_refl8}
    \end{equation}
    From the rule premise we know that:
    \begin{gather}
      [[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM1 ]]
      \label{eq:ctx_refl70} \\
      [[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> iM2 ]]
      \label{eq:ctx_refl71} 
    \end{gather}
    Goal~\ref{eqg:ctx_refl8} follows directly by applying Part 1 of this theorem
    to Equations~\ref{eq:ctx_refl70} and~\ref{eq:ctx_refl71}. \\
  }
\item[Part 3] By case analysis on the first typing derivation. \\
  Similar to Part 1. \\
\item[Part 4] By case analysis on the first typing derivation. \\
  Similar to Part 2. \\
\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Value Relation for Dictionary Values]\leavevmode
  If \([[ SS1 ; TC ; empty |-d idv1 : iq ~> te1 ]]\)
  and \([[ SS2 ; TC ; empty |-d idv2 : iq ~> te2 ]]\) \\
  and  \([[ TC |- SS1 =log SS2 ]]\) \\
  then \([[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; empty ]]\).
  \label{thmA:dval_rel}
\end{theoremB}

\proof
By induction on the size of \(\intermed{[[idv1]]}\) and \(\intermed{[[idv2]]}\). 

From the definition of dictionary values we know that
\begin{gather*}
  [[ idv1 = iD islj idvli ]] \\
  [[ idv2 = iD' islh' idvlk' ]]
\end{gather*}
For some \(\intermed{[[iD]]}\), \(\intermed{[[iD']]}\), \(\intermed{[[islj]]}\), \(\intermed{[[islh']]}\),
\(\intermed{[[idvli]]}\) and \(\intermed{[[idvlk']]}\).

By case analysis on both the 1\textsuperscript{st} and 2\textsuperscript{nd}
hypothesis (\textsc{D-con}), we know that:
\begin{gather}
  [[ (iD : \/ clj . iqli => iq') . im |-> ie in SS1 ]]~
  \textit{where}~[[ iq = [| islj / clj |] iq' ]]
  \label{eq:dval1} \\
  [[ </ TC ; empty |-ty isj ~> ttj // j /> ]]
  \label{eq:dval2} \\
  [[ </ SS1 ; TC ; empty |-d idvi : [| islj / clj |] iqi ~> tei // i /> ]]
  \label{eq:dval3} \\
  [[ SS11 ; TC ; empty |-tm ie : \/ clj . iqli -> is ~> te ]]~
  \textit{where}~[[ SS1 = SS11 , (iD : \/ clj . iqli => iq') . im |-> ie , SS12 ]]
  \label{eq:dval4} \\
  [[ |-ctx SS1 ; TC ; empty ]]
  \label{eq:dval4b} \\
  [[ (iD' : \/ iblh . iqlk' => iq'') . im' |-> ie' in SS2 ]]~
  \textit{where}~[[ iq = [| islh' / iblh |] iq'' ]]
  \label{eq:dval5} \\
  [[ </ TC ; empty |-ty ish' ~> tth' // h /> ]]
  \label{eq:dval6} \\
  [[ </ SS2 ; TC ; empty |-d idvk' : [| islh' / iblh |] iqk' ~> tek' // k /> ]]
  \label{eq:dval7} \\
  [[ SS21 ; TC ; empty |-tm ie' : \/ iblh . iqlk' -> is' ~> te' ]]~
  \textit{where}~[[ SS2 = SS21 , (iD' : \/ iblh . iqlk' => iq'') . im' |-> ie' , SS22 ]]
  \label{eq:dval8} \\
  [[ |-ctx SS2 ; TC ; empty ]]
  \label{eq:dval8b}
\end{gather}
By case analysis on Equations~\ref{eq:dval4b} and~\ref{eq:dval8b} (\textsc{iCtx-MEnv})
and the definition of logical equivalence in the 3\textsuperscript{rd} hypothesis,
it follows from Equations~\ref{eq:dval1} and~\ref{eq:dval5} that:
\begin{gather}
  [[ iD = iD' ]]
  \nonumber \\
  [[ clj = iblh ]]
  \nonumber \\
  [[ iqli = iqlk' ]]
  \nonumber \\
  [[ iq' = iq'' ]]
  \nonumber \\
  [[ im = im' ]]
  \nonumber \\
  [[ TC |- SS11 =log SS21 ]]
  \nonumber \\
  [[ TC |- SS12 =log SS22 ]]
  \nonumber \\
  [[ TC ; empty |- SS11 : ie =log SS21 : ie' : \/ clj . iqli -> is ]]
  \nonumber
\end{gather}
Consequently, we also know that \(\intermed{[[ j ]]} = \intermed{[[ h ]]}\) and \(\intermed{[[ i ]]} = \intermed{[[ k ]]}\).

Furthermore, rule \textsc{iCtx-MEnv} also tells us that
\([[ unambig (\/ clj . iqli => iq') ]]\).
The definition of unambiguity thus gives us
\([[ clj in fv (iq') ]]\). 
This, in combination with Equations~\ref{eq:dval1} and \ref{eq:dval5}
tells us that \([[ islj = islh' ]]\).

Unfolding the definition of the \(\mathcal{V}\) relation, reduces the goal to be
proven to:
\begin{gather}
  [[ </ (SS1 : idvi , SS2 : idvk') in V ([| islj / clj |] iqi) with TC ; empty // i /> ]]
  \label{eq:dval9} \\
  [[ SS1 ; TC ; empty |-d iD islj idvli : iq ~> te1 ]]
  \label{eq:dval10} \\
  [[ SS2 ; TC ; empty |-d iD islj idvlk' : iq ~> te2 ]]
  \label{eq:dval11} \\
  [[ (iD : \/ clj . iqli => iq') . im |-> ie in SS1 ]]~
  \textit{where}~[[ iq = [| islj / clj |] iq' ]]
  \label{eq:dval12}
\end{gather}
Goals~\ref{eq:dval10} and \ref{eq:dval11} are given by the hypothesis.
Goal~\ref{eq:dval12} follows directly from Equation~\ref{eq:dval1}.
Finally, Goal~\ref{eq:dval9} follows by applying the induction hypothesis on
Equations~\ref{eq:dval3} and \ref{eq:dval7}. \\
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Environment Equivalence Preservation]
  If \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
  and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
  then \([[ TC |- SS1 =log SS2 ]]\).
  \label{thmA:env_eq_pres}
\end{theoremB} 

\begin{figure}[htp]
  \centering

  \def\svgscale{0.75}
  \input{mut_dep_graph.pdf_tex}

  %% \includegraphics[height=5cm]{mut_dep_graph.png}
  \caption{Dependency graph for Theorems~\ref{thmA:env_eq_pres},
    \ref{thmA:dict_cohA} and
    \ref{thmA:coh_exprA}}
  \label{fig:dep_graph1}
\end{figure}

\proof 
By structural induction on \([[P]]\) and mutually proven with
Theorems~\ref{thmA:dict_cohA} and~\ref{thmA:coh_exprA} (see
Figure~\ref{fig:dep_graph1}). 
Note that at the dependency between
Theorem~\ref{thmA:env_eq_pres} and~\ref{thmA:coh_exprA}, the size of \([[P]]\) is
strictly decreasing, whereas \([[P]]\) remains constant at every other
dependency. Because of this, the size of \([[P]]\) is strictly decreasing in
every cycle. 
Consequently, the induction remains well-founded. \\
\proofStep{\([[ P = empty ]]\)}{}
{
  By case analysis on the 1\textsuperscript{st} and 2\textsuperscript{nd}
  hypothesis:
  \begin{equation*}
    \intermed{[[ SS1 ]]} = \intermed{[[ SS2 ]]} = \intermed{[[ empty ]]}
  \end{equation*}
  The goal follows from \textsc{ctxLog-empty}. \\
}
\proofStep{\([[ P = P', (sD : sc) . sm |-> empty, blj, sdvarli : sqli, alk,
  sdvarlh : [| st / a |] sqlh : se ]]\)}{}
{
  By case analysis on the 1\textsuperscript{st} and 2\textsuperscript{nd}
  hypothesis (\textsc{sCtx-pgmInst}):
  \begin{gather}
    [[ SS1 = SS1', (iD : ic) . im |-> /\ iblj . \ idvarli : iqli . /\ clk . \
    idvarlh : [| is / c |] iqlh . ie1 ]]
    \nonumber \\
    [[ SS2 = SS2', (iD : ic') . im |-> /\ iblj . \ idvarli : iqli' . /\ clk . \
    idvarlh : [| is / c |] iqlh' . ie2 ]]
    \nonumber \\
    [[ P' ; GC ; empty, blj, sdvarli : sqli, alk, sdvarlh : [| st / a |] sqlh |-tm se <= [|
    st / a |] st' ~> ie1 ]]
    \label{eq:env_pres3} \\
    [[ P' ; GC ; empty, blj, sdvarli : sqli, alk, sdvarlh : [| st / a |] sqlh |-tm se <= [|
    st / a |] st' ~> ie2 ]]
    \label{eq:env_pres4} \\
    [[ |-ctx P' ; GC ; GG ~> SS1' ; TC ; TT ]]
    \label{eq:env_pres5} \\
    [[ |-ctx P' ; GC ; GG ~> SS2' ; TC ; TT ]]
    \label{eq:env_pres6}
  \end{gather}
  Since the elaboration from \srcL{} constraints to \interL{} constraints is
  entirely deterministic (Lemma~\ref{lemma:c_elab_unique}), we know that 
  \([[ ic' = ic ]]\), \([[ iqli' = iqli ]]\), \([[ iqlh' = iqlh ]]\) and
  consequently that \([[ [| is / c |] iqlh' = [| is / c |] iqlh ]]\).

  From the induction hypothesis, together with Equations~\ref{eq:env_pres5}
  and~\ref{eq:env_pres6}, we get that:
  \begin{equation}
    [[ TC |- SS1' =log SS2' ]]
    \label{eq:env_pres7}
  \end{equation}
  From Expression Coherence Theorem A (Theorem~\ref{thmA:coh_exprA}), in
  combination with Equations~\ref{eq:env_pres3}, \ref{eq:env_pres4},
  \ref{eq:env_pres5} and~\ref{eq:env_pres6}, we know:
  \begin{equation}
    [[ TC ; TT |- SS1' : ie1 =log SS2' : ie2 : [| is / c |] is' ]]
    \label{eq:env_pres8}
  \end{equation}
  where \([[ GC ; GG |-ty [| st / a |] st' ~> [| is / c |] is' ]]\).

  % By applying Expression Coherence Theorem B (Theorem~\ref{thmA:coh_exprB}) to
  % this result, we get:
  % \begin{equation}
  %   [[ TC ; TT |- SS1' : ie1 =ctx SS2' : ie2 : [| is / c |] is' ]]
  %   \label{eq:env_pres9}
  % \end{equation}
  The goal follows from \textsc{ctxLog-cons}, together with
  Equations~\ref{eq:env_pres7} and~\ref{eq:env_pres8}. \\
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\renewcommand\itot[1]{#1}
\begin{theoremB}[Contextual Equivalence in \interL{} Implies Contextual
  Equivalence in \srcL{}]\ \\
  If \([[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]\) \\
  and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
  and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
  and \([[ |-ctx P ; GC ; GG ~> GT ]]\) \\
  and there exists an \([[ st ]]\) such that
  \([[ GC ; GG |-ty st ~> is ]]\) \\
  then \([[ P ; GC ; GG |- te1 =ctx te2 : st ]]\).
  \label{thmA:ctx_equiv_pres}
\end{theoremB}

\proof
By unfolding the definition of contextual equivalence, the goal becomes:
\begin{gather}
  \forall [[ sM : (PT ; GC ; GG ==> st) |--> (PT ; GC ; empty ==> sbool) ~~> tM1 ]]
  \label{eqg:ctx_equiv_pres0a} \\
  [[ sM : (PT ; GC ; GG ==> st) |--> (PT ; GC ; empty ==> sbool) ~~> tM2 ]]
  \label{eqg:ctx_equiv_pres0b} \\
  \textit{then}~[[ tM1 (te1) ~= tM2 (te2) ]]
  \label{eqg:ctx_equiv_pres0}
\end{gather}
We thus assume Equations~\ref{eqg:ctx_equiv_pres0a}
and~\ref{eqg:ctx_equiv_pres0b} and prove Equation~\ref{eqg:ctx_equiv_pres0}.

By unfolding the definition of contextual equivalence in the first hypothesis, we
get that:
\begin{gather}
  \forall [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~> tM1 ]]
  \nonumber \\
  \forall [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2 ]]
  \nonumber \\
  \textit{if}~[[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]]
  \nonumber \\
  \textit{then}~[[ tM1 (te1) ~= tM2 (te2) ]]
  \label{eq:ctx_equiv_pres1}
\end{gather}
By applying Lemma~\ref{lemma:env_strengthening} to the fourth hypothesis, we
know that:
\begin{equation*}
  [[ |-ctx P ; GC ; empty ~> tempty ]]
\end{equation*}
By applying context equivalence (Theorem~\ref{thmA:equiv_ctx}) on
Equations~\ref{eqg:ctx_equiv_pres0a} and~\ref{eqg:ctx_equiv_pres0b}, together
with this result and hypotheses 2, 3 and 4, we know that:
\begin{gather}
  [[ sM : (P ; GC ; GG ==> st) |--> (P ; GC ; empty ==> sbool) ~~> iM1' ]]
  \label{eq:ctx_equiv_pres2} \\
  [[ iM1' : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~> tM1' ]]
  \label{eq:ctx_equiv_pres3} \\
  [[ sM : (P ; GC ; GG ==> st) |--> (P ; GC ; empty ==> sbool) ~~> iM2' ]]
  \label{eq:ctx_equiv_pres4} \\
  [[ iM2' : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2' ]]
  \label{eq:ctx_equiv_pres5}
\end{gather}
Similarly, by applying Lemma~\ref{lemma:env_mid_strengthening} to the first and
second hypothesis, we get:
\begin{gather}
  [[ |-ctx P ; GC ; empty ~> SS1 ; TC ; empty ]]
  \nonumber \\
  [[ |-ctx P ; GC ; empty ~> SS1 ; TC ; empty ]]
  \nonumber
\end{gather}
By applying Theorem~\ref{thmA:ctx_reflex} to
Equations~\ref{eq:ctx_equiv_pres2} and~\ref{eq:ctx_equiv_pres4},
together with this result, hypotheses 2, 3 and 5, and \textsc{sTy-bool}, we know
that:
\begin{equation}
  [[ SS1 : iM1' =log SS2 : iM2' : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]]
  \label{eq:ctx_equiv_pres6}
\end{equation}
We take \([[ iM1 = iM1' ]]\) and \([[ iM2 = iM2' ]]\).
Consequently, since \interL{} context elaboration is deterministic
(Theorem~\ref{thmA:ctxelab:det}),
we get that \([[ tM1 = tM1' ]]\) and \([[ tM2 = tM2' ]]\).
Goal~\ref{eqg:ctx_equiv_pres0} follows from Equations~\ref{eq:ctx_equiv_pres1},
\ref{eq:ctx_equiv_pres3}, \ref{eq:ctx_equiv_pres5} and~\ref{eq:ctx_equiv_pres6}.
\\
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Partial Coherence Theorems
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Partial Coherence Theorems}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\renewcommand\itot[1]{}
\begin{theoremB}[Coherence - Dictionaries - Part A]\leavevmode
  If \([[ P ; GC ; GG |= sq ~> id1 ]]\)
  and \([[ P ; GC ; GG |= sq ~> id2 ]]\) \\
  and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
  and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
  then \([[ TC ; TT |- SS1 : id1 =log SS2 : id2 : iq ]]\) \\
  where \([[ GC ; GG |-q sq ~> iq ]]\).
  \label{thmA:dict_cohA}
\end{theoremB}

\proof
By induction on the first constraint entailment derivation.
This theorem is mutually proven with Theorems~\ref{thmA:env_eq_pres}
and~\ref{thmA:coh_exprA} (see Figure~\ref{fig:dep_graph1}). 
Note that at the dependency between
Theorem~\ref{thmA:env_eq_pres} and~\ref{thmA:coh_exprA}, the size of \([[P]]\) is
strictly decreasing, whereas \([[P]]\) remains constant at every other
dependency. Because of this, the size of \([[P]]\) is strictly decreasing in
every cycle.
Consequently, the induction remains well-founded. \\
\proofStepNL{\textsc{sEntail-inst}}
{
  \drule{sEntail-inst}
}
{
  The final step in the second derivation can be either \textsc{sEntail-inst} or
  \textsc{sEntail-local}: 
  \begin{itemize}
  \item \textsc{sEntail-inst}:
    This means that:
    \begin{gather}
      [[ P ; GC ; GG |= sq ~> iD islj idli ]]
      \label{eq:dcoh_ii0a} \\
      [[ P ; GC ; GG |= sq ~> iD' islj' idli' ]]
      \label{eq:dcoh_ii0b}
    \end{gather}
    The goal to be proven is the following:
    \begin{gather}
      [[ TC ; TT |- SS1 : iD islj idli =log SS2 : iD' islj' idli' : iq ]]
      \label{eq:dcoh_ii1} \\
      \textit{where}~[[ GC ; GG |-q sq ~> iq ]]
      \label{eq:dcoh_ii1b}
    \end{gather}
    By repeated case analysis on the 3\textsuperscript{rd} hypothesis
    (\textsc{sCtx-pgmInst}), together with the fact that
    \begin{equation*}
    [[ (sD : \/ alj . sqli => sq') . sm |-> empty, alj, sdvarli : sqli, blk,
    sdvarlh : sqlh : se in P ]]
    \end{equation*}
    (1\textsuperscript{st} rule premise (\textsc{sEntail-inst})), we know that:
    \begin{equation}
      [[ GC ; empty |-c \/ alj . sqli => sq' ~> \/ clj . iqli => iq' ]]
    \end{equation}
    Consequently, by case analysis (\textsc{sQ-TC}) on this result, we get that:
    \begin{equation}
      [[ GC ; empty, alj |-q sq' ~> iq' ]]
    \end{equation}
    By applying Lemma~\ref{lemma:tvar_subst_ctr} to this result, in combination
    with the 4\textsuperscript{th} rule premise (\textsc{sEntail-inst}), we get
    that:
    \begin{equation}
      [[ GC ; empty |-q [| stlj / alj |] sq' ~> [| islj / clj |] iq' ]]
      \label{eq:dcoh_ii1c}
    \end{equation}
    Goal~\ref{eq:dcoh_ii1b} follows directly from Equation~\ref{eq:dcoh_ii1c},
    since we know that \([[ sq = [| stlj / alj |] sq' ]]\)
    (2\textsuperscript{nd} rule premise (\textsc{sEntail-inst})).
    
    By unfolding the definition of logical equivalence in
    Goal~\ref{eq:dcoh_ii1}, the goal reduces to:
    \begin{equation}
      [[ (SS1 : iD islj idli with R ; phi1 ; gamma1 , SS2 : iD' islj' idli' with R ; phi2 ; gamma2) in V (iq) with TC ; R ]]
      \label{eq:dcoh_ii13}
    \end{equation}
    for any \([[ R in F (TT) with TC ]]\),
    \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\) and
    \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\).

    By simplifying the substitutions (note that \([[phi]]\) only substitutes
    term variables, which has no impact on the types or dictionaries),
    Goal~\ref{eq:dcoh_ii13} reduces to:
    \begin{equation}
      [[ (SS1 : iD R (islj) (idli with R ; empty ; gamma1) , SS2 : iD' R (islj') (idli' with R ; empty ; gamma2)) in V (iq) with TC ; R ]]
      \label{eq:dcoh_ii14}
    \end{equation}
    By applying preservation Theorem~\ref{thmA:typing_pres_constraint} on
    Equations~\ref{eq:dcoh_ii0a} and \ref{eq:dcoh_ii0b} respectively, we get:
    \begin{gather}
      [[ SS1 ; TC ; TT |-d iD islj idli : iq ~> te1 ]]
      \label{eq:dcoh_ii15} \\
      [[ SS2 ; TC ; TT |-d iD' islj' idli' : iq ~> te2 ]]
      \label{eq:dcoh_ii16}
    \end{gather}
    By repeatedly applying substitution lemmas~\ref{lemma:var_subst_dict},
    \ref{lemma:dvar_subst_dict} and \ref{lemma:tvar_subst_dict},
    using \([[R]]\) and \([[gamma]]\), Equations~\ref{eq:dcoh_ii15} and
    \ref{eq:dcoh_ii16} simplify to:
    \begin{gather}
      [[ SS1 ; TC ; empty |-d iD R (islj) (idli with R ; empty ; gamma1) : R (iq) ~> te1' ]]
      \label{eq:dcoh_ii17} \\
      [[ SS2 ; TC ; empty |-d iD' R (islj') (idli' with R ; empty ; gamma2) : R (iq) ~> te2' ]]
      \label{eq:dcoh_ii18}
    \end{gather}
    Furthermore, by applying preservation Theorem~\ref{thmA:typing_pres_env} on
    the 3\textsuperscript{rd} and 4\textsuperscript{th} hypothesis, we know
    that \([[ |-ctx SS1 ; TC ; TT ]]\) and \([[ |-ctx SS2 ; TC ; TT ]]\).
    By Theorem~\ref{thmA:env_eq_pres}, we know that \([[ TC |- SS1 =log SS2 ]]\).
    Consequently, by applying Theorem~\ref{thmA:dval_rel} on
    Equations~\ref{eq:dcoh_ii17} and \ref{eq:dcoh_ii18} we get:
    \begin{equation}
      [[ (SS1 : iD R (islj) (idli with R ; empty ; gamma1) , SS2 : iD' R (islj') (idli' with R ; empty ; gamma2)) in V (R(iq)) with TC ; empty ]]
      \label{eq:dcoh_ii19}
    \end{equation}
    Goal~\ref{eq:dcoh_ii14} follows from Equation~\ref{eq:dcoh_ii19} by Lemma~\ref{lemma:dict_Rsubst}.

  \item \textsc{sEntail-local}:
    This means that:
    \begin{gather}
      [[ P ; GC ; GG |= sq ~> iD islj idli ]]
      \label{eq:dcoh_iv0a} \\
      [[ P ; GC ; GG |= sq ~> idvar ]]
      \label{eq:dcoh_iv0b}
    \end{gather}
    The goal to be proven is the following:
    \begin{gather}
      [[ TC ; TT |- SS1 : iD islj idli =log SS2 : idvar : iq ]]
      \label{eq:dcoh_iv1} \\
      \textit{where}~[[ GC ; GG |-q sq ~> iq ]]
      \label{eq:dcoh_iv1b}
    \end{gather}
    Goal~\ref{eq:dcoh_iv1b} follows similarly to Goal~\ref{eq:dcoh_ii1b} in the
    previous part of this proof.
    
    The 1\textsuperscript{st} rule premise (\textsc{sEntail-local}) tells us that:
    \begin{equation}
      [[ (sdvar : sq) in GG ]]
      \label{eq:dcoh_iv6}
    \end{equation}
    Unfolding the definition of logical equivalence reduces Goal~\ref{eq:dcoh_iv1} to:
    \begin{equation}
      [[ (SS1 : iD islj idli with R ; phi1 ; gamma1 , SS2 : idvar with R ; phi2 ; gamma2) in V (iq) with TC ; R ]]
      \label{eq:dcoh_iv7}
    \end{equation}
    for any \([[ R in F (TT) with TC ]]\),
    \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\) and
    \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\).

    By simplifying the substitutions (note that \([[phi]]\) only substitutes
    term variables, which has no impact on the types or dictionaries),
    Goal~\ref{eq:dcoh_iv7} reduces to: 
    \begin{equation}
      [[ (SS1 : iD R (islj) (idli with R ; empty ; gamma1) , SS2 : idvar with R ; phi2 ; gamma2) in V (iq) with TC ; R ]]
      \label{eq:dcoh_iv13}
    \end{equation}
    The definition of \(\mathcal{H}\), together with Equation~\ref{eq:dcoh_iv6},
    combined with the fact that
    \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\) and
    \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\), tells us that:
    \begin{equation}
      [[ idvar |-> (idv1 , idv2) in gamma ]]~
      \textit{where}~[[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R ]]
      \label{eq:dcoh_iv8}
    \end{equation}
    We thus know that:
    \begin{equation*}
      [[ idvar with R ; phi2 ; gamma2 = idv2 ]]
    \end{equation*}
    By unfolding the definition of the \(\mathcal{V}\) relation in
    Equation~\ref{eq:dcoh_iv8}, we get:
    \begin{equation}
      [[ SS2 ; TC ; empty |-d idv2 : R (iq) ~> te' ]]
      \label{eq:dcoh_iv10}
    \end{equation}
    Preservation Theorem~\ref{thmA:typing_pres_env}, applied to the
    3\textsuperscript{rd} and 4\textsuperscript{th} hypothesis, tells us that:
    \begin{gather*}
      [[ |-ctx SS1 ; TC ; TT ]] \\
      [[ |-ctx SS2 ; TC ; TT ]]
    \end{gather*}
    Applying preservation Theorem~\ref{thmA:typing_pres_constraint} to
    Equation~\ref{eq:dcoh_iv0a} results in:
    \begin{equation}
      [[ SS1 ; TC ; TT |-d iD islj idli : iq ~> te ]]
      \label{eq:dcoh_iv11}
    \end{equation}
    By repeatedly applying substitution lemmas~\ref{lemma:var_subst_dict},
    \ref{lemma:dvar_subst_dict} and \ref{lemma:tvar_subst_dict},
    using \([[R]]\) and \([[gamma]]\), Equation~\ref{eq:dcoh_iv11}
    simplifies to:
    \begin{equation}
      [[ SS1 ; TC ; empty |-d iD R (islj) (idli with R ; empty ; gamma1) : R (iq) ~> te'' ]]
      \label{eq:dcoh_iv12}
    \end{equation}
    From Theorem~\ref{thmA:env_eq_pres}, we know that \([[ TC |- SS1 =log SS2 ]]\).
    By applying Theorem~\ref{thmA:dval_rel} to Equations~\ref{eq:dcoh_iv10} and
    \ref{eq:dcoh_iv12} we get:
    \begin{equation}
      [[ (SS1 : iD R (islj) (idli with R ; empty ; gamma1) , SS2 : idv2) in V (R(iq)) with TC ; empty ]]
      \label{eq:dcoh_iv14}
    \end{equation}
    Goal~\ref{eq:dcoh_iv13} follows from Equation~\ref{eq:dcoh_iv14}, in
    combination with Lemma~\ref{lemma:dict_Rsubst}. \\

  \end{itemize}
}
\proofStep{\textsc{sEntail-local}}
{
  \drule{sEntail-local}
}
{
  The final step in the derivation can be either \textsc{sEntail-inst} or
  \textsc{sEntail-local}:
  \begin{itemize}
  \item \textsc{sEntail-inst}: This proof case is identical to the
    2\textsuperscript{nd} part of the previous case.
    
  \item \textsc{sEntail-local}: This means that:
    \begin{gather*}
      [[ P ; GC ; GG |= sq ~> idvar ]] \\
      [[ P ; GC ; GG |= sq ~> idvar' ]]
    \end{gather*}
    The goal to be proven is the following:
    \begin{gather}
      [[ TC ; TT |- SS1 : idvar =log SS2 : idvar' : iq ]]
      \label{eq:dcoh_vv1} \\
      \textit{where}~[[ GC ; GG |-q sq ~> iq ]]
      \label{eq:dcoh_vv1b}
    \end{gather}
    The rule premise tells us that:
    \begin{gather}
      [[ (sdvar : sq) in GG ]]
      \label{eq:dcoh_vv2} \\
      [[ (sdvar' : sq) in GG ]]
      \label{eq:dcoh_vv3}
    \end{gather}
    Goal~\ref{eq:dcoh_vv1b} follows by repeated case analysis
    (\textsc{sCtx-tyEnvD}) on the 3\textsuperscript{rd} hypothesis, together
    with Equation~\ref{eq:dcoh_vv2}.
    
    Unfolding the definition of logical equivalence reduces
    Goal~\ref{eq:dcoh_vv1} to:
    \begin{equation}
      [[ (SS1 : idvar with R ; phi1 ; gamma1 , SS2 : idvar' with R ; phi2 ; gamma2) in V (iq) with TC ; R ]]
      \label{eq:dcoh_vv4}
    \end{equation}
    for any \([[ R in F (TT) with TC ]]\),
    \([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\) and
    \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\).

    The definition of \(\mathcal{H}\), together with Equations~\ref{eq:dcoh_vv2}
    and \ref{eq:dcoh_vv3}, combined with the fact that
    \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\) and
    \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\), tells us that:
    \begin{gather}
      [[ idvar |-> (idv1 , idv2) in gamma ]]~
      \textit{where}~[[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; R ]]
      \label{eq:dcoh_vv5} \\
      [[ idvar' |-> (idv1' , idv2') in gamma ]]~
      \textit{where}~[[ (SS1 : idv1' , SS2 : idv2') in V (iq) with TC ; R ]]
      \label{eq:dcoh_vv6}
    \end{gather}
    We thus know that:
    \begin{gather*}
      [[ idvar with R ; phi1 ; gamma1 = idv1 ]] \\
      [[ idvar' with R ; phi2 ; gamma2 = idv2' ]]
    \end{gather*}
    From the definition of the \(\mathcal{V}\) relation in
    Equations~\ref{eq:dcoh_vv5} and \ref{eq:dcoh_vv6} it follows that:
    \begin{gather}
      [[ SS1 ; TC ; empty |-d idv1 : R (iq) ~> te ]]
      \label{eq:dcoh_vv7} \\
      [[ SS2 ; TC ; empty |-d idv2' : R (iq) ~> te' ]]
      \label{eq:dcoh_vv8}
    \end{gather}
    Applying preservation Theorem~\ref{thmA:typing_pres_env} to our hypothesis that
    \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\) and
    \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) gives us
    \([[ |-ctx SS1 ; TC ; TT ]]\) and
    \([[ |-ctx SS2 ; TC ; TT ]]\), respectively.

    From Theorem~\ref{thmA:env_eq_pres}, we get that \([[ TC |- SS1 =log SS2 ]]\).
    Consequently, by applying Theorem~\ref{thmA:dval_rel} on Equations~\ref{eq:dcoh_vv7} and
    \ref{eq:dcoh_vv8} we get:
    \begin{equation}
      [[ (SS1 : idv1 , SS2 : idv2') in V (R(iq)) with TC ; empty ]]
      \label{eq:dcoh_vv9}
    \end{equation}
    Goal~\ref{eq:dcoh_vv4} follows from Equation~\ref{eq:dcoh_vv9} by Lemma~\ref{lemma:dict_Rsubst}.
    
  \end{itemize}
}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Coherence - Expressions - Part A]\leavevmode
  \begin{itemize}
  \item
    If \([[ P ; GC ; GG |-tm se => st ~> ie1 ]]\)
    and \([[ P ; GC ; GG |-tm se => st ~> ie2 ]]\) \\
    and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
    then \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\)
    where \([[ GC ; GG |-ty st ~> is ]]\).
  \item
    If \([[ P ; GC ; GG |-tm se <= st ~> ie1 ]]\)
    and \([[ P ; GC ; GG |-tm se <= st ~> ie2 ]]\) \\
    and \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\)
    and \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
    then \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\)
    where \([[ GC ; GG |-ty st ~> is ]]\).
  \end{itemize}
  \label{thmA:coh_exprA}
\end{theoremB}

\proof
By mutual induction on the first typing derivation.
This theorem is mutually proven with Theorems~\ref{thmA:env_eq_pres}
and~\ref{thmA:dict_cohA} (see Figure~\ref{fig:dep_graph1}).
Note that at the dependency between
Theorem~\ref{thmA:env_eq_pres} and~\ref{thmA:coh_exprA}, the size of \([[P]]\) is
strictly decreasing, whereas \([[P]]\) remains constant at every other
dependency. Because of this, the size of \([[P]]\) is strictly decreasing in
every cycle. 
Consequently, the induction remains well-founded.

By applying Lemma~\ref{lemma:type_well_source_typing} to the
1\textsuperscript{st} hypothesis, we get that:
\begin{equation}
  [[ GC ; GG |-ty st ~> is ]]
  \label{eq:cohe0}
\end{equation}

\begin{description}
\item[Part 1]~\\
  \proofStep{\textsc{sTm-inf-true}}
  {
    [[ P ; GC ; GG |-tm strue => sbool ~> itrue ]]
  }
  {
    Through case analysis, it is straightforward to see that the final step in
    the second derivation is \textsc{sTm-inf-true} as well.
    This means that \([[ ie1 = ie2 = itrue ]]\).
    From Theorem~\ref{thmA:env_eq_pres}, we know that 
    \([[ TC |- SS1 =log SS2 ]]\).
    The goal follows from reflexivity Theorem~\ref{thmA:expr_reflex}. \\
  }
  \proofStep{\textsc{sTm-inf-false}}
  {
    [[ P ; GC ; GG |-tm strue => sbool ~> itrue ]]
  }
  {
    The proof is identical to the \textsc{sTm-inf-true} case. \\
  }
  \proofStep{\textsc{sTm-inf-let}}
  {
    [[ P ; GC ; GG |-tm slet sx : \/ alj . sqli => st1 = se1 sin se2 => st2 ~>
    ilet ix : \/ clj . iqlk -> is = /\ clj . \ idvarlk : iqlk . ie1 iin ie2 ]]
  }
  {
    Through case analysis, we know that the final step in the second derivation
    has to be \textsc{sTm-inf-let} as well.
    This means that:
    \begin{gather*}
      [[ P ; GC ; GG |-tm slet sx : \/ alj . sqli => st1 = se1 sin se2 => st2 ~>
      ie3 ]] \\
      \textit{where}~[[ ie3 = ilet ix : \/ clj . iqlk -> is = /\ clj . \ idvarlk
      : iqlk . ie1 iin ie2 ]] \\
      [[ P ; GC ; GG |-tm slet sx : \/ alj . sqli => st1 = se1 sin se2 => st2 ~>
      ie4 ]] \\
      \textit{where}~[[ ie4 = ilet ix : \/ clj . iqlk -> is = /\ clj . \ idvarlk : iqlk . ie1' iin ie2' ]]
    \end{gather*}
    The goal to be proven is the following:
    \begin{equation}
      [[ TC ; TT |- SS1 : ie3 =log SS2 : ie4 : is2 ]]~
      \textit{where}~[[ GC ; GG |-ty ss2 ~> is2 ]]
      \label{eq:cohe_let1}
    \end{equation}
    The rule premise tells us that:
    \begin{gather}
      [[ P ; GC ; GG, alj, sdvarlk : sqlk |-tm se1 <= st1 ~> ie1 ]]
      \label{eq:cohe_let2} \\
      [[ P ; GC ; GG, sx : \/ alj . sqlk => st1 |-tm se2 => st2 ~> ie2 ]]
      \label{eq:cohe_let3} \\
      [[ P ; GC ; GG, alj, sdvarlk : sqlk |-tm se1 <= st1 ~> ie1' ]]
      \label{eq:cohe_let4} \\
      [[ P ; GC ; GG, sx : \/ alj . sqlk => st1 |-tm se2 => st2 ~> ie2' ]]
      \label{eq:cohe_let5} \\
      \textit{where}~[[ closure ( GC ; sqli ) = sqlk ]]
      \nonumber
    \end{gather}
    From Lemma~\ref{lemma:ctx_well_source_mid_typing}, together with
    Equations~\ref{eq:cohe_let2}, \ref{eq:cohe_let3}, \ref{eq:cohe_let4}
    and~\ref{eq:cohe_let5}, and through repeated case analysis on the
    results to discover the contents of the elaborated environments, we get that:
    \begin{gather}
      [[ |-ctx P ; GC ; GG, alj, sdvarlk : sqlk ~> SS1 ; TC ; TT, clj, idvarlk : iqlk ]]
      \nonumber \\
      [[ |-ctx P ; GC ; GG, sx : \/ alj . sqlk => st1 ~> SS1 ; TC ; TT, ix : \/ clj . iqlk -> is ]]
      \nonumber \\
      [[ |-ctx P ; GC ; GG, alj, sdvarlk : sqlk ~> SS2 ; TC ; TT, clj, idvarlk : iqlk ]]
      \nonumber \\
      [[ |-ctx P ; GC ; GG, sx : \/ alj . sqlk => st1 ~> SS2 ; TC ; TT, ix : \/ clj . iqlk -> is ]]
      \nonumber
    \end{gather}
    By applying the induction hypothesis to Equations~\ref{eq:cohe_let3} and
    \ref{eq:cohe_let5}, we get:
    \begin{equation}
      [[ TC ; TT, ix : \/ clj . iqlk -> is |- SS1 : ie2 =log SS2 : ie2' : is2 ]]
      \label{eq:cohe_let6}
    \end{equation}
    Furthermore, applying Part 2 of this lemma to
    Equations~\ref{eq:cohe_let2} and \ref{eq:cohe_let4} results in:
    \begin{equation}
      [[ TC ; TT, clj, idvarlk : iqlk |- SS1 : ie1 =log SS2 : ie1' : is ]]
      \label{eq:cohe_let7}
    \end{equation}
    Applying compatibility Lemma~\ref{lemma:compat_let}, together with
    Equation~\ref{eq:cohe_let6}, reduces Goal~\ref{eq:cohe_let1} to:
    \begin{equation}
      [[ TC ; TT |- SS1 : /\ clj . \ idvarlk : iqlk . ie1 =log SS2 : /\ clj . \ idvarlk : iqlk . ie1' : \/ clj . iqlk -> is ]]
      \label{eq:cohe_let8}
    \end{equation}
    Combining compatibility Lemma~\ref{lemma:compat_dabs} with
    Equation~\ref{eq:cohe_let7} gives us:
    \begin{equation}
      [[ TC ; TT, clj |- SS1 : \ idvarlk : iqlk . ie1 =log SS2 : \ idvarlk : iqlk . ie1' : iqlk -> is ]]
      \label{eq:cohe_let9}
    \end{equation}
    Goal~\ref{eq:cohe_let8} follows directly by applying
    Equation~\ref{eq:cohe_let9} to compatibility Lemma~\ref{lemma:compat_tyabs}. \\
  }
  \proofStep{\textsc{sTm-inf-ArrE}}
  {
    [[ P ; GC ; GG |-tm se1 se2 => st2 ~> ie1 ie2 ]]
  }
  {
    Through case analysis, we see that the final step in the second derivation
    can only be \textsc{sTm-inf-ArrE}.
    This means that:
    \begin{gather*}
      [[ P ; GC ; GG |-tm se1 se2 => st2 ~> ie1 ie2 ]] \\
      [[ P ; GC ; GG |-tm se1 se2 => st2 ~> ie1' ie2' ]]
    \end{gather*}
    The goal to be proven is the following:
    \begin{equation}
      [[ TC ; TT |- SS1 : ie1 ie2 =log SS2 : ie1' ie2' : is2 ]]~
      \textit{where}~[[ GC ; GG |-ty st2 ~> is2 ]]
      \label{eq:cohe_arrE7}
    \end{equation}
    The rule premise tells us that:
    \begin{gather}
      [[ P ; GC ; GG |-tm se1 => st1 -> st2 ~> ie1 ]]
      \label{eq:cohe_arrE1} \\
      [[ P ; GC ; GG |-tm se2 <= st1 ~> ie2 ]]
      \label{eq:cohe_arrE2} \\
      [[ P ; GC ; GG |-tm se1 => st1 -> st2 ~> ie1' ]]
      \label{eq:cohe_arrE3} \\
      [[ P ; GC ; GG |-tm se2 <= st1 ~> ie2' ]]
      \label{eq:cohe_arrE4}
    \end{gather}
    Applying the induction hypothesis on Equations~\ref{eq:cohe_arrE1} and
    \ref{eq:cohe_arrE3} results in:
    \begin{equation}
      [[ TC ; TT |- SS1 : ie1 =log SS2 : ie1' : is1 -> is2 ]]~
      \textit{where}~[[ GC ; GG |-ty st1 -> st2 ~> is1 -> is2 ]]
      \label{eq:cohe_arrE5}
    \end{equation}
    By applying Part 2 of this lemma to Equations~\ref{eq:cohe_arrE2} and
    \ref{eq:cohe_arrE4} we get:
    \begin{equation}
      [[ TC ; TT |- SS1 : ie2 =log SS2 : ie2' : is1 ]]~
      \textit{where}~[[ GC ; GG |-ty st1 ~> is1 ]]
      \label{eq:cohe_arrE6}
    \end{equation}
    Goal~\ref{eq:cohe_arrE7} follows by applying Equations~\ref{eq:cohe_arrE5}
    and \ref{eq:cohe_arrE6} to compatibility Lemma~\ref{lemma:compat_app}. \\
  }
  \proofStep{\textsc{sTm-inf-Ann}}
  {
    [[ P ; GC ; GG |-tm se <: st => st ~> ie ]]
  }
  {
    Through case analysis we know that the final step in the second derivation
    is \textsc{sTm-inf-Ann}. This means that:
    \begin{gather*}
      [[ P ; GC ; GG |-tm se <: st => st ~> ie ]] \\
      [[ P ; GC ; GG |-tm se <: st => st ~> ie' ]]
    \end{gather*}
    The goal to be proven is the following:
    \begin{equation}
      [[ TC ; TT |- SS1 : ie =log SS2 : ie' : is ]]~
      \textit{where}~[[ GC ; GG |-ty st ~> is ]]
      \label{eq:cohe_ann1}
    \end{equation}
    From the rule premise we know:
    \begin{gather}
      [[ P ; GC ; GG |-tm se <= st ~> ie ]]
      \label{eq:cohe_ann2} \\
      [[ P ; GC ; GG |-tm se <= st ~> ie' ]]
      \label{eq:cohe_ann3}
    \end{gather}
    The goal follows directly from Part 2 of this lemma, applied to
    Equation~\ref{eq:cohe_ann2} and \ref{eq:cohe_ann3}.
  }
\item[Part 2]~\\
\proofStep{\textsc{sTm-check-var}}
{
  [[ P ; GC ; GG |-tm sx <= [| stlj / alj |] st ~> ix islj idli ]]
}
{
  Through case analysis, we see that the final step in the second typing
  derivation can either be \textsc{sTm-check-var} or \textsc{sTm-check-Inf}.
  However, noting that no matching inference rules exist, we conclude that the
  final derivation step has to be \textsc{sTm-check-var}.
  This means that:
  \begin{gather*}
    [[ P ; GC ; GG |-tm sx <= [| stlj / alj |] st ~> ix islj idli ]] \\
    [[ P ; GC ; GG |-tm sx <= [| stlj / alj |] st ~> ix islj' idli' ]]
  \end{gather*}
  The goal to be proven is the following:
  \begin{equation}
    [[ TC ; TT |- SS1 : ix islj idli =log SS2 : ix islj' idli' : is' ]]~
    \textit{where}~[[ GC ; GG |-ty [| stlj / alj |] st ~> is' ]]
    \label{eq:cohe_var1}
  \end{equation}
  By inversion on Equation~\ref{eq:cohe0}, we know that \([[ is' = [| islj / clj
  |] is ]]\).
  
  The rule premise tells us that:
  \begin{gather}
    [[ ( sx : \/ alj . sqli => st ) in GG ]]
    \label{eq:cohe_var2} \\
    [[ </ P ; GC ; GG |= [| stlj / alj |] sqi ~> idi // i /> ]]
    \label{eq:cohe_var3} \\
    [[ </ GC ; GG |-ty stj ~> isj // j /> ]]
    \label{eq:cohe_var4} \\
    [[ </ P ; GC ; GG |= [| stlj / alj |] sqi ~> idi' // i /> ]]
    \label{eq:cohe_var4b} \\
    [[ </ GC ; GG |-ty stj ~> isj' // j /> ]]
    \label{eq:cohe_var5}
  \end{gather}
  Since type elaboration is completely deterministic (Lemma~\ref{lemma:ty_elab_unique}),
  we know that \([[ islj = islj' ]]\).

  From Lemma~\ref{lemma:pres_env_tm}, 
  combined with the 3\textsuperscript{rd} hypothesis and
  Equation~\ref{eq:cohe_var2}, we know that:
  \begin{equation}
    [[ ( ix : \/ clj . iqli -> is ) in TT ]]
    \label{eq:cohe_var6}
  \end{equation}
  By applying Theorem~\ref{thmA:typing_pres_env} to the 3\textsuperscript{rd} and
  4\textsuperscript{th} hypothesis, we get:
  \begin{gather}
    [[ |-ctx SS1 ; TC ; TT ]]
    \label{eq:cohe_var6b} \\
    [[ |-ctx SS2 ; TC ; TT ]]
    \label{eq:cohe_var6c}
  \end{gather}
  Applying Equations~\ref{eq:cohe_var6}, \ref{eq:cohe_var6b} and~\ref{eq:cohe_var6c} to
  \textsc{iTm-var}, results in:
  \begin{gather}
    [[ SS1 ; TC ; TT |-tm ix : \/ clj . iqli -> is ~> tx ]]
    \label{eq:cohe_var7} \\
    [[ SS2 ; TC ; TT |-tm ix : \/ clj . iqli -> is ~> tx ]]
    \label{eq:cohe_var7b}
  \end{gather}
  From Theorem~\ref{thmA:env_eq_pres}, we know that:
  \begin{equation}
    [[ TC |- SS1 =log SS2 ]]
    \label{eq:cohe_var7c}
  \end{equation}
  From reflexivity Theorem~\ref{thmA:expr_reflex}, applied on
  Equations~\ref{eq:cohe_var7}, \ref{eq:cohe_var7b} and~\ref{eq:cohe_var7c}, we
  know that:
  \begin{equation}
    [[ TC ; TT |- SS1 : ix =log SS2 : ix : \/ clj . iqli -> is ]]
    \label{eq:cohe_var8}
  \end{equation}
  From repeated case analysis on the 3\textsuperscript{rd} hypothesis
  (\textsc{sCtx-pgmInst}), we get:
  \begin{equation}
    [[ |-ctx empty ; GC ; GG ~> empty ; TC ; TT ]]
    \label{eq:cohe_var8a}
  \end{equation}
  By applying Theorem~\ref{thmA:typing_pres_types} to Equations~\ref{eq:cohe_var4}
  and~\ref{eq:cohe_var8a}, we know that:
  \begin{equation}
    [[ </ TC ; TT |-ty isj ~> ttj' // j /> ]]
    \label{eq:cohe_var8b}
  \end{equation}
  Applying compatibility Lemma~\ref{lemma:compat_tyapp} \(j\) times to
  Equations~\ref{eq:cohe_var8} and~\ref{eq:cohe_var8b} results in:
  \begin{equation}
    [[ TC ; TT |- SS1 : ix islj =log SS2 : ix islj : [| islj / clj |] iqli -> [| islj / clj |] is ]]
    \label{eq:cohe_var9}
  \end{equation}
  Applying Theorem~\ref{thmA:dict_cohA} to Equations~\ref{eq:cohe_var3} and
  \ref{eq:cohe_var4b} gives us:
  \begin{gather}
    [[ </ TC ; TT |- SS1 : idi =log SS2 : idi' : iqi' // i /> ]]
    \label{eq:cohe_var10} \\
    \textit{where}~[[ </ GC ; GG |-q [| stlj / alj |] sqi ~> iqi' // i /> ]]
    \label{eq:cohe_var10b}
  \end{gather}
  By inversion on Equation~\ref{eq:cohe_var10b}, we know that
  \([[ </ iqi' = [| islj / clj |] iqi // i /> ]]\).
  
  Goal~\ref{eq:cohe_var1} follows by repeatedly applying compatibility
  Lemma~\ref{lemma:compat_dapp} to Equation~\ref{eq:cohe_var9}, combined with
  Equation~\ref{eq:cohe_var10}. \\
}
\proofStep{\textsc{sTm-check-meth}}
{
  [[ P ; GC ; GG |-tm sm <= [| stlj / alj |] [|st / a |] st' ~> id . im islj
  idli ]]
}
{
  The proof is similar to the \textsc{sTm-check-var} case. \\
}
\proofStep{\textsc{sTm-check-ArrI}}
{
  [[ P ; GC ; GG |-tm \ sx . se <= st1 -> st2 ~> \ ix : is1 . ie ]]
}
{
  Through case analysis, it is straightforward to note that the final step in
  the second typing derivation can be either \textsc{sTm-check-ArrI} or
  \textsc{sTm-check-Inf}. In the latter case however, no matching inference
  rules exist. The \textsc{sTm-check-ArrI} case is the only remaining
  possibility.
  This means that:
  \begin{gather*}
    [[ P ; GC ; GG |-tm \ sx . se <= st1 -> st2 ~> \ ix : is1 . ie ]] \\
    [[ P ; GC ; GG |-tm \ sx . se <= st1 -> st2 ~> \ ix : is1' . ie' ]]
  \end{gather*}
  From the 3\textsuperscript{rd} rule premise we know that:
  \begin{gather}
    [[ GC ; GG |-ty st1 ~> is1 ]]
    \nonumber \\
    [[ GC ; GG |-ty st1 ~> is1' ]]
    \nonumber
  \end{gather}
  Since type elaboration is entirely deterministic (Lemma~\ref{lemma:ty_elab_unique}), it is straightforward to
  note that \([[ is1 = is1' ]]\).
  
  The goal to be proven is the following:
  \begin{equation}
    [[ TC ; TT |- SS1 : \ ix : is1 . ie =log SS2 : \ ix : is1 . ie' : is' ]]~
    \textit{where}~[[ GC ; GG |-ty st1 -> st2 ~> is' ]]
    \label{eq:cohe_arrI1}
  \end{equation}
  By inversion on Equation~\ref{eq:cohe0}, we know that \([[ is' = is1 -> is2 ]]\).

  From the rule premise we know:
  \begin{gather}
    [[ P ; GC ; GG, sx : st1 |-tm se <= st2 ~> ie ]]
    \label{eq:cohe_arrI2} \\
    [[ P ; GC ; GG, sx : st1 |-tm se <= st2 ~> ie' ]]
    \label{eq:cohe_arrI3}
  \end{gather}
  By applying Equation~\ref{eq:cohe_arrI2} to
  Lemma~\ref{lemma:ctx_well_source_mid_typing}, and through repeated case
  analysis on the result to discover the contents of the elaborated
  environments, we know that: 
  \begin{equation*}
    [[ |-ctx P ; GC ; GG , sx : st1 ~> SS1 ; TC ; TT, ix : is1 ]]
  \end{equation*}
  Applying the induction hypothesis on Equations~\ref{eq:cohe_arrI2} and
  \ref{eq:cohe_arrI3} results in:
  \begin{equation}
    [[ TC ; TT, ix : is1 |- SS1 : ie =log SS2 : ie' : is2 ]]~
    \textit{where}~[[ GC ; GG, sx : st1 |-ty st2 ~> is2 ]]
    \label{eq:cohe_arrI4}
  \end{equation}
  Goal~\ref{eq:cohe_arrI1} follows directly from compatibility
  Lemma~\ref{lemma:compat_abs}. \\
}
\proofStep{\textsc{sTm-check-Inf}}
{
  [[ P ; GC ; GG |-tm se <= st ~> ie ]]
}
{
  Through case analysis, we note that the final step in the second typing
  derivation can either be \textsc{sTm-check-var}, \textsc{sTm-check-meth},
  \textsc{sTm-check-ArrI} or \textsc{sTm-check-Inf}. In the first 3 cases, the
  proof is symmetrical to the corresponding proof cases described above. We
  proceed with the last case:
  
  The goal to be proven is the following:
  \begin{equation}
    [[ TC ; TT |- SS1 : ie =log SS2 : ie' : is ]]~
    \textit{where}~[[ GC ; GG |-ty st ~> is ]]
    \label{eq:cohe_inf1}
  \end{equation}
  where we know that:
  \begin{gather}
    [[ P ; GC ; GG |-tm se <= st ~> ie ]]
    \label{eq:cohe_inf2} \\
    [[ P ; GC ; GG |-tm se <= st ~> ie' ]]
    \label{eq:cohe_inf3} 
  \end{gather}
  The rule premise tells us that:
  \begin{gather}
    [[ P ; GC ; GG |-tm se => st ~> ie ]]
    \label{eq:cohe_inf4} \\
    [[ P ; GC ; GG |-tm se => st ~> ie' ]]
    \label{eq:cohe_inf5}
  \end{gather}
  The goal follows directly by applying Part 1 of this lemma to
  Equations~\ref{eq:cohe_inf4} and \ref{eq:cohe_inf5}. Part 1 can be applied on
  \([[se]]\), even though the term size did not decrease, because inference is
  defined to be smaller than type checking in our proof by induction.
}
\end{description}
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Coherence - Expressions - Part B]\ \\
  If \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\)
  then \([[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]\).
  \label{thmA:coh_exprB}
\end{theoremB}

\proof
By unfolding the definition of contextual equivalence, the goal becomes:
\begin{gather}
  \forall [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~>
      tM1 ]]
  \nonumber \\
  \forall [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2 ]]
  \nonumber \\
  \textit{if}~[[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]]
  \label{eq:cohexprB1a} \\
  \textit{then}~[[ SS1 : iM1 (ie1) ~= SS2 : iM2 (ie2) ]]
  \label{eq:cohexprB1}
\end{gather}
We select any \(\intermed{[[iM1]]}\) and \(\intermed{[[iM2]]}\) such that
Equation~\ref{eq:cohexprB1a} holds, and thus need to prove Goal~\ref{eq:cohexprB1}.

From the congruence Theorem~\ref{thmA:congruence_expr} and the
1\textsuperscript{st} hypothesis, we know that:
\begin{equation*}
  [[ TC ; empty |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : ibool ]]
  \label{eq:cohexprB2}
\end{equation*}
By applying the definition of logical equivalence, we get:
\begin{equation}
  [[ (SS1 : iM1 (ie1) with R ; phi1 ; gamma1 , SS2 : iM2 (ie2) with R ; phi2 ; gamma2) in E (ibool) with TC ; R ]]
  \label{eq:cohexprB3}
\end{equation}
for any \([[ R in F (empty) with TC ]]\),
\([[ phi in G (empty) with SS1 ; SS2 ; TC ; R ]]\) and
\([[ gamma in H (empty) with SS1 ; SS2 ; TC ; R ]]\).

However, from the definition of \( \mathcal{F} \), \( \mathcal{G} \)
and \( \mathcal{H} \), it follows that \([[ R = empty ]]\),
\([[ phi = empty ]]\) and
\([[ gamma = empty ]]\).

Equation~\ref{eq:cohexprB3} thus simplifies to:
\begin{equation*}
  [[ (SS1 : iM1 (ie1) , SS2 : iM2 (ie2)) in E (ibool) with TC ; empty ]]
  \label{eq:cohexprB4}
\end{equation*}
Unfolding the definition of the \( \mathcal{E} \) relation, tells us that:
\begin{gather*}
  [[ SS1 ; TC ; empty |-tm iM (ie1) : ibool ~> te1 ]]
  \label{eq:cohexprB5} \\
  [[ SS2 ; TC ; empty |-tm iM (ie2) : ibool ~> te2 ]]
  \label{eq:cohexprB6} \\
  \begin{aligned}
    \exists [[ iv1 ]], [[ iv2 ]] & :
    [[ SS1 |- iM (ie1) -->> iv1 ]]
    \nonumber \\
    & \band [[ SS2 |- iM (ie2) -->> iv2 ]]
    \nonumber \\
    & \band [[ (SS1 : iv1 , SS2 : iv2) in V (ibool) with TC ; empty ]]
    \nonumber
  \end{aligned}
\end{gather*}
From the definition of \( \mathcal{V} \), we know that either
\([[ iv1 = iv2 = itrue ]]\) or \([[ iv1 = iv2 = ifalse ]]\).
The goal follows immediately. \\
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\renewcommand\itot[1]{#1}

\begin{theoremB}[Coherence - Expressions - Part C]\ \\
  If \([[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]\) \\
  and \([[ SS1 ; TC ; TT |-tm ie1 : is ~> te1 ]]\)
  and \([[ SS2 ; TC ; TT |-tm ie2 : is ~> te2 ]]\) \\
  and \([[ TC ; TT ~> GT ]]\) \\
  then \([[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]\).
  \label{thmA:coh_exprC}
\end{theoremB}

\proof
By unfolding the definition of contextual equivalence, the goal becomes:
\begin{gather}
  \forall [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~>
  tM1 ]]
  \nonumber \\
  \forall [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~>
  tM2 ]]
  \nonumber \\
  \textit{if}~[[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]]
  \label{eqg:cohC0a} \\
  \textit{then}~[[ tM1 (te1) ~= tM2 (te2) ]]
  \label{eqg:cohC0}
\end{gather}
We select any \(\intermed{[[iM1]]}\) and \(\intermed{[[iM2]]}\) such that
Equation~\ref{eqg:cohC0a} holds, and thus need to prove Goal~\ref{eqg:cohC0}.

By unfolding the definition of contextual equivalence in the
1\textsuperscript{st} hypothesis, we get that:
\begin{gather}
  \forall [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM1 ]]
  \nonumber \\
  \forall [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2 ]]
  \nonumber \\
  \textit{if}~[[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]]
  \label{eq:cohC1a} \\
  \textit{then}~[[ SS1 : iM1 (ie1) ~= SS2 : iM2 (ie2) ]]
  \label{eq:cohC1}
\end{gather}
By applying Theorem~\ref{thmA:tgt_ctx_compat} to \(\intermed{[[iM1]]}\) and
\(\intermed{[[iM2]]}\), together with the 2\textsuperscript{nd} and
3\textsuperscript{rd} hypothesis, we get:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm iM1 (ie1) : ibool ~> tM1 (te1) ]]
  \nonumber \\
  [[ SS2 ; TC ; empty |-tm iM2 (ie2) : ibool ~> tM2 (te2) ]]
  \nonumber 
\end{gather}
From the definition of kleene equivalence, Equation~\ref{eq:cohC1} reduces to:
\begin{equation*}
  \exists [[iv]] : [[ SS1 |- iM1 (ie1) -->> iv ]] \band [[ SS2 |- iM2 (ie2) -->> iv ]]
\end{equation*}
Finally, Lemma~\ref{lemma:val_sem_pres} applied to these results, tells us that:
\begin{gather}
  [[ SS1 ; TC ; empty |-tm iv : ibool ~> tv1 ]]
  \nonumber \\
  [[ SS2 ; TC ; empty |-tm iv : ibool ~> tv2 ]]
  \nonumber \\
  [[ tM1 (te1) -->> tv1 ]]
  \nonumber \\
  [[ tM2 (te2) -->> tv2 ]]
  \nonumber
\end{gather}
Goal~\ref{eqg:cohC0} follows from the definition of kleene equivalence since either
\([[ tv1 = tv2 = ttrue ]]\) or \([[ tv1 = tv2 = tfalse ]]\). \\
\qed


% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
% Main Theorems
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsection{Main Coherence Theorems}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Coherence]\leavevmode
  If \([[ empty ; empty |-pgm spgm : st ; PT1 ; GC1 ~> te1 ]]\)
  and \([[ empty ; empty |-pgm spgm : st ; PT2 ; GC2 ~> te2 ]]\) \\
  then \([[ GC1 = GC2 ]]\), \([[ PT1 = PT2 ]]\)
  and \([[ PT1 ; GC1 ; empty |- te1 =ctx te2 : st ]]\).
  \label{thmA:coh}
\end{theoremB}

\proof
Since we know from \textsc{sCtxT-empty} that
\begin{equation*}
  [[ |-ctx empty ; empty ; empty ~> tempty ]]
\end{equation*}
the goal follows directly from the Program Coherence Theorem
(Theorem~\ref{thmA:ecoh_programs}). \\
\qed

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Coherence - Expressions]\leavevmode
  \begin{itemize}
  \item If \([[ PT ; GC ; GG |-tm se => st ~> te1 ]]\)
    and \([[ PT ; GC ; GG |-tm se => st ~> te2 ]]\) \\
    then \([[ PT ; GC ; GG |- te1 =ctx te2 : st ]]\).
  \item If \([[ PT ; GC ; GG |-tm se <= st ~> te1 ]]\)
    and \([[ PT ; GC ; GG |-tm se <= st ~> te2 ]]\) \\
    then \([[ PT ; GC ; GG |- te1 =ctx te2 : st ]]\).
  \end{itemize}
  \label{thmA:ecoh}
\end{theoremB}

\proof

By applying Lemma~\ref{lemma:ctx_well_source_typing} to the
1\textsuperscript{st} hypothesis, we know that:
\begin{equation}
  [[ |-ctx P ; GC ; GG ~> GT ]]
  \label{eq:ecoh0}
\end{equation}
\begin{description}
\item[Part 1]
  From environment equivalence (Theorem~\ref{thmA:equiv_env}), we get that:
  \begin{gather}
    [[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]
    \label{eq:ecoh1} \\
    [[ |-ctx P ; GC ; GG ~> SS2 ; TC' ; TT' ]]
    \label{eq:ecoh2} \\
    [[ TC ; TT ~> GT ]]
    \label{eq:ecoh3}
  \end{gather}
  Since class and typing environment elaboration is entirely deterministic (Lemma~\ref{lemma:env_elab_unique}),
  it is easy to see that \([[ TC' = TC ]]\) and \([[ TT' = TT ]]\).

  We know from expression equivalence (Theorem~\ref{thmA:equiv_expr}) that:
  \begin{gather}
    [[ P ; GC ; GG |-tm se <= st ~> ie1 ]]
    \label{eq:ecoh4} \\
    [[ SS1 ; TC ; TT |-tm ie1 : is1 ~> te1 ]]
    \label{eq:ecoh5} \\
    [[ P ; GC ; GG |-tm se <= st ~> ie2 ]]
    \label{eq:ecoh6} \\
    [[ SS2 ; TC ; TT |-tm ie2 : is2 ~> te2 ]]
    \label{eq:ecoh7} \\
    \textit{where}~[[ GC ; GG |-ty st ~> is1 ]]
    \label{eq:ecoh7b} \\
    \textit{and}~[[ GC ; GG |-ty st ~> is2 ]]
    \nonumber
  \end{gather}
  Since type elaboration is entirely deterministic
  (Lemma~\ref{lemma:ty_elab_unique}), it is easy to see that
  \([[ is = is1 = is2 ]]\). 

  By applying Expression Coherence Theorem A (Theorem~\ref{thmA:coh_exprA}) to Equations~\ref{eq:ecoh1},
  \ref{eq:ecoh2}, \ref{eq:ecoh4} and~\ref{eq:ecoh6}, we get:
  \begin{equation}
    [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]
    \label{eq:ecoh8}
  \end{equation}
  By applying Expression Coherence Theorem B (Theorem~\ref{thmA:coh_exprB}) to Equation~\ref{eq:ecoh8},
  we get:
  \begin{equation}
    [[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]
    \label{eq:ecoh9}
  \end{equation}
  By applying Expression Coherence Theorem C (Theorem~\ref{thmA:coh_exprC}) to
  Equations~\ref{eq:ecoh3}, \ref{eq:ecoh5}, \ref{eq:ecoh7} and~\ref{eq:ecoh9},
  we get:
  \begin{equation}
    [[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]
    \label{eq:ecoh10}
  \end{equation}
  The goal follows directly from Theorem~\ref{thmA:ctx_equiv_pres}, together with
  Equations~\ref{eq:ecoh10}, \ref{eq:ecoh0}, \ref{eq:ecoh1}, \ref{eq:ecoh2}
  and~\ref{eq:ecoh7b}. \\
\item[Part 2]
  Similar to Part 1. \\
\end{description}
\qed

\renewcommand\itot[1]{}

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\begin{theoremB}[Coherence - Programs]\ \\
  If \([[ PT ; GC |-pgm spgm : st ; PT1 ; GC1 ~> te1 ]]\), \\
  \([[ PT ; GC |-pgm spgm : st ; PT2 ; GC2 ~> te2 ]]\), \\
  \([[ |-ctx PT ; GC ; empty ~> tempty ]]\), \\
  then \([[ GC1 = GC2 ]]\),
  \([[ PT1 = PT2 ]]\) \\
  and \([[ PT, PT1 ; GC, GC1 ; empty |- te1 =ctx te2 : st ]]\).
  \label{thmA:ecoh_programs}
\end{theoremB}

\proof
By structural induction on \([[spgm]]\). \\
\proofStep{\([[ spgm = scls ; spgm' ]]\)}
{
}
{
  By case analysis on the program typing derivations (\textsc{sPgmT-cls}):
  \begin{gather}
    [[ GC |-cls scls : GC1' ]]
    \label{eq:pcoh:1} \\
    [[ GC |-cls scls : GC2' ]]
    \label{eq:pcoh:2} \\
    [[ PT ; GC, GC1' |-pgm spgm' : st ; PT1 ; GC1'' ~> te1 ]]
    \nonumber \\
    [[ PT ; GC, GC2' |-pgm spgm' : st ; PT2 ; GC2'' ~> te2 ]]
    \nonumber \\
    [[ GC1 = GC1', GC1'' ]]
    \nonumber \\
    [[ GC2 = GC2', GC2'' ]]
    \nonumber 
  \end{gather}
  Since class typing is entirely deterministic, we know that
  \([[ GC1' = GC2' ]]\).
  From Theorem~\ref{thmA:typing_pres_class}, in combination with
  Equations~\ref{eq:pcoh:1} and~\ref{eq:pcoh:2}, we know that:
  \begin{gather}
    [[ |-ctx PT ; GC, GC1' ; empty ~> tempty ]]
    \nonumber \\
    [[ |-ctx PT ; GC, GC2' ; empty ~> tempty ]]
    \nonumber
  \end{gather}
  The goal follows from the induction hypothesis. \\
}
\proofStep{\([[ spgm = sinst ; spgm' ]]\)}
{
}
{
  By case analysis on the program typing derivations (\textsc{sPgmT-inst}):
  \begin{gather}
    [[ PT ; GC |-inst sinst : PT11 ]]
    \label{eq:ecohp1} \\
    [[ PT ; GC |-inst sinst : PT21 ]]
    \label{eq:ecohp2} \\
    [[ PT, PT11 ; GC |-pgm spgm' : st ; PT12 ; GC1 ~> te1 ]]
    \label{eq:ecohp2b} \\
    [[ PT, PT21 ; GC |-pgm spgm' : st ; PT22 ; GC2 ~> te2 ]]
    \label{eq:ecohp2c} \\
    [[ PT1 = PT11 , PT12 ]]
    \nonumber \\
    [[ PT2 = PT21 , PT22 ]]
    \nonumber
  \end{gather}
  The goal to be proven is the following:
  \begin{gather}
    [[ GC1 = GC2 ]]
    \label{eqg:ecohp1} \\
    [[ PT11 , PT12 = PT21 , PT22 ]]
    \label{eqg:ecohp2} \\
    [[ PT, PT11, PT12 ; GC, GC1 ; empty |- te1 =ctx te2 : st ]]
    \label{eqg:ecohp3}
  \end{gather}
  By case analysis on Equations~\ref{eq:ecohp1} and~\ref{eq:ecohp2} (\textsc{sInstT-inst}),
  we know that:
  \begin{gather}
    [[ sinst = instance sqlp => sTC st swhere { sm = se } ]]
    \nonumber \\
    [[ ( sm : sqli' => sTC a : \/ alj . sqlh' => st1 ) in GC ]]
    \label{eq:ecohpe2} \\
    [[ blk = fv (st') ]]
    \nonumber \\
    [[ closure ( GC ; sqlp ) = sqlq1 ]]
    \nonumber \\
    [[ closure ( GC ; sqlp ) = sqlq2 ]]
    \nonumber \\
    [[ unambig ( \/ blk . sqlq1 => sTC st' ) ]]
    \label{eq:ecohpe1} \\
    [[ unambig ( \/ blk . sqlq2 => sTC st' ) ]]
    \nonumber \\
    [[ </ PT ; GC ; empty, blk, sdvarlq1 : sqlq1 |= [| st' / a |] sq'i ~> te1i // i /> ]]
    \nonumber \\
    [[ </ PT ; GC ; empty, blk, sdvarlq2 : sqlq2 |= [| st' / a |] sq'i ~> te2i // i /> ]]
    \nonumber \\
    [[ sD fresh ]]
    \label{eq:ecohpe3} \\
    [[ sdvarlq1 fresh ]]
    \nonumber \\
    [[ sdvarlq2 fresh ]]
    \nonumber \\
    [[ sdvarlh' fresh ]]
    \nonumber
  \end{gather}
  \begin{gather}
    [[ PT ; GC ; empty, blk, sdvarlq1 : sqlq1, alj, sdvarlh' : [| st' / a |] sqlh' |-tm se
    <= [| st' / a |] st1 ~> te1' ]]
    \label{eq:ecohp3} \\
    [[ PT ; GC ; empty, blk, sdvarlq2 : sqlq2, alj, sdvarlh' : [| st' / a |] sqlh' |-tm se
    <= [| st' / a |] st1 ~> te2' ]]
    \label{eq:ecohp4} \\
    [[ PT11 = (sD : \/ blk . sqlq1 => sTC st') . sm |-> empty, blk, sdvarlq1 :
    sqlq1, alj, sdvarlh' : [| st' / a |] sqlh' : se1 ]]
    \label{eq:ecohp7} \\
    [[ PT21 = (sD : \/ blk . sqlq2 => sTC st') . sm |-> empty, blk, sdvarlq2 :
    sqlq2, alj, sdvarlh' : [| st' / a |] sqlh' : se2 ]]
    \label{eq:ecohp8} \\
    [[ GC ; empty, blk |-ty st' ~> tt' ]]
    \label{eq:ecohp29} \\
    [[ </ GC ; empty, blk |-q sqq1 ~> ttq1 // q /> ]]
    \label{eq:ecohp30} \\
    [[ </ GC ; empty, blk |-q sqq2 ~> ttq2 // q /> ]]
    \label{eq:ecohp30b} \\
    [[ (sD' : \/ bls' . sqln' => sTC st2 ) . sm' |-> GG' : se' notin PT : [| stls' / bls' |] st2 = [| stlk' / blk |] st' ]]
    \label{eq:ecohpe4}
  \end{gather}
  Note that since instance typing is entirely deterministic,
  \([[ PT11 = PT21 ]]\).
  Similarly, since the closure over the superclass relation is deterministic, we know that
  \([[ sqlq1 = sqlq2 ]]\).
  Note that we assume that the fresh variables are identical in both program typing derivations.

  We can derive from \textsc{sCtxT-pgmInst} that
  \begin{gather}
    [[ |-ctx PT, PT11 ; GC ; empty ~> tempty ]]
    \label{eq:ecohp14} \\
    [[ |-ctx PT, PT21 ; GC ; empty ~> tempty ]]
    \label{eq:ecohp15}
  \end{gather}
  assuming we can show that:
  \begin{gather}
    [[ unambig (\/ blk . sqlq1 => sTC st') ]]
    \label{eq:ecohp16} \\
    [[ GC ; empty |-c \/ blk . sqlq1 => sTC st' ~> \/ tblk . ttlq1 -> [| tt' / ta |]
    { tl : \/ talj . ttlh' -> tt1 } ]]
    \label{eq:ecohp17} \\
    [[ ( sm : sqli' => sTC a : \/ alj . sqlh' => st1 ) in GC ]]
    \label{eq:ecohp18} \\
    [[ GC ; empty, a |-ty \/ alj . sqlh' => st1 ~> \/ talj . ttlh' -> tt1 ]]
    \label{eq:ecohp19} \\
    [[ GC ; empty, blk |-ty st' ~> tt' ]]
    \label{eq:ecohp20} \\
    [[ PT ; GC ; empty, blk, sdvarlq1 : sqlq1, alj, sdvarlh' : [| st' / a |] sqlh' |-tm se
    <= [| st' / a |] st1 ~> te1' ]]
    \label{eq:ecohp21} \\
    [[ PT ; GC ; empty, blk, sdvarlq2 : sqlq2, alj, sdvarlh' : [| st' / a |] sqlh' |-tm se
    <= [| st' / a |] st1 ~> te2' ]]
    \label{eq:ecohp22} \\
    [[ sD notin dom (PT) ]]
    \label{eq:ecohp23} \\
    [[ ( sD' : \/ blk' . sqlh'' => sTC st'' ) . sm' |-> GG' : se' notin PT ]]~
    where~[[ [| stlk / blk |] st' = [| stlk' / blk' |] st'' ]]
    \label{eq:ecohp25} \\
    [[ |-ctx PT ; GC ; empty ~> tempty ]]
    \label{eq:ecohp28} 
  \end{gather}
  Goals~\ref{eq:ecohp16}, \ref{eq:ecohp18}, \ref{eq:ecohp20}, \ref{eq:ecohp21},
  \ref{eq:ecohp22}, \ref{eq:ecohp23} and~\ref{eq:ecohp25} follow directly from
  Equations~\ref{eq:ecohpe1}, \ref{eq:ecohpe2}, \ref{eq:ecohp29}, \ref{eq:ecohp3},
  \ref{eq:ecohp4}, \ref{eq:ecohpe3} and~\ref{eq:ecohpe4} respectively. 

  Goal~\ref{eq:ecohp28}
  follows directly from the 3\textsuperscript{rd} hypothesis.
  Goal~\ref{eq:ecohp19} follows by applying case analysis on Equation~\ref{eq:ecohp28}
  (\textsc{sCtxT-clsEnv}), in combination with Equation~\ref{eq:ecohp18}.
  Goal~\ref{eq:ecohp17} follows from \textsc{sCT-abs} and \textsc{sQT-TC}, in
  combination with Equations~\ref{eq:ecohp18}, \ref{eq:ecohp19},
  \ref{eq:ecohp29} and~\ref{eq:ecohp30}.

  Finally, Goals~\ref{eqg:ecohp1}, \ref{eqg:ecohp2} and~\ref{eqg:ecohp3} follow
  by applying the induction hypothesis on Equations~\ref{eq:ecohp2b}
  and~\ref{eq:ecohp2c}, in combination with 
  Equations~\ref{eq:ecohp14} and~\ref{eq:ecohp15}. \\
}
\proofStep{\([[ spgm = se ]]\)}
{
}
{
  The goal follows directly from coherence Theorem~\ref{thmA:ecoh}.
}
\qed


\renewcommand\itot[1]{}


% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Aside
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%% \section{Aside}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Compatibility Lemmas
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% \newpage
%% \section{Compatibility Lemmas}

%% \subsection{Application Compatibility Lemma}
%% \[
%% \begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
%%   \inferrule*[right=AppCom]
%%              {
%%                \logEqS{\fDataEnv}{\ityEnv}{t_1}{t_2}{\itype' \to \itype} \\
%%                \logEqS{\fDataEnv}{\ityEnv}{t_1'}{t_2'}{\itype'}
%%              }
%%              { \logEqS{\fDataEnv}{\ityEnv}{t_1~t_1'}{t_2~t_2'}{\itype} }
%% \end{array}
%% \]

%% \proof

%% By def $\logEqName$:
%% \begin{align}
%% &\itceTerm{\fDataEnv}{\ityEnv}{t_1}{\itype' \to \itype}~\band~\itceTerm{\fDataEnv}{\ityEnv}{t_2}{\itype' \to \itype} \\
%% &\band~\forall (\ctxSub_1 ; \ctxSub_2) \in \ctxRel{\ityEnv}{\ityEnv}{\fullTheory}{\fDataEnv},
%% \forall (\datSub_1 ; \datSub_2) \in \datRel{\fDataEnv}{\fDataEnv}{\fullTheory}{\fDataEnv} : \\
%% &(\datSub_1~\ctxSub_1~t_1 ; \datSub_2~\ctxSub_2~t_2) \in \expRel{\itype' \to \itype}{\itype' \to \itype}{\fullTheory}{\fDataEnv}
%% \end{align}
%% \begin{align}
%% &\itceTerm{\fDataEnv}{\ityEnv}{t_1'}{\itype}~\band~\itceTerm{\fDataEnv}{\ityEnv}{t_2'}{\itype'} \\
%% &\band~\forall (\ctxSub_1 ; \ctxSub_2) \in \ctxRel{\ityEnv}{\ityEnv}{\fullTheory}{\fDataEnv},
%% \forall (\datSub_1 ; \datSub_2) \in \datRel{\fDataEnv}{\fDataEnv}{\fullTheory}{\fDataEnv} : \\
%% &(\datSub_1~\ctxSub_1~t_1' ; \datSub_2~\ctxSub_2~t_2') \in \expRel{\itype'}{\itype'}{\fullTheory}{\fDataEnv}
%% \end{align}

%% By def $\expRelName$:
%% \begin{align}
%%   &\itceTerm{\fDataEnv}{\bullet}{\datSub_1~\ctxSub_1~t_1}{\itype' \to \itype}~\band~\itceTerm{\fDataEnv}{\bullet}{\datSub_2~\ctxSub_2~t_2}{\itype' \to \itype} \\
%%   &\band~\exists t_{1v}, t_{2v} : \datSub_1~\ctxSub_1~t_1 \mapsto^{*} t_{1v}~\band~\datSub_2~\ctxSub_2~t_2 \mapsto^{*} t_{2v} \\
%%   &\band~(t_{1v} ; t_{2v}) \in \valRel{\itype' \to \itype}{\itype' \to \itype}{\fullTheory}{\fDataEnv} \label{eq:app-com-val}
%% \end{align}
%% \begin{align}
%%   &\itceTerm{\fDataEnv}{\bullet}{\datSub_1~\ctxSub_1~t_1'}{\itype'}~\band~\itceTerm{\fDataEnv}{\bullet}{\datSub_2~\ctxSub_2~t_2'}{\itype'} \\
%%   &\band~\exists t_{1v}', t_{2v}' : \datSub_1~\ctxSub_1~t_1' \mapsto^{*} t_{1v}'~\band~\datSub_2~\ctxSub_2~t_2' \mapsto^{*} t_{2v}' \\
%%   &\band~(t_{1v}' ; t_{2v}') \in \valRel{\itype'}{\itype'}{\fullTheory}{\fDataEnv}
%% \end{align}

%% By def $\valRelName$ on (\ref{eq:app-com-val}):
%% \begin{align}
%%   &\itceTerm{\fDataEnv}{\bullet}{t_{1v}}{\itype' \to \itype}~\band~\itceTerm{\fDataEnv}{\bullet}{t_{2v}}{\itype' \to \itype} \\
%%   &\band~\itceConstraint{\sconstraint}{\itype'}~\band~\proveConstraint{\fullTheory}{\sconstraint}{t_3} \\
%%   &\band~(t_{1v}~t_3 ; t_{2v}) \in \expRel{\itype}{\itype' \to \itype}{\fullTheory}{\fDataEnv} \label{eq:app-com-exp}
%% \end{align}

%% By def $\expRelName$ on (\ref{eq:app-com-exp}):
%% \begin{align}
%%   &\itceTerm{\fDataEnv}{\bullet}{t_{1v}~t_3}{\itype} \\
%%   &\band~\exists t_4, t_5 : t_{1v}~t_3 \mapsto^{*} t_4~\band~t_{2v} \mapsto^{*} t_5 \\
%%   &\band~(t_4 ; t_5) \in \valRel{\itype}{\itype' \to \itype}{\fullTheory}{\fDataEnv} \label{eq:app-com-val2}
%% \end{align}

%% By def $\valRelName$ on (\ref{eq:app-com-val2}):
%% \begin{align}
%%   &\itceTerm{\fDataEnv}{\bullet}{t_4}{\itype}~\band~\itceTerm{\fDataEnv}{\bullet}{t_5}{\itype} \\
%%   &\band~\itceConstraint{\sconstraint}{\itype'}~\band~\proveConstraint{\fullTheory}{\sconstraint}{t_6} \\
%%   &\band~(t_4 ; t_5~t_6) \in \expRel{\itype}{\itype}{\fullTheory}{\fDataEnv}
%% \end{align}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "./proof"
%%% End:


==> doc/sections/logical.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                              Logical Relations
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\newpage
\section{Logical Relations}
\label{sec:log_rel}
\renewcommand\itot[1]{}
In the definitions for the logical relations below, \([[gamma = gamma' , idvar
|-> (idv1 , idv2)]]\) and \([[phi = phi' , ix |-> (ie1 , ie2)]]\)
are substitutions which map all dictionary variables \([[idvar in TT]]\) and term
variables \([[ix in TT]]\) onto two (possibly different) dictionary values and term
values respectively. Notation-wise, we adopted the convention that \([[ gamma1 ]]\)
maps the dictionary variable \([[idvar]]\) to the leftmost value \([[idv1]]\) and
\([[ gamma2 ]]\) substitutes \([[idvar]]\) for the rightmost value \([[idv2]]\).
Similarly for \([[phi1]]\) and \([[phi2]]\).

The third kind of substitution \([[ R = R' , c |-> (is , r) ]]\) maps all type variables
\([[c in TT]]\) onto closed types \([[is]]\), while also storing a relation
\([[r]]\). This relation \([[r]]\) is an arbitrary member of the set of all
relations \([[ Rel (is) ]]\) which offer the following property:
\begin{equation*}
  [[ Rel (is) ]] = \{ [[r]] \in \mathcal{P} ([[iv]] \times [[iv]])~|~\forall ([[iv1]] , [[iv2]]) \in [[r]] : [[ SS ; TC ; empty |-tm iv1 : is ~> te1 ]] \band [[ SS ; TC ; empty |-tm iv2 : is ~> te2 ]] \}
\end{equation*}

\subsection{Dictionary Relation}
  \begin{flushleft}
    \namedRuleform{[[ ( SS1 : idv1 , SS2 : idv2 ) in V ( iq ) with TC ; R ]]}
                  {Closed Dictionary Value Relation}
  \end{flushleft}
  \begin{align*}
    [[ (SS1 : iD islj idvl1i, SS2 : iD islj idvl2i) in V (iq) with TC ; R ]]
    & \triangleq [[ </ (SS1 : idv1i , SS2 : idv2i) in V ([| islj / clj |] iqi) with TC ; R // i /> ]] \\
    & \land [[ SS1 ; TC ; empty |-d iD islj idvl1i : R (iq) ~> te1 ]] \\
    & \land [[ SS2 ; TC ; empty |-d iD islj idvl2i : R (iq) ~> te2 ]] \\
    & \textit{where } [[ (iD : \/ clj . iqli => iq') . im |-> ie1 in SS1 ]] 
     \land [[ iq = [| islj / clj |] iq' ]] \\
  \end{align*}

  \begin{flushleft}
    \namedRuleform{[[TC ; TT |- SS1 : id1 =log SS2 : id2 : iq]]}
                  {Logical Equivalence for Open Dictionaries}
  \end{flushleft}
  \begin{align*}
    [[TC ; TT |- SS1 : id1 =log SS2 : id2 : iq]]
    & \triangleq \forall [[R in F ( TT ) with TC]],\\
    &  [[phi in G ( TT ) with SS1 ; SS2 ; TC ; R]], \\
    &  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]], \\
    &  [[ (SS1 : id1 with R ; phi1; gamma1, SS2 : id2 with R ; phi2 ; gamma2) in V (iq) with TC ; R]]
  \end{align*}

%% \newpage
\subsection{Expression Relation}
  \begin{flushleft}
  \namedRuleform{[[ ( SS1 : iv1 , SS2 : iv2 ) in V ( is ) with TC ; R ]]}
                {Closed Expression Value Relation}
  \end{flushleft}
  \begin{align*}
    [[ (SS1 : itrue, SS2 : itrue) in V (ibool) with TC ; R ]] \\
    [[ (SS1 : ifalse, SS2 : ifalse) in V (ibool) with TC ; R ]] \\
    [[ (SS1 : iv1 , SS2 : iv2) in V (c) with TC ; R ]]
    & \triangleq [[ (c |-> (is, r)) in R ]] \\
    & \land [[ SS1 ; TC ; empty |-tm iv1 : is ~> te1 ]] \\
    & \land [[ SS2 ; TC ; empty |-tm iv2 : is ~> te2 ]] \\
    & \land [[ (iv1 , iv2) in r ]] \\
    [[ (SS1 : \ ix : is1 . ie1 , SS2 : \ix : is1 . ie2) in V (is1 -> is2) with TC ; R ]]
    & \triangleq [[ SS1 ; TC ; empty |-tm \ix : is . ie1 : R ( is1 -> is2 ) ~> te1 ]] \\
    & \land [[ SS2 ; TC ; empty |-tm \ix : is . ie2 : R ( is1 -> is2 ) ~> te2 ]] \\
    & \land \forall [[ (SS1 : ie3, SS2 : ie4) in E (is1) with TC ; R ]] : \\ 
    & [[ ( SS1 : (\ ix : is . ie1) ie3, SS2 : (\ ix : is . ie2) ie4 ) in E (is2) with TC ; R]] \\
    [[ (SS1 : \idvar : iq . ie1 , SS2 : \idvar : iq . ie2) in V (iq -> is) with TC ; R ]]
    & \triangleq [[ SS1 ; TC ; empty |-tm \idvar : iq . ie1 : R ( iq -> is ) ~> te1 ]] \\
    & \land [[ SS2 ; TC ; empty |-tm \idvar : iq . ie2 : R ( iq -> is ) ~> te2 ]] \\
    & \land \forall [[ (SS1 : idv1, SS2 : idv2) in V (iq) with TC ; R ]] : \\
    & [[ ( SS1 : (\ idvar : iq . ie1) idv1, SS2 : (\ idvar : iq . ie2) idv2 ) in E (is) with TC ; R]] \\
    [[ ( SS1 : /\ c . ie1 , SS2 : /\ c . ie2) in V (\/ c . is) with TC ; R ]]
    & \triangleq [[ SS1 ; TC ; empty |-tm /\ c. ie1 : R (\/ c. is) ~> te1 ]] \\
    & \land [[ SS2 ; TC ; empty |-tm /\ c. ie2 : R (\/ c. is) ~> te2 ]] \\
    & \land \forall \intermed{[[is']]}, \forall [[r in Rel ( is' )]] : \\
    & [[ TC ; empty |-ty is' ~> tt' ]] \Rightarrow \\
    & [[ ( SS1 : (/\ c . ie1) is', SS2 : (/\ c . ie2) is' ) in E (is) with TC ; R , c |-> (is', r) ]]
  \end{align*}


  \begin{flushleft}
  \namedRuleform{[[ ( SS1 : ie1 , SS2 : ie2 ) in E ( is1 ) with TC ; R ]]}
                {Closed Expression Relation}
  \end{flushleft}
  \begin{align*}
    [[ ( SS1 : ie1 , SS2 : ie2 ) in E ( is ) with TC ; R ]]
      & \triangleq [[ SS1 ; TC ; empty |-tm  ie1 : R (is) ~> te1 ]] \\
      & \land [[ SS2 ; TC ; empty |-tm  ie2 : R (is) ~> te2 ]] \\
      & \land \exists \intermed{[[iv1]]} , \intermed{[[iv2]]},
        [[SS1 |- ie1 -->> iv1]],
        [[SS2 |- ie2 -->> iv2]],
        [[ (SS1 : iv1, SS2 : iv2) in V (is) with TC ; R]]
  \end{align*}

  
  \begin{flushleft}
    \namedRuleform{[[TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is]]}
                  {Logical Equivalence for Open Expressions}
  \end{flushleft}
  \begin{align*}
    [[TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is]]
    & \triangleq \forall [[R in F ( TT ) with TC]],\\
    &  [[phi in G ( TT ) with SS1 ; SS2 ; TC ; R]], \\
    &  [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]], \\
    &  [[ (SS1 : ie1 with R ; phi1 ; gamma1, SS2 : ie2 with R ; phi2 ; gamma2) in E (is) with TC ; R]]
  \end{align*}

  \begin{flushleft}
    \namedRuleform{[[SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; TT'
      ==> is')]]}
                  {Logical Equivalence for Contexts}
  \end{flushleft}
  \begin{align*}
    [[SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; TT' ==> is')]]
    & \triangleq \forall \intermed{[[ ie1 ]]}, \intermed{[[ ie2 ]]} :
      [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]] \\
    & \Rightarrow [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]
  \end{align*}

%% \newpage
\begin{definitionA}[Interpretation of type variables in type contexts] 
  \label{def:inter_ty}
  \begin{mathpar}
    \ottaltinferrule{}{}
    {  }
    { [[empty in F (empty) with TC]] } \and

    \ottaltinferrule{}{}
    { [[R in F (TT) with TC]] }
    { [[R in F (TT, ix : is) with TC]]  } \and

    \ottaltinferrule{}{}
    { [[R in F (TT) with TC]]
      \\ [[r in Rel (is)]]
      \\ [[TC ; empty |-ty is ~> tt]]
    }
    { [[ R , c |-> ( is , r ) in F (TT, c) with TC]]  } \and

    \ottaltinferrule{}{}
    { [[R in F (TT) with TC]] }
    { [[R in F (TT, idvar : iq) with TC]] }
  \end{mathpar}
\end{definitionA}

\begin{definitionA}[Interpretation of term variables in type contexts] 
  \label{def:inter_tm}
  \begin{mathpar}
    \ottaltinferrule{}{}
    {  }
    { [[empty in G (empty) with SS1 ; SS2 ; TC ; R]] } \and

    \ottaltinferrule{}{}
    { [[phi in G (TT) with SS1 ; SS2 ; TC ; R]] }
    { [[phi in G (TT, c) with SS1 ; SS2 ; TC ; R]]  } \and

    \ottaltinferrule{}{}
    { [[phi in G (TT) with SS1 ; SS2 ; TC ; R]]
      \\ [[(SS1 : ie1, SS2 : ie2) in E (is) with TC ; R ]]
    }
    { [[ phi , ix |-> (ie1, ie2) in G (TT, ix : is) with SS1 ; SS2 ; TC ; R]]  } \and

    \ottaltinferrule{}{}
    { [[phi in G (TT) with SS1 ; SS2 ; TC ; R]] }
    { [[phi in G (TT, idvar : iq) with SS1 ; SS2 ; TC ; R]] }
  \end{mathpar}
\end{definitionA}

\begin{definitionA}[Interpretation of dictionary variables dictionary contexts] 
  \label{def:inter_d}
  \begin{mathpar}
    \ottaltinferrule{}{}
    {  }
    { [[empty in H (empty) with SS1 ; SS2 ; TC ; R]] } \and

    \ottaltinferrule{}{}
    { [[gamma in H (TT) with SS1 ; SS2 ; TC ; R]] }
    { [[gamma in H (TT, c) with SS1 ; SS2 ; TC ; R]] } \and

    \ottaltinferrule{}{}
    { [[gamma in H (TT) with SS1 ; SS2 ; TC ; R]] }
    { [[gamma in H (TT, ix : is) with SS1 ; SS2 ; TC ; R]] } \and

    \ottaltinferrule{}{}
    { [[gamma in H (TT) with SS1 ; SS2 ; TC ; R]]
      \\ [[(SS1 : idv1, SS2 : idv2) in V (iq) with TC ; R ]]
    }
    { [[ gamma , idvar |-> (idv1, idv2) in H (TT, idvar: iq) with SS1 ; SS2 ; TC ; R]]  }
  \end{mathpar}
\end{definitionA}

\subsection{Environment Relation}
\label{app:log_env_rel}

\drules[ctxLog]{$[[ TC |- SS1 =log SS2 ]]$}{Logical Equivalence for
  Environments}{empty, cons}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Strong Normalization
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\newpage
\section{Strong Normalization Relations}
As opposed to Section~\ref{sec:log_rel}, the relations and substitutions in the
strong normalization relations described below, are unary.
The substitutions \([[ gammaSN = gammaSN' , idvar |-> id ]]\) and
\([[ phiSN = phiSN' , ix |-> ie ]]\) map all dictionary 
variables \([[ idvar in TT ]]\) and term variables \([[ ix in TT ]]\) onto
well-typed dictionaries \([[id]]\) and expressions \([[ ie in SN (is) with SS ;
TC ; RSN ]]\). The final kind of substitution \([[ RSN = RSN' , c |-> (is , r)
]]\) maps all type variables \([[ c in TT ]]\) onto closed types \([[is]]\),
while also storing a relation \([[r]]\).
This relation \([[r]]\) is an arbitrary member of the
set of all relations \([[RelSN (is)]]\) which offer the following property:
\begin{equation*}
  [[ RelSN (is) ]] = \{ [[r]] \in \mathcal{P} ([[ie]])~|~\forall [[ie]] \in [[r]] : [[ SS ; TC ; empty |-tm ie : is ~> te ]] \}
\end{equation*}
We adopted the convention that \([[ RSN1 (c) ]]\) maps the type variable
\([[c]]\) onto the closed type \([[is]]\) and \([[ RSN2 (c) ]]\) denotes the
contained set of expressions \([[r]]\).

  \begin{flushleft}
    \namedRuleform{[[ie in SN ( is ) with SS ; TC ; RSN]]}
                  {Strong Normalization Relation}
  \end{flushleft}
  \begin{align*}
    [[ ie in SN ( ibool ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie : ibool ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    [[ ie in SN ( c ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie : RSN1 ( c ) ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    & \land [[ iv in RSN2 ( c ) ]] \\
    [[ ie in SN ( is1 -> is2 ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie : RSN1 ( is1 -> is2 ) ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    & \land \forall [[ ie' ]] : [[ ie' in SN ( is1 ) with SS ; TC ; RSN ]]
      \Rightarrow [[ ie ie' in SN ( is2 ) with SS ; TC ; RSN ]] \\
    [[ ie in SN ( iq -> is ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie : RSN1 ( iq -> is ) ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    & \land \forall [[ id ]] : [[ SS ; TC ; empty |-d id : RSN1 (iq) ~> te ]]
      \Rightarrow [[ ie id in SN ( is ) with SS ; TC ; RSN ]] \\
    [[ ie in SN ( \/ c . is ) with SS ; TC ; RSN ]]
    & \triangleq [[ SS ; TC ; empty |-tm ie : RSN1 ( \/ c . is ) ~> te ]] \\
    & \land \exists [[ iv ]] : [[ SS |- ie -->> iv ]] \\
    & \land \forall [[ is' ]], [[ r in RelSN ( is' ) ]] :
      [[ ie is' in SN ( is ) with SS ; TC ; RSN, c |-> ( is' , r ) ]]
  \end{align*}

\begin{definitionA}[Interpretation of type variables in type contexts for strong normalization] 
  \label{def:inter_sn_ty}
  \begin{mathpar}
    \ottaltinferrule{}{}
    {  }
    { [[empty in FSN (empty) with SS; TC]] } \and

    \ottaltinferrule{}{}
    { [[RSN in FSN (TT) with SS;TC]] }
    { [[RSN in FSN (TT, ix : is) with SS;TC]]  } \and

    \ottaltinferrule{}{}
    { [[RSN in FSN (TT) with SS;TC]]
      \\ [[ r = SN ( is ) with SS; TC ; RSN ]]
      \\ [[TC ; empty |-ty RSN1(is) ~> tt]]
    }
    { [[ RSN , c |-> ( RSN1(is) , r ) in FSN (TT, c) with SS;TC]]  } \and

    \ottaltinferrule{}{}
    { [[RSN in FSN (TT) with SS;TC]] }
    { [[RSN in FSN (TT, idvar : iq) with SS;TC]] }
  \end{mathpar}
\end{definitionA}

\begin{definitionA}[Interpretation of term variables in type contexts for strong normalization] 
  \label{def:inter_sn_tm}
  \begin{mathpar}
    \ottaltinferrule{}{}
    {  }
    { [[empty in GSN (empty) with SS ; TC ; RSN]] } \and

    \ottaltinferrule{}{}
    { [[phiSN in GSN (TT) with SS ; TC ; RSN]] }
    { [[phiSN in GSN (TT, c) with SS ; TC ; RSN]]  } \and

    \ottaltinferrule{}{}
    { [[phiSN in GSN (TT) with SS ; TC ; RSN]]
      \\ [[ie in SN ( is ) with SS ; TC ; RSN ]]
    }
    { [[ phiSN , ix |-> ie in GSN (TT, ix : is) with SS ; TC ; RSN]]  } \and

    \ottaltinferrule{}{}
    { [[phiSN in GSN (TT) with SS ; TC ; RSN]] }
    { [[phiSN in GSN (TT, idvar : iq) with SS ; TC ; RSN]] }
  \end{mathpar}
\end{definitionA}

\begin{definitionA}[Interpretation of dictionary variables dictionary contexts for strong normalization] 
  \label{def:inter_sn_d}
  \begin{mathpar}
    \ottaltinferrule{}{}
    {  }
    { [[empty in HSN (empty) with SS ; TC ; RSN]] } \and

    \ottaltinferrule{}{}
    { [[gammaSN in HSN (TT) with SS ; TC ; RSN]] }
    { [[gammaSN in HSN (TT, c) with SS ; TC ; RSN]] } \and

    \ottaltinferrule{}{}
    { [[gammaSN in HSN (TT) with SS ; TC ; RSN]] }
    { [[gammaSN in HSN (TT, ix : is) with SS ; TC ; RSN]] } \and

    \ottaltinferrule{}{}
    { [[gammaSN in HSN (TT) with SS ; TC ; RSN]]
      \\ [[ SS ; TC ; empty |-d id : RSN1 (iq) ~> te]]
    }
    { [[ gammaSN , idvar |-> id in HSN (TT, idvar: iq) with SS ; TC ; RSN]]  }
  \end{mathpar}
\end{definitionA}

  
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                                 Equivalence
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\section{Equivalence Relations}

\subsection{Kleene Equivalence Relations}
\label{app:log_kleene}

  \begin{flushleft}
    \namedRuleform{[[ SS1 : ie1 ~= SS2 : ie2 ]]}
                  {Kleene Equivalence for \interL{} Expressions}
  \end{flushleft}
  \begin{align*}
    [[ SS1 : ie1 ~= SS2 : ie2 ]]
    & \triangleq \exists [[ iv ]] : [[ SS1 |- ie1 -->> iv ]]
      \band [[ SS2 |- ie2 -->> iv ]]
  \end{align*}

  \begin{flushleft}
    \namedRuleform{[[ te1 ~= te2 ]]}
                  {Kleene Equivalence for \targetL{} Expressions}
  \end{flushleft}
  \begin{align*}
    [[ te1 ~= te2 ]]
    & \triangleq \exists [[ tv ]] : [[ te1 -->> tv ]]
      \band [[ te2 -->> tv ]]
  \end{align*}

\subsection{Contextual Equivalence Relations}

  \begin{flushleft}
    \namedRuleform{[[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]}
                  {Contextual Equivalence for \interL{} Expressions}
  \end{flushleft}
  \begin{align*}
    [[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]
    & \triangleq \forall [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~> tM1 ]] \\
    & \band \forall [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2 ]] \\
    & \band [[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]] \\
    & \Rightarrow [[ SS1 : iM1 ( ie1 ) ~= SS2 : iM2 ( ie2 ) ]]
  \end{align*}

  \begin{flushleft}
    \namedRuleform{[[ PT ; GC ; GG |- te1 =ctx te2 : st ]]}
                  {Contextual Equivalence for \targetL{} Expressions}
  \end{flushleft}
  \begin{align*}
    [[ PT ; GC ; GG |- te1 =ctx te2 : st ]]
    & \triangleq \forall [[ sM : ( PT ; GC ; GG ==> st ) |--> ( PT ; GC ; empty ==> sbool ) ~~> tM1 ]] \\
    & \band [[ sM : ( PT ; GC ; GG ==> st ) |--> ( PT ; GC ; empty ==> sbool ) ~~> tM2 ]] \\
    & \Rightarrow [[ tM1 ( te1 ) ~= tM2 ( te2 ) ]]
  \end{align*}

  \renewcommand\itot[1]{#1}

  \begin{flushleft}
    \namedRuleform{[[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]}
                  {Contextual Equivalence for \targetL{} Expressions in
                    \interL{} context}
  \end{flushleft}
  \begin{align*}
    [[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]
    & \triangleq \forall [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~> tM1 ]] \\
    & \band \forall [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2 ]] \\
    & \band [[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]] \\
    & \Rightarrow [[ tM1 (te1) ~= tM2 (te2) ]] 
  \end{align*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "./proof"
%%% End:


==> doc/sections/target.tex <==
\newpage
% \newcommand{\pref}[1]{(\ref{#1})}
\newcommand{\pref}[1]{\ref{#1}}
\renewcommand\itot[1]{#1}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                            Target Term Typing
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\section{\interL{}-to-\targetL{} Theorems}

\subsection{Lemmas}
\subsubsection{Determinism / Uniqueness}

\begin{lemmaB}[Dictionary Elaboration Uniqueness]\leavevmode
  \label{lem:det:Q}\ \\
  If \([[ TC ; TT |-q iq ~> tt1 ]]\) and \([[ TC ; TT |-q iq ~> tt2 ]]\),
  then \([[ tt1  =  tt2 ]]\).
\end{lemmaB}

\proof
By straightforward induction on the well-formedness derivation. \\
\qed

\begin{lemmaB}[Type Elaboration Uniqueness]
  \label{lem:det:ty}\ \\
  If \([[ TC ; TT |-ty is ~> tt1 ]]\) and \([[ TC ; TT |-ty is ~> tt2 ]]\),
  then \([[ tt1  =  tt2 ]]\).
\end{lemmaB}

\proof
By straightforward induction on the well-formedness derivation. \\
\qed

\begin{lemmaB}[Context Elaboration Uniqueness]
  \label{lem:det:GT}\ \\
  If $[[TC ; TT ~> GT1]]$
  and $[[TC ; TT ~> GT2]]$
  then $[[GT1 = GT2]]$.
\end{lemmaB}

\proof
By straightforward induction on the well-formedness derivation. \\
\qed

\begin{lemmaB}[Determinism of Evaluation]\ \\
  \label{lem:tgt_eval_unique}
  If \([[ te --> te1 ]]\) and \([[ te --> te2 ]]\)
  then \([[ te1 = te2 ]]\).
\end{lemmaB}

\proof
By straightforward induction on both evaluation derivations. \\
\qed

\subsubsection{Soundness}

\begin{lemmaB}[Dictionary Variable Elaboration Soundness]
  \label{lem:qelab}\ \\
  If \([[TC ; TT |-q iq ~> tt]]\)
%  then, there is a $[[GT]]$ such
  and $[[TC ; TT ~> GT]]$
  then $[[ GT |-ty tt ]]$.
\end{lemmaB}

\proof
By straightforward induction on the dictionary typing derivation. \\
\qed

\begin{lemmaB}[Type Elaboration Soundness]
  \label{lem:tyelab}\ \\
  If \([[ TC ; TT |-ty is ~> tt ]]\)
%  then, there is a $[[GT]]$ such
  and $[[TC ; TT ~> GT]]$
  then \([[ GT |-ty tt ]]\).
\end{lemmaB}

\proof
By straightforward induction on the type well-formedness derivation. \\
\qed

\begin{lemmaB}[Term Variable Elaboration Soundness]
  \label{lem:tmvar:elab}\ \\
  If $[[|-ctx SS ; TC ; TT]]$
  and $[[( ix : is ) in TT ]]$,
  then there are unique $[[GT]]$ and $[[tt]]$ \\
  such that $[[TC ; TT ~> GT]]$
  and $[[TC ; TT |-ty is ~> tt]]$
  and $[[( tx : tt ) in GT]]$.
\end{lemmaB}

\proof
By straightforward induction on the environment well-formedness derivation. \\
\qed

\begin{lemmaB}[Dictionary Variable in Environment Elaboration Soundness]
  \label{lem:elab:dvar}\ \\
  If $[[|-ctx SS ; TC ; TT]]$
  and $[[( idvar : iTC is ) in TT ]]$,
  then there are unique $[[GT]]$ and $[[tt]]$ \\
  such that $[[TC ; TT ~> GT]]$
  and $[[|-ctx GT]]$
  and $[[TC ; TT |-q iTC is ~> tt]]$
  and $[[( txd : tt ) in GT]]$.
\end{lemmaB}

\proof
By straightforward induction on the environment well-formedness derivation. \\
\qed

\begin{lemmaB}[Environment Elaboration Soundness]
  \label{lem:ctx_elab}\ \\
  If $[[|-ctx SS ; TC ; TT]]$,
  then there is a unique $[[GT]]$ such
  that $[[TC ; TT ~> GT]]$
  and $[[|-ctx GT]]$.
\end{lemmaB}

\proof
By straightforward induction on the environment well-formedness derivation. \\
\qed

\subsubsection{Canonical Forms Lemmas}

\begin{lemmaB}[Canonical Forms for Functions]
  \label{lem:canon_func}\ \\
  If $[[ GT |-tm tv : tt1 -> tt2 ]]$ for some value $[[tv]]$,
  then $[[tv]]$ is of the form $\target{[[ \ tx : tt1 . te ]]}$,
  for some $[[tx]]$ and $[[te]]$.
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\begin{lemmaB}[Canonical Forms for Type Abstractions]
  \label{lem:canon_tyabs}\ \\
  If $[[ GT |-tm tv : \/ ta . tt ]]$ for some value $[[tv]]$,
  then $[[tv]]$ is of the form $\target{[[ /\ ta . te ]]}$,
  for some $[[te]]$.
\end{lemmaB}

\proof
By straightforward induction on the typing derivation. \\
\qed

\subsubsection{Evaluation Lemmas}

\begin{lemmaB}[Distribution of \textsc{tEval-app}]
  \label{lem:tEval_app_dist}\ \\
  If $[[tempty |-tm te : tt1 -> tt2]]$
  and $[[tempty |-tm te' : tt1 -> tt2]]$
  and $[[tempty |-tm te1 : tt1]]$
  and $[[te -->> te']]$,
  then $[[te te1 -->> te' te1]]$.
\end{lemmaB}

\proof
The goal follows from Canonical Forms Lemma~\ref{lem:canon_func},
together with the well-known strong normalization
of System F with records. \\
\qed

\begin{lemmaB}[Distribution of \textsc{tEval-Tapp}]
  \label{lem:tEval_tapp_dist}\ \\
  If $[[tempty |-tm te : \/ ta . tt']]$
  and $[[tempty |-tm te' : \/ ta . tt']]$
  and $[[tempty |-ty tt]]$
  and $[[te -->> te']]$,
  then $[[te tt -->> te' tt]]$.
\end{lemmaB}

\proof
The goal follows from Canonical Forms Lemma~\ref{lem:canon_tyabs},
together with the well-known strong normalization
of System F with records. \\
\qed

\subsection{Soundness}
\begin{theoremB}[Term Elaboration Soundness]
  \label{thmA:tmelab}
  % \setcounter{equation}{0}
  \begin{flalign}
  &\text{If}~[[ SS ; TC ; TT |-tm ie : is ~> te ]]\label{tmelab:hyp} &\\
  &\text{then, there are unique}~[[GT]]~\text{and}~[[ tt ]]~\text{such
    that}\nonumber &\\
  &[[TC ; TT ~> GT ]]\label{tmelab:res1} &\\
  &\text{and}~[[ TC ; TT |-ty is ~> tt ]]\label{tmelab:res2} &\\
  &\text{and}~[[GT |-tm te : tt]]\label{tmelab:res3}
  \end{flalign}
\end{theoremB}

\proof This theorem is proved mutually with Theorem~\ref{thmA:delab}. The proof follows
structural induction on Hypothesis~\ref{tmelab:hyp} of the theorem.\\ \\
\proofStep{Case \textsc{iTm-true}}
          {\ottdruleiTmXXtrue{}}
          {We need to show that there are unique $[[GT]]$ and $[[tt]]$ such that
            $[[TC ; TT ~> GT]]$ and $[[TC ; TT |-ty ibool ~> tt]]$ and
            $[[GT |-tm ttrue : tt]]$.
%            \begin{gather*}
%              [[TC ; TT ~> GT]]\\
%              \text{and}~[[TC ; TT |-ty ibool ~> tt]]\\
%              \text{and}~[[GT |-tm ttrue : tt]]
            %            \end{gather*}
            
            Obviously, $[[tt]]$ can only be equal to $[[tbool]]$.
            By Lemma~\ref{lem:ctx_elab} applied on the premise of rule
            \textsc{iTm-true}, there is a unique $[[GT]]$ such that $[[TC ; TT ~> GT ]]$ and
            $[[|-ctx GT]]$. We use the latter result to instantiate rule \textsc{tTm-True},
            which concludes with $[[GT |-tm ttrue : tbool]]$.\\
          }
\proofStep{Case \textsc{iTm-false}}
          {\ottdruleiTmXXfalse{}}
          {Similar to case \textsc{iTm-true}.\\}
\proofStep{Case \textsc{iTm-var}}
          {\ottdruleiTmXXvar{}}
          {
            By Lemma~\ref{lem:ctx_elab}, there is a unique $[[GT]]$ such that
            \begin{gather}
              %\label{tmelab:var:1}
              \nonumber
              [[TC ; TT ~> GT]]\\
              \label{tmelab:var:2}
              \text{and}~[[|-ctx GT]]
            \end{gather}
            With Lemma~\ref{lem:tmvar:elab} applied on the two premises of rule \textsc{iTm-var},
            we also find a unique $[[tt]]$ such that $[[TC ; TT |-ty is ~> tt]]$ and
            $[[( tx : tt ) in GT]]$. Then, by rule \textsc{tTm-Var} applied on the latter
            result and on Equation \pref{tmelab:var:2}, we reach the goal.\\
          }
\proofStep{Case \textsc{iTm-let}}
          {\ottdruleiTmXXlet{}}
          {The induction hypothesis for the first premise of rule \textsc{iTm-let} is
           \begin{gather}
             \text{There are unique}~[[GT]],~\target{[[tt1]]},~\text{such}\nonumber\\
             \label{tmelab:let:IH1:GT}
             \text{that}~[[TC ; TT ~> GT]]\\
             \label{tmelab:let:IH1:ty}
             \text{and}~[[ TC ; TT |-ty is1 ~> tt1 ]]\\
             \label{tmelab:let:IH1:wftm}
             \text{and}~[[ GT |-tm te1 : tt1 ]]
           \end{gather}           
           The induction hypothesis for the second premise of rule \textsc{iTm-let} is
           \begin{gather}
             \text{There are unique}~\target{[[GT']]},~\target{[[tt2]]},~\text{such}\nonumber\\
             \label{tmelab:let:IH2:GT}
             \text{that}~[[TC ; TT , ix : is1 ~> GT']]\\
             \label{tmelab:let:IH2:ty}
             \text{and}~[[ TC ; TT , ix : is1 |-ty is2 ~> tt2]]\\
             \label{tmelan:let:IH2:wftm}
             \text{and}~[[ GT' |-tm te2 : tt2]]
           \end{gather}
           By inversion on Equation~\pref{tmelab:let:IH2:GT}, there are $\target{[[GT0]]}$ and $\target{[[tt1']]}$ such
           that
           \begin{gather}
             \label{tmelab:let:1}
             [[TC ; TT ~> GT0]] \\
             \label{tmelab:let:2}
             \text{and}~[[TC ; TT |-ty is1 ~> tt1']] \\
             \text{and}~[[GT' = GT0 , tx : tt1']]\nonumber
           \end{gather}
           By uniqueness (Lemma~\ref{lem:det:GT} on Equations~\pref{tmelab:let:IH1:GT} and
           \pref{tmelab:let:1} and Lemma~\ref{lem:det:ty} on Equations~\pref{tmelab:let:IH1:ty} and
           \pref{tmelab:let:2}), we get $[[GT0 = GT]]$ and $[[tt1' = tt1]]$.
           This refines Equation \pref{tmelan:let:IH2:wftm} into
           \begin{equation}
             \label{tmelab:let:3}
             [[ GT , tx : tt1 |-tm te2 : tt2]]
           \end{equation}
           By applying Lemma~\ref{lem:tyelab} on Equations \pref{tmelab:let:IH1:ty} and
           \pref{tmelab:let:IH1:GT}, we get
           \begin{equation}
             \label{tmelab:let:4}
             [[ GT |-ty tt1 ]]
           \end{equation}
           By applying rule \textsc{tTm-Let} on Equations \pref{tmelab:let:IH1:wftm},
           \pref{tmelab:let:3} and \pref{tmelab:let:4}, we get
           \begin{equation}
             [[GT |-tm tlet tx : tt1 = te1 tin te2 : tt2]]
           \end{equation}
           It remains to show that $[[TC ; TT |-ty is2 ~> tt2]]$. This is easily derived from
           Equation \pref{tmelab:let:IH2:ty}, since the existence of variable $[[tx]]$ in the
           context does not affect the well-formedness nor the translation of $\intermed{[[is2]]}$.\\
          }
\proofStep{Case \textsc{iTm-method}}
          {\ottdruleiTmXXmethod{}}
          {%Hypothesis \pref{thmA:tmelab:hyp:3} of the theorem becomes
%            \([[ TC ; TT |-ty [| is / c |] is' ~> tt0 ]]\).            
%          The goal becomes \([[ GT |-tm te . tl : tt0 ]]\).
          Applying Theorem~\ref{thmA:delab} to the first premise of rule
          \textsc{iTm-method} results in
          \begin{gather}
            \text{There are unique}~[[GT]]~\text{and}~\target{[[tt1]]}~\text{such}~\nonumber\\
            \label{tmelab:meth:IH1:GT}
            \text{that}~[[TC ; TT ~> GT]]\\
            \label{tmelab:meth:IH1:q}
            \text{and}~[[ TC ; TT |-q iTC is ~> tt1 ]]\\
            \label{tmelab:meth:IH1:wftm}
            \text{and}~[[ GT |-tm te : tt1 ]]
          \end{gather}
          By inversion on Equation \pref{tmelab:meth:IH1:q}, we get
          \begin{gather}
            \label{tmelan:meth:1}
            [[TC = TC1, im' : iTC c' : ism, TC2]]\\ % [[( im' : iTC c' : ism ) in TC]]\\
            \label{tmelan:meth:2}
            [[TC ; TT |-ty is ~> tt]]\\
            \label{tmelan:meth:3}
            [[TC1 ; empty , c' |-ty ism ~> ttm]]
          \end{gather}
          for some $\intermed{[[im']]}$, $\intermed{[[c']]}$, $\intermed{[[ism]]}$, $[[tt]]$ and $\target{[[ttm]]}$.
          However, each dictionary $[[iTC]]$ corresponds to a unique entry in the class
          environment $[[TC]]$. By this uniqueness, we get $[[im' = im]]$,
          $[[c = c']]$, $[[ism = is']]$. % im-in-tc
          Then,
          $[[tt1 =  [| tt / ta |] { tl : ttm } ]]$, and Equations \pref{tmelab:meth:IH1:q}
          and \pref{tmelab:meth:IH1:wftm} become
          \begin{gather}
            [[ TC ; TT |-q iTC is ~> [| tt / ta |] { tl : ttm } ]]\nonumber\\
            \label{tmelab:meth:5}
            \text{and}~[[ GT |-tm te : [| tt / ta |] { tl : ttm } ]]
          \end{gather}
          Lemma~\ref{lemma:tvar_tsubst} applied on Equations~\pref{tmelan:meth:2} and
          \pref{tmelan:meth:3}, results in
          \begin{equation*}
            [[TC ; TT |-ty [| is / c |] is' ~> [| tt / ta |] ttm]]
          \end{equation*}
          and rule \textsc{tTm-Proj} instantiated with Equation~\pref{tmelab:meth:5} gives
          $[[GT |-tm te . tl : [| tt / ta |] ttm]]$.\\
          }
\proofStep{Case \textsc{iTm-arrI}}
          {\ottdruleiTmXXarrI{}}
          {
          The induction hypothesis from the first premise of rule \textsc{iTm-arrI} is
          \begin{gather}
            \text{There are unique}~\target{[[GT']]}~\text{and}~\target{[[tt1]]}~\text{such}~\nonumber\\
            \text{that}~[[TC ; TT , ix : is1 ~> GT']]\nonumber\\
            \label{tmelab:arri:IH:ty}
            \text{and}~[[ TC ; TT , ix : is1 |-ty is2 ~> tt2 ]]\\
            \label{tmelab:arri:IH:wftm}
            \text{and}~[[ GT' |-tm te : tt2 ]]
          \end{gather}
          Similarly to the \textsc{iTm-Let} case, $\target{[[GT']]}$ is of the form $[[GT , tx : tt1]]$,
          where
          \begin{gather}
            \label{tmelab:arri:1}
            [[TC ; TT ~> GT]]\\
            \label{tmelab:arri:2}
            \text{and}~[[TC ; TT |-ty is1 ~> tt1]]
          \end{gather}
          In addition, from Lemma~\ref{lem:tyelab} applied on Equation~\pref{tmelab:arri:1} and the
          second premise of rule \textsc{iTm-arrI}, we obtain \([[ GT |-ty tt1 ]]\).

          By instantiating the premises of rule \textsc{tTm-Abs} with the above result and with
          Equation \pref{tmelab:arri:IH:wftm}, we get
          $[[GT |-tm \ tx : tt1 . te : tt1 -> tt2 ]]$, where $[[TC ; TT |-ty is2 ~> tt2]]$. The
          latter holds from Equation \pref{tmelab:arri:IH:ty}, where $[[tx]]$ has been removed
          from the context (it does not affect the well-formedness of type $\intermed{[[is2]]}$). This, in
          combination with Equation \pref{tmelab:arri:2} in rule \textsc{iTy-Arr}, gives
          $[[TC ; TT |-ty is1 -> is2 ~> tt2 -> tt2]]$.\\
          }
\proofStep{Case \textsc{iTm-arrE}}
          {\ottdruleiTmXXarrE{}}
          {
            The induction hypothesis from the first premise of rule \textsc{iTm-arrE} is
            \begin{gather}
              \text{There are unique}~[[GT]]~\text{and}~[[tt]]~\text{such}~\nonumber\\
              \label{tmelab:arre:IH1:GT}
              \text{that}~[[TC ; TT ~> GT]]\\
              \label{tmelab:arre:IH1:ty}
              \text{and}~[[TC ; TT |-ty is1 -> is2 ~> tt]]\\
              \label{tmelab:arre:IH1:wftm}
             \text{and}~[[ GT |-tm te1 : tt ]]
            \end{gather}
            By inversion on Equation~\pref{tmelab:arre:IH1:ty}, $[[tt]]$ can only be of the form
            $\target{[[tt1 -> tt2]]}$ for the $\target{[[tt1]]}$ and $\target{[[tt2]]}$, uniquely determined by equations
            \begin{gather}
              \label{tmelab:arre:1}
              [[TC ; TT |-ty is1 ~> tt1]]\\
              \text{and}~[[TC ; TT |-ty is2 ~> tt2]]\nonumber
            \end{gather}.
            The induction hypothesis from the second premise of rule \textsc{iTm-arrE} is
            \begin{gather}
              \text{There are unique}~\target{[[GT']]}~\text{and}~\target{[[tt1']]}~\text{such}~\nonumber\\
              \label{tmelab:arre:IH2:GT}
              \text{that}~[[TC ; TT ~> GT']]\\
              \label{tmelab:arre:IH2:ty}
              \text{and}~[[ TC ; TT |-ty is1 ~> tt1' ]]\\
              \label{tmelab:arre:IH2:wftm}
              \text{and}~[[ GT |-tm te2 : tt1' ]]
            \end{gather}
            By uniqueness (Lemma~\ref{lem:det:GT}) on Equations \pref{tmelab:arre:IH1:GT} and \pref{tmelab:arre:IH2:GT},
            it must hold that $[[GT' = GT]]$. Also, uniqueness (Lemma~\ref{lem:det:ty}) on Equations
            \pref{tmelab:arre:1} and \pref{tmelab:arre:IH2:ty}, gives $[[tt1' = tt1]]$.

            Combining Equations \pref{tmelab:arre:IH1:wftm} and \pref{tmelab:arre:IH2:wftm},
            (rewritten with the equalities holding so far) in rule \textsc{tTm-App}, we get
            $[[GT |-tm te1 te2 : tt2]]$.\\
          }
\proofStep{Case \textsc{iTm-constrI}}
          {\ottdruleiTmXXconstrI{}}
          {
          The induction hypothesis from the first premise of rule \textsc{iTm-constrI} is
          \begin{gather}
            \text{There are unique}~\target{[[GT']]}~\text{and}~[[tt]]~\text{such}~\nonumber\\
            \text{that}~[[TC ; TT , idvar : iq ~> GT']]\nonumber\\
            \label{tmelab:constrI:IH:ty}
            \text{and}~[[ TC ; TT , idvar : iq |-ty is ~> tt ]]\\
            \label{tmelab:constrI:IH:wftm}
            \text{and}~[[ GT' |-tm te : tt ]]
          \end{gather}
          Similarly to the \textsc{iTm-Let} case, $\target{[[GT']]}$ is of the form $\target{[[GT , txd : ttq]]}$,
          where
          \begin{gather}
            \label{tmelab:constrI:1}
            [[TC ; TT ~> GT]]\\
            \label{tmelab:constrI:2}
            \text{and}~[[TC ; TT |-q iq ~> ttq]]
          \end{gather}
          In addition, from Lemma~\ref{lem:qelab} applied on Equation~\pref{tmelab:constrI:1} and the
          second premise of rule \textsc{iTm-constrI}, we obtain \([[ GT |-ty tt1 ]]\).

          By instantiating the premises of rule \textsc{tTm-Abs} with the above result and with
          Equation \pref{tmelab:constrI:IH:wftm}, we get
          $[[GT |-tm \ tx : ttq . te : ttq -> tt]]$, where $[[TC ; TT |-ty is ~> tt]]$. The
          latter holds from Equation \pref{tmelab:constrI:IH:ty}, where $[[tx]]$ has been
          removed from the context (it does not affect the well-formedness of type $\intermed{[[is2]]}$).
          This, in combination with Equation \pref{tmelab:constrI:2} in rule \textsc{iTy-Qual},
          gives $[[TC ; TT |-ty iq -> is ~> ttq -> tt]]$.\\
          }
\proofStep{Case \textsc{iTm-constrE}}
          {\ottdruleiTmXXconstrE{}}
          {
            The induction hypothesis from the first premise of rule \textsc{iTm-constrE} is
            \begin{gather}
              \text{There are unique}~[[GT]]~\text{and}~\target{[[tt']]}~\text{such}~\nonumber\\
              \label{tmelab:constrE:IH1:GT}
              \text{that}~[[TC ; TT ~> GT]]\\
              \label{tmelab:constrE:IH1:ty}
              \text{and}~[[TC ; TT |-ty iq -> is ~> tt']] \\
              \label{tmelab:constrE:IH1:wftm}
             \text{and}~[[ GT |-tm te1 : tt ]]
            \end{gather}
            By inversion on Equation~\pref{tmelab:constrE:IH1:ty}, $\target{[[tt']]}$ can only be of the form
            $\target{[[ttq -> tt]]}$ for the $\target{[[ttq]]}$ and $[[tt]]$, uniquely determined by equations
            \begin{gather}
              \label{tmelab:constrE:1}
              [[TC ; TT |-q iq ~> ttq]]\\
              \text{and}~[[TC ; TT |-ty is ~> tt]]\nonumber
            \end{gather}
            Theorem~\ref{thmA:delab}, applied to the second premise of rule
            \textsc{iTm-constrE}, is
            \begin{gather}
              \text{There are unique}~\target{[[GT']]}~\text{and}~\target{[[tt0]]}~\text{such}~\nonumber\\
              \label{tmelab:constrE:IH2:GT}
              \text{that}~[[TC ; TT ~> GT']]\\
              \label{tmelab:constrE:IH2:ty}
              \text{and}~[[ TC ; TT |-q iq ~> tt0 ]]\\
              \label{tmelab:constrE:IH2:wftm}
              \text{and}~[[ GT' |-tm te2 : tt0 ]]
            \end{gather}
            By uniqueness (Lemma~\ref{lem:det:GT}) on Equations \pref{tmelab:constrE:IH1:GT} and
            \pref{tmelab:constrE:IH2:GT},
            it must hold that $[[GT' = GT]]$. Also, uniqueness (Lemma~\ref{lem:det:Q}) on Equations
            \pref{tmelab:constrE:1} and \pref{tmelab:constrE:IH2:ty}, gives
            $[[tt0 = ttq]]$.

            Combining Equations \pref{tmelab:constrE:IH1:wftm} and
            \pref{tmelab:constrE:IH2:wftm}, (rewritten with the above-mentioned equalities) in
            rule \textsc{tTm-App}, we get $[[GT |-tm te1 te2 : tt]]$.\\
          }
\proofStep{Case \textsc{iTm-forallI}}
          {\ottdruleiTmXXforallI{}}
          {The induction hypothesis for the premise of rule \textsc{iTm-forallI} is the
            following.
            \begin{gather}
              \text{There are unique}~\target{[[GT']]}~\text{and}~[[tt]]~\text{such}~\nonumber\\
              \label{tmelab:foralli:IH:GT}
              \text{that}~[[TC ; TT , c ~> GT']]\\
              \label{tmelab:foralli:IH:ty}
              \text{and}~[[TC ; TT , c |-ty is ~> tt]]\\
              \label{tmelab:foralli:IH:wftm}
              \text{and}~[[GT' |-tm te : tt]]
            \end{gather}
            By inversion on Equation~\pref{tmelab:foralli:IH:GT}, $\target{[[GT']]}$ can only be of the form
            $\target{[[GT , ta]]}$, where $[[GT]]$ uniquely determined by
            \begin{equation*}
              [[TC ; TT ~> GT]]
            \end{equation*}
            Then, Equation \pref{tmelab:foralli:IH:wftm} becomes
            \begin{equation*}
              [[GT , ta |-tm te : tt]]
            \end{equation*}
            Using this to instantiate rule \textsc{tTm-Tabs}, we get
            \begin{equation*}
              [[GT |-tm /\ ta . te : \/ ta . tt]]
            \end{equation*}
            where, by rule \textsc{iTy-scheme} on Equation~\pref{tmelab:foralli:IH:ty}, it follows that
            $[[TC ; TT |-ty \/ c . is ~> \/ ta . tt]]$.\\
          }
\proofStep{Case \textsc{iTm-forallE}}
          {\ottdruleiTmXXforallE{}}
          {The induction hypothesis from the first premise of rule \textsc{iTm-forallE} is as
            follows.
            \begin{gather}
              \text{There are unique}~[[GT]]~\text{and}~\target{[[tt0]]}~\text{such}~\nonumber\\
              \label{tmelab:forallE:IH2:GT}
              \text{that}~[[TC ; TT ~> GT]]\\
              \label{tmelab:forallE:IH2:ty}
              \text{and}~[[ TC ; TT |-ty \/ c . is' ~> tt0 ]]\\
              \label{tmelab:forallE:IH2:wftm}
              \text{and}~[[ GT |-tm te : tt0 ]]
            \end{gather}
            By inversion on Equation~\pref{tmelab:forallE:IH2:ty}, $\target{[[tt0]]}$ can only be of the form
            $\target{[[\/ ta . tt']]}$, where $\target{[[tt']]}$ is uniquely determined by equation
            \begin{equation}
              \label{tmelab:forallE:1}
              [[TC ; TT , c |-ty is' ~> tt']]
            \end{equation}
            Lemma~\ref{lemma:tvar_tsubst}, applied on the second premise of rule
            \textsc{iTm-forallE} and on Equation~\pref{tmelab:forallE:1}, results in
            $[[TC ; TT |-ty [| is / c |] is' ~> [| tt / ta |] tt']]$.

            Also, Lemma~\ref{lem:tyelab} applied on the second premise of rule
            \textsc{iTm-forallE} and on Equation~\pref{tmelab:forallE:IH2:GT} results in
            $[[GT |-ty tt]]$.
            We use the latter, together with Equation \pref{tmelab:forallE:IH2:wftm}, to
            instantiate rule \textsc{tTm-Tapp}, which concludes
            $[[GT |-tm te : [| tt / ta |] tt']]$.
          }
\qed

\begin{theoremB}[Dictionary Elaboration Soundness]
\label{thmA:delab}
% \setcounter{equation}{0}
  \begin{flalign}
  &\text{If}~[[ SS ; TC ; TT |-d idvar : iq ~> te ]]\label{delab:hyp} &\\
  &\text{then, there are unique}~[[GT]]~\text{and}~[[ tt ]]~\text{such that}\nonumber &\\
  &[[TC ; TT ~> GT ]]\label{delab:res1} &\\
  &\text{and}~[[ TC ; TT |-q iq ~> tt ]]\label{delab:res2} &\\
  &\text{and}~[[GT |-tm te : tt]]\label{delab:res3}
  \end{flalign}
\end{theoremB}

\proof
This theorem is proved mutually with Theorem~\ref{thmA:tmelab}. The proof follows
structural induction on the first hypothesis.\\
\proofStep{Case \textsc{D-var}}
          {\ottdruleDXXvar{}}
          {By Lemma~\ref{lem:elab:dvar}, there exist $[[GT]]$ and $[[tt]]$ such that
           $[[TC ; TT ~> GT]]$ and
            $[[TC ; TT |-q iTC is ~> tt]]$ and $[[( txd : tt ) in GT]]$. This satisfies
            Equations \pref{delab:res1} and \pref{delab:res2} of the theorem.

            By instantiating rule \textsc{tTm-Var} on $[[( txd : tt ) in GT]]$, we get
            $[[GT |-tm txd : tt]]$, which satisfies Equation \pref{delab:res3} of the
            theorem.\\
          }
\proofStep{Case \textsc{D-con}}
          {\ottdruleDXXcon{}}
          { We need to show that there exist $\target{[[GT0]]}$ and $[[tt]]$ such that
            $[[TC ; TT ~> GT0]]$ and
            \begin{gather}
              \label{delab:dcon:goal:ty}
              [[TC ; TT |-q iTC [| islj / clj |] isq ~> tt ]]\\
              \label{delab:dcon:goal:te_rec}
              [[GT0 |-tm (/\ taj . \ </ txdi : tti' // i />. { tl = te }) ttlj teli : tt]]
            \end{gather}
            From the 2\textsuperscript{nd} premise of rule \textsc{D-con}, applied on Lemma
            \ref{lem:ctx_elab}, there is a unique $[[GT]]$ such that
            \begin{gather}
              \label{delab:dcon:GT}
              [[TC ; TT ~> GT]]\\
              \nonumber
              [[|-ctx GT]]
            \end{gather}
            We thus take $[[GT0 = GT]]$.
            
            Next, we will try to refine type $[[tt]]$.
            By Lemma
            \ref{lemma:inSS2C} applied on the first premise of rule \textsc{D-con}, there are
            $[[c]]$, $\target{[[tt0]]}$ and $\target{[[ttli]]}$ such that
            \begin{gather}
              \label{delab:dcon:im}
              [[( im : iTC c : ism ) in TC ]]\\
              \label{delab:dcon:iqli}
              \text{and}~[[</ TC ; empty , clj |-q iqi ~> tti''// i />]]\\
              \label{delab:dcon:iq}
              \text{and}~[[TC ; empty , clj |-q iTC isq ~> tt0]]
            \end{gather}
            Since Equation \pref{delab:dcon:iq} holds, the premises of the only rule that
            applies, namely rule \textsc{iQ-TC}, must hold as well.
            \begin{gather}
              \label{delab:dcon:isq}
              [[TC ; empty , clj |-ty isq ~> ttq]]\\
              \label{delab:dcon:im'}
              [[TC = TC1, im' : iTC c' : ism', TC2]]\\
              \label{delab:dcon:ism}
              [[TC1 ; empty , c |-ty ism' ~> ttm]]
            \end{gather}
            for some $\intermed{[[im']]}$, $\intermed{[[c']]}$, $\intermed{[[ism']]}$, $\target{[[ttq]]}$ and $\target{[[ttm]]}$, where
            $[[tt0  =  [| ttq / ta' |] { tl' : ttm }]]$.
            By uniqueness on Equations \pref{delab:dcon:im} and \pref{delab:dcon:im'}, we get
            $[[im' = im]]$, $[[c = c']]$,  $[[ism' = ism]]$. Then,
            $[[tt0 =  [| ttq / ta |] { tl : ttm }  = { tl : [| ttq / ta |] ttm }]]$.
            By Lemma~\ref{lemma:tvar_tsubst_iq} applied on Equation~\pref{delab:dcon:isq} and
            the 4\textsuperscript{th} set of premises of rule \textsc{D-con}, Goal
            \pref{delab:dcon:goal:ty} is satisfied with
            $[[tt = { tl : [| </ ttj / taj // j /> |] [| ttq / ta |] ttm }]]$.

            Then, Goal \pref{delab:dcon:goal:te_rec} becomes
            \begin{equation}
              \label{delab:dcon:goal:te_ref}
              [[GT |-tm (/\ taj . \ </ txdi : tti' // i />. { tl = te }) ttlj teli : { tl : [| </ ttj / taj // j /> |] [| ttq / ta |] ttm }]]
            \end{equation}
%            Also, from Lemma~\ref{lem:det:Q} applied on equation \pref{delab:dcon:iq} and on
%            the corresponding premise of rule \textsc{D-con}, we get $[[tti'' = tti']]$.
            For that, it suffices to show that
            \begin{gather}
              \label{delab:dcon:goal:te}
              [[GT , talj , </ txdi : tti'// i /> |-tm te : [| ttq / ta |] ttm]]\\
              \label{delab:dcon:goal:ttjs}
              [[</ GT |-ty ttj // j />]]\\
              \label{delab:dcon:goal:teis}
              \text{and}~[[</ GT |-tm tei : [| </ ttj / taj // j /> |] tti' // i />]]
            \end{gather}
            because, then we can use rules \textsc{tTm-Rec}, \textsc{tTm-Tapp} and
            \textsc{tTm-App} to reach Equation~\pref{delab:dcon:goal:te_ref}.
            
            \paragraph{For Goal~\pref{delab:dcon:goal:ttjs}}
            Passing the 4\textsuperscript{th} set of premises of rule \textsc{D-con} in Lemma
            \ref{lem:qelab}, we get $[[</ GT |-ty ttj // j />]]$, satisfying
            Equation~\pref{delab:dcon:goal:ttjs}. 

            \paragraph{For Goal~\pref{delab:dcon:goal:te}}
            Theorem~\ref{thmA:tmelab}, applied to the 5\textsuperscript{th} premise of rule
            \textsc{D-con}, is:
            \begin{gather}
              \text{There are}~\target{[[GT']]}~\text{and}~\target{[[tt0]]}~\text{such that}\nonumber\\
              [[TC ; empty , clj , idvarli : iqli ~> GT']]\nonumber\\
              \text{and}~[[TC ; empty , clj , idvarli : iqli |-ty [| isq / c |] ism ~> tt0]]\label{delab:dcon:IH5:tt}\\
              \text{and}~[[GT' |-tm te : tt0]].\label{delab:dcon:IH1:wftm}
            \end{gather}
            It is easy to verify that $[[GT' = tempty , talj , </ txdi : tti' //i />]]$.
            From Lemma~\ref{lemma:ty_weakening} on Equation \pref{delab:dcon:ism}, we get
            the weakened equation
            \begin{equation*}
              [[TC ; empty , c |-ty ism ~> ttm]]
            \end{equation*}
            where $[[TC]]$ is specified in Equation~\pref{delab:dcon:im'}.
            Using this result together with Equation \pref{delab:dcon:isq} in Lemma
            \ref{lemma:tvar_tsubst}, we get
            $[[TC ; empty , clj |-ty [|isq / c|] ism ~> [| ttq / ta |] ttm]]$, which we weaken
            as 
            \begin{equation*}
              [[TC ; empty , clj , idvarli : iqli |-ty [|isq / c|] ism ~> [| ttq / ta |] ttm]]
            \end{equation*}
            Then, by uniqueness on the latter and on Equation \pref{delab:dcon:IH5:tt}, we have
            $[[tt0 =  [| ttq / ta |] ttm ]]$, and Equation \pref{delab:dcon:IH1:wftm}
            becomes
            \begin{equation*}
              [[tempty , talj , </ txdi : tti' //i /> |-tm te : [| ttq / ta |] ttm]]
            \end{equation*}
            Prefixing the typing environment of the above with $[[GT]]$, Goal
            \pref{delab:dcon:goal:te} is satisfied.

            \paragraph{For Goal~\pref{delab:dcon:goal:teis}} The 6\textsuperscript{th} set of
            premises of rule \textsc{D-con} induces, for each $i$, the following induction
            hypothesis.
            \begin{gather}
              \text{There are}~\target{[[GTi]]}~\text{and}~\target{[[tt''i]]}~\text{such that}\nonumber\\
              \label{delab:dcon:IHi:GT}
              [[TC ; TT ~> GTi]]\\
              \label{delab:dcon:IHi:q}
              [[TC ; TT |-q [| islj / clj |] iqi ~> tt''i ]] \\
              \label{delab:dcon:IHi:wftm}
              \text{and}~[[GTi |-tm tei : tt''i]]
            \end{gather}
            From Equations \pref{delab:dcon:GT} and \pref{delab:dcon:IHi:GT} in Lemma
            \ref{lem:det:GT}, we have $[[GTi = GT]]$.
            For each equation in the 3\textsuperscript{rd} set of premises of rule
            \textsc{D-con}, we appply Lemma~\ref{lemma:tvar_tsubst_iq} multiple times with the
            4\textsuperscript{th} set of premises of rule \textsc{D-con}, to get
            \begin{equation*}
              [[</ TC ; TT |-q [| islj / clj|] iqi ~> [| </ ttj / taj // j />|] tti' //i />]]
            \end{equation*}
            Then $[[tti'' =  [| </ ttj / taj // j />|] tti' ]]$, for all $i$, and Equation
            \pref{delab:dcon:IHi:wftm} satisfies Goal \pref{delab:dcon:goal:teis}.
            }
\qed

\subsection{Determinism}
\begin{theoremB}[Deterministic Dictionary Elaboration]\ \\
  % \setcounter{equation}{0}
  \label{thmA:delab:det}
  If \([[ SS ; TC ; TT |-d id : iq ~> te1 ]]\)
  and \([[ SS ; TC ; TT |-d id : iq ~> te2 ]]\),
  then \([[ te1  =  te2 ]]\).
\end{theoremB}
\proof This theorem is proved mutually with Theorem~\ref{thmA:tmelab:det}. The proof follows
structural induction on both hypotheses.\\\\
\proofStep{Case \textsc{D-var}}
          {}
          {The first and second hypotheses of the theorem are:
            \begin{gather*}
              [[SS ; TC ; TT |-d idvar : iq ~> txd1]]\\
              \text{and}~[[ SS ; TC ; TT |-d idvar : iq ~> txd2]]
            \end{gather*}
            From the convention regarding namespace translations, explained
            in Section~\ref{sec:namespace_translation}, it follows directly that
            $[[txd1 = txd2 = txd]]$.\\
          }
\proofStep{Case \textsc{D-con}}
          {}
          {The first and second hypotheses of the theorem are:
            \begin{gather}
              \label{delab:det:dcon:1}
              [[SS ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> ( /\ talj . \ </ txdi : tt'i // i /> . { tl = te } ) ttlj teli]]\\
              \label{delab:det:dcon:2}
              \text{and}~
              [[SS ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> ( /\ talj . \ </ txdi' : tt''i // i /> . { tl' = te' } ) ttlj' teli']]
            \end{gather}
            The 5\textsuperscript{th} premise of the two instantiations of rule \textsc{D-con},
            are
            \begin{gather}
              \label{delab:det:dcon:3}
              [[SS1 ; TC ; empty, clj , idvarli : iqli |-tm ie : [| isq / c |] ism ~> te]]\\
              \label{delab:det:dcon:4}
              \text{and}~
              [[SS1 ; TC ; empty, clj , idvarli' : iqli' |-tm ie : [| isq / c |] ism ~> te']]
            \end{gather}
            and the 1\textsuperscript{st} premise of the two \textsc{D-con} rules are
            \begin{gather*}
              [[( iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli . ie in SS]]\\
              [[( iD : \/ clj . iqli' => iTC isq) . im' |-> /\ clj . \ idvarl'i : iql'i . ie in SS]]
            \end{gather*}
            However, a valid method-implementations environment, like $[[SS]]$ in this case,
            contains a unique entry for each constructor $[[iD]]$. From the two above premises
            and this uniqueness property, we have that
            \begin{equation}
              \label{delab:det:dcon:nm_eqs}
            \begin{aligned}
              [[iqli' = iqli]]~~\text{and}~~[[idvarli' = idvarli]] &,~~\text{for all}~i\\
              \text{and}~[[im' = im]]&
            \end{aligned}
            \end{equation}
            By applying these equations to Equations
            \pref{delab:det:dcon:3} and \pref{delab:det:dcon:4}, their typing environment
            becomes identical. We can, now, use Theorem~\ref{thmA:tmelab:det} on these two equations,
            from which we get $[[te = te']]$.
            Also, from the namespace-translation convention, we get $[[tl' = tl]]$ and
            $[[txdli' = txdli]]$.

            If we rewrite Equations \pref{delab:det:dcon:1} and \pref{delab:det:dcon:2} with the
            equations obtained so far, we have
            \begin{gather}
              \label{delab:det:dcon:5}
              [[SS ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> ( /\ talj . \ </ txdi : tt'i // i /> . { tl = te } ) ttlj teli]]\\
              \label{delab:det:dcon:6}
              \text{and}~
              [[SS ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> ( /\ talj . \ </ txdi : tt''i // i /> . { tl = te } ) ttlj' teli']]
            \end{gather}
            From Equations~\pref{delab:det:dcon:nm_eqs} and the 3\textsuperscript{rd} set
            of premises of the two \textsc{D-con} instantiations in Equations~\pref{delab:det:dcon:5} and
            \pref{delab:det:dcon:6}, we get
            \begin{gather*}
              [[</ TC ; empty , clj |-q iqi ~> tt'i // i />]]\\
              \text{and}~[[</ TC ; empty , clj |-q iqi ~> tt''i // i />]]
            \end{gather*}
            By passing the two above in Lemma~\ref{lem:det:Q}, we get
            $[[tt''i = tt'i]]$, for all $i$.

            From the 4\textsuperscript{th} set of premises of the two \textsc{D-con}
            instantiations in Equations~\pref{delab:det:dcon:5} and \pref{delab:det:dcon:6}, we get
            \begin{gather}
              [[</ TC ; TT |-ty isj ~> ttj // j />]]\\
              \text{and}~[[</ TC ; TT |-ty isj ~> ttj' // j />]]
            \end{gather}
            By passing the two above in Lemma~\ref{lem:det:ty}, we get
            $[[tt'j = ttj]]$, for all $j$.

            From the 6\textsuperscript{th} set of premises of the two \textsc{D-con}
            instantiations in Equations~\pref{delab:det:dcon:5} and \pref{delab:det:dcon:6}, we get
            \begin{gather}
              [[</ SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei // i />]]\\
              \text{and}~[[</ SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei' // i />]]
            \end{gather}
            From the induction hypothesis for the two above equations, we have
            $[[tei' = tei]]$, for all $i$.

            Rewritting the derivations in Equations~\pref{delab:det:dcon:5} and \pref{delab:det:dcon:6}
            with the new equations obtained, we have
            \begin{equation*}
              [[( /\ talj . \ </ txdi : tt''i // i /> . { tl = te } ) ttlj' teli' =
                ( /\ talj . \ </ txdi : tt'i // i /> . { tl = te } ) ttlj teli]]
            \end{equation*}
         }
\qed

\begin{theoremB}[Deterministic Term Elaboration]\ \\
  % \setcounter{equation}{0}
  \label{thmA:tmelab:det}
  If \([[ SS ; TC ; TT |-tm ie : is ~> te1 ]]\)
  and \([[ SS ; TC ; TT |-tm ie : is ~> te2 ]]\),
  then \([[ te1  =  te2 ]]\).
\end{theoremB}
\proof This theorem is proved mutually with Theorem~\ref{thmA:delab:det}. The proof follows
structural induction on both hypotheses.\\\\
\proofStep{Case \textsc{iTm-true}}{}
          {The two hypotheses of the theorem are:
            \begin{align*}
              &[[SS ; TC ; TT |-tm itrue : ibool ~> te1]]\\
              \text{and}~&[[SS ; TC ; TT |-tm itrue : ibool ~> te2]]
            \end{align*}
            From rule \textsc{iTm-true}, it must hold that $[[te1 = te2 = ttrue]]$.\\
          }
\proofStep{Case \textsc{iTm-false}}{}
          {The two hypotheses of the theorem are:
            \begin{align*}
              &[[SS ; TC ; TT |-tm ifalse : ibool ~> te1]]\\
              \text{and}~&[[SS ; TC ; TT |-tm ifalse : ibool ~> te2]]
            \end{align*}
            From rule \textsc{iTm-false}, it must hold that $[[te1 = te2 = tfalse]]$.\\
          }
\proofStep{Case \textsc{iTm-var}}{}
          {The two hypotheses of the theorem are:
            \begin{align*}
              [[SS ; TC ; TT |-tm ix : is ~> tx1]]\\
              \text{and}~[[SS ; TC ; TT |-tm ix : is ~> tx2]]
            \end{align*}
            From rule \textsc{iTm-var}, it must hold that $[[tx1 = tx2 = tx]]$, where
            $[[tx]]$ is a target-term-variable with the same identifier as $[[ix]]$.\\
          }
\proofStep{Case \textsc{iTm-let}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmelab:det:let:hyp1}
              &[[SS ; TC ; TT |-tm ilet ix : is1 = ie1 iin ie2 : is2 ~> tlet tx0 : tt1 = te1 tin te2]]\\
              \label{tmelab:det:let:hyp2}
              \text{and}~&[[SS ; TC ; TT |-tm ilet ix : is1 = ie1 iin ie2 : is2 ~> tlet tx0' : tt1' = te1' tin te2']]
            \end{align}
            From our convention regarding translation of identifiers, we have
            \begin{equation}
              \label{tmelab:det:let:tx}
              [[tx0 = tx0' = tx]]
            \end{equation}
            where $[[tx]]$ is a target-term variable with the same identifier as $[[ix]]$.
            
            The first premise of the two \textsc{iTm-let} instantiations above, are
            \begin{align*}
              [[SS ; TC ; TT |-tm ie1 : is1 ~> te1]]\\
              \text{and}~[[SS ; TC ; TT |-tm ie1 : is1 ~> te1']]
            \end{align*}
            By induction hypothesis, we get
            \begin{equation}
              \label{tmelab:det:let:te1}
              [[te1 = te1']]
            \end{equation}
            The 3\textsuperscript{rd} premise of the two instantiations in Equations
            \pref{tmelab:det:let:hyp1} and \pref{tmelab:det:let:hyp2} of rule \text{iTm-let}
            are:
            \begin{align*}
              [[TC ; TT |-ty is1 ~> tt1]]\\
              \text{and}~[[TC ; TT |-ty is1 ~> tt1']]
            \end{align*}
            By uniqueness (Lemma~\ref{lem:det:ty}), we get
            \begin{equation}
              \label{tmelab:det:let:tt1}
              [[tt1 = tt1']]
            \end{equation}
            The 2\textsuperscript{nd} premise of the two instantiations in Equations
            \pref{tmelab:det:let:hyp1} and \pref{tmelab:det:let:hyp2} of rule \text{iTm-let}
            are:
            \begin{align*}
              [[SS ; TC ; TT , ix : is1 |-tm ie2 : is2 ~> te2]]\\
              \text{and}~[[SS ; TC ; TT , ix : is1 |-tm ie2 : is2 ~> te2']]
            \end{align*}
            By induction hypothesis, we get
            \begin{equation}
              \label{tmelab:det:let:te2}
              [[te2 = te2']]
            \end{equation}
            From Equations~\pref{tmelab:det:let:tx}, \pref{tmelab:det:let:te1},
            \pref{tmelab:det:let:tt1} and \pref{tmelab:det:let:te2}, we obtain
            \begin{equation*}
              [[tlet tx0 : tt1 = te1 tin te2 =
                tlet tx0' : tt1' = te1' tin te2']]
            \end{equation*}
          }
\proofStep{Case \textsc{iTm-method}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmelab:det:meth:hyp1}
              &[[SS ; TC ; TT |-tm id . im : [| isq / c |] ism ~> te . tl0]]\\
              \label{tmelab:det:meth:hyp2}
              \text{and}~&[[SS ; TC ; TT |-tm id . im : [| isq / c |] ism ~> te' . tl0']]
            \end{align}
            By our convention for dictionary labels, we have
            \begin{equation*}
              [[tl0 = tl0' = tl]]
            \end{equation*}
            where $[[tl]]$ is a record field with the same identifier as class method $[[im]]$.

            The first premise of the two \textsc{iTm-method} instantiations in Equations
            \pref{tmelab:det:meth:hyp1} and \pref{tmelab:det:meth:hyp2} are:
            \begin{align*}
                         &[[SS ; TC ; TT |-d id : iTC isq ~> te]]\\
              \text{and}~&[[SS ; TC ; TT |-d id : iTC isq ~> te']]
            \end{align*}
            By Theorem~\ref{thmA:delab:det}, we have
            \begin{equation*}
              [[te = te']]
            \end{equation*}
            Then, $[[te . tl0 = te' . tl0']]$.\\
          }
\proofStep{Case \textsc{iTm-arrI}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmelab:det:arri:hyp1}
              &[[SS ; TC ; TT |-tm \ ix : is1 . ie : is1 -> is2 ~> \ tx0 : tt1 . te]]\\
              \label{tmelab:det:arri:hyp2}
              \text{and}~&[[SS ; TC ; TT |-tm \ ix : is1 . ie : is1 -> is2 ~> \ tx0' : tt1' . te']]
          \end{align}
          From our identifiers' translation, it is implied that
          \begin{equation}
            \label{tmelab:det:arri:eq_tx}
            [[tx0 = tx0']]= [[tx]]
          \end{equation}
          where $[[tx]]$ is the target-term variable with the same identifier as $[[ix]]$.

          The 2\textsuperscript{nd} premise of the two \textsc{iTm-arrI} instantiations above
          are:
          \begin{align*}
                       &[[TC ; TT |-ty is1 ~> tt1]]\\
            \text{and}~&[[TC ; TT |-ty is1 ~> tt1']]
          \end{align*}
          By uniqueness (Lemma~\ref{lem:det:ty}), we have
          \begin{equation}
            \label{tmelab:det:arri:eq_tt1}
            [[tt1 = tt1']]
          \end{equation}
          The first premise of the two \textsc{iTm-arrI} instantiations in Equations
          \pref{tmelab:det:arri:hyp1} and \pref{tmelab:det:arri:hyp2} are:
          \begin{align*}
                       &[[SS ; TC ; TT , ix : is1 |-tm ie : is2 ~> te]]\\
            \text{and}~&[[SS ; TC ; TT , ix : is1 |-tm ie : is2 ~> te']]
          \end{align*}
          By the induction hypothesis, we get
          \begin{equation}
            \label{tmelab:det:arri:eq_te}
            [[te = te']]
          \end{equation}
          From Equations~\pref{tmelab:det:arri:eq_tx}, \pref{tmelab:det:arri:eq_tt1} and
          \pref{tmelab:det:arri:eq_te}, we obtain
          \begin{equation*}
            [[\ tx0 : tt1 . te = \ tx0' : tt1' . te']]
          \end{equation*}
          }
\proofStep{Case \textsc{iTm-arrE}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmelab:det:arre:hyp1}
                         &[[SS ; TC ; TT |-tm ie1 ie2 : is2 ~> te1 te2]]\\
              \label{tmelab:det:arre:hyp2}
              \text{and}~&[[SS ; TC ; TT |-tm ie1 ie2 : is2 ~> te1' te2']]
            \end{align}
            The first premise of the above two instantiated \textsc{iTm-arrE} rules are:
            \begin{align*}
                         &[[SS ; TC ; TT |-tm ie1 : is1 -> is2 ~> te1]]\\
              \text{and}~&[[SS ; TC ; TT |-tm ie1 : is1 -> is2 ~> te1']]
            \end{align*}
            By induction hypothesis, we have
            \begin{equation}
              \label{tmelab:det:arre:eq_te1}
              [[te1 = te1']]
            \end{equation}
            Similarly, from the second premise of the two \textsc{iTm-arrE} rules, and the
            induction hypothesis, we get
            \begin{equation}
              \label{tmelab:det:arre:eq_te2}
              [[te2 = te2']]
            \end{equation}
            Then, we obtain
            \begin{equation*}
              [[te1 te2 = te1' te2']]
            \end{equation*}
            by Equations~\pref{tmelab:det:arre:eq_te1} and \pref{tmelab:det:arre:eq_te2}.\\
          }
\proofStep{Case \textsc{iTm-constrI}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmelab:det:constri:hyp1}
              &[[SS ; TC ; TT |-tm \ idvar : iq . ie : iq -> is ~> \ txd0 : tt . te]]\\
              \label{tmelab:det:constri:hyp2}
              \text{and}~&[[SS ; TC ; TT |-tm \ idvar : iq . ie : iq -> is ~> \ txd0' : tt' . te']]
            \end{align}
            From our identifiers' translation, it is implied that
          \begin{equation}
            \label{tmelab:det:constri:eq_txd}
            [[txd0 = txd0']]= [[txd]]
          \end{equation}
          where $[[txd]]$ is the target-term variable with the same identifier as the
          dictionary variable $[[idvar]]$.

          The 2\textsuperscript{nd} premise of the two \textsc{iTm-constrI} instantiations above
          are:
          \begin{align*}
                       &[[TC ; TT |-q iq ~> tt]]\\
            \text{and}~&[[TC ; TT |-q iq ~> tt']]
          \end{align*}
          By uniqueness (Lemma~\ref{lem:det:Q}), we have
          \begin{equation}
            \label{tmelab:det:constri:eq_tt}
            [[tt = tt']]
          \end{equation}
          The first premise of the two \textsc{iTm-constrI} instantiations in Equations
          \pref{tmelab:det:constri:hyp1} and \pref{tmelab:det:constri:hyp2} are:
          \begin{align*}
                       &[[SS ; TC ; TT , idvar : iq |-tm ie : is ~> te]]\\
            \text{and}~&[[SS ; TC ; TT , idvar : iq |-tm ie : is ~> te']]
          \end{align*}
          By the induction hypothesis, we get
          \begin{equation}
            \label{tmelab:det:constri:eq_te}
            [[te = te']]
          \end{equation}
          From Equations~\pref{tmelab:det:constri:eq_txd}, \pref{tmelab:det:constri:eq_tt} and
          \pref{tmelab:det:constri:eq_te}, we obtain
          \begin{equation*}
            [[\ txd0 : tt . te = \ txd0' : tt' . te']]
          \end{equation*}
          }
\proofStep{Case \textsc{iTm-constrE}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmelab:det:constre:hyp1}
                         &[[SS ; TC ; TT |-tm ie id : is ~> te1 te2]]\\
              \label{tmelab:det:constre:hyp2}
              \text{and}~&[[SS ; TC ; TT |-tm ie id : is ~> te1' te2']]
            \end{align}
            The first premise of the above two instantiated \textsc{iTm-constrE} rules are:
            \begin{align*}
                         &[[SS ; TC ; TT |-tm ie : iq -> is ~> te1]]\\
              \text{and}~&[[SS ; TC ; TT |-tm ie : iq -> is ~> te1']]
            \end{align*}
            By induction hypothesis, we have
            \begin{equation}
              \label{tmelab:det:constre:eq_te1}
              [[te1 = te1']]
            \end{equation}
            Similarly, from the second premise of the two \textsc{iTm-constrE} rules, and the
            induction hypothesis, we get
            \begin{equation}
              \label{tmelab:det:constre:eq_te2}
              [[te2 = te2']]
            \end{equation}
            Then, we obtain
            \begin{equation*}
              [[te1 te2 = te1' te2']]
            \end{equation*}
            by Equations~\pref{tmelab:det:constre:eq_te1} and \pref{tmelab:det:constre:eq_te2}.\\}
\proofStep{Case \textsc{iTm-forallI}}{}
          {The two hypotheses of the theorem are:
            \begin{align*}
                         &[[SS ; TC ; TT |-tm /\ c . ie : \/ c . is ~> /\ ta0 . te]]\\
              \text{and}~&[[SS ; TC ; TT |-tm /\ c . ie : \/ c . is ~> /\ ta0' . te']]
            \end{align*}
            It is implied by our identifiers' translation convention, that
            \begin{equation}
              \label{tmelab:det:foralli:eq_ta}
              [[ta0 = ta0' = ta]]
            \end{equation}
            where $[[ta]]$ is the target-type variable with the same identifier as the $[[c]]$.

            The premise of the two \textsc{iTm-forallI} instantiations above are:
            \begin{align*}
                         &[[SS ; TC ; TT , c |-tm ie : is ~> te]]\\
              \text{and}~&[[SS ; TC ; TT , c |-tm ie : is ~> te']]
            \end{align*}
            By the induction hypothesis, we have
            \begin{equation}
              \label{tmelab:det:foralli:eq_te}
              [[te = te']]
            \end{equation}
            Equations~\pref{tmelab:det:foralli:eq_ta} and \pref{tmelab:det:foralli:eq_te}
            result in
            \begin{equation*}
              [[/\ ta0 . te = /\ ta0' . te']]
            \end{equation*}
          }
\proofStep{Case \textsc{iTm-forallE}}{}
          {The two hypotheses of the theorem are:
            \begin{align}
              \label{tmleba:det:foralle:prem1}
                         &[[SS ; TC ; TT |-tm ie is : [| is / c |] is' ~> te tt]]\\
              \label{tmleba:det:foralle:prem1'}
              \text{and}~&[[SS ; TC ; TT |-tm ie is : [| is / c |] is' ~> te' tt']]
            \end{align}
            The first premise of the above two instantiations of rule \textsc{iTm-forallE} are:
            \begin{align*}
                         &[[SS ; TC ; TT |-tm ie : \/ c . is' ~> te]]\\
              \text{and}~&[[SS ; TC ; TT |-tm ie : \/ c . is' ~> te']]
            \end{align*}
            From the induction hypothesis, we get
            \begin{equation}
              \label{tmelab:det:foralle:eq_te}
              [[te = te']]
            \end{equation}
            The second premise of the two instantiations of rule
            \textsc{iTm-forallE} in Equations
            \pref{tmleba:det:foralle:prem1} and \pref{tmleba:det:foralle:prem1'} are:
            \begin{align*}
                          [[TC ; TT |-ty is ~> tt]]
              \text{and}~&[[TC ; TT |-ty is ~> tt']]
            \end{align*}
            Applying Lemma~\ref{lem:det:ty} on these equations gives
            \begin{equation}
              \label{tmelab:det:foralle:eq_tt}
              [[tt = tt']]
            \end{equation}
            From Equations~\pref{tmelab:det:foralle:eq_te} and \pref{tmelab:det:foralle:eq_tt}
            we have
            \begin{equation*}
              [[te tt = te' tt']]
            \end{equation*}
          }
\qed

\begin{theoremB}[Deterministic Context Elaboration]\ \\
  \label{thmA:ctxelab:det}
  If \([[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM1 ]]\)
  and \([[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM2
  ]]\), \\
  then \([[ tM1 = tM2 ]]\).
\end{theoremB}

\proof
This proof proceeds by straightforward structural induction on both hypotheses,
in combination with Lemmas~\ref{lem:det:Q} and~\ref{lem:det:ty} and
Theorems~\ref{thmA:delab:det} and~\ref{thmA:tmelab:det}. \\
\qed

\subsection{Semantic Preservation}
\begin{theoremB}[Semantic Preservation]
  \label{thmA:sem_pres}
  % \setcounter{equation}{0}
  \begin{flalign}
    &\text{If}~[[ SS |- ie --> ie' ]]\nonumber &\\
    \label{semelab:hyp1}
    &\text{and}~[[ SS ; TC ; empty |-tm ie : is ~> te ]] &\\
    \label{semelab:hyp2}
    &\text{and}~[[ SS ; TC ; empty |-tm ie' : is ~> te' ]] &\\
    &\text{for some}~[[is]],~[[te]]~\text{and}~\target{[[te']]},\nonumber &\\
    &\text{then, there is an}~\target{[[teh]]}~\text{such that}\nonumber &\\
    &[[ te -->> teh ]]~\text{and}~[[ te' -->> teh]].\nonumber
  \end{flalign}
\end{theoremB}

\proof This proof proceeds by induction on the first hypothesis.

\proofStep{Case \textsc{iEval-app}}{\drule{iEval-app}}
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align*}
                         &[[SS ; TC ; empty |-tm ie1 ie2 : is2 ~> te1 te2]]\\
              \text{and}~&[[SS ; TC ; empty |-tm ie1' ie2 : is2 ~> te1' te2]]
            \end{align*}
            for some $\intermed{[[is2]]}$, $\target{[[te1]]}$, $\target{[[te1']]}$ and $\target{[[te2]]}$.
            
            The last rule of these derivations must be instances of \textsc{iTm-arrE}. For
            Hypothesis \pref{semelab:hyp1}, we have:
            \begin{equation}
              \label{semelab:app:der1}
            \ottdrule['']{
              \ottpremise{[[SS ; TC ; empty |-tm ie1 : is1 -> is2 ~> te1]]}
              \ottpremise{[[SS ; TC ; empty |-tm ie2 : is1 ~> te2]]}
            }{
              [[SS ; TC ; empty |-tm ie1 ie2 : is2 ~> te1 te2]]
            }{\textsc{iTm-arrE}
            }
            \end{equation}
            and for Hypothesis \pref{semelab:hyp2}, we have:
            \begin{equation}
              \label{semelab:app:der2}
            \ottdrule['']{
              \ottpremise{[[SS ; TC ; empty |-tm ie1' : is1' -> is2 ~> te1']]}
              \ottpremise{[[SS ; TC ; empty |-tm ie2 : is1' ~> te2]]}
            }{
              [[SS ; TC ; empty |-tm ie1' ie2 : is2 ~> te1' te2]]
            }{\textsc{iTm-arrE}
            }
            \end{equation}
            From the second premise of the two above rules and by uniqueness (Lemma~\ref{lem:det:ty}), we get
            $[[is1 = is1']]$.

            The induction hypothesis is:
            \begin{align*}
              \text{If}~[[ SS ; TC ; empty |-tm ie1 : ish ~> tep ]]\\
              \text{and}~[[ SS ; TC ; empty |-tm ie1' : ish ~> teq ]]\\
              \text{for some}~\intermed{[[ish]]},~\target{[[tep]]}~\text{and}~\target{[[teq]]},\nonumber\\
              \text{then, there is an}~\target{[[te']]}~\text{such that}\nonumber\\
              [[tep -->> te']]~\text{and}~[[teq --> te']]
            \end{align*}
            Then, an appropriate choice for $\target{[[teh]]}$ is $\target{[[te' te2]]}$, since from Lemma~
            \pref{lem:tEval_app_dist}, we have $[[te1 te2 -->> te' te2]]$ and
            $[[te1' te2 -->> te' te2]]$.\\
          }
\proofStep{Case \textsc{iEval-appAbs}}{\drule{iEval-appAbs}}
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align}
              \label{semelab:appabs:der1}
                         &[[SS ; TC ; empty |-tm ( \ ix : is . ie1 ) ie2 : is' ~> te0]]\\
              \label{semelab:appabs:der2}
              \text{and}~&[[SS ; TC ; empty |-tm [| ie2 / ix |] ie1 : is' ~> te0']]
            \end{align}
            for some $\intermed{[[is']]}$, $\target{[[te0]]}$ and $\target{[[te0']]}$. We need to show that
            there exists an \(\target{[[teh]]}\) such that \([[ te0 -->> teh ]]\) and
            \([[ te0' -->> teh ]]\). We do this by showing that $[[te0 -->> te0']]$.
            
            By inversion, the last part of Derivation \pref{semelab:appabs:der1} must be an
            instance of \textsc{iTm-arrI} directly followed by \textsc{iTm-arrE}, as shown
            below.
            \begin{equation*}
            \ottdrule{
              \ottpremise{
                \ottdrule{
                  \ottpremise{[[SS ; TC ; empty , ix : is |-tm ie1 : is' ~> te1]]}
                  \ottpremise{[[TC ; empty |-ty is ~> tt]]}
                }{
                  [[SS ; TC ; empty |-tm \ ix : is . ie1 : is -> is' ~> \ tx : tt . te1]]
                }{\textsc{iTm-arrI}}}
              \ottpremise{[[SS ; TC ; empty |-tm ie2 : is ~> te2]]}
            }{
              [[SS ; TC ; empty |-tm ( \ ix : is . ie1 ) ie2 : is' ~> (\ tx : tt . te1) te2]]
            }{\textsc{iTm-arrE}
            }
            \end{equation*}
            where $[[te0 = (\ tx : tt . te1) te2]]$. From the above equation, we can use
            premises
            \begin{align*}
                         &[[SS ; TC ; empty , ix : is |-tm ie1 : is' ~> te1]]\\
              \text{and}~&[[SS ; TC ; empty |-tm ie2 : is ~> te2]]
            \end{align*}
            in Lemma~\ref{lemma:var_subst}, to obtain
            \begin{equation*}
              [[SS ; TC ; empty |-tm [| ie2 / ix |] ie1 : is' ~> [| te1 / tx |] te2 ]]
            \end{equation*}
            Then, by uniqueness (Theorem~\ref{thmA:tmelab:det} on the latter and on
            Equation~\pref{semelab:appabs:der2}), we have $[[te0' =  [| te1 / tx |] te2 ]]$.

            We set $[[teh =  [| te1 / tx |] te2 ]]$, since
            $[[(\ tx : tt . te1) te2 -->> [| te1 / tx |] te2 ]]$, by evaluation rule
            \textsc{tEval-AppAbs}, and $[[ [| te1 / tx |] te2 -->> [| te1 / tx |] te2 ]]$, by
            reflexivity of $[[-->>]]$.\\
          }
\proofStep{Case \textsc{iEval-tyApp}}{\drule{iEval-tyApp}}
          {Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align*}
                         &[[SS ; TC ; empty |-tm ie is : [| is / c |] isp ~> te tt]]\\
              \text{and}~&[[SS ; TC ; empty |-tm ie' is : [| is / c' |] isq ~> te' tt]]
            \end{align*}
            for some $\intermed{[[c]]}$, $\intermed{[[c']]}$, $\intermed{[[isp]]}$, $\intermed{[[isq]]}$, $[[te]]$, $\target{[[te']]}$ and $[[tt]]$.

            The last rule of both derivations above must be instances of \textsc{iTm-forallE}.
            For the first, we have:
            \begin{equation}
              \label{semelab:tyapp:der1}
              \ottdrule{
                \ottpremise{[[SS ; TC ; empty |-tm ie : \/ c . isp ~> te]]}
                \ottpremise{[[TC ; empty |-ty is ~> tt]]}
              }{
                [[SS ; TC ; empty |-tm ie is : [| is / c |] isp ~> te tt]]
              }{\textsc{iTm-forallE}}
            \end{equation}
            and for the second:
            \begin{equation}
              \label{semelab:tyapp:der2}
              \ottdrule{
                \ottpremise{[[SS ; TC ; empty |-tm ie' : \/ c' . isq ~> te']]}
                \ottpremise{[[TC ; empty |-ty is ~> tt]]}
              }{
                [[SS ; TC ; empty |-tm ie is : [| is / c' |] isq ~> te' tt]]
              }{\textsc{iTm-forallE}}
            \end{equation}
            By applying Theorem~\ref{thmA:intermediate_preservation} on the first premise of
            Equation \pref{semelab:tyapp:der1} and on the premise of rule \textsc{iEval-tyApp},
            we have that $[[\/ c . isp = \/ c' . isq]]$.

            The induction hypothesis is:
            \begin{align*}
              \text{If}~[[ SS ; TC ; empty |-tm ie1 : ish ~> tep ]]\\
              \text{and}~[[ SS ; TC ; empty |-tm ie1' : ish ~> teq ]]\\
              \text{for some}~\intermed{[[ish]]},~\target{[[tep]]}~\text{and}~\target{[[teq]]},\nonumber\\
              \text{then, there is an}~\target{[[teh']]}~\text{such that}\nonumber\\
              [[tep -->> teh']]~\text{and}~[[teq --> teh']]
            \end{align*}
            For $[[ish = \/ c . isp]]$, $[[tep = te]]$ and $[[teq = te']]$, the two
            conditions are fulfilled by the first premise of Equations
            \pref{semelab:tyapp:der1} and \pref{semelab:tyapp:der2}.

            We choose $[[teh = teh' tt]]$, because from Lemma~\pref{lem:tEval_tapp_dist},
            we have $[[te tt -->> teh' tt]]$ and $[[te' tt -->> teh' tt]]$.\\
          }
\proofStep{Case \textsc{iEval-tyAppAbs}}{\drule{iEval-tyAppAbs}}
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align}
              \label{semelab:tyappabs:der1}
                         &[[SS ; TC ; empty |-tm ( /\ c . ie ) is : is0 ~> te0]]\\
              \label{semelab:tyappabs:der2}
              \text{and}~&[[SS ; TC ; empty |-tm [| is / c |] ie : is0 ~> te0']]
            \end{align}
            for some $\intermed{[[is0]]}$, $\target{[[te0]]}$ and $\target{[[te0']]}$.
            We need to show that
            there exists an \(\target{[[teh]]}\) such that \([[ te0 -->> teh ]]\) and
            \([[ te0' -->> teh ]]\). We do this by showing that $[[te0 -->> te0']]$.
            
            By inversion, the last part of Derivation \pref{semelab:tyappabs:der1} must be an
            instance of \textsc{iTm-forallI} directly followed by \textsc{iTm-forallE}, as shown
            below.
            \begin{equation*}
            \ottdrule{
              \ottpremise{
                \ottdrule{
                  \ottpremise{[[SS ; TC ; empty , c |-tm ie : is' ~> te]]}
                }{
                  [[SS ; TC ; empty |-tm /\ c . ie : \/ c . is' ~> /\ ta . te]]
                }{\textsc{iTm-forallI}}}
              \ottpremise{[[TC ; empty |-ty is ~> tt]]}
            }{
              [[SS ; TC ; empty |-tm ( /\ c . ie ) is : [| is / c |] is' ~> ( /\ ta . te ) tt]]
            }{\textsc{iTm-forallE}
            }
            \end{equation*}
            where $[[is0 =  [| is / c |] is' ]]$ and $[[te0 = ( /\ ta . te ) tt]]$. From
            the above equation, we can use premises
            \begin{align*}
                         &[[SS ; TC ; empty , c |-tm ie : is' ~> te]]\\
              \text{and}~&[[TC ; empty |-ty is ~> tt]]
            \end{align*}
            in Lemma~\ref{lemma:tvar_subst}, to obtain
            \begin{equation*}
              [[SS ; TC ; empty |-tm [| is / c |] ie : [| is / c |] is' ~> [| tt / ta |] te ]]
            \end{equation*}
            Then, by uniqueness (Theorem~\ref{thmA:tmelab:det} on the latter and on
            Equation~\pref{semelab:tyappabs:der2}), we have $[[te0' =  [| tt / ta |] te ]]$.

            We set $[[teh =  [| tt / ta |] te ]]$, since
            $[[( /\ ta . te ) tt -->> [| tt / ta |] te ]]$, by evaluation rule
            \textsc{tEval-TAppAbs}, and $[[ [| tt / ta |] te -->> [| tt / ta |] te ]]$, by
            reflexivity of $[[-->>]]$.\\
          }
\proofStep{Case \textsc{iEval-DApp}}{\drule{iEval-DApp}}
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align*}
                         &[[SS ; TC ; empty |-tm ie id : is ~> te1 te2]]\\
              \text{and}~&[[SS ; TC ; empty |-tm ie' id : is ~> te1' te2]]
            \end{align*}
            for some $\target{[[te1]]}$, $\target{[[te1']]}$ and $\target{[[te2]]}$.
            
            The last rule of these derivations must be instances of \textsc{iTm-constrE}. For
            Hypothesis \pref{semelab:hyp1}, we have:
            \begin{equation}
              \label{semelab:dapp:der1}
            \ottdrule{
              \ottpremise{[[SS ; TC ; empty |-tm ie : iq -> is ~> te1]]}
              \ottpremise{[[SS ; TC ; empty |-d id : iq ~> te2]]}
            }{
              [[SS ; TC ; empty |-tm ie id : is ~> te1 te2]]
            }{\textsc{iTm-constrE}
            }
            \end{equation}
            and for Hypothesis \pref{semelab:hyp2}, we have:
            \begin{equation}
              \label{semelab:dapp:der2}
            \ottdrule['']{
              \ottpremise{[[SS ; TC ; empty |-tm ie' : iq' -> is ~> te1']]}
              \ottpremise{[[SS ; TC ; empty |-d id : iq' ~> te2]]}
            }{
              [[SS ; TC ; empty |-tm ie1' id : is ~> te1' te2]]
            }{\textsc{iTm-constrE}
            }
            \end{equation}
            From the second premise of the two above rules and by uniqueness, we get
            $[[iq = iq']]$.

            The induction hypothesis is:
            \begin{align*}
              \text{If}~[[ SS ; TC ; empty |-tm ie : ish ~> tep ]]\\
              \text{and}~[[ SS ; TC ; empty |-tm ie' : ish ~> teq ]]\\
              \text{for some}~\intermed{[[ish]]},~\target{[[tep]]}~\text{and}~\target{[[teq]]},\nonumber\\
              \text{then, there is an}~\target{[[teh']]}~\text{such that}\nonumber\\
              [[tep -->> teh']]~\text{and}~[[teq --> teh']]
            \end{align*}
            Then, the conditions of the above hold from the first premise of Derivations
            \pref{semelab:dapp:der1} and \pref{semelab:dapp:der2}, where
            $[[ish = iq -> is]]$, $[[tep = te1]]$ and $[[teq = te1']]$.

            Then, an appropriate choice for $\target{[[teh]]}$ is $\target{[[teh' te2]]}$, since from Lemma~
            \pref{lem:tEval_app_dist}, we have $[[te1 te2 -->> teh' te2]]$ and
            $[[te1' te2 -->> teh' te2]]$.\\
          }
\proofStep{Case \textsc{iEval-DAppAbs}}{\drule{iEval-DAppAbs}}
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align}
              \label{semelab:dappabs:der1}
                         &[[SS ; TC ; empty |-tm ( \ idvar : iq . ie ) id : is ~> te0]]\\
              \label{semelab:dappabs:der2}
              \text{and}~&[[SS ; TC ; empty |-tm [| id / idvar |] ie : is ~> te0']]
            \end{align}
            for some $\intermed{[[is']]}$, $\target{[[te0]]}$ and $\target{[[te0']]}$.
            We need to show that
            there exists an \(\target{[[teh]]}\) such that \([[ te0 -->> teh ]]\) and
            \([[ te0' -->> teh ]]\). We do this by showing that $[[te0 -->> te0']]$.
            
            By inversion, the last part of Derivation \pref{semelab:dappabs:der1} must be an
            instance of \textsc{iTm-constrI} directly followed by \textsc{iTm-constrE}, as shown
            below.
            \begin{equation*}
            \ottdrule{
              \ottpremise{
                \ottdrule{
                  \ottpremise{[[SS ; TC ; empty , idvar : iq |-tm ie : is ~> te1]]}
                  \ottpremise{[[TC ; empty |-ty is ~> tt]]}
                }{
                  [[SS ; TC ; empty |-tm \ idvar : iq . ie : iq -> is ~> \ txd : tt . te1]]
                }{\textsc{iTm-constrI}}}
              \ottpremise{[[SS ; TC ; empty |-d id : iq ~> te2]]}
            }{
              [[SS ; TC ; empty |-tm ( \ idvar : iq . ie ) id : is ~> (\ txd : tt . te1) te2]]
            }{\textsc{iTm-constrE}
            }
            \end{equation*}
            where $[[te0 = (\ txd : tt . te1) te2]]$. From the above equation, we can use
            premises
            \begin{align*}
                         &[[SS ; TC ; empty , idvar : iq |-tm ie : is ~> te1]]\\
              \text{and}~&[[SS ; TC ; empty |-d id : iq ~> te2]]
            \end{align*}
            in Lemma~\ref{lemma:dvar_subst}, to obtain
            \begin{equation*}
              [[SS ; TC ; empty |-tm [| id / idvar |] ie : is ~> [| te1 / txd |] te2 ]]
            \end{equation*}
            Then, by uniqueness (Theorem~\ref{thmA:delab:det} on the latter and on
            Equation~\pref{semelab:dappabs:der2}), we have $[[te0' =  [| te1 / txd |] te2 ]]$.

            We set $[[teh =  [| te1 / txd |] te2 ]]$, since
            $[[(\ txd : tt . te1) te2 -->> [| te1 / txd |] te2 ]]$, by evaluation rule
            \textsc{tEval-AppAbs}, and $[[ [| te1 / txd |] te2 -->> [| te1 / txd |] te2 ]]$, by
            reflexivity of $[[-->>]]$.\\
%            Indeed, by evaluation rule \textsc{tEval-AppAbs}, we get
%            $[[(\ txd : tt . te1) te2 --> [| te1 / txd |] te2 ]]$.\\
          }
\proofStep{Case \textsc{iEval-method}}
          {
            \ottdrule{
              \ottpremise{[[(iD : \/ clj . iqli => iTC isq).im |-> ie in SS]]}
            }{[[SS |- (iD islj idli).im --> ie islj idli]]
            }{\textsc{iEval-method}}
          }
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align}
              \label{semelab:meth:der1}
                         &[[SS ; TC ; empty |-tm (iD islj idli).im : is0 ~> te0]]\\
              \label{semelab:meth:der2}
              \text{and}~&[[SS ; TC ; empty |-tm ie islj idli : is0 ~> te0']]
            \end{align}
            for some $\intermed{[[is0]]}$, $\target{[[te0]]}$ and $\target{[[te0']]}$. We need to show that there is a
            $\target{[[teh]]}$ such that $[[te0 -->> teh]]$ and $[[te0' -->> teh]]$.
            
            By inversion on Equation~\pref{semelab:meth:der1}, we have
            $[[te0 = (( /\ talj . \ </ txdi : tt'i // i /> . { tl = tem } ) ttlj teli) . tl]]$
            and $[[is0 =  [| [| islj / clj |] isq / c |] ism ]]$, for some $\intermed{[[ism]]}$,
            $\intermed{[[iem]]}$, $\intermed{[[c]]}$, $\target{[[tti']]}$, $\target{[[tem]]}$, $\target{[[ttj]]}$ and $\target{[[tei]]}$,
            such that 
            \begin{gather*}
              %\label{semelab:meth:iTC}
              [[(im : iTC c : ism) in TC]]\\
              %\label{semelab:meth:ism}
              [[TC ; empty , c |-ty ism ~> ttm]]\\
              %\label{semelab:meth:D}
              [[( iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli . iem in SS]]\\
              %\label{semelab:meth:tem}
              [[SS1 ; TC ; empty , clj , idvarli : iqli |-tm iem : [| isq / c |] ism ~> tem]]\\
              %\label{semelab:meth:iqi}
              [[</ TC ; empty , clj |-q iqi ~> tti' // i />]]\\
              %\label{semelab:meth:isj}
              [[</ TC ; empty |-ty isj ~> ttj // j />]]\\
              %\label{semelab:meth:id}
              [[</ SS ; TC ; empty |-d idi : [| islj / clj |] iqi ~> tei // i />]]
            \end{gather*}
            Because $[[SS]]$ contains a unique method implementation per class instance, we
            also have
            \begin{equation}
              \label{semelab:meth:ie}
              [[ie = /\ clj . \ idvarli : iqli . iem]]
            \end{equation}
            Then, term $\intermed{[[ie islj idli]]}$, equal to
            $\intermed{[[(/\ clj . \ idvarli : iqli . iem) islj idli]]}$, is deterministcally elaborated to
            $\target{[[(/\ talj . \ </ txdi : tti' // i /> . tem) ttlj teli]]}$.

            Indeed, $[[teh =  [| </ tei / txi // i /> |] [| </ ttj / taj // j /> |] tem ]]$
            is an appropriate choice, since
            \begin{equation*}
            \begin{aligned}
              \target{[[te0]]} &= \target{[[(( /\ talj . \ </ txdi : tt'i // i />. { tl = tem } ) ttlj teli) . tl]]}\\
              &\to \target{[[(\ </ txdi : [| </ ttj / taj // j /> |] tt'i // i /> . { tl = [| </ ttj / taj // j /> |] tem }) . tl]]}\\
              &\to \target{[[ {tl = [| </ tei / txdi // i /> |] [| </ ttj / taj // j /> |] tem } . tl]]}\\
              &\to \target{[[ [| </ tei / txdi // i /> |] [| </ ttj / taj // j /> |] tem ]]}
            \end{aligned}
            \end{equation*}
            and
            \begin{equation*}
              \begin{aligned}
                \target{[[te0']]} &= \target{[[(/\ talj . \ </ txdi : tti' // i /> . tem) ttlj teli]]}\\
                &\to \target{[[\ </ txdi : [| </ ttj / taj // j /> |] tt'i // i />. [| </ ttj / taj // j /> |] tem ]]}\\
                &\to \target{[[ [| </ tei / txdi // i /> |] [| </ ttj / taj // j /> |] tem ]]}
              \end{aligned}
            \end{equation*}
          }
\proofStep{Case \textsc{iEval-let}}{\drule{iEval-let}}
          {
            Hypotheses \pref{semelab:hyp1} and \pref{semelab:hyp2} of the theorem, adapted to
            this case, are:
            \begin{align}
              \label{semelab:let:der1}
                         &[[SS ; TC ; empty |-tm ilet ix : is = ie1 iin ie : is' ~> te0]]\\
              \label{semelab:let:der2}
              \text{and}~&[[SS ; TC ; empty |-tm [| ie1 / ix |] ie2 : is' ~> te0']]
            \end{align}
            for some $\intermed{[[is']]}$, $\target{[[te0]]}$ and $\target{[[te0']]}$. 
            We need to show that
            there exists an \(\target{[[teh]]}\) such that \([[ te0 -->> teh ]]\) and
            \([[ te0' -->> teh ]]\). We do this by showing that $[[te0 -->> te0']]$.
            
            By inversion, the last rule used for Derivation \pref{semelab:let:der1} must be an
            instance of \textsc{iTm-let}.
            \begin{equation*}
                \ottdrule{
                  \ottpremise{[[SS ; TC ; empty |-tm ie1 : is ~> te1]]}
                  \ottpremise{[[SS ; TC ; empty , ix : is |-tm ie2 : is' ~> te2]]}
                  \ottpremise{[[TC ; empty |-ty is ~> tt]]}
                }{
                  [[SS ; TC ; empty |-tm ilet ix : is = ie1 iin ie : is' ~> tlet tx : tt = te1 tin te2]]
                }{\textsc{iTm-constrI}}
            \end{equation*}
            where $[[te0 = tlet tx : tt = te1 tin te2]]$. From the above equation, we can use
            the first two premises in Lemma~\ref{lemma:var_subst}, to obtain
            \begin{equation*}
              [[SS ; TC ; empty |-tm [| ie1 / ix |] ie2 : is' ~> [| te1 / tx |] te2 ]]
            \end{equation*}
            Then, by uniqueness (Theorem~\ref{thmA:tmelab:det} on the latter and on
            Equation~\pref{semelab:let:der2}), we have $[[te0' =  [| te1 / tx |] te2 ]]$.

            We set $[[teh =  [| te1 / tx |] te2 ]]$, since
            $[[(\ tx : tt . te1) te2 -->> [| te1 / tx |] te2 ]]$, by evaluation rule
            \textsc{tEval-AppAbs}, and $[[ [| te1 / tx |] te2 -->> [| te1 / tx |] te2 ]]$, by
            reflexivity of $[[-->>]]$.\\
          }
\qed

\begin{lemmaB}[\targetL{} Preservation of Values]\ \\
  \label{lemma:val_pres}
  If \([[ SS ; TC ; empty |-tm iv : is ~> te ]]\)
  then \([[ te ]]\) is a value.
\end{lemmaB}
\proof By straightforward case analysis on the typing derivation.

\begin{theoremB}[Value Semantic Preservation]\ \\
  \label{lemma:val_sem_pres}
  If \([[ SS ; TC ; empty |-tm ie : is ~> te ]]\)
  and \([[ SS |- ie -->> iv ]]\)
  then \([[ SS ; TC ; empty |-tm iv : is ~> tv ]]\)
  and \([[ te ~= tv ]]\).
\end{theoremB}
\proof
From the Preservation Theorem~\ref{thmA:intermediate_preservation} and Progress
Theorem~\ref{thmA:progress_expressions}, in combination with the hypothesis,
we know that:
\begin{equation*}
  [[ SS ; TC ; empty |-tm iv : is ~> te' ]]
\end{equation*}
Lemma~\ref{lemma:val_pres} teaches us that \([[te']]\) is some value \([[tv]]\).

The goal follows by repeatedly applying Theorem~\ref{thmA:sem_pres}, in
combination with the fact that evaluation in both \interL{} and \targetL{} is
deterministic (Lemmas~\ref{lemma:eval_unique} and~\ref{lem:tgt_eval_unique}). \\
\qed

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                                Definitions
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "./proof"
%%% End:


==> doc/sections/typesystem.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                                   Syntax
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\section{Syntax}
\label{app:syntax}
\subsection{\srcL{} : Source Language}

\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  % Program
  \Mytabular{
    \syntaxLine{[[spgm]]}
               {::=}
               {\source { [[se]] } \mid \source { [[scls ; spgm]] } \mid \source { [[sinst ; spgm]] }}
               {spgm}
    \\
    \syntaxLine{[[scls]]}
               {::=}
               {\source { [[class sTCl => sTC a swhere { sm : ss}]] }}
               {class decl.}
    \\
    \syntaxLine{[[sinst]]}
               {::=}
               {\source { [[instance sql => sTC st swhere { sm = se }]] }}
               {instance decl.}
  }
  \\\\
  % Expression
  \Mytabular{
    \syntaxLine{[[se]]}
               {::=}
               {\source { [[strue]] } \mid \source { [[sfalse]] } \mid \source {
  [[sx]] }
  \mid \source { [[sm]] } \mid \source { [[\sx. se]] } \mid \source { [[se1 se2]] }
  \mid \source { [[slet sx : ss = se1 sin se2]] } \mid \source { [[se <: st]] }}{term}
  }
  \\\\
  % Types
  \Mytabular{
    \syntaxLine{[[st]]}
               {::=}
               {\source { [[sbool]] } \mid \source { [[a]] } \mid \source { [[st1 -> st2]] }}
               {monotype}
    \\
    \syntaxLine{[[sp]]}
               {::=}
               {\source { [[st]] } \mid \source { [[sq => sp]] }}
               {qualified type}
    \\
    \syntaxLine{[[ss]]}
               {::=}
               {\source { [[sp]] } \mid \source { [[\/a. ss]] }}
               {type scheme}
  }
  \\\\
  % Constraints
  \Mytabular{
    \syntaxLine{[[sq]]}
               {::=}
               {\source { [[sTC st]] }}
               {class constraint}
    \\
    \syntaxLine{[[sc]]}
               {::=}
               {\source { [[\/ al . sql => sq]] }}
               {constraint}
  }
  \\\\
  % Contexts
  \Mytabular{
    \syntaxLine{[[GG]]}
               {::=}
               {\source { [[empty]] } \mid \source { [[GG, sx : ss]] } \mid \source { [[GG, a]] } \mid \source { [[GG, sdvar : sq]] } }
               {typing environment}
     \\
    \syntaxLine{[[GC]]}
               {::=}
               {\source { [[empty]] } \mid \source { [[GC, sm : sTCl => sTC a : ss]] }}
               {class environment}
     \\
    \syntaxLine{[[PT]]}
               {::=}
               {\source { [[empty]] } \mid \source { [[PT, (sD : sc) . sm |-> GG : se]] }}
               {program context}
     \\
    \syntaxLine{[[sM]]}
               {::=}
               {\source { [[ [empty] ]] } \mid \source { [[\ sx . sM]] } \mid \source { [[sM se]] } \mid \source { [[se sM]] } \mid \source { [[sM <: st]] }}
               {evaluation context}
     \\
    \syntaxLine{}
               {}
               { \mid \source { [[slet sx : ss = sM sin se]] } \mid \source { [[slet sx : ss = se sin sM]] } }
               {}
  }
\end{array}
\]


\subsection{\interL{} : Intermediate Language}
\label{app:mid_syntax}

\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  \Mytabular{
  % Expression
    \syntaxLine{[[ie]]}
               {::=}
               {\intermed { [[itrue]] } \mid \intermed { [[ifalse]] } \mid \intermed { [[ix]] } \mid \intermed { [[\ ix : is . ie]] } \mid
  \intermed { [[ie1 ie2]] } \mid \intermed { [[\idvar : iq . ie]] } \mid \intermed { [[ie id]] }}
               {expression}
    \\
    \syntaxLine{}
               {}
               {\intermed { [[/\ c. ie]] } \mid \intermed { [[ie is]] } \mid \intermed { [[id . im]] } \mid \intermed { [[ilet ix : is = ie1 iin ie2]] }}
               {}
    \\
    \syntaxLine{[[iv]]}
               {::=}
               {\intermed { [[itrue]] } \mid \intermed { [[ifalse]] } \mid \intermed { [[\ ix : is . ie]] } \mid \intermed { [[\ idvar : iq . ie]] }
  \mid \intermed { [[/\ c . ie]] }}
               {value}
  }
\end{array}
\]

\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  \Mytabular{
  % Types
    \syntaxLine{[[is]]}
               {::=}
               {\intermed { [[ibool]] } \mid \intermed { [[c]] } \mid \intermed { [[is1 -> is2]] } \mid \intermed { [[iq -> is]] } \mid \intermed { [[\/ c. is]] }}
               {type}
    \\
  % Class Constraints
    \syntaxLine{[[iq]]}
               {::=}
               {\intermed { [[iTC is]] }}
               {class constraint}
    \\
  % Constraints
    \syntaxLine{[[ic]]}
               {::=}
               {\intermed { [[\/ cl . iql => iq]] }}
               {constraint}
  }
\end{array}
\]

\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  \Mytabular{
  % Typing Context
    \syntaxLine{[[TT]]}
               {::=}
               {\intermed { [[empty]] } \mid \intermed { [[TT, ix : is]] } \mid \intermed { [[TT, c]] } \mid \intermed { [[TT, idvar : iq]] } }
               {typing environment}
  \\
  % Class Context
    \syntaxLine{[[TC]]}
               {::=}
               {\intermed { [[empty]] } \mid \intermed { [[TC, im : iTC c : is]] }}
               {class environment}
  \\
  % method environment
    \syntaxLine{[[SS]]}
               {::=}
               {\intermed { [[empty]] } \mid \intermed { [[SS , (iD : ic) . im |-> ie]] }}
               {method environment}
  \\
  % evaluation context
    \syntaxLine{[[iM]]}
               {::=}
               {\intermed { [[ [empty] ]] } \mid \intermed { [[ \ ix : is . iM]] } \mid \intermed { [[ \ idvar : iq . iM ]] }
  \mid \intermed { [[ ie iM ]] } \mid \intermed { [[ iM ie ]] } \mid \intermed { [[ iM id ]] }}
               {evaluation context}
  \\
    \syntaxLine{}
               {}
               {\mid \intermed { [[ /\ c . iM ]] } \mid \intermed { [[ iM is ]] } \mid \intermed { [[ ilet ix : is = iM iin ie ]] }}
               {}
  \\
    \syntaxLine{}
               {}
               {\mid \intermed { [[ ilet ix : is = ie iin iM ]] }}
               {}
  }
\end{array}
\]

\subsubsection{Dictionaries}
\[
  \begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  % Dictionary
  \Mytabular{
    \syntaxLine{[[id]]}
               {::=}
               {\intermed { [[idvar]] } \mid \intermed { [[iD isl idl]] }}
               {dictionary}
    \\
    \syntaxLine{[[idv]]}
               {::=}
               {\intermed { [[iD isl idvl]] }}
               {dictionary value}
  }
\end{array}
\]

\subsection{\targetL{} : Target language}
\[
  \begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  % Dictionary
  \Mytabular{
    \syntaxLine{[[te]]}
               {::=}
               {\target { [[ttrue]] } \mid \target { [[tfalse]] } \mid \target { [[tx]] } \mid \target { [[\ tx : tt . te]] }
    \mid \target { [[te1 te2]] } \mid \target { [[/\ ta . te]] } \mid \target { [[te tt]] }}
               {target term}
    \\
    \syntaxLine{}
               {}
    {\mid \target { [[{ </ tli = tei // i IN n /> }]] } \mid \target { [[te . tl]] } \mid \target { [[tlet tx : tt = te1 tin te2]] }}
               {}
    \\
    \syntaxLine{[[tv]]}
               {::=}
               {\target { [[ttrue]] } \mid \target { [[tfalse]] } \mid \target { [[\ tx : tt . te]] } \mid \target { [[/\ ta . te]] } \mid \target { [[{ </ tli = tei // i IN n /> }]] }}
               {target value}
    \\
    \syntaxLine{[[tt]]}
               {::=}
               {\target { [[tbool]] } \mid \target { [[ta]] } \mid \target { [[\/ ta . tt]] } \mid \target { [[tt1 -> tt2]] } \mid \target { [[{ </ tli : tti // i IN n /> }]] }}
               {target type}
    \\
    \syntaxLine{[[GT]]}
               {::=}
               {\target { [[tempty]] } \mid \target { [[GT , ta]] } \mid \target { [[GT , tx : tt]] }}
               {target context}
    \\
    \syntaxLine{[[tM]]}
               {::=}
               {\target { [[ [ empty ] ]] } \mid \target { [[\ tx : tt . tM]] } \mid \target { [[te tM]] } \mid [[tM
    te]] \mid \target { [[/\ ta . tM]] } \mid \target { [[tM tt]] } \mid \target { [[ { </ tli = tMi // i IN 1 .. n /> } ]] } }
               {target evaluation context}
    \\
    \syntaxLine{}
               {}
               {\mid \target { [[tM . tl]] } \mid \target { [[tlet tx : tt = tM tin te]] } \mid \target { [[tlet tx : tt = te tin tM]] }}
               {}
  }
\end{array}
\]

\newpage
\section{\srcL{} Judgments and Elaboration}
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Type & Constraint WF
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{\srcL{} Type \& Constraint Well-Formedness}
\label{app:src_ty_wf}

\drules[sQT]{$[[ GC ;  GG |-q sq ~> tt ]]$}{\srcL{} Class Constraint Well-Formedness}{TC}
\drules[sCT]{$[[ GC ; GG |-c sc ~> tt ]]$}{\srcL{} Constraint Well-Formedness}{abs}
\drules[sTyT]{$[[ GC ; GG |-ty ss ~> tt ]]$}{\srcL{} Type Well-Formedness}{bool, var,
  arrow, qual, scheme}


% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                                 Term Typing
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% \newpage
\subsection{\srcL{} Term Typing}
\label{app:src_tm_typing}

\drules[sTm-infT]{$[[ PT ; GC ; GG |-tm se => st ~> te ]]$}{\srcL{} Term Inference}{true, false,
  let, ArrE, Ann}
\drules[sTm-checkT]{$[[ PT ; GC ; GG |-tm se <= st ~> te ]]$}{\srcL{} Term Checking}{var,
meth, ArrI, Inf}
\drules[sClsT]{$[[ GC |-cls scls : GC' ]]$}{Class Decl Typing}{cls}
\drules[sInstT]{$[[ PT ; GC |-inst sinst : PT' ]]$}{Instance Decl Typing}{inst}
\drules[sPgmT]{$[[ PT ; GC |-pgm spgm : st ; PT' ; GC' ~> te ]]$}{\srcL{}
  Program Typing}{cls, inst, expr}
\drules[sClosure]{$[[ closure ( GC ; sqli ) = sqlj ]]$}{Closure over Superclass
  Relation}{empty, TC}
\drules[sUnambig]{$[[ unambig ( ss ) ]]$}{Unambiguity for Type Schemes}{scheme}
\drules[sUnambig]{$[[ unambig ( sc ) ]]$}{Unambiguity for Constraints}{constraint}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Constraint Proving
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Constraint Proving}

\drules[sEntailT]{$[[ PT ; GC ; GG |= sq ~> te ]]$}{Constraint Entailment}{inst, local}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                          Environment Well-formedness
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{\srcL{} Environment Well-Formedness}
\label{app:src_env_wf}

\drules[sCtxT]{$[[ |-ctx PT ; GC ; GG ~> GT ]]$}{\srcL{} Environment
  Well-Formedness}{empty, clsEnv, tyEnvTm, tyEnvTy, tyEnvD, pgmInst}

\newpage
\section{\srcL{} Judgments and Elaboration through \interL{}}
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Type & Constraint WF
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{\srcL{} Type \& Constraint Well-Formedness}

\drules[sQ]{$[[ GC ;  GG |-q sq ~> iq ]]$}{\srcL{} Class Constraint Well-Formedness}{TC}
\drules[sC]{$[[ GC ; GG |-c sc ~> ic ]]$}{\srcL{} Constraint Well-Formedness}{abs}
\drules[sTy]{$[[ GC ; GG |-ty ss ~> is ]]$}{\srcL{} Type Well-Formedness}{bool, var,
  arrow, qual, scheme}


% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                                 Term Typing
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% \newpage
\subsection{\srcL{} Term Typing}
\label{app:srcmid_tm_typing}

\drules[sTm-inf]{$[[ P ; GC ; GG |-tm se => st ~> ie ]]$}{\srcL{} Term Inference}{true, false,
  let, ArrE, Ann}
\drules[sTm-check]{$[[ P ; GC ; GG |-tm se <= st ~> ie ]]$}{\srcL{} Term Checking}{var,
meth, ArrI, Inf}
\drules[sCls]{$[[ GC |-clsM scls : GC' ]]$}{Class Decl Typing}{cls}
\drules[sInst]{$[[ P ; GC |-instM sinst : P' ]]$}{Instance Decl Typing}{inst}
\drules[sPgm]{$[[ P ; GC |-pgmM spgm : st ; P' ; GC' ~> ie ]]$}{\srcL{}
  Program Typing}{cls, inst, expr}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                             Constraint Proving
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Constraint Proving}

\drules[sEntail]{$[[ P ; GC ; GG |= sq ~> id ]]$}{Constraint Entailment}{inst, local}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                          Environment Well-formedness
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{\srcL{} Environment Well-Formedness}

\renewcommand\itot[1]{}
\drules[sCtx]{$[[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]$}{\srcL{} Environment
  Well-Formedness}{empty, clsEnv, tyEnvTm, tyEnvTy, tyEnvD, pgmInst}
\renewcommand\itot[1]{#1}

\newpage
\section{\interL{} Judgments and Elaboration}
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                       Intermediate Type & Constraint WF
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{\interL{} Type \& Constraint Well-Formedness}

\drules[iQ]{$[[ TC ; TT |-q iq ~> tt ]]$}{\interL{} Dictionary Type Well-Formedness}{TC}
\drules[iC]{$[[ TC ; TT |-c ic ]]$}{\interL{} Constraint Well-Formedness}{abs}
\drules[iTy]{$[[ TC ; TT |-ty is ~> tt ]]$}{\interL{} Type Well-Formedness}{bool, var,
  arrow, qual, scheme}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                          Dictionary Witness Typing
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{Dictionary Typing}

\drules[D]{$[[ SS ; TC ; TT |-d id : iq ~> te ]]$}{Dictionary Typing}{var, con}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                            Intermediate Term Typing
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% \clearpage
\subsection{\interL{} Term Typing}

\drules[iTm]{$[[ SS ; TC ; TT |-tm ie : is ~> te ]]$}{\interL{} Term Typing}{true,
  false, var, let, method, arrI, arrE, constrI, constrE, forallI, forallE}


% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                       MID Environment well-formedness
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% \newpage
\subsection{\interL{} Environment Well-Formedness}
\drules[iCtx]{$[[ |-ctx SS ; TC ; TT]]$}{\interL{} Environment
  Well-Formedness}{empty, clsEnv, tyEnvTm, tyEnvTy, tyEnvD, MEnv}
\drules[iUnambig]{$[[ unambig (ic) ]]$}{Unambiguity for Constraints}{constraint}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                         Phase 2 - Context translation
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\subsection{\interL{} Environment Elaboration}
\label{sec:namespace_translation}
\drules[Ctx]{$[[TC ; TT ~> GT]]$}{\interL{}-to-\targetL{} environment translation}{Empty, Var, DVar, TVar}

In the translation mechanism, we have assumed namespace translation functions which take a
\interL{} type, term or dictionary-variable name and return the same identifier
representing a \targetL{} type or term variable. There are four such functions, each with
a different namespace as domain:

\begin{center}
%% \begin{minipage}[c]{10cm}
\begin{itemize}
  \item[\textbf{Type variables:}] It translates a type variable of the \interL{} language,
    $[[c]]$, to the \targetL{} type variable with the same name, $[[ta]]$.
  \item[\textbf{Term variables:}] Similar to type variables, but for the term sort.
  \item[\textbf{Dictionary variables:}] It translates a dictionary variable, $[[idvar]]$, to a \targetL{}
    term variable with the same name.
  \item[\textbf{Dictionary labels:}] It translates a dictionary method, $[[im]]$, to a record-field
    label, $[[tl]]$, with the same name.
\end{itemize}
%% \end{minipage}
\end{center}

This identifier translation is assumed in all judgments that involve elaboration, such as
the \interL{} term typing. When we regard identifiers, the font-color change
implies such a translation. However, this convention is not used in other language sorts
(types, non-variable terms, etc.). For example, two types with the same identifier but of
different color mean only two types, a \interL{} and a \targetL{} type, that are not related
to each other. Any specification of the relation between the two types is given by the
judgments they appear in.

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                                  Evaluation
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% \newpage
\subsection{\interL{} Operational Semantics}

\drules[iEval]{$[[ SS |- ie --> ie' ]]$}{\interL{} Evaluation}{app, appAbs,
  tyApp, tyAppAbs, DApp, DAppAbs, method, let}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                               TARGET JUDGMENTS
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\newpage
\section{\targetL{} Judgments}
\label{app:tgt}

\subsection{\targetL{} Type Well-Formedness}
\drules[tTy]{$[[GT |-ty tt]]$}{Well-formed \targetL{} types}{Bool, Var, Abs, Arr, Rec}

\subsection{\targetL{} Term Typing}
\drules[tTm]{$[[GT |-tm te : tt]]$}{Well typed \targetL{} terms}{True, False, Var, Abs, App, Tabs, Tapp, Rec, Proj, Let}

\subsection{\targetL{} Environment Well-Formedness}
\drules[tCx]{$[[|-ctx GT]]$}{Well-formed \targetL{} environment}{Empty, Tvar, Var}

\subsection{\targetL{} Operational Semantics}
\label{app:tgt_op}
\drules[tEval]{$[[te --> te']]$}{\targetL{} evaluation}{AppAbs, TappTabs, Proj, Let , App, Tapp, Rec}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%                               Context Typing
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\newpage
\section{Context Typing}
\label{app:context_typing}

\subsection{\srcL{} Context Typing and Elaboration}
\renewcommand\itot[1]{#1}

\drules[sM-inf-infT]{$[[ sM : (PT ; GC ; GG ==> st) |--> (PT ; GC ; GG' ==> st') ~~> tM ]]$}{\srcL{}
  Context Inference - Inference}{empty, appL, appR, letL, letR, ann}
\drules[sM-inf-checkT]{$[[ sM : (PT ; GC ; GG ==> st) |--> (PT ; GC ; GG' <== st') ~~> tM ]]$}{\srcL{}
  Context Inference - Checking}{abs, inf}
\drules[sM-check-infT]{$[[ sM : (PT ; GC ; GG <== st) |--> (PT ; GC ; GG' ==> st') ~~> tM ]]$}{\srcL{}
  Context Checking - Inference}{appL, appR, letL, letR, ann}
\drules[sM-check-checkT]{$[[ sM : (PT ; GC ; GG <== st) |--> (PT ; GC ; GG' <== st') ~~> tM ]]$}{\srcL{}
  Context Checking - Checking}{empty, abs, inf}

\subsection{\srcL{} Context Typing and Elaboration through \interL{}}

\drules[sM-inf-inf]{$[[ sM : (P ; GC ; GG ==> st) |--> (P ; GC ; GG' ==> st') ~~> iM ]]$}{\srcL{}
  Context Inference - Inference}{empty, appL, appR, letL, letR, ann}
\drules[sM-inf-check]{$[[ sM : (P ; GC ; GG ==> st) |--> (P ; GC ; GG' <== st') ~~> iM ]]$}{\srcL{}
  Context Inference - Checking}{abs, inf}
\drules[sM-check-inf]{$[[ sM : (P ; GC ; GG <== st) |--> (P ; GC ; GG' ==> st') ~~> iM ]]$}{\srcL{}
  Context Checking - Inference}{appL, appR, letL, letR, ann}
\drules[sM-check-check]{$[[ sM : (P ; GC ; GG <== st) |--> (P ; GC ; GG' <== st') ~~> iM ]]$}{\srcL{}
  Context Checking - Checking}{empty, abs, inf}

\subsection{\interL{} Context Typing and Elaboration}

\drules[iM]{$[[ iM : ( SS ; TC ; TT ==> is ) |--> ( SS ; TC ; TT' ==> is' ) ~> tM ]]$}{\interL{}
  Context Typing}{empty, abs, appL, appR, dictAbs, dictApp, tyAbs, tyApp, letL, letR}

\subsection{\targetL{} Context Typing}

\drules[tM]{$[[ tM : ( GT ==> tt ) |--> ( GT' ==> tt' ) ]]$}{\targetL{}
  Context Typing}{empty, abs, appL, appR, tyAbs, tyApp, letL, letR}

\renewcommand\itot[1]{#1}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "./proof"
%%% End:


==> examples/itelab_exp1.tex <==
%\newcommand{\tname}[1]{\target {#1}}
%\newcommand{\tlet}[4]{&\textbf{\target {let}} \, \target {#1} &\ottsym{:} #2\\ & &\ottsym{=} #3\\
%                      &\begin{aligned}\textbf{\target {in}} \, #4\end{aligned}}
%\newcommand{\ttall}[2]{\forall \target {#1} \ottsym{.} #2}
%\newcommand{\trec}[2]{\target {\ottsym{\{}} \target {#1} \, \ottsym{:} \, #2 \target {\ottsym{\}}}}
%\newcommand{\ra}{\, \target{\rightarrow} \,}
%\newcommand{\tbool}{\tname{Bool}}
%\newcommand{\tint}{\tname{Int}}
%\newcommand{\Labs}[2]{\Lambda \tname{#1} \ottsym{.} #2}
%\newcommand{\labs}[3]{\lambda \tname{#1} \ottsym{:} #2 \ottsym{.} #3}
%\newcommand{\Eqrec}[1]{\trec{(==)}{\tname{#1} \ra \tname{#1} \ra \tbool}}
%\newcommand{\ntlet}[4]{\textbf{\target {let}} \, \target {#1} &\ottsym{:} #2\\ &\ottsym{=} #3\\ &\begin{aligned}\textbf{\target {in}} \, #4\end{aligned}}
\lstdefinelanguage{TGT}{%
  identifierstyle=\target\itshape,
%  classoffset=1,
  keywords={[1]let,in},
  keywordstyle={[1]\upshape\bfseries\target},
%  classoffset=2,
%  keywords=[2]{labs,Labs,forall},
%  keywordstyle={[2]\rmfamily\color{black}}
%  classoffset=3,
  alsoletter={:,=,-,>,\{,\}},
  morekeywords=[3]{:,=,->,\{,\},labs,Labs,forall},
  %  classoffset=0,
  morekeywords={[0]Int,Bool},   % types go here
  keywordstyle={[0]\itshape\target}, % style for types
%  otherkeywords={:,=,->,\{,\},\(,\)}, % operators go here
  keywordstyle={[3]\color{black}\upshape},
  classoffset=0,
  mathescape=true,
  literate={% replace strings with symbols
    {->}{{$\to$}}{1}
    {labs}{{$\lambda$}}{1}
    {Labs}{{$\Lambda$}}{1}
    {forall}{$\forall$}{1}
    {delta1}{{\target{$\delta$}}{\textsubscript{1}}}{2}
    {delta2}{{\target{$\delta$}}{\textsubscript{2}}}{2}
    {delta3}{{\target{$\delta$}}{\textsubscript{3}}}{2}
    {x1}{{\target{\textit{x}}}{\textsubscript{1}}}{2}
    {x2}{{\target{\textit{x}}}{\textsubscript{2}}}{2}
    {y1}{{\target{\textit{y}}}{\textsubscript{1}}}{2}
    {y2}{{\target{\textit{y}}}{\textsubscript{2}}}{2}
    {va}{\textit{\target{a}}}{1}
    {vb}{\textit{\target{b}}}{1}
    {vx}{\target{\textit{x}}}{1}
    {eqm}{\target{(==)}}{4}
    {land}{\target{(\&\&)}}{4}
    {primEqInt}{\textit{\target{primEqInt}}}{10}
    {refl}{\textit{\target{refl}}}{4}
    {main}{\textit{\target{main}}}{4}
    {Int}{\textit{\target{Int}}}{3}
  },
  basicstyle={\rmfamily},
  keepspaces,
  columns=fullflexible,
  tabsize=2
%  breaklines=true,
%  breakatwhitespace=true
}%[keywords,comments,strings]%
\begin{lstlisting}[language=TGT]
let refl : $\forall$va. { eqm : va -> va -> Bool } -> va -> Bool
           = Labsva.labsdelta3 : { eqm : va -> va -> Bool }.labsvx : va. delta3.eqm vx vx
in let main : Bool
           = refl (Int, Int)
               (Labsva.Labsvb.
                labsdelta1 : { eqm : va -> va -> Bool }.
                labsdelta2 : { eqm : vb -> vb -> Bool }.
                { eqm = labs(x1, y1) : (va, vb). labs(x2, y2) : (va, vb).
                           land (delta1.eqm x1 x2) (delta2.eqm y1 y2)
                } Int Int { eqm = primEqInt } { eqm = primEqInt })
                (5,42)
in main
\end{lstlisting}
%\[
%\begin{fleqn}
%\begin{aligned}[l]
%  \tlet{refl}
%       {\ttall{a}{\Eqrec{a} \ra \tname{a} \ra \tbool}}
%       {\Labs{a}{\labs{\delta_3}{\Eqrec{a}}{\labs{x}{\tname{a}}{\tname{\delta_3}.\tname{(==) \, x \, x}}}}}
%       {\ntlet{main}{\tbool}{\tname{refl} \, (\tint,\,\tint)\\
%           &\begin{aligned}\target {\ottsym{\{}} \tname{(==)} &\ottsym{=} \Labs{a}{\Labs{b}{\\&
%                  \labs{\delta_1}{\Eqrec{a}}{\\&\labs{\delta_2}{\Eqrec{b}}{\\
%                      &\labs{(x_1 , y_1)}{(\tname{a} , \tname{b})}{\\
%                        &\labs{(x_2, y_2)}{(\tname{a} , \tname{b})}{}}}}}}\\
%         &\target {\ottsym{\}}}\end{aligned}
%       }{\tname{main}}}
%\end{aligned}
%\end{fleqn}
%\]
%\let\tname\undefined
%\let\ttall\undefined
%\let\ra\undefined


==> examples/sielab_example1_env.tex <==
\begin{fleqn}
  \begin{align*}
    [[ TC ]] &= \intermed { [[ iequal : iEq c : c -> c -> ibool ]] }
  \end{align*}
\end{fleqn}
\begin{fleqn}
  \begin{align*}
    [[ SS ]] =~&\intermed{ [[ (iD1 : iEq iint) . iequal |-> iprimEqInt ]]}
    \\ \intermed {,}~& \intermed{ [[ (iD2 : \/ empty, c, ib . empty, iEq c, iEq ib => iEq (c , ib)) . iequal |-> /\ c . /\ ib . \ idvar1 : iEq c . \ idvar2 : iEq ib . \ (ix1 , iy1) : (c , ib) . \ (ix2 , iy2) : (c , ib) . ((iand (((idvar1 . iequal) ix1) ix2)) (((idvar2 . iequal) iy1) iy2)) ]] }
  \end{align*}
\end{fleqn}

==> examples/sielab_example1_expr.tex <==
\begin{equation*}
  [[ ilet irefl : \/ c . iEq c -> c -> ibool
  = /\ c . \ idvar3 : iEq c . \ ix : c . (((idvar3 . iequal) ix) ix)
  iin ilet imain : ibool
  = (((irefl ( iint , iint )) (iD2 (empty, iint, iint) (empty, iD1 empty empty, iD1 empty empty))) ( 5 , 42 ))
  iin imain ]]
\end{equation*}

==> examples/sielab_example2_env.tex <==
\begin{fleqn}
  \begin{align*}
    \qquad [[ TC ]] =~&\intermed{ [[ ibase : iBase c : c -> ibool ]] }
    \\ \intermed{,}~&\intermed{ [[ isub1 : iSub1 c : c -> ibool ]] }
    \\ \intermed{,}~&\intermed{ [[ isub2 : iSub2 c : c -> ibool ]] }
  \end{align*}
\end{fleqn}


==> examples/sielab_example2_expr.tex <==
\begin{equation*}
  [[ ilet itest : \/ c . empty, iBase c, iSub1 c, iBase c, iSub2 c -> c -> ibool
  = /\ c . \ idvar1 : iBase c . \ idvar2 : iSub1 c . \idvar3 : iBase c . \ idvar4 : iSub2 c . \ ix : c . ((idvar1 . ibase) ix)
  iin itrue ]]
\end{equation*}

==> examples/stelab_example1_env.tex <==
\begin{fleqn}
  \begin{align*}
    [[ GC ]] &= \source { [[ sequal : empty => sEq a : a -> a -> sbool ]] }
  \end{align*}
\end{fleqn}
\begin{fleqn}
  \begin{align*}
    [[ P ]] &= \source { [[ ( sD1 : sEq sint ) . sequal |-> empty : sprimEqInt ]] }
    \\ & \source { , [[ ( sD2 : \/ empty, a , b . empty, sEq a, sEq b => sEq (a , b) ) .sequal |-> empty, a, b, sdvar1 : sEq a, sdvar2 : sEq b : \ (sx1 , sy1) . \ (sx2 , sy2) . ( ( sand ( (sequal sx1) sx2 ) ) ( (sequal sy1) sy2 ) ) ]] }
  \end{align*}
\end{fleqn}

==> examples/stelab_example1_expr.tex <==
\begin{equation*}
  \target { [[ tlet trefl : \/ ta . { tequal : ta -> ta -> tbool } -> ta -> tbool
  = /\ ta . \ txd3 : { tequal : ta -> ta -> tbool } . \ tx : ta . (((txd3 . tequal) tx) tx)
  tin tlet tmain : tbool
  = (((trefl ( tint , tint )) ( ((((( /\ ta . /\ tb . \ txd4 : { tequal : ta -> ta -> tbool } . \ txd5 : { tequal : tb -> tb -> tbool } . { tequal = \ (tx1 , ty1) : (ta , tb) . \ (tx2 , ty2) : (ta , tb) . (( tand (((txd4 . tequal) tx1 ) tx2) ) (((txd5 . tequal) ty1 ) ty2 ) ) } ) tint ) tint ) {tequal = tprimEqInt} ) {tequal = tprimEqInt} ) )) ( 5 , 42 ))
  tin tmain ]] }
\end{equation*}

==> examples/stelab_example2_env.tex <==
\begin{fleqn}
  \begin{align*}
    [[ GC ]] =~&\source { [[ sbase : empty => sBase a : a -> sbool ]] }
    \\ \source {,}~& \source{ [[ ssub1 : empty, sBase a => sSub1 a : a -> sbool ]] }
    \\ \source {,}~& \source{ [[ ssub2 : empty, sBase a => sSub2 a : a -> sbool ]] }
  \end{align*}
\end{fleqn}

==> examples/stelab_example2_expr.tex <==
\begin{equation*}
  [[ tlet ttest2 : \/ ta . {tbase : ta -> tbool} -> {tsub1 : ta -> tbool} -> {tbase : ta -> tbool} -> {tsub2 : ta -> tbool} -> ta -> tbool
  = /\ ta . \ txd1 : {tbase : ta -> tbool} . \ txd2 : {tsub1 : ta -> tbool} .
  \ tx : ta . ((txd1 . tbase) tx)
  tin ttrue ]]
\end{equation*}

==> figures/inter_envwf.tex <==
\begin{drulepar}{$[[ |-ctx SS ; TC ; TT ]]$}{\interL{} Environment
  Well-Formedness}{
  \ottaltinferrule{iCtx-MEnv}{}{
    [[ unambig ( \/ clj . iqli => iTC is ) ]] \\
    [[ TC ; empty |-c \/ clj . iqli => iTC is ]] \\
    [[ ( im : iTC c : is' ) in TC ]] \\
    [[ SS ; TC ; empty |-tm ie : \/ clj . iqli -> [| is / c |] is' ~> te ]] \\
    [[ iD notin dom (SS) ]] \\
    [[ ( iD' : \/ clm' . iqln' => iTC is' ) . im' |-> ie' notin SS ]] \\
    [[ where [| islj / clj |] is = [| islm' / clm' |] is' ]] \\
    [[ |-ctx SS ; TC ; TT ]]
  }{
    [[ |-ctx SS , ( iD : \/ clj . iqli => iTC is ) . im |-> ie ; TC ; TT ]]
   }
  }
\end{drulepar}%

==> figures/inter_eval.tex <==
\drules[iEval]{$[[ SS |- ie --> ie' ]]$}{\interL{} Evaluation}{DApp, DAppAbs, method}

==> figures/inter_syntax.tex <==
\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  \Mytabular{
  % Types
    \syntaxLine{[[is]] , [[istau]]}
               {::=}
               {\ldots \mid \intermed { [[iq -> is]] } }
               {type}
    \\
  % Class Constraints
    \syntaxLine{[[iq]]}
               {::=}
               {[[iTC is]]}
               {class constraint}
    \\
  % Constraints
    \syntaxLine{[[ic]]}
               {::=}
               {\intermed{ [[\/ cl . iql => iq]] } }
               {constraint}
    \\
  }
\end{array}
\]

\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  \Mytabular{
  % Expression
    \syntaxLine{[[id]]}
               {::=}
               {[[idvar]] \mid \intermed { [[iD isl idl]] } }
               {dictionary}
    \\
    \syntaxLine{[[idv]]}
               {::=}
               {\intermed{[[iD isl idvl]]}}
               {dictionary value}
    \\
    \syntaxLine{[[ie]]}
               {::=}
               {\ldots \mid \intermed{ [[\idvar : iq . ie]] } \mid [[ie id]]
  \mid \intermed{ [[id . im]] } }
               {expression}
    \\
  }
\end{array}
\]

\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  \Mytabular{
  % Typing Context
    \syntaxLine{[[TT]]}
               {::=}
               {\intermed{ [[empty]] } \mid \intermed{ [[TT, ix : is]] } \mid
  \intermed { [[TT, c]] } \mid \intermed { [[TT, idvar : iq]] } }
               {typing environment}
  \\
  % Class Context
    \syntaxLine{[[TC]]}
               {::=}
               {\intermed{[[empty]]} \mid \intermed{[[TC, im : iTC c : is]] } }
               {class environment}
  \\
  % method environment
    \syntaxLine{[[SS]]}
               {::=}
               {\intermed{ [[empty]] } \mid \intermed { [[SS , (iD : ic) . im
  |-> ie]] } }
               {method environment}
    \\
  }
\end{array}
\]

==> figures/inter_typing.tex <==
\drules[iTm]{$[[ SS ; TC ; TT |-tm ie : is ~> te ]]$}{\interL{} Term Typing}{method, constrE}

\[
\ottaltinferrule{iTm-constrI}{}{
  [[ SS ; TC ; TT, idvar : iq |-tm ie : is ~> te ]] \\
  [[ TC ; TT |-q iq ~> tt ]] \\
  [[ te' = \ txd : tt . te ]]
}{
  [[ SS ; TC ; TT |-tm \ idvar : iq . ie : iq -> is ~> te' ]]
}
\]


==> figures/inter_typing_dict.tex <==
\drules[D]{$[[ SS ; TC ; TT |-d id : iq ~> te ]]$}{Dictionary Typing}{}

\[
  \ottaltinferrule{D-var}{}{
    [[ ( idvar : iq ) in TT ]] \\
    [[ |-ctx SS ; TC ; TT ]]
  }{
    [[ SS ; TC ; TT |-d idvar : iq ~> txd ]]
  }
\]

\[
  \ottaltinferrule{D-con}{}{
    [[ ( iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli . ie in SS ]] \\
    \repeated{[[ TC ; empty , clj |-q iqi ~> tt'i ]]}{i} \\
    \repeated{[[ TC ; TT |-ty isj ~> ttj ]]}{j} \\
    [[ SS1 ; TC ; empty, clj , idvarli : iqli |-tm ie : [| isq / c |] ism ~> te ]] \\
    \repeated{[[SS ; TC ; TT |-d idi : [| islj / clj |] iqi ~> tei]]}{i} \\
    [[ SS = SS1, ( iD : \/ clj . iqli => iTC isq) . im |-> /\ clj . \ idvarli : iqli . ie, SS2 ]]
  }{
[[ SS ; TC ; TT |-d iD islj idli : iTC [| islj / clj |] isq ~> ( /\ talj . \ </ txdi : tt'i // i />. { tl = te } ) ttlj teli ]]
   }
\]


==> figures/sourceM_resolution.tex <==
\drules[sEntail]{$[[ P ; GC ; GG |= sq ~> id ]]$}{Constraint Entailment}{}

\[
  \ottaltinferrule{sEntail-local}{}{
    [[ ( sdvar : sq ) in GG ]] \\
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
  }{
    [[ P ; GC ; GG |= sq ~> idvar ]]
  }
\]

\[
  \ottaltinferrule{sEntail-inst}{}{
    [[ P = (? P1, (sD : \/ alj . sqli => sq') . sm |-> GG' : se ?), P2 ]] \\
    [[ GG' = empty, alj, sdvarli : sqli, blk, sdvarlh : sqlh ]] \\
    [[ sq = [| stlj / alj |] sq' ]] \\
    \repeated{[[ GC ; GG |-ty stj ~> isj ]]}{j} \\
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]] \\
    \repeated{[[ P ; GC ; GG |= [| stlj / alj |] sqi ~> idi ]]}{i}
  }{
    [[ P ; GC ; GG |= sq ~> iD islj idli ]]
  }
\]  


==> figures/sourceM_typing.tex <==
  \begin{drulepar}{$[[ P ; GC ; GG |-tm se <= st ~> ie ]]$}{Source Term Checking}{
  \ottaltinferrule{sTm-check-meth}{}{
    [[ ( sm : sqlk' => sTC a : \/ alj . sqli => st' ) in GC ]] \\
    [[ unambig ( \/ alj, a . sqli => st' ) ]] \\
    [[ P ; GC ; GG |= sTC st ~> id ]] \\
    [[ GC ; GG |-ty st ~> is ]] \\
    \repeated{[[ P ; GC ; GG |= [| stlj / alj |] [|st / a |] sqi ~> idi ]]}{i} \\
    \repeated{[[ GC ; GG |-ty stj ~> isj ]]}{j} \\
    [[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]
  }{
    [[ P ; GC ; GG |-tm sm <= [| stlj / alj |] [|st / a |] st' ~> id . im
    istaulj idli ]]
   }
  }
  \end{drulepar}%


==> figures/source_inst_typing.tex <==
\begin{drulepar}{$[[ P ; GC |-inst sinst :  P' ]]$}{Instance Decl Typing}{
  \ottaltinferrule{\textsc{sInstT-inst}}{}{
    [[ ( sm : sqli' => sTC a : \/ alj . sqlh' => st1 ) in GC ]] \\
    [[ blk = fv (st) ]] \\
    [[ GC ; empty, blk |-ty st ~> tt ]] \\
    [[ closure ( GC ; sqlp ) = sqlq ]] \\
    [[ unambig ( \/ blk . sqlq => sTC st ) ]] \\
    \repeated{[[ GC ; empty, blk |-q sqq ~> ttq ]]}{q} \\
    [[ sD fresh ]] \\
    [[ sdvarlq fresh ]] \\
    [[ sdvarlh' fresh ]] \\
    \repeated{[[ PT ; GC ; empty, blk, sdvarlq : sqlq |= [| st / a |] sq'i ~> tei ]]}{i} \\
    [[ GG' = empty, blk, sdvarlq : sqlq , alj, sdvarlh' : [| st / a |] sqlh' ]] \\
    [[ PT ; GC ; GG' |-tm se <= [| st / a |] st1 ~> te ]] \\
    [[ (sD' : \/ blm' . sqln' => sTC st2 ) . sm' |-> GG'' : se' notin PT ]] \\
    \textit{where}~[[ [| stlm' / blm' |] st2 = [| stlk' / blk |] st ]]
    }{
    [[ P ; GC |-inst instance sqlp => sTC st swhere { sm = se } : (sD : \/ blk . sqlq => sTC st) . sm |-> GG' : se ]]
    }
} 
\end{drulepar}


==> figures/source_inst_typing_gen.tex <==
%%% !!! WARNING: AUTO GENERATED. DO NOT MODIFY !!! %%%
\begin{drulepar}{$ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}  \source {  {\source {inst} }  } : \source {  { \source P }'  } $}{Instance Decl Typing}{
  \ottaltinferrule{}{}{
     ( \source {  {\source m}  } : \source {  {\overline {\source Q} }'_{\ottmv{i}}  }  \Rightarrow  \source {  {\source {\mathit{TC} } }  } \source {  {\source a }  } : \source {  \forall  {\overline {\source a} }_{\ottmv{j}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{h}}  \Rightarrow  {\source \tau }_{{\mathrm{1}}}  } )  \in  \source {  {\source { \Gamma_C } }  }  \\
     \source {  {\overline {\source b} }_{\ottmv{k}}  } =  \textbf {fv}  ( \source {  {\source \tau }  } )  \qquad
     \textbf {closure}  ( \source {  {\source { \Gamma_C } }  } ; \source {  {\overline {\source Q} }_{\ottmv{p}}  } ) = \source {  {\overline {\source Q} }_{\ottmv{q}}  }  \\
     \textbf {unambig}  ( \source {  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  } )  \qquad
     \source {  {\source D }  }~ \textbf {fresh}  \\
    \ottcomp{ \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  }  \vDash  \source {  [  {\source \tau }  /  {\source a }  ]  {\source Q}'_{\ottmv{i}}  } \stoi{ \rightsquigarrow  \target {  {\target e }_{\ottmv{i}}  } } }{\ottmv{i}} \\
     \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  } ; \source {  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }'_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  }  \vdash_{tm}  \source {  {\source e}  } \xLeftarrow{c} \source {  [  {\source \tau }  /  {\source a }  ]  {\source \tau }_{{\mathrm{1}}}  } \stoi{ \rightsquigarrow  \target {  {\target e }  } }  \\
     ( \source {  {\source D }'  } : \source {  \forall  {\overline {\source b} }'_{\ottmv{m}}  \ottsym{.}  {\overline {\source Q} }'_{\ottmv{n}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }_{{\mathrm{2}}}  } ) . \source {  {\source m}'  }  \mapsto  \source {  {\source \Gamma}'  } : \source {  {\source e}'  }  \notin  \source {  { \source P }  } : \source {  [  {\overline {\source \tau} }'_{\ottmv{m}}  /  {\overline {\source b} }'_{\ottmv{m}}  ]  {\source \tau }_{{\mathrm{2}}}  } = \source {  [  {\overline {\source \tau} }'_{\ottmv{k}}  /  {\overline {\source b} }_{\ottmv{k}}  ]  {\source \tau }  }  \\
     \source {  { \source P }'  } = \source {  \ottsym{(}  {\source D }  \ottsym{:}  \forall  {\overline {\source b} }_{\ottmv{k}}  \ottsym{.}  {\overline {\source Q} }_{\ottmv{q}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau }  \ottsym{)}  \ottsym{.}  {\source m}  \mapsto  \bullet  \ottsym{,}  {\overline {\source b} }_{\ottmv{k}}  \ottsym{,}  {\overline {\source \delta} }_{\ottmv{q}}  \ottsym{:}  {\overline {\source Q} }_{\ottmv{q}}  \ottsym{,}  {\overline {\source a} }_{\ottmv{j}}  \ottsym{,}  {\overline {\source \delta} }'_{\ottmv{h}}  \ottsym{:}  [  {\source \tau }  /  {\source a }  ]  {\overline {\source Q} }'_{\ottmv{h}}  \ottsym{:}  {\source e}  }  
    \scriptsize{\textsc{sInstT-inst-simp}} \qquad \qquad \qquad \qquad \qquad \qquad
    \qquad \qquad \qquad \qquad \qquad 
    }{
     \source {  { \source P }  } ; \source {  {\source { \Gamma_C } }  }  \vdash_{inst}  \source {  \textbf{\source {instance} } \, {\overline {\source Q} }_{\ottmv{p}}  \Rightarrow  {\source {\mathit{TC} } } \, {\source \tau } \, \textbf{\source {where} } \, \ottsym{\{}  {\source m}  \ottsym{=}  {\source e}  \ottsym{\}}  } : \source {  { \source P }'  } 
    }
} 
\end{drulepar}

==> figures/source_resolution.tex <==
\drules[sEntailT]{$[[ P ; GC ; GG |= sq ~> te ]]$}{Constraint Entailment}{}

\[
  \ottaltinferrule{sEntailT-local}{}{
    [[ ( sdvar : sq ) in GG ]] \\
    [[ |-ctx P ; GC ; GG ~> GT ]]
  }{
    [[ P ; GC ; GG |= sq ~> txd ]]
  }
\]  

\[
  \ottaltinferrule{sEntailT-inst}{}{
    [[ PT = (? PT1, (sD : \/ alj . sqli' => sq') . sm |-> GG' : se ?) , PT2 ]] \\
    [[ GG' = empty, alj, sdvarli : sqli', blk, sdvarlh : sqlh ]] \\
    [[ sq = [| stlj / alj |] sq' ]] \\
    [[ PT1 ; GC ; GG' |-tm se => st ~> te ]] \\
    [[ |-ctx PT ; GC ; GG ~> GT ]] \\
    \repeated{[[ GC ; GG |-ty stj ~> ttj ]]}{j} \\
    \repeated{[[ GC ; empty, alj |-q sqi' ~> tti' ]]}{i} \\
    \repeated{[[ GC ; empty, alj, blk |-q sqh ~> tth'' ]]}{h} \\
    \repeated{[[ PT ; GC ; GG |= [| stlj / alj |] sqi' ~> tei ]]}{i}
  }{
    [[ PT ; GC ; GG |= sq ~> (/\ talj . \ </ txdi' : tti' // i /> . {tl = /\ tblk . \ </ txdh : tth'' // h /> . te}) ttlj teli ]]
  }
\]  


==> figures/source_syntax.tex <==
\[
\begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  % Types
  \Mytabular{
    \syntaxLine{[[st]]}
               {::=}
               {\source { [[sbool]] } \mid \source { [[a]] } \mid \source { [[st1 -> st2]] }}
               {monotype}
    \\
    \syntaxLine{[[sp]]}
               {::=}
               {\source { [[st]] } \mid \source { [[sq => sp]] }}
               {qualified type}
    \\
    \syntaxLine{[[ss]]}
               {::=}
               {\source { [[sp]] } \mid \source { [[\/a. ss]] }}
               {type scheme}
  }
  \\\\
  % Constraints
  \Mytabular{
    \syntaxLine{[[sq]]}
               {::=}
               {\source { [[sTC st]] }}
               {class constraint}
    \\
    \syntaxLine{[[sc]]}
               {::=}
               {\source { [[\/ al . sql => sq]] }}
               {constraint scheme}
  }
  \\\\
  % Expression
  \Mytabular{
    \syntaxLine{[[se]]}
               {::=}
               {\source { [[strue]] } \mid \source { [[sfalse]] } \mid \source { [[sx]] } \mid \source { [[sm]] } \mid \source { [[\sx. se]] } \mid \source { [[se1 se2]] } \mid \source { [[slet sx : ss = se1 sin se2]] } \mid \source { [[se <: st]] }}{term}
  }
  \\\\
  % Program
  \Mytabular{
    \syntaxLine{[[spgm]]}
               {::=}
               {\source { [[se]] } \mid \source { [[scls ; spgm]] } \mid \source { [[sinst ; spgm]] }}
               {\srcL{} program}
    \\
    \syntaxLine{[[scls]]}
               {::=}
               {\source { [[class sTCl => sTC a swhere { sm : ss}]] }}
               {class decl.}
    \\
    \syntaxLine{[[sinst]]}
               {::=}
               {\source { [[instance sql => sTC st swhere { sm = se }]] }}
               {instance decl.}
  }
  \\\\
  % Contexts
  \Mytabular{
    \syntaxLine{[[GG]]}
               {::=}
               {\source { [[empty]] } \mid \source { [[GG, sx : ss]] } \mid \source { [[GG, a]] } \mid \source { [[GG, sdvar : sq]] } }
               {typing environment}
     \\
    \syntaxLine{[[GC]]}
               {::=}
               {\source { [[empty]] } \mid \source { [[GC, sm : sTCl => sTC a : ss]] }}
               {class environment}
     \\
    \syntaxLine{[[PT]]}
               {::=}
               {\source { [[empty]] } \mid \source { [[PT, (sD : sc) . sm |-> GG : se]] }}
               {program context}
     \\
    \syntaxLine{[[sM]]}
               {::=}
               {\source { [[ [empty] ]] } \mid \source { [[\ sx . sM]] } \mid \source { [[sM se]] } \mid \source { [[se sM]] } \mid \source { [[sM <: st]] }}
               {evaluation context}
     \\
    \syntaxLine{}
               {}
               { \mid \source { [[slet sx : ss = sM sin se]] } \mid \source { [[slet sx : ss = se sin sM]] } }
               {}
  }
\end{array}
\]


==> figures/source_typing.tex <==
  \begin{drulepar}{$[[ P ; GC ; GG |-tm se => st ~> te ]]$}{\srcL{} Term Inference}{
  \ottaltinferrule{\textsc{sTm-infT-let}}{}{
    [[sx notin dom ( GG )]] \\
    [[unambig ( \/ alj . sqli => st1 ) ]] \\
    [[closure ( GC ; sqli ) = sqlk]] \\
    \repeated{[[GC ; GG |-q sqk ~> ttk]]}{k} \\
    [[ GC ; GG |-ty \/ alj . sqlk => st1 ~> \/ talj . ttlk -> tt ]] \\
    [[ sdvarlk fresh ]] \\
    [[P ; GC ; GG, alj, sdvarlk : sqlk |-tm se1 <= st1 ~> te1]] \\
    [[P ; GC ; GG, sx : \/ alj . sqlk => st1 |-tm se2 => st2 ~> te2]]
  }{
    \renewcommand\stot[1]{}
    [[ P ; GC ; GG |-tm slet sx : \/ alj . sqli => st1 = se1 sin se2 => st2 ~> te]] \\
    [[~>]] \target{[[tlet tx : \/ talj . ttlk -> tt1 = /\ talj . \ </ txdk : ttk // k /> . te1 tin te2]]}
   }
  }
  \end{drulepar}%
  \begin{drulepar}{$[[ P ; GC ; GG |-tm se <= st ~> te ]]$}{\srcL{} Term Checking}{
  \ottaltinferrule{\textsc{sTm-checkT-meth}}{}{
    [[ ( sm : sqlk' => sTC a : \/ alj . sqli => st' ) in GC ]] \\
    [[ unambig ( \/ alj, a . sqli => st' ) ]] \\
    [[ P ; GC ; GG |= sTC st ~> te ]] \\
    [[ GC ; GG |-ty st ~> tt ]] \\
    \repeated{[[ P ; GC ; GG |= [| stlj / alj |] [|st / a |] sqi ~> tei ]]}{i} \\
    \repeated{[[ GC ; GG |-ty stj ~> ttj ]]}{j} \\
    [[ |-ctx PT ; GC ; GG ~> GT ]] 
  }{
    [[ P ; GC ; GG |-tm sm <= [| stlj / alj |] [|st / a |] st' ~> te . tl
    ttlj teli ]]
   }
  }
  \end{drulepar}%


==> figures/source_typing_extra.tex <==
\drules[sClosure]{$[[ closure ( GC ; sqli ) = sqlj ]]$}{Superclass Closure}{empty, TC}

==> figures/source_typing_extra2.tex <==
\drules[sUnambig]{$[[ unambig ( ss ) ]]$}{Unambiguity for Type Schemes}{scheme}
\drules[sUnambig]{$[[ unambig ( sc ) ]]$}{Unambiguity for Constraints}{constraint}

==> figures/target_Q.tex <==
\drules[iQ]{$[[ TC ; TT |-q iq ~> tt ]]$}{Constr. Well-Formedness}{TC}


==> figures/target_syntax.tex <==
\[
  \begin{array}{@{\hspace{0mm}}c@{\hspace{0mm}}}
  % Dictionary
  \Mytabular{
    \syntaxLine{[[tt]]}
               {::=}
               {\target { [[tbool]] } \mid \target { [[ta]] } \mid \target { [[\/ ta . tt]] } \mid \target { [[tt1 -> tt2]] } \mid \target { [[{ </ tli : tti // i IN n /> }]] }}
               {\targetL{} type}
    \\
    \syntaxLine{[[te]]}
               {::=}
               {\target { [[ttrue]] } \mid \target { [[tfalse]] } \mid \target { [[tx]] } \mid \target { [[\ tx : tt . te]] }
    \mid \target { [[te1 te2]] } \mid \target { [[/\ ta . te]] } \mid \target { [[te tt]] }}
               {\targetL{} term}
    \\
    \syntaxLine{}
               {}
    {\mid \target { [[{ </ tli = tei // i IN n /> }]] } \mid \target { [[te . tl]] } \mid \target { [[tlet tx : tt = te1 tin te2]] }}
               {}
    \\
    \syntaxLine{[[GT]]}
               {::=}
               {\target { [[tempty]] } \mid \target { [[GT , ta]] } \mid \target { [[GT , tx : tt]] }}
               {\targetL{} context}
    \\
  }
\end{array}
\]


==> sections/coherence.tex <==
\section{Coherence}
\label{sec:coherence}
\renewcommand\stoi[1]{{#1}} 
\renewcommand\itot[1]{}

This section provides an outline for our coherence proof, and defines the
required notions.
We first provide a definition of
\textit{contextual equivalence}~\citep{morris1969lambda}, which captures that
two expressions have the same meaning.

\subsection{Contextual Equivalence}

In order to formally discuss the concept of contextual equivalence, we first define the notion of an
\textit{expression context}.

\paragraph{\textbf{Expression Contexts.}}
An expression context $[[sM]]$ is an expression
with a single hole, for which another expression \([[se]]\) can be filled in,
denoted as \(\source{[[sM]] [ [[se]] ]}\).
The syntax can be found in Figure~\ref{fig:source_syntax}.

The typing judgment for an expression context \([[sM]]\) is of the form
$[[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' ==> st' ) ~~> tM ]]$.
This means that for any
expression \([[se]]\) such that $[[P ; GC ; GG |-tm se => st ~> te]]$,
we have $[[P ; GC ; GG' |-tm sM ( se ) => st' ~> te']]$.
Following regular \srcL{} term typing, context typing spans all combinations
of type inference and checking mode:
$[[ sM : ( P ; GC ; GG ==> st ) |--> ( P ; GC ; GG' <== st' ) ~~> tM ]]$, 
$[[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' ==> st' ) ~~> tM ]]$ and
$[[ sM : ( P ; GC ; GG <== st ) |--> ( P ; GC ; GG' <== st' ) ~~> tM ]]$.

For example, the simplest expression context is the
empty context $[[ [empty] : (P ; GC ; GG ==> st) |--> (P ; GC ; GG ==> st) ~~>
[tempty] ]]$.

Now we can formally define contextual equivalence. Note that the small step
operational semantics can be found in Section~\ref{app:tgt_op} of the appendix.
The environment and type well-formedness judgments can be found in
Sections~\ref{app:src_env_wf} and~\ref{app:src_ty_wf} of the appendix respectively.
\begin{definition}[Kleene Equivalence]\leavevmode \\
  Two \targetL{} expressions \gsp $\target{[[te1]]}$ \gsp and \gsp
  $\target{[[te2]]}$ \gsp are
  Kleene equivalent, written \gsp $[[ te1 ~= te2 ]]$, \\ if there exists 
    a value \gsp $[[ tv ]]$ \gsp such that \gsp $[[ te1 -->> tv ]]$, and \gsp $[[ te2 -->> tv ]]$.
  \label{def:kleene_tgt}
\end{definition}

\begin{definition}[Contextual Equivalence]\leavevmode \\
  Two expressions \gsp
  $[[ GT |-tm te1 : tt ]]$ \gsp and \gsp $[[ GT |-tm te2 : tt ]]$, \\ where \gsp
  $[[ |-ctx P ; GC ; GG ~> GT ]]$ \gsp and \gsp $[[ GC ; GG |-ty st ~> tt ]]$, \\
  are contextually equivalent, written \gsp
  $[[ P ; GC ; GG |- te1 =ctx te2 : st ]]$, \\ if forall \gsp
  $[[ sM : (P ; GC ; GG ==> st) |--> (P ; GC ; empty ==> sbool) ~~> tM1
  ]]$ \\
  and \gsp $[[ sM : (P ; GC ; GG ==> st) |--> (P ; GC ; empty ==> sbool) ~~> tM2 ]]$ \\
  implies \gsp $[[ tM1 (te1) ~= tM2 (te2) ]]$.
  \label{def:ctx_tgt}
\end{definition}

The definition is adapted from~\citet[Chapter 46]{PFPL46}.
Intuitively, contextual equivalence means that two open expressions are
observationally indistinguishable, when used in any program that instantiates
the expressions' free variables.

\subsection{Coherence}

We can now make a first attempt to prove 
that different translations of the same
source program are contextually equivalent. The program typing judgment
can be found in Section~\ref{app:src_tm_typing} of the appendix.

\begin{theoremB}[Coherence]\leavevmode \\
  If \gsp \([[ empty ; empty |-pgm spgm : st ; PT1 ; GC1 ~> te1 ]]\) \gsp
  and \gsp \([[ empty ; empty |-pgm spgm : st ; PT2 ; GC2 ~> te2 ]]\) \\
  then \gsp \([[ GC1 = GC2 ]]\), \([[ PT1 = PT2 ]]\) \gsp
  and \gsp \([[ PT1 ; GC1 ; empty |- te1 =ctx te2 : st ]]\).
  \label{thm:coh}
\end{theoremB}

We first set out to prove the simpler variant, which only considers
expressions~\footnote{Theorem~\ref{thm:ecoh} also has a type checking mode
  counterpart, which has been omitted here for space reasons.}.

\begin{theoremB}[Expression Coherence]\leavevmode \\
  If \gsp \([[ PT ; GC ; GG |-tm se => st ~> te1 ]]\) \gsp
  and \gsp \([[ PT ; GC ; GG |-tm se => st ~> te2 ]]\) \\
  then \gsp \([[ PT ; GC ; GG |- te1 =ctx te2 : st ]]\).
  \label{thm:ecoh}
\end{theoremB}

The main requirement which makes type class resolution coherent is that type
class instances do not overlap. However, since \targetL{} uses records to encode
dictionaries, the \targetL{} language does not enforce this crucial uniqueness property.
In order to prove Theorem~\ref{thm:coh}, we introduce an
additional intermediate language \interL{}, which captures the invariant that
type class instances do not overlap, and makes it explicit. 

\renewcommand\itot[1]{#1}

%%% Local Variables:
%%% mode: latex
%%% org-ref-default-bibliography: ../paper.bib
%%% End:


==> sections/coherence2.tex <==
\section{Coherence Revisited}
\label{sec:coherence2}
\renewcommand\stoi[1]{{#1}} 
\renewcommand\itot[1]{}

As mentioned previously in Section~\ref{sec:coherence}, the invariant that type
class instances do not overlap is crucial in proving Theorem~\ref{thm:coh}.
This uniqueness property is made explicit in \interL{}.
Our proof thus proceeds by elaborating the \srcL{} expression to two possibly
different \interL{} expressions and subsequently elaborating these \interL{}
expressions to \targetL{} expressions.
Consequently, the proof is split in two main steps.
The first part is the most involved, where we use a technique based on logical
relations to prove that any two \interL{} expressions originating from the same
\srcL{} expression are contextually equivalent.
The second part proves that the elaboration from \interL{} to
\targetL{} is contextual equivalence preserving. This step follows
straightforwardly from the fact that the \interL{}-to-\targetL{} elaboration is deterministic.
Together, these prove that the elaboration from \srcL{} to \targetL{} through
\interL{} is coherent. Theorem~\ref{thm:ecoh} follows from this result,
together with Theorem~\ref{thm:equiv_expr}. 

The remainder of this section explains the techniques we used to prove
Theorem~\ref{thm:coh} in detail.

\subsection{Coherent Elaboration from \srcL{} to \interL{}}

\subsubsection{\textbf{Logical Relations.}}
\renewcommand\itot[1]{}

Logical relations~\citep{plotkin1973lambda, statman1985logical,
tait1967intensional} are key to proving contextual equivalence. In
our type system, the logical relation for expressions is mostly standard,
though the relation for dictionaries is novel.

\paragraph{\textbf{Dictionaries.}}

The logical relation over two open dictionaries is defined by means of an
auxiliary relation on closed dictionaries.
We define this value relation for closed dictionaries as follows.
Note that from now on, we will omit elaborations when they are entirely
irrelevant. The appendix uses the same convention.

\begin{definition}[Value Relation for Dictionaries] \leavevmode \\
  The dictionary values \gsp
  $\intermed{[[iD islj idvl1i]]}$ \gsp
  and \gsp
  $\intermed{[[iD islj idvl2i]]}$ \gsp
  are in the value relation, defined as:

  \begin{flalign*}
    &[[ (SS1 : iD islj idvl1i, SS2 : iD islj idvl2i) in V (iq) with TC ; R ]] \triangleq
    \repeated{[[ (SS1 : idv1i , SS2 : idv2i) in V ([| islj / clj |] iqi) with TC ; R ]]}{i} &\\
    &\qquad
      \begin{aligned}
        & \land \gsp [[ SS1 ; TC ; empty |-d iD islj idvl1i : R (iq) ~> te1 ]] \gsp
        \land \gsp [[ SS2 ; TC ; empty |-d iD islj idvl2i : R (iq) ~> te2 ]], \\
        & \textit{where } [[ (iD : \/ clj . iqli => iq') . im |-> ie1 in SS1 ]] 
        \land [[ iq = [| islj / clj |] iq' ]]
      \end{aligned}
  \end{flalign*}
\end{definition}

The value relation is indexed by the dictionary type \([[iq]]\).
We require both dictionaries to be well-typed, and their dictionary arguments to
be in the value relation as well.
The relation has four additional parameters:
the contexts \(\intermed{[[SS1]]}\) and \(\intermed{[[SS2]]}\), which annotate the dictionaries, the
class environment \([[TC]]\), used in the well-typing condition,
and the type substitution \([[R]]\).

In order to define logical equivalence between open dictionaries, we substitute
all free variables with closed terms, thus reducing them to closed dictionary
values. Three kinds of variables exist (term variables \([[ix]]\), type
variables \([[c]]\) and dictionary variables \([[idvar]]\)). This results in three
separate semantic interpretations of the typing context \([[TT]]\).
The type substitution \([[ R in F (TT) with TC ]]\) maps all type variables
\([[ c in TT ]]\) onto closed types.
\([[ phi in G (TT) with SS1 ; SS2 ; TC ; R ]]\) maps each term
variable \([[ ix in TT ]]\) to two expressions \(\intermed{[[ie1]]}\) and
\(\intermed{[[ie2]]}\) that are in the
expression value relation (see Definition~\ref{def:expr_val_rel}),
and \([[ gamma in H (TT) with SS1 ; SS2 ; TC ; R ]]\) maps each dictionary
variable \([[ idvar in TT ]]\) to two logically related dictionary values.
We use \(\intermed{[[phi1]]}\) and \(\intermed{[[phi2]]}\) to denote the substitution for the first
and second expression, respectively.

\begin{definition}[Logical Equivalence for Dictionaries]\leavevmode \\
  Two dictionaries \gsp
  $\intermed{[[id1]]}$ \gsp
  and \gsp
  $\intermed{[[id2]]}$ \gsp
  are logically equivalent, defined as:
  \begin{flalign*}
    &[[TC ; TT |- SS1 : id1 =log SS2 : id2 : iq]]
    \triangleq \gsp \forall [[R in F ( TT ) with TC]], \gsp
       [[phi in G ( TT ) with SS1 ; SS2 ; TC ; R]], \gsp
       [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]] : &\\
    &\qquad [[ (SS1 : id1 with R ; phi1; gamma1, SS2 : id2 with R ; phi2 ; gamma2) in V (iq) with TC ; R]]
  \end{flalign*}
\end{definition}

Two dictionaries \(\intermed{[[id1]]}\) and \(\intermed{[[id2]]}\) are logically
equivalent if any substitution of their free variables (with related expressions
/ dictionaries) results in related dictionary values. 

\paragraph{\textbf{Expressions.}}

The value relation for expressions is mostly standard, with two notable
deviations. Firstly, the relation is defined over two different method
environments \(\intermed{[[SS1]]}\) and \(\intermed{[[SS2]]}\).
Hence, both expressions are annotated with their respective
environment. Secondly, the dictionary abstraction case is novel.

\begin{definition}[Value Relation for Expressions]\leavevmode \\
  Two values \gsp
  $\intermed{[[iv1]]}$ \gsp
  and \gsp
  $\intermed{[[iv2]]}$ \gsp
  are in the value relation, defined as:
  \begin{flalign*}
    &[[ (SS1 : itrue, SS2 : itrue) in V (ibool) with TC ; R ]] &\\
    &[[ (SS1 : ifalse, SS2 : ifalse) in V (ibool) with TC ; R ]] &\\
    &[[ (SS1 : iv1 , SS2 : iv2) in V (c) with TC ; R ]]
    \triangleq &\\
    &\qquad [[ (c |-> (is, r)) in R ]] \gsp
    \land \gsp [[ (iv1 , iv2) in r ]] \gsp
    \land \gsp [[ SS1 ; TC ; empty |-tm iv1 : is ~> te1 ]] \gsp
      \land \gsp [[ SS2 ; TC ; empty |-tm iv2 : is ~> te2 ]] &\\
    &[[ (SS1 : \ ix : is1 . ie1 , SS2 : \ix : is1 . ie2) in V (is1 -> is2) with TC ; R ]]
    \triangleq &\\
    &\qquad [[ SS1 ; TC ; empty |-tm \ix : is . ie1 : R ( is1 -> is2 ) ~> te1 ]] \gsp
    \land \gsp [[ SS2 ; TC ; empty |-tm \ix : is . ie2 : R ( is1 -> is2 ) ~> te2 ]] &\\
    &\qquad \land \forall [[ (SS1 : ie3, SS2 : ie4) in E (is1) with TC ; R ]] :
    [[ ( SS1 : (\ ix : is . ie1) ie3, SS2 : (\ ix : is . ie2) ie4 ) in E (is2) with TC ; R]] &\\
    &[[ (SS1 : \idvar : iq . ie1 , SS2 : \idvar : iq . ie2) in V (iq -> is) with
    TC ; R ]]
    \triangleq &\\
    &\qquad [[ SS1 ; TC ; empty |-tm \idvar : iq . ie1 : R ( iq -> is ) ~> te1 ]] \gsp
    \land \gsp [[ SS2 ; TC ; empty |-tm \idvar : iq . ie2 : R ( iq -> is ) ~> te2 ]] &\\
    &\qquad \land \forall [[ (SS1 : idv1, SS2 : idv2) in V (iq) with TC ; R ]] :
    [[ ( SS1 : (\ idvar : iq . ie1) idv1, SS2 : (\ idvar : iq . ie2) idv2 ) in E (is) with TC ; R]] &\\
    &[[ ( SS1 : /\ c . ie1 , SS2 : /\ c . ie2) in V (\/ c . is) with TC ; R ]]
    \triangleq &\\
    &\qquad [[ SS1 ; TC ; empty |-tm /\ c. ie1 : R (\/ c. is) ~> te1 ]] \gsp
    \land \gsp [[ SS2 ; TC ; empty |-tm /\ c. ie2 : R (\/ c. is) ~> te2 ]] &\\
    &\qquad \land \forall \intermed{[[is']]}, \forall [[r in Rel ( is' )]] : \gsp
      [[ TC ; empty |-ty is' ~> tt' ]] \Rightarrow
      [[ ( SS1 : (/\ c . ie1) is', SS2 : (/\ c . ie2) is' ) in E (is) with TC ; R , c |-> (is', r) ]]
  \end{flalign*}
  \label{def:expr_val_rel}
\end{definition}

Consider the interesting case of dictionary abstraction. The relation
requires the terms to be
well-typed, and the applications for all related input dictionaries
to be in the expression relation \(\mathcal{E}\). The definition of this \(\mathcal{E}\) relation
is as follows:

\begin{definition}[Expression Relation]\leavevmode \\
  Two expressions \gsp
  $\intermed{[[ie1]]}$ \gsp
  and \gsp
  $\intermed{[[ie2]]}$ \gsp
  are in the expression relation, defined as:
  \begin{flalign*}
    &[[ ( SS1 : ie1 , SS2 : ie2 ) in E ( is ) with TC ; R ]]
    \triangleq [[ SS1 ; TC ; empty |-tm  ie1 : R (is) ~> te1 ]] \gsp
    \land [[ SS2 ; TC ; empty |-tm  ie2 : R (is) ~> te2 ]] &\\
    &\qquad \land \exists \intermed{[[iv1]]} , \intermed{[[iv2]]},
    [[SS1 |- ie1 -->> iv1]],
    [[SS2 |- ie2 -->> iv2]],
    [[ (SS1 : iv1, SS2 : iv2) in V (is) with TC ; R]]
  \end{flalign*}
\end{definition}

In this definition, expressions are reduced to values and those values must be
in the value relation. This is well-defined because \interL{} is
strongly normalizing~(Theorem~\ref{theorem:inter-sn}).

Finally, we can give the definition of logical equivalence for open expressions:

\begin{definition}[Logical Equivalence for Expressions]\leavevmode \\
  Two expressions \gsp
  $\intermed{[[ie1]]}$ \gsp
  and \gsp
  $\intermed{[[ie2]]}$ \gsp
  are logically equivalent, defined as:
  \begin{flalign*}
    &[[TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is]]
    \triangleq \forall [[R in F ( TT ) with TC]], \gsp
       [[phi in G ( TT ) with SS1 ; SS2 ; TC ; R]], \gsp
       [[ gamma in H ( TT ) with SS1 ; SS2 ; TC ; R ]] : &\\
    &\qquad  [[ (SS1 : ie1 with R ; phi1 ; gamma1, SS2 : ie2 with R ; phi2 ; gamma2) in E (is) with TC ; R]]
  \end{flalign*}
\end{definition}

We also provide a definition of logical equivalence for contexts:

\begin{definition}[Logical Equivalence for Contexts]\leavevmode \\
  \label{def:log_M}
  Two contexts \gsp \(\intermed{[[iM1]]}\) \gsp and \gsp \(\intermed{[[iM2]]}\) \gsp
  are logically equivalent, defined as:
  \begin{flalign*}
    &[[SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; TT' ==>
    is')]]
    \triangleq &\\
    &\qquad \forall \intermed{[[ ie1 ]]}, \intermed{[[ ie2 ]]}:
    [[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]] \gsp \Rightarrow \gsp
    [[ TC ; TT' |- SS1 : iM1 (ie1) =log SS2 : iM2 (ie2) : is' ]]
  \end{flalign*}
\end{definition}


\subsubsection{\textbf{Proof of \srcL{}-to-\interL{} Coherence.}}

With the above definitions we are ready to formally state the metatheory and
establish the coherence theorems from \srcL{} to \interL{}.

\paragraph{\textbf{Design Principle of \interL.}} 

We emphasize that \interL{} captures the intention of type class
instances. Theorem~\ref{thm:dval_rel} states that any two dictionary
values for the same constraint are logically related:

\begin{theoremB}[Value Relation for Dictionary Values]\leavevmode \\
  \label{thm:dval_rel}
  If \gsp \([[ SS1 ; TC ; empty |-d idv1 : iq ~> te1 ]]\) \gsp and \gsp \([[ SS2 ; TC ; empty |-d idv2 : iq ~> te2 ]]\) \gsp
  and \gsp \([[ TC |- SS1 =log SS2 ]]\) \\
  then \gsp \([[ (SS1 : idv1 , SS2 : idv2) in V (iq) with TC ; empty ]]\).
\end{theoremB}

Note that two environments \(\intermed{[[SS1]]}\) and \(\intermed{[[SS2]]}\) are
logically equivalent under \([[TC]]\), written \([[ TC |- SS1 =log SS2 ]]\),
when they contain the same dictionary constructors and the corresponding method
implementations are logically equivalent. The full definition can be found in
Section~\ref{app:log_env_rel} of the appendix.

\paragraph{\textbf{Coherent Resolution.}} 
\renewcommand\itot[1]{{#1}}

We now prove that constraint resolution is semantically
coherent, that is, if multiple resolutions of the same
constraint exist, they are logically equivalent.

\begin{theoremB}[Logical Coherence of Dictionary Resolution]\leavevmode \\
  If \gsp \([[ P ; GC ; GG |= sq ~> id1 ]]\) \gsp
  and \gsp \([[ P ; GC ; GG |= sq ~> id2 ]]\) \\
  and \gsp \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\) \gsp
  and \gsp \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
  then \gsp \([[ TC ; TT |- SS1 : id1 =log SS2 : id2 : iq ]]\) \gsp
  where \gsp \([[ GC ; GG |-q sq ~> iq ]]\).
  \label{thm:dict_cohA}
\end{theoremB}

\paragraph{\textbf{Coherent Elaboration.}} 

Furthermore, in order to prove that the elaboration from \srcL to \interL is coherent,
we show that all elaborations of the same expression are logically
equivalent~\footnote{Theorem~\ref{thm:coh_exprA} also has a type checking mode
  counterpart, which has been omitted here for space reasons.}.

\begin{theoremB}[Logical Coherence of Expression Elaboration]\leavevmode \\
  If \gsp \([[ P ; GC ; GG |-tm se => st ~> ie1 ]]\) \gsp
  and \gsp \([[ P ; GC ; GG |-tm se => st ~> ie2 ]]\) \\
  and \gsp \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\) \gsp
  and \gsp \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \\
  then \gsp \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\) \gsp
  where \gsp \([[ GC ; GG |-ty st ~> is ]]\).
  \label{thm:coh_exprA}
\end{theoremB}

\paragraph{\textbf{Contextual Equivalence.}}
We prove that all logically equivalent expressions are contextually
equivalent. Together with Theorem~\ref{thm:coh_exprA}, this shows coherence of the
\srcL{}-to-\interL{} elaboration.

We first provide a formal definition of
contextual equivalence for \interL{} expressions.
Kleene equivalence for \interL{} is defined similarly to
Definition~\ref{def:kleene_tgt} and can be found in Section~\ref{app:log_kleene} of the appendix.

\renewcommand\itot[1]{}
\begin{definition}[Contextual Equivalence for \interL{} Expressions]\leavevmode \\
  Two expressions \gsp $[[ SS1 ; TC ; TT |-tm ie1 : is ~> te1 ]]$ \gsp
  and \gsp $[[ SS2 ; TC ; TT |-tm ie2 : is ~> te2 ]]$, \\
  are contextually equivalent, written 
  \gsp $[[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]$, \\
  if forall \gsp $[[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~> tM1 ]]$ \\
  and forall \gsp $[[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~> tM2 ]]$ \\
  where \gsp $[[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==> ibool) ]]$, \\
  we have that \gsp $[[ SS1 : iM1 ( ie1 ) ~= SS2 : iM2 ( ie2 ) ]]$.
  \label{def:ctx_mid}
\end{definition}
\renewcommand\itot[1]{#1}

\begin{theoremB}[Logical Equivalence implies Contextual Equivalence]\leavevmode \\
  \label{thm:coh_exprB}
  If \gsp \([[ TC ; TT |- SS1 : ie1 =log SS2 : ie2 : is ]]\) \gsp
  then \gsp \([[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]\).
\end{theoremB}
% \qed

\subsection{Deterministic Elaboration from \interL{} to \targetL{}}
\subsubsection{\textbf{Contextual Equivalence.}}
\renewcommand\itot[1]{{#1}}

Similarly to expressions, the elaboration from a \srcL{} context \([[sM]]\) to a
\targetL{} context \([[tM]]\) can always be decomposed into two elaborations,
through a \interL{} context \([[iM]]\).
The syntax and typing judgments can be found in Sections~\ref{app:syntax} and~\ref{app:context_typing} of
the appendix, respectively. 

We now formally define contextual equivalence for \targetL{} expressions through
\interL{} contexts.
\begin{definition}[Contextual Equivalence in \interL{} Context]\leavevmode \\
  Two expressions \gsp $[[ GT |-tm te1 : tt ]]$ \gsp and \gsp $[[ GT |-tm te2 : tt ]]$, \\
  where \gsp $[[ |-ctx P ; GC ; GG ~> GT ]]$ \gsp and \gsp $[[ GC ; GG |-ty st ~> tt ]]$, \\
  are contextually equivalent, written \gsp $[[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 :
  is ]]$, \\
  if forall \gsp $ [[ iM1 : (SS1 ; TC ; TT ==> is) |--> (SS1 ; TC ; empty ==> ibool) ~>
  tM1 ]]$ \\
  and forall \gsp $ [[ iM2 : (SS2 ; TC ; TT ==> is) |--> (SS2 ; TC ; empty ==> ibool) ~>
  tM2 ]]$ \\
  where \gsp $[[ SS1 : iM1 =log SS2 : iM2 : (TC ; TT ==> is) |--> (TC ; empty ==>
  ibool) ]]$, \\
  we have that \gsp $[[ tM1 (te1) ~= tM2 (te2) ]]$, \\
  where \gsp $[[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]$ \gsp and \gsp $[[ TC ; TT
  ~> GT ]]$ \gsp and \gsp $[[ GC ; GG |-ty st ~> is ]]$ \gsp and \gsp $[[ TC ;
  TT |-ty is ~> tt ]]$. 
  \label{def:ctx_tgt_mid}
\end{definition}

\subsubsection{\textbf{Proof of \interL{}-to-\targetL{} Coherence.}}

We continue by proving that contextual equivalence is preserved by the
elaboration from \interL{} to \targetL{}:

\begin{theoremB}[Elaboration preserves Contextual Equivalence]\leavevmode \\
  If \gsp \([[ TC ; TT |- SS1 : ie1 =ctx SS2 : ie2 : is ]]\) \\
  and \gsp \([[ SS1 ; TC ; TT |-tm ie1 : is ~> te1 ]]\) \gsp
  and \gsp \([[ SS2 ; TC ; TT |-tm ie2 : is ~> te2 ]]\) \gsp
  and \gsp \([[ TC ; TT ~> GT ]]\) \\
  then \gsp \([[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]\).
  \label{thm:coh_exprC}
\end{theoremB}
% \qed

\subsubsection{\textbf{Proof of \srcL{}-to-\targetL{} Coherence.}}

Finally, in order to link back to Theorem~\ref{thm:ecoh} (which has no notion of
\interL{}), we prove that contextual equivalence with \interL{} contexts implies
contextual equivalence with \srcL{} contexts:

\begin{theoremB}[Contextual Equivalence in \interL{} implies Contextual
    Equivalence in \srcL{}]\ \\
  If \gsp \([[ TC ; TT |- SS1 : te1 =ctx SS2 : te2 : is ]]\) \\
  and \gsp \([[ |-ctx P ; GC ; GG ~> SS1 ; TC ; TT ]]\) \gsp
  and \gsp \([[ |-ctx P ; GC ; GG ~> SS2 ; TC ; TT ]]\) \gsp
  and \gsp \([[ GC ; GG |-ty st ~> is ]]\) \\
  then \gsp \([[ P ; GC ; GG |- te1 =ctx te2 : st ]]\).
  \label{thm:ctx_equiv_pres}
\end{theoremB}

For clarity, we restate coherence Theorems~\ref{thm:ecoh} and~\ref{thm:coh}:

\newtheorem*{thm:ecoh}{Theorem \ref*{thm:ecoh}}
\begin{thm:ecoh}[Expression Coherence - Restated]\leavevmode \\
  If \gsp \([[ PT ; GC ; GG |-tm se => st ~> te1 ]]\) \gsp
  and \gsp \([[ PT ; GC ; GG |-tm se => st ~> te2 ]]\) \\
  then \gsp \([[ PT ; GC ; GG |- te1 =ctx te2 : st ]]\).
\end{thm:ecoh}

Theorem~\ref{thm:ecoh} follows by combining
Theorems~\ref{thm:equiv_expr}, \ref{thm:coh_exprA}, \ref{thm:coh_exprB},
\ref{thm:coh_exprC} and~\ref{thm:ctx_equiv_pres}. 

\newtheorem*{thm:coh}{Theorem \ref*{thm:coh}}
\begin{thm:coh}[Coherence - Restated]\leavevmode \\
  If \gsp \([[ empty ; empty |-pgm spgm : st ; PT1 ; GC1 ~> te1 ]]\) \gsp
  and \gsp \([[ empty ; empty |-pgm spgm : st ; PT2 ; GC2 ~> te2 ]]\) \\
  then \gsp \([[ GC1 = GC2 ]]\), \([[ PT1 = PT2 ]]\) \gsp
  and \gsp \([[ PT1 ; GC1 ; empty |- te1 =ctx te2 : st ]]\).
\end{thm:coh}

Finally, we show that Theorem~\ref{thm:coh} follows from
Theorem~\ref{thm:ecoh}.
The full proofs can be found in Section~\ref{app:coh} of the appendix.
% \qed

\renewcommand\itot[1]{#1}

%%% Local Variables:
%%% mode: latex
%%% org-ref-default-bibliography: ../paper.bib
%%% End:


==> sections/inter.tex <==
\section{Intermediate Language \interL{}}\label{sec:inter}

This section presents our intermediate language \interL{}.
The language is modeled with three main goals in mind:
\begin{inparaenum}[(a)]
\item \interL{} should explicitly pass type class dictionaries, which are 
      implicit in \srcL;
\item the \interL{} type system should capture the uniqueness of
  dictionaries, thus enforcing the elaboration from
  \srcL{} to preserve full abstraction; and
\item \interL{} expressions should elaborate straightforwardly and
  deterministically to the target language \targetL{} (System F with records, see
  Section~\ref{sec:target}).
\end{inparaenum}

To this end, \interL{} is an extension of System F, with built-in support for
dictionaries. These dictionaries differ from those commonly used in
Haskell compilers in that they are special constants rather than a record of
method implementations. A separate global map \([[SS]]\) from dictionaries
to method implementations gives access to the latter. Note that this setup does
not allow programs to introduce new (and possibly overlapping) dictionaries dynamically.
All dictionaries have to be provided upfront, where uniqueness is easily enforced.

\paragraph{\textbf{Syntax.}}
Figure~\ref{fig:inter_syntax} shows selected syntax of \interL{};
the basic System F constructs are omitted and can be found in 
Section~\ref{app:mid_syntax} of the appendix.

\boxedfigure
  {\input{figures/inter_syntax.mng}}
  {\interL{}, selected syntax}
  {fig:inter_syntax}

\interL{} introduces a new syntactic sort of 
dictionaries \([[id]]\) that can either be a dictionary variable
\([[idvar]]\) or a dictionary constructor \([[iD]]\). A dictionary
constructor has a number (possibly zero) of type and dictionary parameters and always
appears in fully-applied form.
Each constructor corresponds to a unique instance declaration, and is
mapped to its method implementation by the global environment \([[SS]]\).

Expressions have explicit application and abstraction forms for dictionaries.
Furthermore, similarly to \targetL{}, method names can no longer
be used on their own. Instead, they have to be applied explicitly to a
dictionary, in the form \([[id . im]]\).

\interL{} types \([[is]]\) or \([[istau]]\) are identical to the well-known
System F types, with the addition of a special function type \(\intermed{[[iq -> is]]}\)
for dictionary abstractions. 

Similarly to \srcL{}, \interL{} features two global
and a single local environment \([[TT]]\). The latter is similar to the \srcL{}
typing environment \([[GG]]\). However, there are notable differences between
the global environments. The \interL{} class environment \([[TC]]\)
does not contain any superclass information.
The reason for this is that, as previously mentioned in Section~\ref{sec:source},
superclass constraints in the source language \srcL{} are flattened into local
constraints, and stored in the typing environment \([[GG]]\).
The analog to the \srcL{} program context
\([[P]]\) is the \interL{} method environment \([[SS]]\), storing
information about all dictionary constructors \([[iD]]\).
Each constructor corresponds to a unique instance declaration,
and stores the accompanying method implementations.

\paragraph{\textbf{Typing.}}
\renewcommand\itot[1]{} 
Figure~\ref{fig:inter_typing} (left-hand side) shows selected typing rules for
\interL{} expressions.
The red parts can be safely ignored
for now, as they will be explained in detail in Section~\ref{sec:elabIT}.
The judgment \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\) expresses that the \interL{}
term \([[ie]]\) of type \([[is]]\) is well-typed under environments \([[SS]]\),
\([[TC]]\) and \([[TT]]\).
As shown by rule~\textsc{iTm-method}, the type of a method variable applied to a
dictionary is simply the corresponding method type (as stored in the
static class environment), where the type variable has been substituted for the
corresponding dictionary type.
\renewcommand\itot[1]{#1} 

\boxedfigure
{
  \begin{subfigure}[t]{0.49\textwidth}
    \vskip 0pt
    \input{figures/inter_typing.mng}
  \end{subfigure}
  \vrulesep
  \begin{subfigure}[t]{0.49\textwidth}
    \vskip 0pt
    \input{figures/target_Q.mng}
    \hrulesep
    \input{figures/inter_eval.mng}
  \end{subfigure}
}
{\interL{} typing and operational semantics, selected rules}
{fig:inter_typing}

\boxedfigure
  {\input{figures/inter_envwf.mng}}
  {\interL{} environment well-formedness, selected rules}
  {fig:inter_env_wf}

\boxedfigure
  {\input{figures/inter_typing_dict.mng}}
  {\interL{} dictionary typing}
  {fig:inter_dict_typing}

\renewcommand\itot[1]{} 
Figure~\ref{fig:inter_dict_typing} shows the typing rules for
dictionaries. The relation
\([[ SS ; TC ; TT |-d id : iq ~> te ]]\) denotes that dictionary \([[id]]\) of
dictionary type \([[iq]]\) is well-formed
under environments \([[SS]]\), \([[TC]]\) and \([[TT]]\).
Similarly to regular term variables \([[ix]]\) (\textsc{iTm-var}),
the type of a dictionary variable \([[idvar]]\) (\textsc{D-var}) is obtained
from the typing environment \([[TT]]\).
The type of a dictionary constructor \([[iD]]\) (\textsc{D-con}), on the other
hand, is obtained by finding the corresponding entry in the method environment \([[SS]]\) and
substituting any types \(\intermed{[[islj]]}\) applied to it in the
corresponding class constraint \(\intermed{[[iTC isq]]}\). All
applied dictionaries \(\intermed{[[idli]]}\) have to be well-typed with the corresponding
constraint. Finally, the corresponding method implementation has to be
well-typed in the reduced method environment \(\intermed{[[SS1]]}\), which only contains
the instances declared before \([[iD]]\). As mentioned in
Section~\ref{sec:source}, this reduced environment disallows
recursive method implementations, as this would significantly clutter the
coherence proof while, as a feature, recursion is completely orthogonal to the desired property.
\renewcommand\itot[1]{#1} 

\paragraph{\textbf{Non-Overlapping Instances.}}
The main requirement for achieving coherence of type class resolution, is that
type class instances do not overlap. This requirement is common in Haskell and
is for example enforced in GHC (though strongly discouraged, 
the \texttt{OverlappingInstances} pragma disables it).
By storing all method implementations (with their corresponding instances) in a
single environment \([[SS]]\), this invariant can easily be made explicit.

Figure~\ref{fig:inter_env_wf} shows the
environment well-formedness condition \([[ |-ctx SS ; TC ; TT ]]\) for the method environment.
Besides stating well-scopedness, it denotes that the method
environment \([[SS]]\) cannot contain a second instance, for which the head of
the constraint overlaps with \(\intermed{[[iTC is]]}\), up to renaming.
This key property will be exploited in our coherence proof. 

\paragraph{\textbf{Operational Semantics.}}
As \interL{} is an extension of System F, its call-by-name operational
semantics  are mostly standard. The non-standard rules can be found
in Figure~\ref{fig:inter_typing} (bottom right), where \([[ SS |- ie --> ie' ]]\) denotes
expression \([[ie]]\) evaluating to \(\intermed{[[ie']]}\) in a single step, under method
environment \([[SS]]\).

The evaluation rules for dictionary application (\textsc{iEval-DApp} and
\textsc{iEval-DAppAbs}) are identical to those for term and type application.
More interesting, however, is the evaluation for methods (\textsc{iEval-method}).
A method name applied to a dictionary evaluates in one step to the method
implementation, as stored in the environment \([[SS]]\). 

\renewcommand\itot[1]{} 
\paragraph{\textbf{Metatheory.}}
\interL{} is type safe. That is, the
common progress and preservation properties hold:
\begin{theoremB}[Progress]\leavevmode \\
  If \gsp $[[SS ; empty ; empty |-tm ie : is ~> te]]$,
  then either \gsp $[[ie]]$ \gsp is a value, 
  or there exists \gsp $\intermed{[[ie']]}$ \gsp such that \gsp $[[SS |- ie --> ie']]$.
\label{thm:progress_expressions}
\end{theoremB}
\begin{theoremB}[Preservation]\leavevmode \\
  If \gsp $[[ SS ; TC ; TT |-tm ie : is ~> te ]]$,
  and \gsp $[[SS |- ie --> ie']]$, 
  then \gsp $[[ SS ; TC ; TT |-tm ie' : is ~> te' ]]$.
  \label{thm:intermediate_preservation}
\end{theoremB}
Analogously to \srcL{}, \interL{}
rejects recursive expressions (including mutual recursion and recursive
methods). This allows for a normalizing language, that is,
any well-typed expression evaluates to a value, after a finite number of steps.
Note that since the small step operational semantics are deterministic,
normalization implies strong normalization.
\begin{theoremB}[Strong Normalization]\leavevmode \\
  If \([[ SS ; TC ; empty |-tm ie : is ~> te ]]\)
  then all possible evaluation derivations for \([[ie]]\) terminate :
  \( \exists [[iv]] : [[ SS |- ie -->> iv ]]\).
  \label{theorem:inter-sn}
\end{theoremB}
The proof follows the familiar structure for proving normalization using logical
relations, as presented by Ahmed~\cite{Ahmed2015}, and can be found in
Section~\ref{app:sn} of the appendix.
\renewcommand\itot[1]{#1} 

%-------------------------------------------------------------------------------
\subsection{Elaboration from \srcL{} to \interL{}}
\label{sec:elabSI}

The green aspects in Figure~\ref{fig:sourceM_typing} denote the elaboration of
\srcL{} terms to \interL{}. Similarly to the elaboration from \srcL{} to
\targetL{}, we have adopted the convention
that any green \interL{} types or constraints are the elaborated forms of their
identically named blue \srcL{} counterparts.
This elaboration works analogously to the elaboration from \srcL{} to \targetL{},
as shown in Figure~\ref{fig:source_typing}.
The full set of rules can be found in Section~\ref{app:srcmid_tm_typing} of the appendix.

The only notable case is \textsc{sTm-check-meth}, where the entailment relation
for solving the type class constraint \([[ sTC st ]]\) now results in a
dictionary \([[id]]\). As explained at the start of Section~\ref{sec:inter},
unlike \targetL{},
\interL{} differentiates syntactically between dictionaries and normal
expressions.

\boxedfigure
  {\input{figures/sourceM_typing.mng}}
  {\srcL{} typing with elaboration to \interL{}, selected rules}
  {fig:sourceM_typing}

\boxedfigure
  {\input{figures/sourceM_resolution.mng}}
  {\srcL{} constraint entailment with elaboration to \interL{}}
  {fig:sourceM_entail}

Type class resolution (Figure~\ref{fig:sourceM_entail}) of a \srcL{}
constraint \([[sq]]\) results in a \interL{} dictionary \([[id]]\).
When using a locally available constraint to resolve the wanted constraint
(\textsc{sEntail-local}), the corresponding dictionary variable \([[idvar]]\) is returned.
On the other hand, when resolving using a global instance declaration (\textsc{sEntail-inst}), a
dictionary is constructed by taking the corresponding constructor
\([[iD]]\) and applying
\begin{inparaenum}[(a)]
\item the types \(\intermed{[[ islj ]]}\) needed for matching the wanted constraint to the instance
  declaration and
\item the dictionaries \(\intermed{[[ idli ]]}\), constructed by resolving the
  instance context constraints.
\end{inparaenum}

\renewcommand\itot[1]{} 
\paragraph{\textbf{Metatheory.}}
We discuss the coherence of the elaboration from \srcL{} to \interL{} in detail
in Section~\ref{sec:coherence2}, and mention here
that it is type preserving:
\begin{theoremB}[Typing Preservation - Expressions]\leavevmode \\
If \gsp $[[P ; GC ; GG |-tm se => st ~> ie]]$,
and \gsp $[[|-ctx P ; GC ; GG ~> SS ; TC ; TT]]$,
and \gsp $[[GC ; GG |-ty st ~> is]]$, \\
then \gsp $[[SS ; TC ; TT |-tm ie : is ~> te]]$.
\label{thm:typing_pres_expr}
\end{theoremB}
The same theorem holds for check mode, but is omitted for space
reasons. The full proofs can be found in Section~\ref{app:type_pres} of the appendix.
\renewcommand\itot[1]{#1} 

\paragraph{\textbf{Example~\ref{fig:ex1} \srcL{} to \interL{}.}}
Elaborating the \srcL{} environments that originate from Example~\ref{fig:ex1},
results in the following \interL{} environments:
\input{examples/sielab_example1_env_gen.tex} 
Note that both the class environment \([[ TC ]]\) and the program context \([[SS]]\)
are largely direct translations of their \srcL{} counterparts. One notable
difference is the fact that the environment \([[GG]]\) under which to interpret
the \srcL{} method implementation is now explicitly abstracted over in the
\interL{} method implementation.
Consider for instance the case of \(\intermed{[[iD2]]}\), where the variables
\([[c]]\), \([[ib]]\), \(\intermed{[[idvar1]]}\) and \(\intermed{[[idvar2]]}\),
which in \srcL{} are implicitly provided by the typing environment, are now
explicit in the term level. 

Elaborating the \srcL{} expression results in the following \interL{}
expression:
\input{examples/sielab_example1_expr_gen.tex}
Unlike the corresponding \targetL{} expression, shown in Section~\ref{sec:elabST},
records storing the method types and implementations do not need to be passed
around explicitly.
In \interL{}, they are replaced by class constraints and dictionaries,
respectively. The construction of these dictionaries through type class
resolution is shown in Figure~\ref{fig:sourceM_entail}. 

\paragraph{\textbf{Example~\ref{fig:ex2} \srcL{} to \interL{}.}}
Elaborating Example~\ref{fig:ex2}, including the extension from
Section~\ref{sec:nondet}, results in the following \interL{} class environment
(since no instance declarations exist, the method environment \([[SS]]\) remains empty):
\input{examples/sielab_example2_env.mng} 
The \interL{} class environment no longer needs to
store superclasses, as these are all flattened into additional local
constraints during elaboration.

Similarly to Section~\ref{sec:elabST}, we focus solely on elaborating
\texttt{test2}, which results in the following \interL{} expression:

\input{examples/sielab_example2_expr_gen.tex}
The only difference with the \targetL{} elaboration is that we now use class
constraints instead of passing around a record type (storing the method types).

\subsection{Elaboration from \interL{} to \targetL{}}
\label{sec:elabIT}

As both \interL{} and \targetL{} are extensions of System F, the elaboration
from former to latter is mostly trivial, leaving common features unchanged. 
The mapping of \interL{} dictionaries into \targetL{}
records, however, is non-trivial.
Briefly, dictionary types are elaborated into record types, as shown in
Figure~\ref{fig:inter_typing} (top right), and dictionaries into record expressions,
possibly nested within type and term abstractions and applications, as shown in
Figure~\ref{fig:inter_dict_typing}.

In particular, a dictionary type, $[[iTC]]$, which corresponds to a unique entry
$(\intermed{[[im]] : [[iTC c]] : [[is']]})$ in the class environment $[[TC]]$, elaborates to a record
type whose field has the same name as the dictionary type's method name, $[[im]]$, and the type of
that field is determined by the elaboration of $\intermed{[[is']]}$. A $[[iTC is]]$ dictionary
elaborates to a record expression which is surrounded, firstly, by abstractions over
type and term variables that arise from the method type's class constraints and, secondly,
by type and term applications that properly instantiate those abstractions.

% \targetL{} is a thoroughly studied language and, thus, can serve well for the verification of
% the dictionaries' good-behavior. However, the method of elaborating a source language to a
% target one, to use the latter's well-studied operational semantics, does not straight-forwardly
% solve the problem, but transfers it to verifying that the translation is suitable.

\paragraph{\textbf{Metatheory.}}
The following theorems confirm that the \interL{}-to-\targetL{} elaboration is
indeed appropriate. 

The first theorem states that a well-typed \interL{} expression always elaborates to
a \targetL{} expression that is also well-typed in the translated context. 
\begin{theoremB}[Type Preservation]\leavevmode \\
  If \gsp $[[SS ; TC ; TT |-tm ie : is ~> te]]$, \\
  then there are unique \gsp $[[GT]]$ \gsp and \gsp $[[tt]]$ \gsp such that \gsp
  $[[GT |-tm te : tt]]$, \\
  where \gsp $[[ TC ; TT |-ty is ~> tt ]]$ \gsp and \gsp $[[TC ; TT ~> GT]]$.
\end{theoremB}
Secondly, and more importantly, the dynamic semantics is also preserved by the
elaboration.
\begin{theoremB}[Semantic Preservation]\leavevmode \\
  If \gsp \([[ SS ; TC ; empty |-tm ie : is ~> te ]]\) \gsp
  and \gsp \([[ SS |- ie -->> iv ]]\) \\
  then there exists a \gsp \([[tv]]\) \gsp such that \gsp \([[ SS ; TC ; empty
  |-tm iv : is ~> tv ]]\) \gsp
  and \gsp \([[ te ~= tv ]]\).
\end{theoremB}
Thirdly, the elaboration is entirely deterministic.
\begin{theoremB}[Determinism]\leavevmode \\
  \label{thm:mid-tgt-deter}
    If \gsp $[[ SS ; TC ; TT |-tm ie : is ~> te1 ]]$ \gsp and \gsp $[[ SS ; TC ; TT |-tm ie :
    is ~> te2 ]]$,  
    then \gsp $[[te1 = te2]]$.
\end{theoremB}

\subsection{Elaboration Decomposition}
\renewcommand\itot[1]{{#1}}

An elaboration from \srcL{} to \targetL{} can always be decomposed into two
elaborations through \interL{}.
This intuition is formalized in
Theorems~\ref{thm:equiv_expr} and~\ref{thm:equiv_dict} respectively.

\begin{theoremB}[Elaboration Equivalence - Expressions]\leavevmode \\
  If \gsp \([[ PT ; GC ; GG |-tm se => st ~> te ]]\) \gsp
  and \gsp \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
  then \gsp \([[ P ; GC ; GG |-tm se => st ~> ie ]]\) \gsp
  and \gsp \([[ SS ; TC ; TT |-tm ie : is ~> te ]]\) \\
  where \gsp \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\) \gsp
  and \gsp \([[ TC ; TT ~> GT ]]\) \gsp
  and \gsp \([[ GC ; GG |-ty st ~> is ]]\).
  \label{thm:equiv_expr}
\end{theoremB} 

\begin{theoremB}[Elaboration Equivalence - Dictionaries]\leavevmode \\
  If \gsp \([[ PT ; GC ; GG |= sq ~> te ]]\) \gsp
  and \gsp \([[ |-ctx PT ; GC ; GG ~> GT ]]\) \\
  then \gsp \([[ P ; GC ; GG |= sq ~> id ]]\) \gsp
  and \gsp \([[ SS ; TC ; TT |-d id : iq ~> te ]]\) \\
  where \gsp \([[ |-ctx P ; GC ; GG ~> SS ; TC ; TT ]]\) \gsp
  and \gsp \([[ TC ; TT ~> GT ]]\).
  \label{thm:equiv_dict}
\end{theoremB} 

Theorem~\ref{thm:equiv_expr} also has a type checking mode counterpart, which
has been omitted for space reasons. The full proofs can be
found in Section~\ref{app:equiv} of the appendix.


==> sections/source.tex <==
\section{Source Language \srcL{}}\label{sec:source}

This section presents our source language \srcL{}, a basic calculus which
isolates nondeterministic resolution.
The calculus only supports features that are
essential for type class resolution and its coherence.

Consequently, the language is strongly normalizing, and thus does not support
recursive let expressions, mutual recursion or recursive methods.
This is a sensible choice, as recursion does not affect the fundamentals of the
coherence proof.
This work could include recursion through step
indexing~\citep{ahmed2006step}, a well-known technique,
but this would significantly clutter the proof.
Recursion is discussed in more detail in Section~\ref{sec:features}.

Furthermore, two notable design decisions were made in the support of
superclasses in \srcL{}.
Firstly, similar to GHC, \srcL{} derives all possible superclass constraints
from their subclass constraints in advance, instead of deriving them
``just-in-time'' during resolution. The advantage of this approach is that it
streamlines the actual resolution process.

Secondly, similar to Coq~\cite{Sozeau2008} and unlike \citet{AdHocPolymorphism}, we pass superclass
dictionaries alongside their subclass dictionaries, i.e., in a \emph{flattened}
form, instead of nesting them inside their subclass dictionaries.
% Both approaches are isomorphic, since the fact that elaboration is determined by
% \srcL{} typing implies an isomorphism between said elaboration relations.
% Because of this isomorphism, flattening the superclasses does not
% fundamentally change the proof.
As it is not too difficult to see that both approaches are isomorphic,
flattening the superclasses does not impact the coherence of resolution.
% As both approaches are isomorphic, flattening the superclasses does not
% fundamentally change the proof.
It does, however, considerably simplify the
proof, since this way neither our type class
resolution mechanism, nor the intermediate language \interL{}
(Section~\ref{sec:inter}) need to have any
support for superclasses and can treat them as regular local constraints.
A more structured representation would give rise to additional complexity, but
would not alter the essence of the proof.

\paragraph{\textbf{Syntax.}} Figure~\ref{fig:source_syntax} presents the, mostly
standard, syntax.
Programs consist of a number of class (with superclasses) and instance
declarations, and an expression.
For the sake of simplicity and well-foundedness, the declarations are ordered
and can only refer to previous declarations.

\boxedfigure
  {\input{figures/source_syntax.mng}}
  {\srcL{} syntax}
  {fig:source_syntax}

Following \citet{jones-94}'s qualified types framework, we distinguish between three
sorts of types: monotypes \([[st]]\), qualified types \([[sp]]\) which include
constraints, and type schemes \([[ss]]\) which include type abstractions.
Constraints differentiate between full constraint schemes \([[sc]]\)
and simple class constraints \([[sq]]\). Observe that we allow flexible contexts
in the qualified types; they are not restricted to constraints on type variables.

The definition of expressions \([[se]]\) is standard, but with a few notable exceptions.
Firstly, the language differentiates syntactically between regular
variables \([[sx]]\) and method names \([[sm]]\), which are introduced
in class declarations.
Secondly, type annotations \(\source{[[ se <: st ]]}\) allow the programmer to manually
assign a monotype to an expression. This is useful for resolving ambiguity---see
the \textit{Typing} paragraph below.
Finally, let bindings include type annotations with a type scheme \([[ss]]\),
allowing the programmer to introduce local constraints---also discussed
in the \textit{Typing} paragraph.
Note that we use Haskell syntax for class and instance declarations. 

There are three \srcL{} environments: two global ones and one local
environment.
Firstly, the global class environment \([[GC]]\) stores all class declarations.
Each entry in \([[GC]]\) contains the method name \([[sm]]\), any superclasses \(\source{[[sTCl]]}\), the
class \([[sTC a]]\) itself and the corresponding method type \([[ss]]\).

Secondly, the global program context \([[P]]\) contains all instance declarations.
Each entry in \([[P]]\) consists of a unique dictionary constructor \([[sD]]\), its corresponding
constraint \([[sc]]\), the method name \([[sm]]\) and its implementation
\([[se]]\), together with the context \([[GG]]\) under which \([[se]]\) should be
interpreted. This context contains the local axioms available in this
instance declaration, as well as any axioms which explicitly annotate the method
type signature. 

Thirdly, the local typing environment \([[GG]]\), besides containing the
default term and type variables \([[sx]]\) and \([[a]]\), also stores any local
axioms \([[sq]]\). As opposed to the program context \([[P]]\),
\([[GG]]\) does not contain any type class instances. Instead, the (local) axioms
are associated with a dictionary variable \([[sdvar]]\).
Sections~\ref{sec:inter} and \ref{sec:elabSI} explain the use of these dictionaries.


\paragraph{\textbf{Typing.}}
Our type system features two design choices to
eliminate the possibility of ambiguous type schemes.
This allows us to focus on the coherence of type class
resolution, by making our proof orthogonal to ambiguous type schemes, the source
of ambiguity which has already been studied by \citet{jones}.
We thus side-step an already solved problem and focus on tackling the full
problem of resolution coherence.

Firstly, we require type signatures to be unambiguous
(Figure~\ref{fig:source_typing_extra}, right-hand side)
to make sure that all newly introduced type variables
are bound in the head of the type (the remaining monotype after dropping all type
and constraint abstractions).
This prevents ambiguous expressions such as:
\begin{verbatim}
    > let f : forall a . Eq a => Int -> Int -- ambiguous
    >       = \ x . x + 1 in f 42
\end{verbatim}

Secondly, we use a bidirectional type system rather than
a fully declarative one. A bidirectional type system distinguishes between two
typing modes: \emph{inference} and \emph{check} mode.
% The former outputs a type,
% while the latter takes it as a given input.
The former synthesizes a type from the given expression, while the latter checks
whether a given expression is of a given type. 
Special in our setting is that
variables can only be typed in check mode, to ensure that only a single
instantiation exists.
This avoids the ambiguity that can arise when instantiating type
variables in inference mode.
Consider the following example:
\begin{verbatim}
    > let y : forall a . Eq a => a -> a = ...
    > in const 1 y
\end{verbatim}
where \texttt{const x} is the constant function, which evaluates to \texttt{x}
for any input.
The instantiation of \texttt{y}'s type scheme is not uniquely determined by the
context in which it is used.  In a declarative type system or in inference mode,
this ambiguity would result in multiple distinct typings and corresponding
elaborations. While this ambiguity is harmless, it is not the focus of this
work. Hence, to focus exclusively on the resolution, we use a bidirectional type
system with check mode for variables to eliminate this irrelevant source of ambiguity. 

Figure~\ref{fig:source_typing}~
\footnote{Note that lists, such as \(\source{[[stli]]}\),
  are denoted by overlines, whereas collections of predicates are annotated by
  their range. For instance,
  \( \repeated{[[GC ; GG |-ty sti ~> tti]]}{i} \) iterates over \(i\).}
shows selected typing rules.
The full set of rules can be found in Section~\ref{app:src_tm_typing} of the appendix.
We ignore the red (elaboration-related) parts for now and explain them in
detail in Section~\ref{sec:elabST}.
\renewcommand\stoi[1]{}
\renewcommand\stot[1]{}
The judgments \([[ P ; GC ; GG |-tm se => st ~> te ]]\) and
\([[ P ; GC ; GG |-tm se <= st ~> te ]]\) denote \emph{infer}ring a monotype 
\([[ st ]]\) for expression \([[ se ]]\) and \emph{check}ing \([[ se ]]\) to have a
monotype \([[ st ]]\) respectively, in environments \([[P]]\), \([[GC]]\) and
\([[GG]]\).
Note that the constraint and type well-formedness relations \(\vdash_{Q}\) and
\(\vdash_{ty}\) are omitted, as they are standard
well-scopedness checks.
They can be found in Section~\ref{app:src_ty_wf} of the appendix.

\renewcommand\stoi[1]{{#1}}
\renewcommand\stot[1]{{#1}}

\newcommand{\vrulesep}{\unskip\ \vrule\ }
\newcommand{\hrulesep}{\hrule}
\boxedfigureH
  {
    \input{figures/source_typing.mng}
  }
  {\srcL{} typing, selected rules}
  {fig:source_typing}

\boxedfigureH
  {
    \begin{subfigure}[t]{0.49\textwidth}
      \input{figures/source_typing_extra.mng}
    \end{subfigure}
    \vrulesep
    \begin{subfigure}[t]{0.49\textwidth}
      \input{figures/source_typing_extra2.mng}
    \end{subfigure}
  }
  {Closure and unambiguity relations}
  {fig:source_typing_extra}

\boxedfigureH
  {\input{figures/source_resolution.mng}}
  {\srcL{} constraint entailment}
  {fig:source_entail}

\boxedfigureH
  {\input{figures/source_inst_typing.mng}}
  {\srcL{} instance declaration typing}
  {fig:source_inst}

Through a let binding (rule \textsc{sTm-infT-let}), the programmer provides a
type scheme for a variable, thus potentially introducing local constraints.
As explained above, the unambiguity check from
Figure~\ref{fig:source_typing_extra} (right-hand side) requires the
provided type scheme to be unambiguous.
In order to flatten the superclasses, the rule takes the closure
over the superclass relation (left-hand side of Figure~\ref{fig:source_typing_extra}) of the
user provided constraints \(\source{[[sqli]]}\). It then adds the resulting set of constraints
\(\source{[[sqlk]]}\) to the typing environment, under which to typecheck \(\source{[[se1]]}\).
Finally, the type of \(\source{[[se2]]}\) is inferred under the extended environment. 

Rule~\textsc{sTm-checkT-meth} types a method call \([[sm]]\) in
check mode, like regular variables, to avoid any ambiguity in the instantiation of the type variables in
the  method's type scheme.
This includes both the type variable \([[a]]\) from the class and any
additional free variables \(\source{[[alj]]}\) in the method type.
Furthermore, the rules uses the unambig-relation to avoid ambiguity in the
method type scheme itself, by requiring that both sets
of type variables have to occur in the head of the method type.
The rule also checks that all required constraints
\(\source{[[sqli]]}\) from the method type can be
entailed.

\renewcommand{\stoi}[1]{}
The instance typing rule can be found in
Figure~\ref{fig:source_inst}. The relation
\([[ P ; GC |-inst sinst : P' ]]\) denotes that an instance declaration
\([[sinst]]\) results in a \srcL{} program context \(\source{[[P']]}\),
while being typed under environments \([[P]]\) and \([[GC]]\).
The unambig-relation for constraints
(Figure~\ref{fig:source_typing_extra}, bottom right),
similarly to the unambig-relation for types,
checks that all free type variables \(\source{[[blk]]}\) in the instance context
occur in the instance type \([[st]]\) as well, in order to avoid ambiguity.
Like in the \textsc{sTm-infT-let} rule explained above, the
superclasses of the instance context \(\source{[[sqlp]]}\) are flattened into additional local
constraints \(\source{[[sqlq]]}\) and added to the environment.
The superclasses \(\source{[[sqli']]}\) of the instantiated type
class are then checked to be entailed under this extended environment.
The rule checks that no overlapping instance declarations \(\source{[[sD']]}\) have been defined.
Finally, the program context is extended with the new instance axiom \([[sD]]\), consisting
of a constraint scheme that requires the full set of local constraints \(\source{[[sqlq]]}\).


\paragraph{\textbf{Type Class Resolution.}}
\renewcommand\stoi[1]{}
\renewcommand\stot[1]{}
The type class resolution rules can be found in
Figure~\ref{fig:source_entail}, where
\([[ P ; GC ; GG |= sq ~> te ]]\) denotes that a class constraint \([[sq]]\)
is entailed under the environments \([[P]]\), \([[GC]]\) and \([[GG]]\).
A wanted constraint \([[sq]]\) can either be resolved
using a locally available constraint \([[sdvar]]\) (\textsc{sEntailT-local}) or through a
global instance declaration \([[sD]]\)
(\textsc{sEntailT-inst}). 
\renewcommand\stoi[1]{{#1}}
\renewcommand\stot[1]{{#1}}
The former is entirely straightforward. The latter is more involved as
an instance \([[sD]]\) may have an instance context \(\source{[[sqli']]}\), which has to be
recursively resolved. Before resolving the context, the type variables
\(\source{[[alj]]}\) are instantiated with the
corresponding concrete types \(\source{[[stlj]]}\), originating from the wanted
constraint \([[sq]]\).

Note that the type class resolution mechanism does not require any specific
support for superclasses, as these have all been flattened into regular local
constraints.




==> sections/target.tex <==
\section{Target Language \targetL{}}
\label{sec:target}

This section covers our target language \targetL{}, and the elaboration from
\srcL{} to \targetL{}. 

The target language is System F with records, which we consider a
reasonable subcalculus of those used by
Haskell compilers. Its syntax is shown in Figure~\ref{fig:target_syntax}.
We omit its standard typing rules and call-by-name operational semantics and refer the reader
to \citet[Chapter 23]{TAPL}, or Section~\ref{app:tgt} of the appendix.

\boxedfigure
  {\input{figures/target_syntax.mng}}
  {Target language syntax}
  {fig:target_syntax}

\subsection{Elaboration from \srcL{} to \targetL{}}
\label{sec:elabST}

The red aspects in Figure~\ref{fig:source_typing} denote the elaboration of
\srcL{} terms to \targetL{}. We have adopted the convention
that any red \targetL{} types are the elaborated forms of their
identically named blue \srcL{} counterparts. 
This elaboration maps most \srcL{} forms on identical \targetL{} terms,
with the exception of a few notable cases:
\begin{inparaenum}[(a)]
\item The interesting aspect of elaborating let expressions
  (\textsc{sTm-infT-let}) is that, as mentioned previously, superclasses are
  flattened into additional local constraints.
  The elaborated expression thus explicitly requires both the type
  variables and the full closure of the local constraints.
\item As opposed to \srcL{}, dictionary and type application are made explicit in
  \targetL{}. When elaborating variables \([[sx]]\) and method references
  \([[sm]]\) (\textsc{sTm-checkT-meth}), all previously substituted types
  \(\source{[[stlj]]}\) are now explicitly applied, together with the dictionary expressions \(\target{[[teli]]}\).
  Furthermore, method names \([[sm]]\) are elaborated to \targetL{} record
  labels \([[tl]]\) and therefore cannot appear by themselves, but must be
  applied to a record expression \([[te]]\), which originates from resolving the
  class constraint.
\end{inparaenum}

Type class resolution (Figure~\ref{fig:source_entail}) of a \srcL{}
constraint \([[sq]]\) results in a \targetL{} expression \([[te]]\).
When resolving the wanted constraint using a locally available constraint \([[sdvar]]\)
(\textsc{sEntailT-local}), this results in a regular term variable \([[txd]]\)
(which keeps the name of its \srcL{} counterpart for readability).
On the other hand, when resolving with the use of a global instance declaration \([[sD]]\) (\textsc{sEntailT-inst}), a record
expression is constructed, containing the method name \([[tl]]\) and its corresponding
implementation \([[te]]\). This method implementation now explicitly abstracts over the
type variables \(\target{[[tblk]]}\) and term variables \(\target{[[txdlh]]}\)
originating from the method types's class constraints \(\source{[[sqlh]]}\), which
annotate the class declaration.
Furthermore, the record expression is nested in abstractions
over the type variables \(\target{[[talj]]}\) and term variables \(\target{[[txdli']]}\) arising from the corresponding instance
constraints \(\source{[[sqli']]}\).
These abstractions are immediately instantiated by applying
\begin{inparaenum}[(a)]
\item the types \(\target{[[ttlj]]}\) needed for matching the wanted constraint \([[sq]]\) to the instance
  declaration \(\source{[[sq']]}\) and
\item the expressions \(\target{[[teli]]}\) constructed by resolving the
  instance context constraints \(\source{[[ sqli' ]]}\).
\end{inparaenum}

\paragraph{\textbf{Example~\ref{fig:ex1} \srcL{} to \targetL{}.}}
Typing the Example~\ref{fig:ex1} program results in the following
environments:
\input{examples/stelab_example1_env_gen.tex} 
The \([[sEq]]\)~class straightforwardly gets stored in the class environment
\([[GC]]\). Instances are stored in the \srcL{} program context \([[P]]\)
(containing the dictionary constructor, the corresponding constraint, the method
implementation and the environment under which to interpret this expression).
Storing the instance declaration for \([[ sEq sint ]]\) is
clear-cut. The instance for tuples on the other hand is somewhat more complex, since it
requires an instance context, containing the local constraints \([[sEq a]]\) and
\([[sEq b]]\). These constraints are made explicit, that is, the
corresponding dictionaries are required by the elaborated
implementation.

Elaborating the \srcL{} expression results in the following \targetL{}
expression:
\input{examples/stelab_example1_expr_gen.tex} 
Note that the \([[ sEq a ]]\) constraint is made explicit in the implementation
of \([[ trefl ]]\), by abstracting over the constraint
(elaborated to \targetL{} as the record type
\( \target {[[ { tequal : ta -> ta -> tbool } ]]}\), which stores the method name and its
corresponding type)
with the use of the record variable \(\target{[[ txd3 ]]}\). 
When this function is called in \([[ tmain ]]\), both the type and the
dictionary variable are instantiated. The latter is performed by (recursively) constructing a
dictionary expression, using the type class resolution mechanism, as explained
above in Section~\ref{sec:elabST}.

\paragraph{\textbf{Example~\ref{fig:ex2} \srcL{} to \targetL{}.}}
Below is the environment generated by typing the Example~\ref{fig:ex2} program (including
the Section~\ref{sec:nondet} extension), which features superclasses.
\input{examples/stelab_example2_env_gen.tex}
The class environment \([[GC]]\) contains three classes, two of which have superclasses.
However, since the example does not contain any instance declarations, the resulting
program context \([[P]]\) is empty.

For space reasons, we focus solely on elaborating \texttt{test2}, which results in
the following \targetL{} expression:

\input{examples/stelab_example2_expr_gen.tex}
Note that the \srcL{} expression requires two local constraints:
\(\source{[[ sSub1 a ]]}\) and \(\source{[[ sSub2 a ]]}\).
However, after flattening the superclasses and adding them to the local
constraints, the elaborated \targetL{} expression requires (the elaborated form
of) the
\(\source{[[ sBase a ]]}\), \(\source{[[ sSub1 a ]]}\), \(\source{[[ sBase a ]]}\) and
\(\source{[[ sSub2 a ]]}\) constraints. Notice the duplicate \(\source{[[sBase a]]}\) entry.
Either of these two entries can be used for calling
the method \([[ tbase ]]\). 
We have arbitrarily selected the first here. 
The next section proves that both options are equivalent
and can be used interchangeably.


